Lingering Issues in Distributed Scheduling

Recent advances have resulted in queue-based algorithms for medium access control which operate in a distributed fashion, and yet achieve the optimal throughput performance of centralized scheduling algorithms. However, fundamental performance bounds reveal that the "cautious" activation rules involved in establishing throughput optimality tend to produce extremely large delays, typically growing exponentially in 1/(1-r), with r the load of the system, in contrast to the usual linear growth. Motivated by that issue, we explore to what extent more "aggressive" schemes can improve the delay performance. Our main finding is that aggressive activation rules induce a lingering effect, where individual nodes retain possession of a shared resource for excessive lengths of time even while a majority of other nodes idle. Using central limit theorem type arguments, we prove that the idleness induced by the lingering effect may cause the delays to grow with 1/(1-r) at a quadratic rate. To the best of our knowledge, these are the first mathematical results illuminating the lingering effect and quantifying the performance impact. In addition extensive simulation experiments are conducted to illustrate and validate the various analytical results.

==> fig/full.tex <==
\addplot[color=red, mark=none, line width=10pt, smooth] plot coordinates {
	(0,	1407)
	(10,	1412)
	(20,	1417)
	(30,	1425)
	(40,	1433)
	(50,	1438)
	(60,	1454)
	(70,	1454)
	(80,	1460)
	(90,	1464)
	(100,	1472)
	(110,	1477)
	(120,	1481)
	(130,	1486)
	(140,	1493)
	(150,	1494)
	(160,	1496)
	(170,	1500)
	(180,	1505)
	(190,	1513)
	(200,	1520)
	(210,	1528)
	(220,	1531)
	(230,	1539)
	(240,	1547)
	(250,	1552)
	(260,	1560)
	(270,	1564)
	(280,	1568)
	(290,	1571)
	(300,	1572)
	(310,	1574)
	(320,	1584)
	(330,	1585)
	(340,	1592)
	(350,	1594)
	(360,	1601)
	(370,	1603)
	(380,	1607)
	(390,	1613)
	(400,	1615)
	(410,	1618)
	(420,	1622)
	(430,	1625)
	(440,	1626)
	(450,	1632)
	(460,	1637)
	(470,	1642)
	(480,	1652)
	(490,	1656)
	(500,	1661)
	(510,	1664)
	(520,	1669)
	(530,	1671)
	(540,	1683)
	(550,	1689)
	(560,	1690)
	(570,	1695)
	(580,	1699)
	(590,	1704)
	(600,	1708)
	(610,	1709)
	(620,	1716)
	(630,	1725)
	(640,	1731)
	(650,	1737)
	(660,	1742)
	(670,	1746)
	(680,	1751)
	(690,	1757)
	(700,	1766)
	(710,	1775)
	(720,	1782)
	(730,	1792)
	(740,	1797)
	(750,	1803)
	(760,	1806)
	(770,	1814)
	(780,	1816)
	(790,	1819)
	(800,	1824)
	(801,	1824)
	(802,	1827)
	(803,	1827)
	(804,	1827)
	(805,	1827)
	(806,	1828)
	(807,	1828)
	(808,	1828)
	(809,	1828)
	(810,	1828)
	(811,	1828)
	(812,	1828)
	(813,	1828)
	(814,	1828)
	(815,	1828)
	(816,	1828)
	(817,	1829)
	(818,	1829)
	(819,	1829)
	(820,	1829)
	(821,	1829)
	(822,	1829)
	(823,	1829)
	(824,	1830)
	(825,	1830)
	(826,	1830)
	(827,	1830)
	(828,	1830)
	(829,	1830)
	(830,	1831)
	(831,	1833)
	(832,	1833)
	(833,	1834)
	(834,	1834)
	(835,	1834)
	(836,	1834)
	(837,	1834)
	(838,	1834)
	(839,	1837)
	(840,	1837)
	(841,	1837)
	(842,	1838)
	(843,	1839)
	(844,	1839)
	(845,	1840)
	(846,	1840)
	(847,	1840)
	(848,	1840)
	(849,	1840)
	(850,	1840)
	(851,	1841)
	(852,	1842)
	(853,	1842)
	(854,	1842)
	(855,	1844)
	(856,	1845)
	(857,	1845)
	(858,	1846)
	(859,	1847)
	(860,	1847)
	(861,	1847)
	(862,	1847)
	(863,	1847)
	(864,	1847)
	(865,	1848)
	(866,	1848)
	(867,	1849)
	(868,	1852)
	(869,	1853)
	(870,	1853)
	(871,	1853)
	(872,	1853)
	(873,	1853)
	(874,	1853)
	(875,	1853)
	(876,	1853)
	(877,	1853)
	(878,	1853)
	(879,	1853)
	(880,	1853)
	(881,	1853)
	(882,	1853)
	(883,	1853)
	(884,	1853)
	(885,	1853)
	(886,	1853)
	(887,	1853)
	(888,	1853)
	(889,	1853)
	(890,	1853)
	(891,	1853)
	(892,	1853)
	(893,	1854)
	(894,	1854)
	(895,	1854)
	(896,	1854)
	(897,	1854)
	(898,	1854)
	(899,	1855)
	(900,	1855)
	(901,	1856)
	(902,	1856)
	(903,	1856)
	(904,	1856)
	(905,	1856)
	(906,	1856)
	(907,	1857)
	(908,	1857)
	(909,	1858)
	(910,	1858)
	(911,	1861)
	(912,	1862)
	(913,	1862)
	(914,	1862)
	(915,	1862)
	(916,	1862)
	(917,	1863)
	(918,	1863)
	(919,	1863)
	(920,	1863)
	(921,	1865)
	(922,	1865)
	(923,	1867)
	(924,	1867)
	(925,	1869)
	(926,	1869)
	(927,	1870)
	(928,	1870)
	(929,	1871)
	(930,	1872)
	(931,	1872)
	(932,	1872)
	(933,	1872)
	(934,	1872)
	(935,	1872)
	(936,	1872)
	(937,	1873)
	(938,	1874)
	(939,	1874)
	(940,	1875)
	(941,	1875)
	(942,	1877)
	(943,	1877)
	(944,	1877)
	(945,	1877)
	(946,	1877)
	(947,	1877)
	(948,	1879)
	(949,	1879)
	(950,	1879)
	(951,	1880)
	(952,	1880)
	(953,	1880)
	(954,	1880)
	(955,	1880)
	(956,	1880)
	(957,	1880)
	(958,	1881)
	(959,	1881)
	(960,	1883)
	(961,	1884)
	(962,	1884)
	(963,	1884)
	(964,	1886)
	(965,	1886)
	(966,	1887)
	(967,	1888)
	(968,	1888)
	(969,	1888)
	(970,	1888)
	(971,	1888)
	(972,	1889)
	(973,	1890)
	(974,	1890)
	(975,	1890)
	(976,	1890)
	(977,	1890)
	(978,	1890)
	(979,	1890)
	(980,	1890)
	(981,	1895)
	(982,	1895)
	(983,	1896)
	(984,	1896)
	(985,	1897)
	(986,	1897)
	(987,	1899)
	(988,	1899)
	(989,	1899)
	(990,	1899)
	(991,	1899)
	(992,	1899)
	(993,	1900)
	(994,	1900)
	(995,	1900)
	(996,	1901)
	(997,	1902)
	(998,	1903)
	(999,	1903)
	(1000,	1903)
	(1001,	1903)
	(1002,	1903)
	(1003,	1904)
	(1004,	1904)
	(1005,	1905)
	(1006,	1907)
	(1007,	1908)
	(1008,	1908)
	(1009,	1908)
	(1010,	1909)
	(1011,	1909)
	(1012,	1910)
	(1013,	1911)
	(1014,	1912)
	(1015,	1912)
	(1016,	1913)
	(1017,	1914)
	(1018,	1914)
	(1019,	1915)
	(1020,	1917)
	(1021,	1917)
	(1022,	1917)
	(1023,	1919)
	(1024,	1924)
	(1025,	1924)
	(1026,	1924)
	(1027,	1924)
	(1028,	1925)
	(1029,	1925)
	(1030,	1925)
	(1031,	1926)
	(1032,	1926)
	(1033,	1927)
	(1034,	1928)
	(1035,	1930)
	(1036,	1931)
	(1037,	1932)
	(1038,	1932)
	(1039,	1932)
	(1040,	1932)
	(1041,	1934)
	(1042,	1935)
	(1043,	1937)
	(1044,	1937)
	(1045,	1937)
	(1046,	1938)
	(1047,	1938)
	(1048,	1941)
	(1049,	1940)
	(1050,	1939)
	(1051,	1938)
	(1052,	1937)
	(1053,	1937)
	(1054,	1936)
	(1055,	1935)
	(1056,	1934)
	(1057,	1933)
	(1058,	1935)
	(1059,	1934)
	(1060,	1934)
	(1061,	1933)
	(1062,	1932)
	(1063,	1931)
	(1064,	1930)
	(1065,	1929)
	(1066,	1928)
	(1067,	1927)
	(1068,	1926)
	(1069,	1925)
	(1070,	1924)
	(1071,	1924)
	(1072,	1926)
	(1073,	1925)
	(1074,	1925)
	(1075,	1924)
	(1076,	1923)
	(1077,	1922)
	(1078,	1922)
	(1079,	1923)
	(1080,	1922)
	(1081,	1921)
	(1082,	1920)
	(1083,	1919)
	(1084,	1918)
	(1085,	1917)
	(1086,	1916)
	(1087,	1915)
	(1088,	1914)
	(1089,	1913)
	(1090,	1913)
	(1091,	1912)
	(1092,	1912)
	(1093,	1911)
	(1094,	1910)
	(1095,	1909)
	(1096,	1911)
	(1097,	1910)
	(1098,	1909)
	(1099,	1908)
	(1100,	1908)
	(1101,	1908)
	(1102,	1908)
	(1103,	1907)
	(1104,	1907)
	(1105,	1906)
	(1106,	1906)
	(1107,	1906)
	(1108,	1909)
	(1109,	1909)
	(1110,	1908)
	(1111,	1907)
	(1112,	1907)
	(1113,	1906)
	(1114,	1905)
	(1115,	1905)
	(1116,	1904)
	(1117,	1904)
	(1118,	1903)
	(1119,	1902)
	(1120,	1902)
	(1121,	1903)
	(1122,	1904)
	(1123,	1903)
	(1124,	1902)
	(1125,	1902)
	(1126,	1901)
	(1127,	1901)
	(1128,	1900)
	(1129,	1899)
	(1130,	1900)
	(1131,	1899)
	(1132,	1899)
	(1133,	1898)
	(1134,	1897)
	(1135,	1898)
	(1136,	1897)
	(1137,	1897)
	(1138,	1898)
	(1139,	1898)
	(1140,	1899)
	(1141,	1901)
	(1142,	1900)
	(1143,	1899)
	(1144,	1898)
	(1145,	1899)
	(1146,	1901)
	(1147,	1900)
	(1148,	1899)
	(1149,	1898)
	(1150,	1897)
	(1151,	1896)
	(1152,	1895)
	(1153,	1895)
	(1154,	1894)
	(1155,	1893)
	(1156,	1892)
	(1157,	1891)
	(1158,	1891)
	(1159,	1891)
	(1160,	1890)
	(1161,	1890)
	(1162,	1889)
	(1163,	1888)
	(1164,	1889)
	(1165,	1889)
	(1166,	1889)
	(1167,	1888)
	(1168,	1887)
	(1169,	1886)
	(1170,	1885)
	(1171,	1884)
	(1172,	1884)
	(1173,	1884)
	(1174,	1884)
	(1175,	1884)
	(1176,	1883)
	(1177,	1882)
	(1178,	1881)
	(1179,	1880)
	(1180,	1879)
	(1181,	1878)
	(1182,	1877)
	(1183,	1876)
	(1184,	1875)
	(1185,	1875)
	(1186,	1874)
	(1187,	1877)
	(1188,	1876)
	(1189,	1875)
	(1190,	1874)
	(1191,	1874)
	(1192,	1876)
	(1193,	1876)
	(1194,	1875)
	(1195,	1874)
	(1196,	1873)
	(1197,	1874)
	(1198,	1873)
	(1199,	1872)
	(1200,	1871)
	(1210,	1862)
	(1220,	1855)
	(1230,	1848)
	(1240,	1841)
	(1250,	1841)
	(1260,	1835)
	(1270,	1827)
	(1280,	1818)
	(1290,	1820)
	(1300,	1813)
	(1310,	1806)
	(1320,	1804)
	(1330,	1796)
	(1340,	1791)
	(1350,	1785)
	(1360,	1782)
	(1370,	1775)
	(1380,	1773)
	(1390,	1772)
	(1400,	1764)
	(1410,	1758)
	(1420,	1755)
	(1430,	1751)
	(1440,	1749)
	(1450,	1748)
	(1460,	1739)
	(1470,	1733)
	(1480,	1731)
	(1490,	1725)
	(1500,	1718)
	(1510,	1715)
	(1520,	1710)
	(1530,	1705)
	(1540,	1699)
	(1550,	1691)
	(1560,	1682)
	(1570,	1675)
	(1580,	1666)
	(1590,	1659)
	(1600,	1653)
	(1610,	1650)
	(1620,	1646)
	(1630,	1642)
	(1640,	1638)
	(1650,	1631)
	(1660,	1624)
	(1670,	1620)
	(1680,	1617)
	(1690,	1609)
	(1700,	1603)
	(1710,	1598)
	(1720,	1592)
	(1730,	1586)
	(1740,	1590)
	(1750,	1583)
	(1760,	1579)
	(1770,	1573)
	(1780,	1564)
	(1790,	1559)
	(1800,	1558)
	(1810,	1554)
	(1820,	1550)
	(1830,	1547)
	(1840,	1545)
	(1850,	1537)
	(1860,	1528)
	(1870,	1524)
	(1880,	1523)
	(1890,	1517)
	(1900,	1512)
	(1910,	1504)
	(1920,	1497)
	(1930,	1499)
	(1940,	1492)
	(1950,	1483)
	(1960,	1478)
	(1970,	1477)
	(1980,	1472)
	(1990,	1467)
	(2000,	1465)
	(2010,	1457)
	(2020,	1454)
	(2030,	1449)
	(2040,	1442)
	(2050,	1436)
	(2060,	1428)
	(2070,	1422)
	(2080,	1414)
	(2090,	1406)
	(2100,	1399)
	(2110,	1396)
	(2120,	1394)
	(2130,	1391)
	(2140,	1384)
	(2150,	1377)
	(2160,	1371)
	(2170,	1366)
	(2180,	1361)
	(2190,	1358)
	(2200,	1353)
	(2210,	1346)
	(2220,	1341)
	(2230,	1336)
	(2240,	1329)
	(2250,	1322)
	(2260,	1316)
	(2270,	1307)
	(2280,	1306)
	(2290,	1300)
	(2300,	1300)
	(2310,	1295)
	(2320,	1293)
	(2330,	1288)
	(2340,	1282)
	(2350,	1273)
	(2360,	1269)
	(2370,	1267)
	(2380,	1259)
	(2390,	1256)
	(2400,	1250)
	(2410,	1246)
	(2420,	1245)
	(2430,	1240)
	(2440,	1235)
	(2450,	1227)
	(2460,	1222)
	(2470,	1217)
	(2480,	1211)
	(2490,	1203)
	(2500,	1200)
	(2510,	1191)
	(2520,	1183)
	(2530,	1176)
	(2540,	1173)
	(2550,	1164)
	(2560,	1164)
	(2570,	1156)
	(2580,	1151)
	(2590,	1150)
	(2600,	1145)
	(2610,	1137)
	(2620,	1128)
	(2630,	1124)
	(2640,	1122)
	(2650,	1118)
	(2660,	1118)
	(2670,	1114)
	(2680,	1110)
	(2690,	1108)
	(2700,	1103)
	(2710,	1097)
	(2720,	1095)
	(2730,	1090)
	(2740,	1086)
	(2750,	1080)
	(2760,	1074)
	(2770,	1067)
	(2780,	1061)
	(2790,	1060)
	(2800,	1055)
	(2810,	1050)
	(2820,	1043)
	(2830,	1036)
	(2840,	1035)
	(2850,	1030)
	(2860,	1025)
	(2870,	1018)
	(2880,	1012)
	(2890,	1009)
	(2900,	1004)
	(2910,	998)
	(2920,	996)
	(2930,	989)
	(2940,	982)
	(2950,	975)
	(2960,	966)
	(2970,	958)
	(2980,	954)
	(2990,	950)
	(3000,	949)
	(3010,	948)
	(3020,	940)
	(3030,	934)
	(3040,	932)
	(3050,	925)
	(3060,	916)
	(3070,	912)
	(3080,	905)
	(3090,	898)
	(3100,	893)
	(3110,	888)
	(3120,	882)
	(3130,	881)
	(3140,	876)
	(3150,	873)
	(3160,	867)
	(3170,	863)
	(3180,	854)
	(3190,	847)
	(3200,	842)
	(3210,	841)
	(3220,	835)
	(3230,	828)
	(3240,	823)
	(3250,	818)
	(3260,	812)
	(3270,	804)
	(3280,	796)
	(3290,	793)
	(3300,	787)
	(3310,	781)
	(3320,	778)
	(3330,	772)
	(3340,	768)
	(3350,	761)
	(3360,	755)
	(3370,	749)
	(3380,	745)
	(3390,	743)
	(3400,	736)
	(3410,	733)
	(3420,	733)
	(3430,	730)
	(3440,	721)
	(3450,	711)
	(3460,	703)
	(3470,	694)
	(3480,	690)
	(3490,	693)
	(3500,	685)
	(3510,	677)
	(3520,	668)
	(3530,	663)
	(3540,	658)
	(3550,	650)
	(3560,	644)
	(3570,	641)
	(3580,	639)
	(3590,	633)
	(3600,	626)
	(3610,	623)
	(3620,	617)
	(3630,	611)
	(3640,	603)
	(3650,	594)
	(3660,	586)
	(3670,	580)
	(3680,	574)
	(3690,	569)
	(3700,	563)
	(3710,	554)
	(3720,	550)
	(3730,	546)
	(3740,	542)
	(3750,	533)
	(3760,	534)
	(3770,	525)
	(3780,	520)
	(3790,	513)
	(3800,	504)
	(3810,	506)
	(3820,	497)
	(3830,	490)
	(3840,	486)
	(3850,	481)
	(3860,	471)
	(3870,	464)
	(3880,	460)
	(3890,	462)
	(3900,	454)
	(3910,	451)
	(3920,	447)
	(3930,	445)
	(3940,	438)
	(3950,	434)
	(3960,	428)
	(3970,	422)
	(3980,	416)
	(3990,	408)
	(4000,	405)
	(4010,	399)
	(4020,	394)
	(4030,	397)
	(4040,	388)
	(4050,	384)
	(4060,	379)
	(4070,	373)
	(4080,	367)
	(4090,	365)
	(4100,	358)
	(4110,	355)
	(4120,	351)
	(4130,	345)
	(4140,	345)
	(4150,	347)
	(4160,	340)
	(4170,	341)
	(4180,	334)
	(4190,	327)
	(4200,	320)
	(4210,	317)
	(4220,	311)
	(4230,	314)
	(4240,	305)
	(4250,	298)
	(4260,	292)
	(4270,	286)
	(4280,	280)
	(4290,	273)
	(4300,	266)
	(4310,	263)
	(4320,	263)
	(4330,	258)
	(4340,	254)
	(4350,	247)
	(4360,	243)
	(4370,	238)
	(4380,	234)
	(4390,	226)
	(4400,	222)
	(4410,	213)
	(4420,	212)
	(4430,	209)
	(4440,	201)
	(4450,	193)
	(4460,	192)
	(4470,	187)
	(4480,	183)
	(4490,	183)
	(4500,	176)
	(4510,	171)
	(4520,	165)
	(4530,	159)
	(4540,	157)
	(4550,	151)
	(4560,	145)
	(4570,	141)
	(4580,	136)
	(4590,	128)
	(4600,	122)
	(4610,	117)
	(4620,	113)
	(4630,	106)
	(4640,	102)
	(4650,	95)
	(4660,	89)
	(4670,	85)
	(4680,	81)
	(4690,	72)
	(4700,	66)
	(4701,	66)
	(4702,	65)
	(4703,	66)
	(4704,	65)
	(4705,	64)
	(4706,	63)
	(4707,	62)
	(4708,	61)
	(4709,	61)
	(4710,	62)
	(4711,	62)
	(4712,	61)
	(4713,	61)
	(4714,	61)
	(4715,	60)
	(4716,	59)
	(4717,	58)
	(4718,	57)
	(4719,	57)
	(4720,	56)
	(4721,	55)
	(4722,	54)
	(4723,	57)
	(4724,	57)
	(4725,	57)
	(4726,	57)
	(4727,	57)
	(4728,	56)
	(4729,	55)
	(4730,	54)
	(4731,	53)
	(4732,	52)
	(4733,	53)
	(4734,	52)
	(4735,	52)
	(4736,	52)
	(4737,	51)
	(4738,	50)
	(4739,	49)
	(4740,	48)
	(4741,	47)
	(4742,	46)
	(4743,	48)
	(4744,	47)
	(4745,	46)
	(4746,	45)
	(4747,	44)
	(4748,	43)
	(4749,	42)
	(4750,	42)
	(4751,	41)
	(4752,	41)
	(4753,	40)
	(4754,	40)
	(4755,	40)
	(4756,	40)
	(4757,	40)
	(4758,	39)
	(4759,	39)
	(4760,	39)
	(4761,	38)
	(4762,	37)
	(4763,	36)
	(4764,	35)
	(4765,	35)
	(4766,	34)
	(4767,	34)
	(4768,	35)
	(4769,	34)
	(4770,	33)
	(4771,	34)
	(4772,	34)
	(4773,	33)
	(4774,	35)
	(4775,	35)
	(4776,	34)
	(4777,	35)
	(4778,	35)
	(4779,	34)
	(4780,	33)
	(4781,	34)
	(4782,	33)
	(4783,	32)
	(4784,	32)
	(4785,	32)
	(4786,	31)
	(4787,	30)
	(4788,	29)
	(4789,	30)
	(4790,	31)
	(4791,	31)
	(4792,	30)
	(4793,	30)
	(4794,	29)
	(4795,	28)
	(4796,	27)
	(4797,	26)
	(4798,	25)
	(4799,	24)
	(4800,	23)
	(4801,	22)
	(4802,	21)
	(4803,	20)
	(4804,	19)
	(4805,	18)
	(4806,	17)
	(4807,	16)
	(4808,	15)
	(4809,	14)
	(4810,	13)
	(4811,	12)
	(4812,	12)
	(4813,	11)
	(4814,	11)
	(4815,	10)
	(4816,	9)
	(4817,	9)
	(4818,	9)
	(4819,	8)
	(4820,	7)
	(4821,	7)
	(4822,	6)
	(4823,	5)
	(4824,	4)
	(4825,	3)
	(4826,	5)
	(4827,	5)
	(4828,	4)
	(4829,	3)
	(4830,	2)
	(4831,	1)
	(4832,	1)
	(4833,	1)
	(4834,	2)
	(4835,	1)
	(4836,	2)
	(4837,	3)
	(4838,	2)
	(4839,	1)
	(4840,	0)
	(4841,	0)
	(4842,	0)
	(4843,	0)
	(4844,	0)
	(4845,	0)
	(4846,	1)
	(4847,	0)
	(4848,	0)
	(4849,	0)
	(4850,	0)
	(4851,	0)
	(4852,	0)
	(4853,	0)
	(4854,	0)
	(4855,	0)
	(4856,	0)
	(4857,	2)
	(4858,	1)
	(4859,	0)
	(4860,	0)
	(4861,	0)
	(4862,	0)
	(4863,	0)
	(4864,	0)
	(4865,	0)
	(4866,	0)
	(4867,	0)
	(4868,	2)
	(4869,	1)
	(4870,	1)
	(4871,	0)
	(4872,	0)
	(4873,	0)
	(4874,	0)
	(4875,	0)
	(4876,	0)
	(4877,	0)
	(4878,	0)
	(4879,	1)
	(4880,	3)
	(4881,	2)
	(4882,	2)
	(4883,	3)
	(4884,	2)
	(4885,	2)
	(4886,	1)
	(4887,	0)
	(4888,	0)
	(4889,	0)
	(4890,	0)
	(4891,	0)
	(4892,	0)
	(4893,	0)
	(4894,	0)
	(4895,	0)
	(4896,	1)
	(4897,	0)
	(4898,	0)
	(4899,	0)
	(4900,	1)
	(4901,	0)
	(4902,	0)
	(4903,	0)
	(4904,	2)
	(4905,	1)
	(4906,	1)
	(4907,	0)
	(4908,	0)
	(4909,	0)
	(4910,	0)
	(4911,	0)
	(4912,	2)
	(4913,	1)
	(4914,	0)
	(4915,	0)
	(4916,	0)
	(4917,	0)
	(4918,	0)
	(4919,	0)
	(4920,	0)
	(4921,	2)
	(4922,	1)
	(4923,	0)
	(4924,	0)
	(4925,	0)
	(4926,	0)
	(4927,	0)
	(4928,	1)
	(4929,	0)
	(4930,	0)
	(4931,	0)
	(4932,	0)
	(4933,	0)
	(4934,	0)
	(4935,	1)
	(4936,	2)
	(4937,	2)
	(4938,	2)
	(4939,	2)
	(4940,	4)
	(4941,	4)
	(4942,	5)
	(4943,	5)
	(4944,	5)
	(4945,	6)
	(4946,	6)
	(4947,	6)
	(4948,	7)
	(4949,	8)
	(4950,	9)
	(4951,	9)
	(4952,	9)
	(4953,	9)
	(4954,	11)
	(4955,	14)
	(4956,	15)
	(4957,	16)
	(4958,	16)
	(4959,	19)
	(4960,	20)
	(4961,	21)
	(4962,	21)
	(4963,	24)
	(4964,	26)
	(4965,	26)
	(4966,	26)
	(4967,	27)
	(4968,	27)
	(4969,	27)
	(4970,	27)
	(4971,	28)
	(4972,	30)
	(4973,	30)
	(4974,	30)
	(4975,	30)
	(4976,	30)
	(4977,	30)
	(4978,	30)
	(4979,	30)
	(4980,	30)
	(4981,	30)
	(4982,	30)
	(4983,	30)
	(4984,	31)
	(4985,	31)
	(4986,	31)
	(4987,	32)
	(4988,	32)
	(4989,	32)
	(4990,	32)
	(4991,	32)
	(4992,	32)
	(4993,	32)
	(4994,	33)
	(4995,	33)
	(4996,	33)
	(4997,	33)
	(4998,	35)
	(4999,	38)
	(5000,	39)
	(5001,	39)
	(5002,	39)
	(5003,	40)
	(5004,	40)
	(5005,	40)
	(5006,	41)
	(5007,	41)
	(5008,	42)
	(5009,	42)
	(5010,	42)
	(5011,	42)
	(5012,	42)
	(5013,	42)
	(5014,	42)
	(5015,	42)
	(5016,	42)
	(5017,	43)
	(5018,	43)
	(5019,	43)
	(5020,	43)
	(5021,	43)
	(5022,	43)
	(5023,	46)
	(5024,	46)
	(5025,	47)
	(5026,	47)
	(5027,	47)
	(5028,	47)
	(5029,	47)
	(5030,	47)
	(5031,	47)
	(5032,	47)
	(5033,	50)
	(5034,	52)
	(5035,	54)
	(5036,	54)
	(5037,	58)
	(5038,	58)
	(5039,	58)
	(5040,	58)
	(5041,	58)
	(5042,	58)
	(5043,	58)
	(5044,	58)
	(5045,	58)
	(5046,	60)
	(5047,	62)
	(5048,	62)
	(5049,	62)
	(5050,	62)
	(5051,	62)
	(5052,	62)
	(5053,	62)
	(5054,	62)
	(5055,	62)
	(5056,	66)
	(5057,	69)
	(5058,	69)
	(5059,	69)
	(5060,	69)
	(5061,	70)
	(5062,	70)
	(5063,	70)
	(5064,	70)
	(5065,	70)
	(5066,	70)
	(5067,	71)
	(5068,	71)
	(5069,	73)
	(5070,	75)
	(5071,	75)
	(5072,	75)
	(5073,	76)
	(5074,	76)
	(5075,	76)
	(5076,	76)
	(5077,	76)
	(5078,	76)
	(5079,	76)
	(5080,	76)
	(5081,	76)
	(5082,	76)
	(5083,	76)
	(5084,	76)
	(5085,	78)
	(5086,	79)
	(5087,	79)
	(5088,	80)
	(5089,	80)
	(5090,	80)
	(5091,	81)
	(5092,	83)
	(5093,	83)
	(5094,	83)
	(5095,	83)
	(5096,	83)
	(5097,	83)
	(5098,	83)
	(5099,	84)
	(5100,	84)
	(5110,	86)
	(5120,	92)
	(5130,	95)
	(5140,	105)
	(5150,	106)
	(5160,	109)
	(5170,	116)
	(5180,	123)
	(5190,	127)
	(5200,	130)
	(5210,	131)
	(5220,	138)
	(5230,	143)
	(5240,	146)
	(5250,	152)
	(5260,	161)
	(5270,	171)
	(5280,	171)
	(5290,	176)
	(5300,	186)
	(5310,	195)
	(5320,	199)
	(5330,	204)
	(5340,	211)
	(5350,	219)
	(5360,	227)
	(5370,	229)
	(5380,	230)
	(5390,	233)
	(5400,	240)
	(5410,	241)
	(5420,	249)
	(5430,	251)
	(5440,	253)
	(5450,	259)
	(5460,	263)
	(5470,	272)
	(5480,	278)
	(5490,	285)
	(5500,	289)
	(5510,	289)
	(5520,	294)
	(5530,	299)
	(5540,	307)
	(5550,	307)
	(5560,	311)
	(5570,	316)
	(5580,	320)
	(5590,	332)
	(5600,	334)
	(5610,	341)
	(5620,	347)
	(5630,	352)
	(5640,	354)
	(5650,	358)
	(5660,	358)
	(5670,	366)
	(5680,	370)
	(5690,	370)
	(5700,	375)
	(5710,	383)
	(5720,	389)
	(5730,	395)
	(5740,	401)
	(5750,	406)
	(5760,	412)
	(5770,	421)
	(5780,	424)
	(5790,	426)
	(5800,	432)
	(5810,	439)
	(5820,	441)
	(5830,	442)
	(5840,	444)
	(5850,	456)
	(5860,	460)
	(5870,	461)
	(5880,	471)
	(5890,	474)
	(5900,	477)
	(5910,	479)
	(5920,	481)
	(5930,	488)
	(5940,	490)
	(5950,	493)
	(5960,	500)
	(5970,	506)
	(5980,	511)
	(5990,	514)
	(6000,	518)
	(6010,	524)
	(6020,	526)
	(6030,	529)
	(6040,	534)
	(6050,	540)
	(6060,	547)
	(6070,	550)
	(6080,	551)
	(6090,	557)
	(6100,	560)
	(6110,	567)
	(6120,	571)
	(6130,	573)
	(6140,	577)
	(6150,	581)
	(6160,	586)
	(6170,	600)
	(6180,	609)
	(6190,	620)
	(6200,	624)
	(6210,	632)
	(6220,	637)
	(6230,	639)
	(6240,	643)
	(6250,	648)
	(6260,	656)
	(6270,	661)
	(6280,	664)
	(6290,	670)
	(6300,	673)
	(6310,	676)
	(6320,	685)
	(6330,	690)
	(6340,	693)
	(6350,	697)
	(6360,	704)
	(6370,	706)
	(6380,	711)
	(6390,	714)
	(6400,	717)
	(6410,	718)
	(6420,	723)
	(6430,	732)
	(6440,	733)
	(6450,	740)
	(6460,	742)
	(6470,	746)
	(6480,	750)
	(6490,	753)
	(6500,	758)
	(6510,	767)
	(6520,	775)
	(6530,	781)
	(6540,	783)
	(6550,	785)
	(6560,	787)
	(6570,	792)
	(6580,	801)
	(6590,	807)
	(6600,	810)
	(6610,	814)
	(6620,	819)
	(6630,	827)
	(6640,	831)
	(6650,	835)
	(6660,	838)
	(6670,	845)
	(6680,	849)
	(6690,	853)
	(6700,	858)
	(6710,	861)
	(6720,	864)
	(6730,	867)
	(6740,	869)
	(6750,	877)
	(6760,	886)
	(6770,	894)
	(6780,	894)
	(6790,	898)
	(6800,	899)
	(6810,	902)
	(6820,	909)
	(6830,	911)
	(6840,	918)
	(6850,	925)
	(6860,	929)
	(6870,	933)
	(6880,	939)
	(6890,	946)
	(6900,	953)
	(6910,	958)
	(6920,	969)
	(6930,	973)
	(6940,	976)
	(6950,	977)
	(6960,	986)
	(6970,	992)
	(6980,	999)
	(6990,	1002)
	(7000,	1008)
	(7010,	1011)
	(7020,	1016)
	(7030,	1020)
	(7040,	1025)
	(7050,	1030)
	(7060,	1035)
	(7070,	1037)
	(7080,	1041)
	(7090,	1046)
	(7100,	1061)
	(7110,	1063)
	(7120,	1074)
	(7130,	1080)
	(7140,	1085)
	(7150,	1088)
	(7160,	1095)
	(7170,	1107)
	(7180,	1109)
	(7190,	1115)
	(7200,	1116)
	(7210,	1124)
	(7220,	1126)
	(7230,	1139)
	(7240,	1152)
	(7250,	1159)
	(7260,	1162)
	(7270,	1169)
	(7280,	1171)
	(7290,	1177)
	(7300,	1181)
	(7310,	1184)
	(7320,	1186)
	(7330,	1189)
	(7340,	1195)
	(7350,	1196)
	(7360,	1204)
	(7370,	1209)
	(7380,	1213)
	(7390,	1221)
	(7400,	1221)
	(7410,	1224)
	(7420,	1228)
	(7430,	1231)
	(7440,	1247)
	(7450,	1250)
	(7460,	1251)
	(7470,	1252)
	(7480,	1258)
	(7490,	1269)
	(7500,	1275)
	(7510,	1283)
	(7520,	1286)
	(7530,	1289)
	(7540,	1294)
	(7550,	1303)
	(7560,	1304)
	(7570,	1307)
	(7580,	1311)
	(7590,	1320)
	(7600,	1328)
	(7610,	1333)
	(7620,	1343)
	(7630,	1346)
	(7640,	1348)
	(7650,	1355)
	(7660,	1359)
	(7670,	1370)
	(7680,	1377)
	(7690,	1380)
	(7700,	1386)
	(7710,	1394)
	(7720,	1400)
	(7730,	1404)
	(7740,	1410)
	(7750,	1417)
	(7760,	1422)
	(7770,	1429)
	(7780,	1432)
	(7790,	1435)
	(7800,	1440)
	(7810,	1448)
	(7820,	1452)
	(7830,	1458)
	(7840,	1459)
	(7850,	1465)
	(7860,	1471)
	(7870,	1475)
	(7880,	1480)
	(7890,	1482)
	(7900,	1483)
	(7910,	1491)
	(7920,	1501)
	(7930,	1509)
	(7940,	1516)
	(7950,	1527)
	(7960,	1529)
	(7970,	1534)
	(7980,	1551)
	(7990,	1561)
	(8000,	1573)
	(8010,	1577)
	(8020,	1579)
	(8030,	1584)
	(8040,	1589)
	(8050,	1594)
	(8060,	1597)
	(8070,	1601)
	(8080,	1606)
	(8090,	1609)
	(8100,	1614)
	(8110,	1619)
	(8120,	1623)
	(8130,	1630)
	(8140,	1642)
	(8150,	1644)
	(8160,	1647)
	(8170,	1654)
	(8180,	1661)
	(8190,	1666)
	(8200,	1672)
	(8210,	1675)
	(8220,	1677)
	(8230,	1690)
	(8240,	1692)
	(8250,	1699)
	(8260,	1704)
	(8270,	1710)
	(8280,	1718)
	(8290,	1723)
	(8300,	1724)
	(8310,	1727)
	(8320,	1729)
	(8330,	1734)
	(8340,	1741)
	(8350,	1747)
	(8360,	1757)
	(8370,	1758)
	(8380,	1761)
	(8390,	1765)
	(8400,	1769)
	(8410,	1775)
	(8420,	1783)
	(8430,	1784)
	(8440,	1790)
	(8450,	1794)
	(8460,	1795)
	(8470,	1802)
	(8480,	1804)
	(8490,	1806)
	(8500,	1814)
	(8510,	1819)
	(8520,	1822)
	(8530,	1827)
	(8540,	1831)
	(8550,	1833)
	(8560,	1836)
	(8570,	1837)
	(8580,	1842)
	(8590,	1855)
	(8600,	1859)
	(8601,	1859)
	(8602,	1859)
	(8603,	1859)
	(8604,	1859)
	(8605,	1859)
	(8606,	1859)
	(8607,	1859)
	(8608,	1860)
	(8609,	1860)
	(8610,	1861)
	(8611,	1861)
	(8612,	1861)
	(8613,	1861)
	(8614,	1861)
	(8615,	1861)
	(8616,	1861)
	(8617,	1861)
	(8618,	1861)
	(8619,	1861)
	(8620,	1862)
	(8621,	1862)
	(8622,	1862)
	(8623,	1863)
	(8624,	1863)
	(8625,	1863)
	(8626,	1864)
	(8627,	1865)
	(8628,	1865)
	(8629,	1870)
	(8630,	1870)
	(8631,	1871)
	(8632,	1873)
	(8633,	1874)
	(8634,	1874)
	(8635,	1874)
	(8636,	1877)
	(8637,	1877)
	(8638,	1877)
	(8639,	1877)
	(8640,	1877)
	(8641,	1878)
	(8642,	1878)
	(8643,	1878)
	(8644,	1878)
	(8645,	1878)
	(8646,	1878)
	(8647,	1878)
	(8648,	1878)
	(8649,	1878)
	(8650,	1878)
	(8651,	1878)
	(8652,	1878)
	(8653,	1878)
	(8654,	1879)
	(8655,	1880)
	(8656,	1881)
	(8657,	1881)
	(8658,	1881)
	(8659,	1881)
	(8660,	1881)
	(8661,	1881)
	(8662,	1881)
	(8663,	1881)
	(8664,	1881)
	(8665,	1882)
	(8666,	1882)
	(8667,	1882)
	(8668,	1882)
	(8669,	1882)
	(8670,	1882)
	(8671,	1882)
	(8672,	1882)
	(8673,	1882)
	(8674,	1882)
	(8675,	1882)
	(8676,	1882)
	(8677,	1882)
	(8678,	1883)
	(8679,	1883)
	(8680,	1883)
	(8681,	1883)
	(8682,	1884)
	(8683,	1885)
	(8684,	1885)
	(8685,	1886)
	(8686,	1886)
	(8687,	1886)
	(8688,	1886)
	(8689,	1888)
	(8690,	1890)
	(8691,	1890)
	(8692,	1890)
	(8693,	1890)
	(8694,	1891)
	(8695,	1891)
	(8696,	1891)
	(8697,	1892)
	(8698,	1897)
	(8699,	1899)
	(8700,	1899)
	(8701,	1900)
	(8702,	1901)
	(8703,	1901)
	(8704,	1901)
	(8705,	1901)
	(8706,	1901)
	(8707,	1901)
	(8708,	1902)
	(8709,	1904)
	(8710,	1905)
	(8711,	1907)
	(8712,	1909)
	(8713,	1909)
	(8714,	1909)
	(8715,	1910)
	(8716,	1910)
	(8717,	1911)
	(8718,	1912)
	(8719,	1912)
	(8720,	1915)
	(8721,	1915)
	(8722,	1916)
	(8723,	1916)
	(8724,	1916)
	(8725,	1916)
	(8726,	1916)
	(8727,	1916)
	(8728,	1916)
	(8729,	1918)
	(8730,	1918)
	(8731,	1920)
	(8732,	1920)
	(8733,	1920)
	(8734,	1920)
	(8735,	1920)
	(8736,	1920)
	(8737,	1920)
	(8738,	1920)
	(8739,	1920)
	(8740,	1920)
	(8741,	1921)
	(8742,	1921)
	(8743,	1921)
	(8744,	1921)
	(8745,	1922)
	(8746,	1922)
	(8747,	1922)
	(8748,	1922)
	(8749,	1922)
	(8750,	1922)
	(8751,	1925)
	(8752,	1925)
	(8753,	1925)
	(8754,	1928)
	(8755,	1928)
	(8756,	1931)
	(8757,	1931)
	(8758,	1933)
	(8759,	1934)
	(8760,	1934)
	(8761,	1934)
	(8762,	1934)
	(8763,	1934)
	(8764,	1936)
	(8765,	1938)
	(8766,	1938)
	(8767,	1938)
	(8768,	1938)
	(8769,	1938)
	(8770,	1939)
	(8771,	1940)
	(8772,	1940)
	(8773,	1941)
	(8774,	1941)
	(8775,	1942)
	(8776,	1942)
	(8777,	1942)
	(8778,	1942)
	(8779,	1942)
	(8780,	1942)
	(8781,	1942)
	(8782,	1942)
	(8783,	1942)
	(8784,	1942)
	(8785,	1942)
	(8786,	1942)
	(8787,	1942)
	(8788,	1942)
	(8789,	1942)
	(8790,	1942)
	(8791,	1942)
	(8792,	1943)
	(8793,	1947)
	(8794,	1947)
	(8795,	1947)
	(8796,	1947)
	(8797,	1949)
	(8798,	1950)
	(8799,	1950)
	(8800,	1950)
	(8801,	1950)
	(8802,	1950)
	(8803,	1950)
	(8804,	1950)
	(8805,	1950)
	(8806,	1950)
	(8807,	1950)
	(8808,	1950)
	(8809,	1950)
	(8810,	1950)
	(8811,	1950)
	(8812,	1950)
	(8813,	1950)
	(8814,	1950)
	(8815,	1950)
	(8816,	1951)
	(8817,	1951)
	(8818,	1956)
	(8819,	1958)
	(8820,	1958)
	(8821,	1958)
	(8822,	1958)
	(8823,	1958)
	(8824,	1958)
	(8825,	1958)
	(8826,	1961)
	(8827,	1962)
	(8828,	1962)
	(8829,	1964)
	(8830,	1965)
	(8831,	1965)
	(8832,	1965)
	(8833,	1965)
	(8834,	1965)
	(8835,	1965)
	(8836,	1965)
	(8837,	1966)
	(8838,	1966)
	(8839,	1966)
	(8840,	1966)
	(8841,	1966)
	(8842,	1966)
	(8843,	1966)
	(8844,	1968)
	(8845,	1969)
	(8846,	1969)
	(8847,	1969)
	(8848,	1969)
	(8849,	1972)
	(8850,	1972)
	(8851,	1978)
	(8852,	1978)
	(8853,	1979)
	(8854,	1979)
	(8855,	1981)
	(8856,	1981)
	(8857,	1981)
	(8858,	1982)
	(8859,	1983)
	(8860,	1983)
	(8861,	1983)
	(8862,	1983)
	(8863,	1983)
	(8864,	1983)
	(8865,	1984)
	(8866,	1984)
	(8867,	1984)
	(8868,	1985)
	(8869,	1988)
	(8870,	1989)
	(8871,	1991)
	(8872,	1991)
	(8873,	1991)
	(8874,	1991)
	(8875,	1990)
	(8876,	1989)
	(8877,	1988)
	(8878,	1988)
	(8879,	1987)
	(8880,	1986)
	(8881,	1987)
	(8882,	1986)
	(8883,	1986)
	(8884,	1985)
	(8885,	1984)
	(8886,	1983)
	(8887,	1982)
	(8888,	1981)
	(8889,	1982)
	(8890,	1982)
	(8891,	1983)
	(8892,	1982)
	(8893,	1982)
	(8894,	1981)
	(8895,	1980)
	(8896,	1981)
	(8897,	1980)
	(8898,	1979)
	(8899,	1979)
	(8900,	1978)
	(8901,	1978)
	(8902,	1979)
	(8903,	1978)
	(8904,	1978)
	(8905,	1978)
	(8906,	1978)
	(8907,	1978)
	(8908,	1977)
	(8909,	1976)
	(8910,	1975)
	(8911,	1974)
	(8912,	1973)
	(8913,	1972)
	(8914,	1971)
	(8915,	1971)
	(8916,	1972)
	(8917,	1972)
	(8918,	1971)
	(8919,	1970)
	(8920,	1971)
	(8921,	1970)
	(8922,	1969)
	(8923,	1970)
	(8924,	1969)
	(8925,	1969)
	(8926,	1968)
	(8927,	1967)
	(8928,	1968)
	(8929,	1967)
	(8930,	1966)
	(8931,	1965)
	(8932,	1968)
	(8933,	1967)
	(8934,	1966)
	(8935,	1965)
	(8936,	1965)
	(8937,	1964)
	(8938,	1964)
	(8939,	1963)
	(8940,	1963)
	(8941,	1962)
	(8942,	1961)
	(8943,	1960)
	(8944,	1959)
	(8945,	1959)
	(8946,	1958)
	(8947,	1957)
	(8948,	1957)
	(8949,	1956)
	(8950,	1955)
	(8951,	1954)
	(8952,	1954)
	(8953,	1953)
	(8954,	1952)
	(8955,	1951)
	(8956,	1950)
	(8957,	1951)
	(8958,	1951)
	(8959,	1950)
	(8960,	1950)
	(8961,	1950)
	(8962,	1949)
	(8963,	1948)
	(8964,	1947)
	(8965,	1946)
	(8966,	1948)
	(8967,	1947)
	(8968,	1946)
	(8969,	1945)
	(8970,	1947)
	(8971,	1946)
	(8972,	1946)
	(8973,	1945)
	(8974,	1944)
	(8975,	1944)
	(8976,	1943)
	(8977,	1942)
	(8978,	1941)
	(8979,	1940)
	(8980,	1939)
	(8981,	1938)
	(8982,	1937)
	(8983,	1938)
	(8984,	1938)
	(8985,	1938)
	(8986,	1938)
	(8987,	1937)
	(8988,	1937)
	(8989,	1936)
	(8990,	1935)
	(8991,	1936)
	(8992,	1935)
	(8993,	1935)
	(8994,	1935)
	(8995,	1934)
	(8996,	1933)
	(8997,	1933)
	(8998,	1932)
	(8999,	1931)
	(9000,	1930)
	(9010,	1928)
	(9020,	1919)
	(9030,	1914)
	(9040,	1912)
	(9050,	1903)
	(9060,	1901)
	(9070,	1895)
	(9080,	1895)
	(9090,	1887)
	(9100,	1880)
	(9110,	1872)
	(9120,	1864)
	(9130,	1857)
	(9140,	1853)
	(9150,	1851)
	(9160,	1845)
	(9170,	1840)
	(9180,	1834)
	(9190,	1830)
	(9200,	1825)
	(9210,	1819)
	(9220,	1816)
	(9230,	1808)
	(9240,	1807)
	(9250,	1798)
	(9260,	1794)
	(9270,	1792)
	(9280,	1784)
	(9290,	1779)
	(9300,	1774)
	(9310,	1771)
	(9320,	1767)
	(9330,	1765)
	(9340,	1759)
	(9350,	1753)
	(9360,	1752)
	(9370,	1748)
	(9380,	1744)
	(9390,	1738)
	(9400,	1732)
	(9410,	1724)
	(9420,	1717)
	(9430,	1711)
	(9440,	1702)
	(9450,	1696)
	(9460,	1691)
	(9470,	1687)
	(9480,	1683)
	(9490,	1677)
	(9500,	1671)
	(9510,	1665)
	(9520,	1665)
	(9530,	1665)
	(9540,	1661)
	(9550,	1656)
	(9560,	1650)
	(9570,	1653)
	(9580,	1649)
	(9590,	1646)
	(9600,	1643)
	(9610,	1639)
	(9620,	1634)
	(9630,	1634)
	(9640,	1631)
	(9650,	1624)
	(9660,	1615)
	(9670,	1609)
	(9680,	1606)
	(9690,	1606)
	(9700,	1607)
	(9710,	1599)
	(9720,	1591)
	(9730,	1586)
	(9740,	1581)
	(9750,	1571)
	(9760,	1568)
	(9770,	1562)
	(9780,	1557)
	(9790,	1551)
	(9800,	1546)
	(9810,	1544)
	(9820,	1537)
	(9830,	1530)
	(9840,	1525)
	(9850,	1522)
	(9860,	1513)
	(9870,	1507)
	(9880,	1500)
	(9890,	1497)
	(9900,	1495)
	(9910,	1491)
	(9920,	1484)
	(9930,	1477)
	(9940,	1471)
	(9950,	1463)
	(9960,	1456)
	(9970,	1449)
	(9980,	1444)
	(9990,	1438)
	(10000,	1430)
};
\addplot[color=blue, mark=none, line width=10pt, smooth] plot coordinates {
	(0,	1539)
	(10,	1543)
	(20,	1548)
	(30,	1553)
	(40,	1554)
	(50,	1554)
	(60,	1557)
	(70,	1562)
	(80,	1569)
	(90,	1579)
	(100,	1585)
	(110,	1591)
	(120,	1595)
	(130,	1600)
	(140,	1610)
	(150,	1612)
	(160,	1614)
	(170,	1624)
	(180,	1635)
	(190,	1636)
	(200,	1638)
	(210,	1641)
	(220,	1646)
	(230,	1653)
	(240,	1655)
	(250,	1661)
	(260,	1663)
	(270,	1667)
	(280,	1671)
	(290,	1679)
	(300,	1683)
	(310,	1692)
	(320,	1698)
	(330,	1702)
	(340,	1714)
	(350,	1719)
	(360,	1720)
	(370,	1724)
	(380,	1727)
	(390,	1731)
	(400,	1738)
	(410,	1744)
	(420,	1749)
	(430,	1753)
	(440,	1759)
	(450,	1762)
	(460,	1768)
	(470,	1769)
	(480,	1771)
	(490,	1778)
	(500,	1780)
	(510,	1783)
	(520,	1785)
	(530,	1789)
	(540,	1793)
	(550,	1799)
	(560,	1802)
	(570,	1811)
	(580,	1821)
	(590,	1822)
	(600,	1823)
	(610,	1825)
	(620,	1827)
	(630,	1835)
	(640,	1836)
	(650,	1838)
	(660,	1844)
	(670,	1851)
	(680,	1856)
	(690,	1856)
	(700,	1861)
	(710,	1866)
	(720,	1869)
	(730,	1877)
	(740,	1883)
	(750,	1888)
	(760,	1894)
	(770,	1898)
	(780,	1898)
	(790,	1910)
	(800,	1912)
	(801,	1912)
	(802,	1912)
	(803,	1912)
	(804,	1913)
	(805,	1913)
	(806,	1915)
	(807,	1915)
	(808,	1915)
	(809,	1915)
	(810,	1915)
	(811,	1916)
	(812,	1916)
	(813,	1916)
	(814,	1916)
	(815,	1916)
	(816,	1916)
	(817,	1917)
	(818,	1917)
	(819,	1920)
	(820,	1920)
	(821,	1920)
	(822,	1922)
	(823,	1922)
	(824,	1922)
	(825,	1922)
	(826,	1924)
	(827,	1925)
	(828,	1928)
	(829,	1928)
	(830,	1928)
	(831,	1928)
	(832,	1929)
	(833,	1930)
	(834,	1931)
	(835,	1931)
	(836,	1931)
	(837,	1932)
	(838,	1932)
	(839,	1932)
	(840,	1933)
	(841,	1933)
	(842,	1933)
	(843,	1934)
	(844,	1935)
	(845,	1936)
	(846,	1936)
	(847,	1936)
	(848,	1937)
	(849,	1937)
	(850,	1937)
	(851,	1937)
	(852,	1938)
	(853,	1938)
	(854,	1938)
	(855,	1939)
	(856,	1939)
	(857,	1939)
	(858,	1940)
	(859,	1941)
	(860,	1941)
	(861,	1942)
	(862,	1942)
	(863,	1943)
	(864,	1943)
	(865,	1943)
	(866,	1943)
	(867,	1943)
	(868,	1943)
	(869,	1944)
	(870,	1944)
	(871,	1945)
	(872,	1945)
	(873,	1946)
	(874,	1946)
	(875,	1946)
	(876,	1946)
	(877,	1946)
	(878,	1946)
	(879,	1946)
	(880,	1946)
	(881,	1947)
	(882,	1951)
	(883,	1951)
	(884,	1951)
	(885,	1952)
	(886,	1953)
	(887,	1954)
	(888,	1955)
	(889,	1956)
	(890,	1956)
	(891,	1957)
	(892,	1958)
	(893,	1959)
	(894,	1959)
	(895,	1959)
	(896,	1959)
	(897,	1959)
	(898,	1959)
	(899,	1959)
	(900,	1959)
	(901,	1959)
	(902,	1961)
	(903,	1964)
	(904,	1964)
	(905,	1965)
	(906,	1965)
	(907,	1965)
	(908,	1966)
	(909,	1966)
	(910,	1966)
	(911,	1966)
	(912,	1966)
	(913,	1966)
	(914,	1967)
	(915,	1968)
	(916,	1968)
	(917,	1968)
	(918,	1968)
	(919,	1968)
	(920,	1970)
	(921,	1972)
	(922,	1973)
	(923,	1973)
	(924,	1973)
	(925,	1973)
	(926,	1973)
	(927,	1974)
	(928,	1974)
	(929,	1974)
	(930,	1974)
	(931,	1975)
	(932,	1975)
	(933,	1975)
	(934,	1975)
	(935,	1976)
	(936,	1976)
	(937,	1976)
	(938,	1977)
	(939,	1979)
	(940,	1982)
	(941,	1982)
	(942,	1982)
	(943,	1983)
	(944,	1983)
	(945,	1983)
	(946,	1985)
	(947,	1985)
	(948,	1985)
	(949,	1985)
	(950,	1986)
	(951,	1986)
	(952,	1986)
	(953,	1987)
	(954,	1987)
	(955,	1987)
	(956,	1988)
	(957,	1988)
	(958,	1988)
	(959,	1988)
	(960,	1988)
	(961,	1988)
	(962,	1989)
	(963,	1989)
	(964,	1989)
	(965,	1989)
	(966,	1990)
	(967,	1990)
	(968,	1992)
	(969,	1993)
	(970,	1994)
	(971,	1994)
	(972,	1996)
	(973,	1996)
	(974,	1996)
	(975,	1996)
	(976,	1996)
	(977,	1996)
	(978,	1997)
	(979,	1999)
	(980,	1999)
	(981,	1999)
	(982,	1999)
	(983,	1999)
	(984,	2000)
	(985,	2000)
	(986,	2000)
	(987,	2000)
	(988,	2001)
	(989,	2001)
	(990,	2001)
	(991,	2002)
	(992,	2002)
	(993,	2002)
	(994,	2004)
	(995,	2004)
	(996,	2005)
	(997,	2005)
	(998,	2005)
	(999,	2006)
	(1000,	2006)
	(1001,	2006)
	(1002,	2006)
	(1003,	2006)
	(1004,	2006)
	(1005,	2006)
	(1006,	2006)
	(1007,	2006)
	(1008,	2006)
	(1009,	2007)
	(1010,	2007)
	(1011,	2007)
	(1012,	2007)
	(1013,	2008)
	(1014,	2009)
	(1015,	2010)
	(1016,	2010)
	(1017,	2012)
	(1018,	2012)
	(1019,	2012)
	(1020,	2015)
	(1021,	2015)
	(1022,	2015)
	(1023,	2017)
	(1024,	2019)
	(1025,	2020)
	(1026,	2020)
	(1027,	2020)
	(1028,	2020)
	(1029,	2020)
	(1030,	2020)
	(1031,	2020)
	(1032,	2020)
	(1033,	2021)
	(1034,	2021)
	(1035,	2021)
	(1036,	2021)
	(1037,	2022)
	(1038,	2022)
	(1039,	2023)
	(1040,	2023)
	(1041,	2023)
	(1042,	2023)
	(1043,	2023)
	(1044,	2023)
	(1045,	2024)
	(1046,	2024)
	(1047,	2026)
	(1048,	2026)
	(1049,	2025)
	(1050,	2026)
	(1051,	2025)
	(1052,	2024)
	(1053,	2023)
	(1054,	2022)
	(1055,	2021)
	(1056,	2022)
	(1057,	2021)
	(1058,	2020)
	(1059,	2019)
	(1060,	2018)
	(1061,	2020)
	(1062,	2019)
	(1063,	2020)
	(1064,	2019)
	(1065,	2018)
	(1066,	2021)
	(1067,	2020)
	(1068,	2019)
	(1069,	2018)
	(1070,	2017)
	(1071,	2016)
	(1072,	2016)
	(1073,	2015)
	(1074,	2014)
	(1075,	2015)
	(1076,	2014)
	(1077,	2016)
	(1078,	2015)
	(1079,	2014)
	(1080,	2013)
	(1081,	2012)
	(1082,	2011)
	(1083,	2010)
	(1084,	2009)
	(1085,	2008)
	(1086,	2008)
	(1087,	2007)
	(1088,	2006)
	(1089,	2005)
	(1090,	2004)
	(1091,	2003)
	(1092,	2002)
	(1093,	2001)
	(1094,	2000)
	(1095,	1999)
	(1096,	1998)
	(1097,	1997)
	(1098,	1997)
	(1099,	1997)
	(1100,	1996)
	(1101,	1995)
	(1102,	1994)
	(1103,	1993)
	(1104,	1992)
	(1105,	1991)
	(1106,	1990)
	(1107,	1989)
	(1108,	1988)
	(1109,	1987)
	(1110,	1987)
	(1111,	1986)
	(1112,	1987)
	(1113,	1987)
	(1114,	1987)
	(1115,	1986)
	(1116,	1985)
	(1117,	1986)
	(1118,	1986)
	(1119,	1985)
	(1120,	1984)
	(1121,	1983)
	(1122,	1983)
	(1123,	1984)
	(1124,	1983)
	(1125,	1983)
	(1126,	1982)
	(1127,	1981)
	(1128,	1980)
	(1129,	1979)
	(1130,	1980)
	(1131,	1979)
	(1132,	1978)
	(1133,	1977)
	(1134,	1976)
	(1135,	1975)
	(1136,	1974)
	(1137,	1974)
	(1138,	1975)
	(1139,	1975)
	(1140,	1974)
	(1141,	1973)
	(1142,	1972)
	(1143,	1971)
	(1144,	1970)
	(1145,	1969)
	(1146,	1968)
	(1147,	1967)
	(1148,	1966)
	(1149,	1965)
	(1150,	1965)
	(1151,	1964)
	(1152,	1965)
	(1153,	1965)
	(1154,	1964)
	(1155,	1963)
	(1156,	1963)
	(1157,	1962)
	(1158,	1962)
	(1159,	1961)
	(1160,	1961)
	(1161,	1960)
	(1162,	1960)
	(1163,	1959)
	(1164,	1958)
	(1165,	1957)
	(1166,	1957)
	(1167,	1958)
	(1168,	1958)
	(1169,	1958)
	(1170,	1959)
	(1171,	1958)
	(1172,	1957)
	(1173,	1956)
	(1174,	1956)
	(1175,	1955)
	(1176,	1954)
	(1177,	1953)
	(1178,	1952)
	(1179,	1951)
	(1180,	1950)
	(1181,	1949)
	(1182,	1949)
	(1183,	1953)
	(1184,	1952)
	(1185,	1954)
	(1186,	1954)
	(1187,	1953)
	(1188,	1956)
	(1189,	1958)
	(1190,	1957)
	(1191,	1956)
	(1192,	1955)
	(1193,	1955)
	(1194,	1954)
	(1195,	1953)
	(1196,	1952)
	(1197,	1951)
	(1198,	1950)
	(1199,	1950)
	(1200,	1951)
	(1210,	1947)
	(1220,	1939)
	(1230,	1930)
	(1240,	1925)
	(1250,	1923)
	(1260,	1921)
	(1270,	1919)
	(1280,	1913)
	(1290,	1907)
	(1300,	1901)
	(1310,	1904)
	(1320,	1898)
	(1330,	1896)
	(1340,	1890)
	(1350,	1886)
	(1360,	1878)
	(1370,	1875)
	(1380,	1872)
	(1390,	1863)
	(1400,	1860)
	(1410,	1856)
	(1420,	1853)
	(1430,	1850)
	(1440,	1843)
	(1450,	1840)
	(1460,	1832)
	(1470,	1824)
	(1480,	1817)
	(1490,	1812)
	(1500,	1805)
	(1510,	1803)
	(1520,	1798)
	(1530,	1792)
	(1540,	1790)
	(1550,	1782)
	(1560,	1780)
	(1570,	1773)
	(1580,	1767)
	(1590,	1766)
	(1600,	1761)
	(1610,	1753)
	(1620,	1749)
	(1630,	1742)
	(1640,	1735)
	(1650,	1733)
	(1660,	1727)
	(1670,	1722)
	(1680,	1719)
	(1690,	1716)
	(1700,	1711)
	(1710,	1705)
	(1720,	1697)
	(1730,	1694)
	(1740,	1685)
	(1750,	1678)
	(1760,	1671)
	(1770,	1663)
	(1780,	1655)
	(1790,	1650)
	(1800,	1644)
	(1810,	1641)
	(1820,	1635)
	(1830,	1630)
	(1840,	1627)
	(1850,	1622)
	(1860,	1615)
	(1870,	1612)
	(1880,	1605)
	(1890,	1598)
	(1900,	1591)
	(1910,	1587)
	(1920,	1581)
	(1930,	1574)
	(1940,	1569)
	(1950,	1567)
	(1960,	1564)
	(1970,	1562)
	(1980,	1552)
	(1990,	1545)
	(2000,	1536)
	(2010,	1527)
	(2020,	1524)
	(2030,	1520)
	(2040,	1512)
	(2050,	1504)
	(2060,	1496)
	(2070,	1497)
	(2080,	1489)
	(2090,	1484)
	(2100,	1477)
	(2110,	1472)
	(2120,	1465)
	(2130,	1457)
	(2140,	1449)
	(2150,	1445)
	(2160,	1440)
	(2170,	1436)
	(2180,	1436)
	(2190,	1434)
	(2200,	1432)
	(2210,	1424)
	(2220,	1418)
	(2230,	1409)
	(2240,	1407)
	(2250,	1405)
	(2260,	1397)
	(2270,	1389)
	(2280,	1383)
	(2290,	1375)
	(2300,	1374)
	(2310,	1366)
	(2320,	1363)
	(2330,	1358)
	(2340,	1352)
	(2350,	1346)
	(2360,	1342)
	(2370,	1337)
	(2380,	1335)
	(2390,	1331)
	(2400,	1326)
	(2410,	1324)
	(2420,	1318)
	(2430,	1321)
	(2440,	1313)
	(2450,	1303)
	(2460,	1298)
	(2470,	1293)
	(2480,	1287)
	(2490,	1281)
	(2500,	1275)
	(2510,	1269)
	(2520,	1270)
	(2530,	1263)
	(2540,	1255)
	(2550,	1249)
	(2560,	1240)
	(2570,	1232)
	(2580,	1225)
	(2590,	1218)
	(2600,	1217)
	(2610,	1212)
	(2620,	1205)
	(2630,	1201)
	(2640,	1193)
	(2650,	1188)
	(2660,	1178)
	(2670,	1174)
	(2680,	1175)
	(2690,	1169)
	(2700,	1161)
	(2710,	1165)
	(2720,	1158)
	(2730,	1155)
	(2740,	1150)
	(2750,	1144)
	(2760,	1137)
	(2770,	1134)
	(2780,	1131)
	(2790,	1123)
	(2800,	1118)
	(2810,	1108)
	(2820,	1104)
	(2830,	1096)
	(2840,	1092)
	(2850,	1084)
	(2860,	1079)
	(2870,	1074)
	(2880,	1073)
	(2890,	1070)
	(2900,	1060)
	(2910,	1058)
	(2920,	1055)
	(2930,	1049)
	(2940,	1045)
	(2950,	1038)
	(2960,	1034)
	(2970,	1031)
	(2980,	1024)
	(2990,	1018)
	(3000,	1012)
	(3010,	1004)
	(3020,	1002)
	(3030,	996)
	(3040,	993)
	(3050,	987)
	(3060,	984)
	(3070,	987)
	(3080,	987)
	(3090,	981)
	(3100,	971)
	(3110,	963)
	(3120,	955)
	(3130,	952)
	(3140,	947)
	(3150,	941)
	(3160,	931)
	(3170,	924)
	(3180,	920)
	(3190,	913)
	(3200,	906)
	(3210,	899)
	(3220,	890)
	(3230,	883)
	(3240,	874)
	(3250,	872)
	(3260,	866)
	(3270,	860)
	(3280,	853)
	(3290,	855)
	(3300,	847)
	(3310,	844)
	(3320,	838)
	(3330,	835)
	(3340,	829)
	(3350,	823)
	(3360,	815)
	(3370,	810)
	(3380,	804)
	(3390,	800)
	(3400,	794)
	(3410,	787)
	(3420,	782)
	(3430,	775)
	(3440,	770)
	(3450,	770)
	(3460,	764)
	(3470,	761)
	(3480,	754)
	(3490,	749)
	(3500,	745)
	(3510,	742)
	(3520,	736)
	(3530,	733)
	(3540,	726)
	(3550,	724)
	(3560,	716)
	(3570,	710)
	(3580,	709)
	(3590,	711)
	(3600,	708)
	(3610,	704)
	(3620,	703)
	(3630,	694)
	(3640,	689)
	(3650,	686)
	(3660,	679)
	(3670,	670)
	(3680,	663)
	(3690,	657)
	(3700,	649)
	(3710,	644)
	(3720,	639)
	(3730,	637)
	(3740,	629)
	(3750,	623)
	(3760,	617)
	(3770,	608)
	(3780,	601)
	(3790,	597)
	(3800,	593)
	(3810,	586)
	(3820,	579)
	(3830,	572)
	(3840,	567)
	(3850,	561)
	(3860,	556)
	(3870,	551)
	(3880,	544)
	(3890,	537)
	(3900,	533)
	(3910,	526)
	(3920,	518)
	(3930,	509)
	(3940,	504)
	(3950,	500)
	(3960,	497)
	(3970,	489)
	(3980,	480)
	(3990,	472)
	(4000,	469)
	(4010,	465)
	(4020,	458)
	(4030,	455)
	(4040,	447)
	(4050,	442)
	(4060,	438)
	(4070,	432)
	(4080,	424)
	(4090,	423)
	(4100,	417)
	(4110,	410)
	(4120,	408)
	(4130,	405)
	(4140,	402)
	(4150,	400)
	(4160,	395)
	(4170,	391)
	(4180,	382)
	(4190,	376)
	(4200,	370)
	(4210,	366)
	(4220,	365)
	(4230,	364)
	(4240,	363)
	(4250,	355)
	(4260,	350)
	(4270,	343)
	(4280,	340)
	(4290,	331)
	(4300,	324)
	(4310,	318)
	(4320,	310)
	(4330,	305)
	(4340,	308)
	(4350,	302)
	(4360,	296)
	(4370,	291)
	(4380,	284)
	(4390,	278)
	(4400,	279)
	(4410,	274)
	(4420,	271)
	(4430,	267)
	(4440,	259)
	(4450,	253)
	(4460,	245)
	(4470,	242)
	(4480,	240)
	(4490,	236)
	(4500,	234)
	(4510,	224)
	(4520,	220)
	(4530,	214)
	(4540,	204)
	(4550,	195)
	(4560,	191)
	(4570,	186)
	(4580,	181)
	(4590,	177)
	(4600,	174)
	(4610,	172)
	(4620,	166)
	(4630,	159)
	(4640,	154)
	(4650,	147)
	(4660,	139)
	(4670,	132)
	(4680,	137)
	(4690,	132)
	(4700,	125)
	(4701,	124)
	(4702,	123)
	(4703,	123)
	(4704,	122)
	(4705,	123)
	(4706,	122)
	(4707,	121)
	(4708,	120)
	(4709,	120)
	(4710,	123)
	(4711,	122)
	(4712,	121)
	(4713,	120)
	(4714,	120)
	(4715,	121)
	(4716,	120)
	(4717,	119)
	(4718,	118)
	(4719,	118)
	(4720,	117)
	(4721,	116)
	(4722,	115)
	(4723,	115)
	(4724,	114)
	(4725,	113)
	(4726,	112)
	(4727,	111)
	(4728,	111)
	(4729,	110)
	(4730,	111)
	(4731,	110)
	(4732,	111)
	(4733,	110)
	(4734,	110)
	(4735,	109)
	(4736,	108)
	(4737,	107)
	(4738,	106)
	(4739,	105)
	(4740,	104)
	(4741,	106)
	(4742,	106)
	(4743,	105)
	(4744,	108)
	(4745,	107)
	(4746,	106)
	(4747,	105)
	(4748,	104)
	(4749,	103)
	(4750,	102)
	(4751,	105)
	(4752,	105)
	(4753,	104)
	(4754,	106)
	(4755,	106)
	(4756,	108)
	(4757,	107)
	(4758,	107)
	(4759,	106)
	(4760,	105)
	(4761,	109)
	(4762,	108)
	(4763,	107)
	(4764,	106)
	(4765,	106)
	(4766,	105)
	(4767,	105)
	(4768,	104)
	(4769,	103)
	(4770,	103)
	(4771,	102)
	(4772,	101)
	(4773,	100)
	(4774,	99)
	(4775,	99)
	(4776,	99)
	(4777,	98)
	(4778,	97)
	(4779,	98)
	(4780,	98)
	(4781,	97)
	(4782,	96)
	(4783,	95)
	(4784,	94)
	(4785,	94)
	(4786,	94)
	(4787,	93)
	(4788,	92)
	(4789,	92)
	(4790,	92)
	(4791,	91)
	(4792,	92)
	(4793,	91)
	(4794,	90)
	(4795,	90)
	(4796,	91)
	(4797,	91)
	(4798,	90)
	(4799,	89)
	(4800,	90)
	(4801,	90)
	(4802,	89)
	(4803,	89)
	(4804,	88)
	(4805,	87)
	(4806,	88)
	(4807,	87)
	(4808,	86)
	(4809,	85)
	(4810,	85)
	(4811,	84)
	(4812,	83)
	(4813,	82)
	(4814,	81)
	(4815,	81)
	(4816,	81)
	(4817,	80)
	(4818,	79)
	(4819,	78)
	(4820,	77)
	(4821,	76)
	(4822,	75)
	(4823,	75)
	(4824,	74)
	(4825,	74)
	(4826,	73)
	(4827,	72)
	(4828,	73)
	(4829,	72)
	(4830,	71)
	(4831,	70)
	(4832,	70)
	(4833,	69)
	(4834,	68)
	(4835,	68)
	(4836,	67)
	(4837,	66)
	(4838,	65)
	(4839,	64)
	(4840,	63)
	(4841,	62)
	(4842,	61)
	(4843,	61)
	(4844,	60)
	(4845,	59)
	(4846,	58)
	(4847,	58)
	(4848,	57)
	(4849,	59)
	(4850,	58)
	(4851,	57)
	(4852,	56)
	(4853,	55)
	(4854,	54)
	(4855,	54)
	(4856,	53)
	(4857,	52)
	(4858,	51)
	(4859,	50)
	(4860,	49)
	(4861,	48)
	(4862,	47)
	(4863,	46)
	(4864,	45)
	(4865,	44)
	(4866,	43)
	(4867,	42)
	(4868,	41)
	(4869,	40)
	(4870,	39)
	(4871,	38)
	(4872,	37)
	(4873,	36)
	(4874,	35)
	(4875,	34)
	(4876,	33)
	(4877,	34)
	(4878,	34)
	(4879,	33)
	(4880,	32)
	(4881,	31)
	(4882,	30)
	(4883,	29)
	(4884,	28)
	(4885,	30)
	(4886,	29)
	(4887,	28)
	(4888,	27)
	(4889,	26)
	(4890,	25)
	(4891,	24)
	(4892,	23)
	(4893,	23)
	(4894,	22)
	(4895,	21)
	(4896,	20)
	(4897,	19)
	(4898,	18)
	(4899,	17)
	(4900,	17)
	(4901,	16)
	(4902,	15)
	(4903,	14)
	(4904,	13)
	(4905,	12)
	(4906,	11)
	(4907,	10)
	(4908,	11)
	(4909,	10)
	(4910,	9)
	(4911,	8)
	(4912,	8)
	(4913,	10)
	(4914,	9)
	(4915,	8)
	(4916,	7)
	(4917,	6)
	(4918,	5)
	(4919,	5)
	(4920,	5)
	(4921,	5)
	(4922,	4)
	(4923,	3)
	(4924,	4)
	(4925,	4)
	(4926,	5)
	(4927,	4)
	(4928,	3)
	(4929,	2)
	(4930,	2)
	(4931,	2)
	(4932,	2)
	(4933,	1)
	(4934,	0)
	(4935,	0)
	(4936,	2)
	(4937,	2)
	(4938,	3)
	(4939,	3)
	(4940,	3)
	(4941,	4)
	(4942,	5)
	(4943,	5)
	(4944,	5)
	(4945,	7)
	(4946,	7)
	(4947,	8)
	(4948,	10)
	(4949,	10)
	(4950,	10)
	(4951,	10)
	(4952,	11)
	(4953,	11)
	(4954,	11)
	(4955,	12)
	(4956,	12)
	(4957,	12)
	(4958,	12)
	(4959,	12)
	(4960,	12)
	(4961,	12)
	(4962,	12)
	(4963,	14)
	(4964,	15)
	(4965,	15)
	(4966,	15)
	(4967,	17)
	(4968,	22)
	(4969,	23)
	(4970,	25)
	(4971,	25)
	(4972,	26)
	(4973,	26)
	(4974,	28)
	(4975,	31)
	(4976,	31)
	(4977,	31)
	(4978,	31)
	(4979,	31)
	(4980,	31)
	(4981,	31)
	(4982,	31)
	(4983,	32)
	(4984,	32)
	(4985,	32)
	(4986,	32)
	(4987,	32)
	(4988,	35)
	(4989,	35)
	(4990,	35)
	(4991,	35)
	(4992,	35)
	(4993,	36)
	(4994,	37)
	(4995,	37)
	(4996,	37)
	(4997,	37)
	(4998,	37)
	(4999,	37)
	(5000,	40)
	(5001,	40)
	(5002,	42)
	(5003,	42)
	(5004,	42)
	(5005,	42)
	(5006,	43)
	(5007,	43)
	(5008,	43)
	(5009,	43)
	(5010,	46)
	(5011,	46)
	(5012,	46)
	(5013,	46)
	(5014,	47)
	(5015,	48)
	(5016,	49)
	(5017,	50)
	(5018,	50)
	(5019,	52)
	(5020,	52)
	(5021,	53)
	(5022,	53)
	(5023,	54)
	(5024,	54)
	(5025,	55)
	(5026,	55)
	(5027,	55)
	(5028,	55)
	(5029,	55)
	(5030,	55)
	(5031,	55)
	(5032,	56)
	(5033,	57)
	(5034,	57)
	(5035,	57)
	(5036,	58)
	(5037,	58)
	(5038,	59)
	(5039,	59)
	(5040,	59)
	(5041,	60)
	(5042,	60)
	(5043,	61)
	(5044,	61)
	(5045,	61)
	(5046,	62)
	(5047,	62)
	(5048,	64)
	(5049,	65)
	(5050,	66)
	(5051,	67)
	(5052,	68)
	(5053,	68)
	(5054,	68)
	(5055,	68)
	(5056,	69)
	(5057,	70)
	(5058,	71)
	(5059,	72)
	(5060,	73)
	(5061,	73)
	(5062,	73)
	(5063,	74)
	(5064,	74)
	(5065,	75)
	(5066,	75)
	(5067,	75)
	(5068,	75)
	(5069,	77)
	(5070,	78)
	(5071,	78)
	(5072,	79)
	(5073,	79)
	(5074,	80)
	(5075,	80)
	(5076,	80)
	(5077,	80)
	(5078,	80)
	(5079,	80)
	(5080,	80)
	(5081,	81)
	(5082,	81)
	(5083,	81)
	(5084,	81)
	(5085,	81)
	(5086,	81)
	(5087,	82)
	(5088,	82)
	(5089,	82)
	(5090,	82)
	(5091,	82)
	(5092,	82)
	(5093,	85)
	(5094,	85)
	(5095,	86)
	(5096,	86)
	(5097,	87)
	(5098,	89)
	(5099,	89)
	(5100,	89)
	(5110,	99)
	(5120,	103)
	(5130,	111)
	(5140,	120)
	(5150,	125)
	(5160,	131)
	(5170,	136)
	(5180,	147)
	(5190,	150)
	(5200,	157)
	(5210,	160)
	(5220,	163)
	(5230,	170)
	(5240,	172)
	(5250,	175)
	(5260,	179)
	(5270,	183)
	(5280,	188)
	(5290,	196)
	(5300,	203)
	(5310,	209)
	(5320,	218)
	(5330,	222)
	(5340,	225)
	(5350,	233)
	(5360,	237)
	(5370,	242)
	(5380,	248)
	(5390,	251)
	(5400,	257)
	(5410,	261)
	(5420,	263)
	(5430,	267)
	(5440,	270)
	(5450,	273)
	(5460,	277)
	(5470,	285)
	(5480,	293)
	(5490,	299)
	(5500,	306)
	(5510,	309)
	(5520,	315)
	(5530,	320)
	(5540,	325)
	(5550,	328)
	(5560,	329)
	(5570,	338)
	(5580,	343)
	(5590,	350)
	(5600,	355)
	(5610,	361)
	(5620,	369)
	(5630,	372)
	(5640,	379)
	(5650,	381)
	(5660,	393)
	(5670,	396)
	(5680,	401)
	(5690,	408)
	(5700,	411)
	(5710,	414)
	(5720,	417)
	(5730,	423)
	(5740,	425)
	(5750,	433)
	(5760,	436)
	(5770,	441)
	(5780,	445)
	(5790,	453)
	(5800,	460)
	(5810,	460)
	(5820,	469)
	(5830,	476)
	(5840,	484)
	(5850,	491)
	(5860,	494)
	(5870,	497)
	(5880,	505)
	(5890,	508)
	(5900,	512)
	(5910,	515)
	(5920,	519)
	(5930,	524)
	(5940,	527)
	(5950,	531)
	(5960,	533)
	(5970,	538)
	(5980,	545)
	(5990,	547)
	(6000,	549)
	(6010,	558)
	(6020,	569)
	(6030,	572)
	(6040,	579)
	(6050,	584)
	(6060,	589)
	(6070,	593)
	(6080,	597)
	(6090,	599)
	(6100,	604)
	(6110,	607)
	(6120,	613)
	(6130,	615)
	(6140,	621)
	(6150,	629)
	(6160,	633)
	(6170,	641)
	(6180,	642)
	(6190,	647)
	(6200,	652)
	(6210,	659)
	(6220,	674)
	(6230,	682)
	(6240,	686)
	(6250,	697)
	(6260,	698)
	(6270,	707)
	(6280,	714)
	(6290,	719)
	(6300,	730)
	(6310,	734)
	(6320,	745)
	(6330,	753)
	(6340,	759)
	(6350,	762)
	(6360,	762)
	(6370,	770)
	(6380,	775)
	(6390,	779)
	(6400,	784)
	(6410,	787)
	(6420,	791)
	(6430,	796)
	(6440,	797)
	(6450,	802)
	(6460,	805)
	(6470,	809)
	(6480,	811)
	(6490,	815)
	(6500,	816)
	(6510,	823)
	(6520,	825)
	(6530,	831)
	(6540,	842)
	(6550,	844)
	(6560,	848)
	(6570,	852)
	(6580,	857)
	(6590,	860)
	(6600,	860)
	(6610,	868)
	(6620,	875)
	(6630,	876)
	(6640,	881)
	(6650,	885)
	(6660,	891)
	(6670,	899)
	(6680,	905)
	(6690,	910)
	(6700,	912)
	(6710,	923)
	(6720,	927)
	(6730,	928)
	(6740,	931)
	(6750,	934)
	(6760,	939)
	(6770,	942)
	(6780,	947)
	(6790,	951)
	(6800,	957)
	(6810,	962)
	(6820,	964)
	(6830,	965)
	(6840,	968)
	(6850,	975)
	(6860,	980)
	(6870,	982)
	(6880,	989)
	(6890,	993)
	(6900,	997)
	(6910,	997)
	(6920,	998)
	(6930,	1000)
	(6940,	1005)
	(6950,	1010)
	(6960,	1016)
	(6970,	1018)
	(6980,	1021)
	(6990,	1025)
	(7000,	1030)
	(7010,	1035)
	(7020,	1044)
	(7030,	1046)
	(7040,	1053)
	(7050,	1055)
	(7060,	1058)
	(7070,	1066)
	(7080,	1075)
	(7090,	1079)
	(7100,	1083)
	(7110,	1088)
	(7120,	1090)
	(7130,	1095)
	(7140,	1104)
	(7150,	1108)
	(7160,	1114)
	(7170,	1120)
	(7180,	1127)
	(7190,	1135)
	(7200,	1140)
	(7210,	1145)
	(7220,	1155)
	(7230,	1158)
	(7240,	1164)
	(7250,	1171)
	(7260,	1177)
	(7270,	1184)
	(7280,	1187)
	(7290,	1191)
	(7300,	1196)
	(7310,	1202)
	(7320,	1206)
	(7330,	1211)
	(7340,	1214)
	(7350,	1217)
	(7360,	1222)
	(7370,	1229)
	(7380,	1232)
	(7390,	1242)
	(7400,	1246)
	(7410,	1253)
	(7420,	1264)
	(7430,	1265)
	(7440,	1272)
	(7450,	1273)
	(7460,	1276)
	(7470,	1281)
	(7480,	1287)
	(7490,	1293)
	(7500,	1295)
	(7510,	1300)
	(7520,	1302)
	(7530,	1316)
	(7540,	1322)
	(7550,	1328)
	(7560,	1334)
	(7570,	1340)
	(7580,	1347)
	(7590,	1356)
	(7600,	1363)
	(7610,	1366)
	(7620,	1371)
	(7630,	1380)
	(7640,	1384)
	(7650,	1388)
	(7660,	1393)
	(7670,	1397)
	(7680,	1398)
	(7690,	1401)
	(7700,	1404)
	(7710,	1409)
	(7720,	1416)
	(7730,	1418)
	(7740,	1424)
	(7750,	1427)
	(7760,	1428)
	(7770,	1429)
	(7780,	1432)
	(7790,	1433)
	(7800,	1440)
	(7810,	1442)
	(7820,	1447)
	(7830,	1450)
	(7840,	1454)
	(7850,	1460)
	(7860,	1462)
	(7870,	1468)
	(7880,	1474)
	(7890,	1475)
	(7900,	1478)
	(7910,	1483)
	(7920,	1487)
	(7930,	1491)
	(7940,	1496)
	(7950,	1500)
	(7960,	1505)
	(7970,	1507)
	(7980,	1511)
	(7990,	1517)
	(8000,	1519)
	(8010,	1525)
	(8020,	1527)
	(8030,	1531)
	(8040,	1539)
	(8050,	1542)
	(8060,	1550)
	(8070,	1557)
	(8080,	1563)
	(8090,	1571)
	(8100,	1576)
	(8110,	1584)
	(8120,	1588)
	(8130,	1596)
	(8140,	1602)
	(8150,	1612)
	(8160,	1626)
	(8170,	1629)
	(8180,	1632)
	(8190,	1639)
	(8200,	1644)
	(8210,	1649)
	(8220,	1653)
	(8230,	1655)
	(8240,	1658)
	(8250,	1660)
	(8260,	1664)
	(8270,	1666)
	(8280,	1674)
	(8290,	1682)
	(8300,	1684)
	(8310,	1692)
	(8320,	1701)
	(8330,	1707)
	(8340,	1709)
	(8350,	1714)
	(8360,	1718)
	(8370,	1723)
	(8380,	1728)
	(8390,	1731)
	(8400,	1736)
	(8410,	1742)
	(8420,	1745)
	(8430,	1746)
	(8440,	1749)
	(8450,	1755)
	(8460,	1765)
	(8470,	1772)
	(8480,	1775)
	(8490,	1775)
	(8500,	1780)
	(8510,	1784)
	(8520,	1788)
	(8530,	1794)
	(8540,	1802)
	(8550,	1805)
	(8560,	1813)
	(8570,	1818)
	(8580,	1825)
	(8590,	1826)
	(8600,	1841)
	(8601,	1842)
	(8602,	1843)
	(8603,	1845)
	(8604,	1846)
	(8605,	1846)
	(8606,	1846)
	(8607,	1847)
	(8608,	1847)
	(8609,	1847)
	(8610,	1848)
	(8611,	1849)
	(8612,	1849)
	(8613,	1851)
	(8614,	1851)
	(8615,	1851)
	(8616,	1852)
	(8617,	1852)
	(8618,	1852)
	(8619,	1853)
	(8620,	1853)
	(8621,	1853)
	(8622,	1854)
	(8623,	1855)
	(8624,	1855)
	(8625,	1858)
	(8626,	1858)
	(8627,	1858)
	(8628,	1858)
	(8629,	1859)
	(8630,	1859)
	(8631,	1859)
	(8632,	1859)
	(8633,	1859)
	(8634,	1863)
	(8635,	1863)
	(8636,	1863)
	(8637,	1863)
	(8638,	1863)
	(8639,	1863)
	(8640,	1863)
	(8641,	1863)
	(8642,	1863)
	(8643,	1864)
	(8644,	1865)
	(8645,	1865)
	(8646,	1865)
	(8647,	1865)
	(8648,	1866)
	(8649,	1866)
	(8650,	1866)
	(8651,	1867)
	(8652,	1867)
	(8653,	1867)
	(8654,	1867)
	(8655,	1867)
	(8656,	1867)
	(8657,	1867)
	(8658,	1867)
	(8659,	1867)
	(8660,	1867)
	(8661,	1867)
	(8662,	1867)
	(8663,	1867)
	(8664,	1867)
	(8665,	1870)
	(8666,	1870)
	(8667,	1870)
	(8668,	1871)
	(8669,	1871)
	(8670,	1871)
	(8671,	1871)
	(8672,	1871)
	(8673,	1875)
	(8674,	1875)
	(8675,	1875)
	(8676,	1875)
	(8677,	1875)
	(8678,	1877)
	(8679,	1878)
	(8680,	1880)
	(8681,	1880)
	(8682,	1880)
	(8683,	1880)
	(8684,	1881)
	(8685,	1881)
	(8686,	1881)
	(8687,	1881)
	(8688,	1881)
	(8689,	1881)
	(8690,	1882)
	(8691,	1883)
	(8692,	1883)
	(8693,	1883)
	(8694,	1883)
	(8695,	1883)
	(8696,	1883)
	(8697,	1884)
	(8698,	1884)
	(8699,	1889)
	(8700,	1889)
	(8701,	1889)
	(8702,	1889)
	(8703,	1889)
	(8704,	1889)
	(8705,	1889)
	(8706,	1891)
	(8707,	1892)
	(8708,	1892)
	(8709,	1892)
	(8710,	1894)
	(8711,	1895)
	(8712,	1897)
	(8713,	1897)
	(8714,	1897)
	(8715,	1897)
	(8716,	1898)
	(8717,	1900)
	(8718,	1900)
	(8719,	1900)
	(8720,	1901)
	(8721,	1902)
	(8722,	1902)
	(8723,	1903)
	(8724,	1903)
	(8725,	1904)
	(8726,	1904)
	(8727,	1904)
	(8728,	1904)
	(8729,	1904)
	(8730,	1904)
	(8731,	1906)
	(8732,	1906)
	(8733,	1906)
	(8734,	1906)
	(8735,	1906)
	(8736,	1906)
	(8737,	1906)
	(8738,	1906)
	(8739,	1906)
	(8740,	1906)
	(8741,	1906)
	(8742,	1906)
	(8743,	1907)
	(8744,	1907)
	(8745,	1909)
	(8746,	1910)
	(8747,	1910)
	(8748,	1911)
	(8749,	1912)
	(8750,	1912)
	(8751,	1913)
	(8752,	1913)
	(8753,	1913)
	(8754,	1914)
	(8755,	1914)
	(8756,	1919)
	(8757,	1919)
	(8758,	1919)
	(8759,	1919)
	(8760,	1919)
	(8761,	1921)
	(8762,	1921)
	(8763,	1923)
	(8764,	1924)
	(8765,	1924)
	(8766,	1924)
	(8767,	1924)
	(8768,	1924)
	(8769,	1924)
	(8770,	1924)
	(8771,	1926)
	(8772,	1932)
	(8773,	1932)
	(8774,	1932)
	(8775,	1932)
	(8776,	1932)
	(8777,	1934)
	(8778,	1935)
	(8779,	1936)
	(8780,	1936)
	(8781,	1938)
	(8782,	1938)
	(8783,	1938)
	(8784,	1938)
	(8785,	1938)
	(8786,	1938)
	(8787,	1938)
	(8788,	1939)
	(8789,	1939)
	(8790,	1939)
	(8791,	1939)
	(8792,	1939)
	(8793,	1939)
	(8794,	1939)
	(8795,	1939)
	(8796,	1939)
	(8797,	1940)
	(8798,	1940)
	(8799,	1941)
	(8800,	1941)
	(8801,	1942)
	(8802,	1942)
	(8803,	1943)
	(8804,	1943)
	(8805,	1943)
	(8806,	1945)
	(8807,	1945)
	(8808,	1946)
	(8809,	1946)
	(8810,	1946)
	(8811,	1946)
	(8812,	1946)
	(8813,	1948)
	(8814,	1950)
	(8815,	1950)
	(8816,	1951)
	(8817,	1951)
	(8818,	1952)
	(8819,	1954)
	(8820,	1954)
	(8821,	1954)
	(8822,	1954)
	(8823,	1954)
	(8824,	1954)
	(8825,	1954)
	(8826,	1957)
	(8827,	1957)
	(8828,	1959)
	(8829,	1959)
	(8830,	1959)
	(8831,	1959)
	(8832,	1960)
	(8833,	1960)
	(8834,	1960)
	(8835,	1960)
	(8836,	1960)
	(8837,	1960)
	(8838,	1962)
	(8839,	1963)
	(8840,	1963)
	(8841,	1964)
	(8842,	1965)
	(8843,	1965)
	(8844,	1965)
	(8845,	1965)
	(8846,	1966)
	(8847,	1966)
	(8848,	1966)
	(8849,	1967)
	(8850,	1967)
	(8851,	1967)
	(8852,	1968)
	(8853,	1968)
	(8854,	1968)
	(8855,	1974)
	(8856,	1974)
	(8857,	1974)
	(8858,	1974)
	(8859,	1975)
	(8860,	1975)
	(8861,	1975)
	(8862,	1975)
	(8863,	1975)
	(8864,	1976)
	(8865,	1977)
	(8866,	1977)
	(8867,	1977)
	(8868,	1977)
	(8869,	1978)
	(8870,	1978)
	(8871,	1980)
	(8872,	1980)
	(8873,	1980)
	(8874,	1980)
	(8875,	1980)
	(8876,	1979)
	(8877,	1978)
	(8878,	1977)
	(8879,	1976)
	(8880,	1975)
	(8881,	1974)
	(8882,	1973)
	(8883,	1972)
	(8884,	1971)
	(8885,	1970)
	(8886,	1972)
	(8887,	1971)
	(8888,	1970)
	(8889,	1969)
	(8890,	1968)
	(8891,	1969)
	(8892,	1969)
	(8893,	1968)
	(8894,	1968)
	(8895,	1967)
	(8896,	1966)
	(8897,	1965)
	(8898,	1964)
	(8899,	1963)
	(8900,	1962)
	(8901,	1961)
	(8902,	1960)
	(8903,	1959)
	(8904,	1961)
	(8905,	1960)
	(8906,	1959)
	(8907,	1960)
	(8908,	1963)
	(8909,	1966)
	(8910,	1965)
	(8911,	1964)
	(8912,	1964)
	(8913,	1968)
	(8914,	1967)
	(8915,	1967)
	(8916,	1966)
	(8917,	1965)
	(8918,	1964)
	(8919,	1963)
	(8920,	1962)
	(8921,	1961)
	(8922,	1960)
	(8923,	1959)
	(8924,	1959)
	(8925,	1958)
	(8926,	1957)
	(8927,	1956)
	(8928,	1956)
	(8929,	1957)
	(8930,	1956)
	(8931,	1958)
	(8932,	1959)
	(8933,	1960)
	(8934,	1960)
	(8935,	1959)
	(8936,	1958)
	(8937,	1957)
	(8938,	1960)
	(8939,	1960)
	(8940,	1961)
	(8941,	1961)
	(8942,	1960)
	(8943,	1962)
	(8944,	1961)
	(8945,	1960)
	(8946,	1959)
	(8947,	1958)
	(8948,	1957)
	(8949,	1957)
	(8950,	1956)
	(8951,	1956)
	(8952,	1955)
	(8953,	1954)
	(8954,	1953)
	(8955,	1952)
	(8956,	1951)
	(8957,	1950)
	(8958,	1949)
	(8959,	1948)
	(8960,	1947)
	(8961,	1946)
	(8962,	1945)
	(8963,	1945)
	(8964,	1944)
	(8965,	1943)
	(8966,	1942)
	(8967,	1941)
	(8968,	1940)
	(8969,	1939)
	(8970,	1939)
	(8971,	1938)
	(8972,	1937)
	(8973,	1936)
	(8974,	1935)
	(8975,	1935)
	(8976,	1936)
	(8977,	1935)
	(8978,	1934)
	(8979,	1933)
	(8980,	1932)
	(8981,	1931)
	(8982,	1930)
	(8983,	1929)
	(8984,	1928)
	(8985,	1928)
	(8986,	1929)
	(8987,	1928)
	(8988,	1927)
	(8989,	1926)
	(8990,	1926)
	(8991,	1925)
	(8992,	1925)
	(8993,	1924)
	(8994,	1923)
	(8995,	1922)
	(8996,	1922)
	(8997,	1922)
	(8998,	1922)
	(8999,	1921)
	(9000,	1921)
	(9010,	1915)
	(9020,	1906)
	(9030,	1899)
	(9040,	1893)
	(9050,	1891)
	(9060,	1884)
	(9070,	1882)
	(9080,	1875)
	(9090,	1867)
	(9100,	1860)
	(9110,	1856)
	(9120,	1856)
	(9130,	1849)
	(9140,	1842)
	(9150,	1836)
	(9160,	1830)
	(9170,	1825)
	(9180,	1818)
	(9190,	1814)
	(9200,	1816)
	(9210,	1812)
	(9220,	1806)
	(9230,	1800)
	(9240,	1795)
	(9250,	1789)
	(9260,	1782)
	(9270,	1778)
	(9280,	1772)
	(9290,	1768)
	(9300,	1762)
	(9310,	1757)
	(9320,	1750)
	(9330,	1741)
	(9340,	1736)
	(9350,	1732)
	(9360,	1727)
	(9370,	1720)
	(9380,	1722)
	(9390,	1716)
	(9400,	1712)
	(9410,	1705)
	(9420,	1700)
	(9430,	1693)
	(9440,	1685)
	(9450,	1680)
	(9460,	1673)
	(9470,	1663)
	(9480,	1655)
	(9490,	1652)
	(9500,	1645)
	(9510,	1637)
	(9520,	1629)
	(9530,	1624)
	(9540,	1623)
	(9550,	1618)
	(9560,	1608)
	(9570,	1602)
	(9580,	1594)
	(9590,	1590)
	(9600,	1584)
	(9610,	1588)
	(9620,	1581)
	(9630,	1574)
	(9640,	1576)
	(9650,	1574)
	(9660,	1571)
	(9670,	1564)
	(9680,	1556)
	(9690,	1553)
	(9700,	1550)
	(9710,	1544)
	(9720,	1543)
	(9730,	1541)
	(9740,	1535)
	(9750,	1530)
	(9760,	1527)
	(9770,	1524)
	(9780,	1519)
	(9790,	1511)
	(9800,	1507)
	(9810,	1505)
	(9820,	1506)
	(9830,	1505)
	(9840,	1504)
	(9850,	1501)
	(9860,	1494)
	(9870,	1489)
	(9880,	1487)
	(9890,	1480)
	(9900,	1475)
	(9910,	1469)
	(9920,	1465)
	(9930,	1460)
	(9940,	1456)
	(9950,	1448)
	(9960,	1443)
	(9970,	1439)
	(9980,	1439)
	(9990,	1433)
	(10000,	1427)
};
\addplot[color=green, mark=none, line width=10pt, smooth] plot coordinates {
	(0,	456)
	(10,	451)
	(20,	445)
	(30,	440)
	(40,	436)
	(50,	431)
	(60,	425)
	(70,	424)
	(80,	419)
	(90,	411)
	(100,	408)
	(110,	407)
	(120,	403)
	(130,	398)
	(140,	389)
	(150,	380)
	(160,	377)
	(170,	372)
	(180,	373)
	(190,	371)
	(200,	365)
	(210,	360)
	(220,	353)
	(230,	346)
	(240,	342)
	(250,	335)
	(260,	330)
	(270,	327)
	(280,	321)
	(290,	316)
	(300,	310)
	(310,	302)
	(320,	297)
	(330,	295)
	(340,	293)
	(350,	287)
	(360,	281)
	(370,	277)
	(380,	271)
	(390,	264)
	(400,	259)
	(410,	254)
	(420,	248)
	(430,	242)
	(440,	244)
	(450,	237)
	(460,	232)
	(470,	224)
	(480,	219)
	(490,	220)
	(500,	220)
	(510,	216)
	(520,	206)
	(530,	204)
	(540,	196)
	(550,	193)
	(560,	187)
	(570,	182)
	(580,	177)
	(590,	172)
	(600,	163)
	(610,	160)
	(620,	156)
	(630,	152)
	(640,	146)
	(650,	137)
	(660,	128)
	(670,	124)
	(680,	119)
	(690,	115)
	(700,	112)
	(710,	110)
	(720,	106)
	(730,	96)
	(740,	95)
	(750,	90)
	(760,	81)
	(770,	79)
	(780,	74)
	(790,	69)
	(800,	66)
	(801,	67)
	(802,	67)
	(803,	67)
	(804,	66)
	(805,	65)
	(806,	64)
	(807,	63)
	(808,	64)
	(809,	63)
	(810,	65)
	(811,	66)
	(812,	66)
	(813,	65)
	(814,	64)
	(815,	63)
	(816,	62)
	(817,	61)
	(818,	60)
	(819,	59)
	(820,	58)
	(821,	57)
	(822,	56)
	(823,	56)
	(824,	57)
	(825,	57)
	(826,	56)
	(827,	55)
	(828,	55)
	(829,	57)
	(830,	56)
	(831,	55)
	(832,	54)
	(833,	53)
	(834,	52)
	(835,	51)
	(836,	50)
	(837,	50)
	(838,	49)
	(839,	50)
	(840,	49)
	(841,	49)
	(842,	50)
	(843,	50)
	(844,	49)
	(845,	51)
	(846,	50)
	(847,	49)
	(848,	48)
	(849,	47)
	(850,	46)
	(851,	47)
	(852,	46)
	(853,	46)
	(854,	48)
	(855,	47)
	(856,	46)
	(857,	45)
	(858,	44)
	(859,	43)
	(860,	42)
	(861,	41)
	(862,	40)
	(863,	39)
	(864,	38)
	(865,	37)
	(866,	36)
	(867,	35)
	(868,	35)
	(869,	34)
	(870,	34)
	(871,	33)
	(872,	32)
	(873,	32)
	(874,	31)
	(875,	31)
	(876,	33)
	(877,	33)
	(878,	32)
	(879,	31)
	(880,	32)
	(881,	31)
	(882,	30)
	(883,	30)
	(884,	29)
	(885,	30)
	(886,	30)
	(887,	29)
	(888,	28)
	(889,	27)
	(890,	26)
	(891,	25)
	(892,	24)
	(893,	24)
	(894,	23)
	(895,	22)
	(896,	21)
	(897,	20)
	(898,	19)
	(899,	19)
	(900,	18)
	(901,	17)
	(902,	16)
	(903,	15)
	(904,	15)
	(905,	14)
	(906,	13)
	(907,	12)
	(908,	11)
	(909,	11)
	(910,	11)
	(911,	12)
	(912,	11)
	(913,	10)
	(914,	9)
	(915,	8)
	(916,	8)
	(917,	7)
	(918,	8)
	(919,	8)
	(920,	7)
	(921,	8)
	(922,	7)
	(923,	6)
	(924,	5)
	(925,	4)
	(926,	4)
	(927,	3)
	(928,	4)
	(929,	3)
	(930,	3)
	(931,	2)
	(932,	2)
	(933,	1)
	(934,	0)
	(935,	0)
	(936,	0)
	(937,	0)
	(938,	1)
	(939,	0)
	(940,	0)
	(941,	0)
	(942,	0)
	(943,	1)
	(944,	1)
	(945,	2)
	(946,	1)
	(947,	1)
	(948,	1)
	(949,	2)
	(950,	1)
	(951,	0)
	(952,	0)
	(953,	0)
	(954,	0)
	(955,	0)
	(956,	0)
	(957,	0)
	(958,	0)
	(959,	0)
	(960,	0)
	(961,	0)
	(962,	0)
	(963,	0)
	(964,	0)
	(965,	0)
	(966,	0)
	(967,	0)
	(968,	0)
	(969,	0)
	(970,	1)
	(971,	1)
	(972,	1)
	(973,	1)
	(974,	1)
	(975,	0)
	(976,	1)
	(977,	0)
	(978,	0)
	(979,	0)
	(980,	0)
	(981,	0)
	(982,	0)
	(983,	1)
	(984,	0)
	(985,	0)
	(986,	0)
	(987,	0)
	(988,	1)
	(989,	1)
	(990,	0)
	(991,	2)
	(992,	1)
	(993,	2)
	(994,	1)
	(995,	1)
	(996,	0)
	(997,	0)
	(998,	1)
	(999,	2)
	(1000,	2)
	(1001,	3)
	(1002,	2)
	(1003,	1)
	(1004,	1)
	(1005,	0)
	(1006,	0)
	(1007,	0)
	(1008,	2)
	(1009,	1)
	(1010,	1)
	(1011,	0)
	(1012,	0)
	(1013,	1)
	(1014,	0)
	(1015,	0)
	(1016,	0)
	(1017,	0)
	(1018,	0)
	(1019,	0)
	(1020,	1)
	(1021,	1)
	(1022,	0)
	(1023,	0)
	(1024,	0)
	(1025,	0)
	(1026,	1)
	(1027,	0)
	(1028,	0)
	(1029,	0)
	(1030,	0)
	(1031,	0)
	(1032,	0)
	(1033,	0)
	(1034,	0)
	(1035,	0)
	(1036,	0)
	(1037,	0)
	(1038,	1)
	(1039,	0)
	(1040,	0)
	(1041,	1)
	(1042,	1)
	(1043,	0)
	(1044,	1)
	(1045,	0)
	(1046,	0)
	(1047,	0)
	(1048,	3)
	(1049,	3)
	(1050,	4)
	(1051,	5)
	(1052,	5)
	(1053,	5)
	(1054,	5)
	(1055,	5)
	(1056,	6)
	(1057,	6)
	(1058,	6)
	(1059,	6)
	(1060,	7)
	(1061,	8)
	(1062,	8)
	(1063,	8)
	(1064,	8)
	(1065,	8)
	(1066,	9)
	(1067,	9)
	(1068,	9)
	(1069,	9)
	(1070,	10)
	(1071,	10)
	(1072,	11)
	(1073,	11)
	(1074,	11)
	(1075,	11)
	(1076,	11)
	(1077,	13)
	(1078,	16)
	(1079,	16)
	(1080,	16)
	(1081,	16)
	(1082,	18)
	(1083,	18)
	(1084,	18)
	(1085,	18)
	(1086,	18)
	(1087,	19)
	(1088,	19)
	(1089,	20)
	(1090,	20)
	(1091,	20)
	(1092,	21)
	(1093,	21)
	(1094,	21)
	(1095,	22)
	(1096,	22)
	(1097,	22)
	(1098,	22)
	(1099,	22)
	(1100,	22)
	(1101,	23)
	(1102,	24)
	(1103,	24)
	(1104,	24)
	(1105,	25)
	(1106,	25)
	(1107,	25)
	(1108,	25)
	(1109,	27)
	(1110,	28)
	(1111,	29)
	(1112,	29)
	(1113,	29)
	(1114,	29)
	(1115,	30)
	(1116,	30)
	(1117,	30)
	(1118,	30)
	(1119,	30)
	(1120,	30)
	(1121,	30)
	(1122,	30)
	(1123,	30)
	(1124,	30)
	(1125,	30)
	(1126,	30)
	(1127,	30)
	(1128,	30)
	(1129,	31)
	(1130,	31)
	(1131,	31)
	(1132,	31)
	(1133,	31)
	(1134,	31)
	(1135,	33)
	(1136,	33)
	(1137,	35)
	(1138,	36)
	(1139,	36)
	(1140,	36)
	(1141,	36)
	(1142,	37)
	(1143,	37)
	(1144,	37)
	(1145,	38)
	(1146,	38)
	(1147,	38)
	(1148,	38)
	(1149,	41)
	(1150,	41)
	(1151,	41)
	(1152,	41)
	(1153,	41)
	(1154,	44)
	(1155,	45)
	(1156,	45)
	(1157,	45)
	(1158,	45)
	(1159,	45)
	(1160,	47)
	(1161,	47)
	(1162,	48)
	(1163,	48)
	(1164,	48)
	(1165,	49)
	(1166,	49)
	(1167,	49)
	(1168,	49)
	(1169,	49)
	(1170,	49)
	(1171,	49)
	(1172,	49)
	(1173,	51)
	(1174,	51)
	(1175,	51)
	(1176,	51)
	(1177,	51)
	(1178,	51)
	(1179,	51)
	(1180,	51)
	(1181,	51)
	(1182,	51)
	(1183,	51)
	(1184,	51)
	(1185,	51)
	(1186,	51)
	(1187,	51)
	(1188,	51)
	(1189,	52)
	(1190,	52)
	(1191,	56)
	(1192,	57)
	(1193,	58)
	(1194,	59)
	(1195,	60)
	(1196,	61)
	(1197,	61)
	(1198,	62)
	(1199,	62)
	(1200,	62)
	(1210,	64)
	(1220,	69)
	(1230,	72)
	(1240,	75)
	(1250,	80)
	(1260,	86)
	(1270,	93)
	(1280,	98)
	(1290,	103)
	(1300,	104)
	(1310,	109)
	(1320,	113)
	(1330,	116)
	(1340,	119)
	(1350,	124)
	(1360,	128)
	(1370,	131)
	(1380,	133)
	(1390,	137)
	(1400,	141)
	(1410,	147)
	(1420,	153)
	(1430,	156)
	(1440,	161)
	(1450,	169)
	(1460,	172)
	(1470,	180)
	(1480,	186)
	(1490,	195)
	(1500,	200)
	(1510,	209)
	(1520,	216)
	(1530,	220)
	(1540,	228)
	(1550,	236)
	(1560,	243)
	(1570,	249)
	(1580,	252)
	(1590,	254)
	(1600,	261)
	(1610,	265)
	(1620,	271)
	(1630,	275)
	(1640,	276)
	(1650,	282)
	(1660,	292)
	(1670,	296)
	(1680,	303)
	(1690,	310)
	(1700,	315)
	(1710,	318)
	(1720,	322)
	(1730,	335)
	(1740,	337)
	(1750,	341)
	(1760,	351)
	(1770,	354)
	(1780,	360)
	(1790,	368)
	(1800,	382)
	(1810,	385)
	(1820,	389)
	(1830,	392)
	(1840,	394)
	(1850,	398)
	(1860,	403)
	(1870,	405)
	(1880,	406)
	(1890,	413)
	(1900,	419)
	(1910,	426)
	(1920,	427)
	(1930,	432)
	(1940,	437)
	(1950,	445)
	(1960,	452)
	(1970,	456)
	(1980,	464)
	(1990,	468)
	(2000,	473)
	(2010,	475)
	(2020,	482)
	(2030,	484)
	(2040,	488)
	(2050,	493)
	(2060,	499)
	(2070,	503)
	(2080,	505)
	(2090,	507)
	(2100,	512)
	(2110,	518)
	(2120,	528)
	(2130,	531)
	(2140,	533)
	(2150,	538)
	(2160,	546)
	(2170,	551)
	(2180,	560)
	(2190,	565)
	(2200,	568)
	(2210,	577)
	(2220,	585)
	(2230,	593)
	(2240,	599)
	(2250,	604)
	(2260,	610)
	(2270,	616)
	(2280,	619)
	(2290,	623)
	(2300,	626)
	(2310,	632)
	(2320,	634)
	(2330,	638)
	(2340,	640)
	(2350,	644)
	(2360,	647)
	(2370,	648)
	(2380,	654)
	(2390,	660)
	(2400,	667)
	(2410,	673)
	(2420,	689)
	(2430,	693)
	(2440,	697)
	(2450,	708)
	(2460,	714)
	(2470,	721)
	(2480,	725)
	(2490,	731)
	(2500,	735)
	(2510,	740)
	(2520,	745)
	(2530,	747)
	(2540,	752)
	(2550,	753)
	(2560,	757)
	(2570,	760)
	(2580,	761)
	(2590,	767)
	(2600,	774)
	(2610,	783)
	(2620,	787)
	(2630,	792)
	(2640,	795)
	(2650,	795)
	(2660,	801)
	(2670,	801)
	(2680,	807)
	(2690,	812)
	(2700,	812)
	(2710,	817)
	(2720,	819)
	(2730,	826)
	(2740,	831)
	(2750,	832)
	(2760,	837)
	(2770,	845)
	(2780,	849)
	(2790,	854)
	(2800,	861)
	(2810,	872)
	(2820,	877)
	(2830,	881)
	(2840,	884)
	(2850,	887)
	(2860,	890)
	(2870,	894)
	(2880,	901)
	(2890,	904)
	(2900,	909)
	(2910,	914)
	(2920,	921)
	(2930,	930)
	(2940,	939)
	(2950,	944)
	(2960,	946)
	(2970,	948)
	(2980,	951)
	(2990,	952)
	(3000,	956)
	(3010,	964)
	(3020,	968)
	(3030,	973)
	(3040,	979)
	(3050,	982)
	(3060,	987)
	(3070,	993)
	(3080,	993)
	(3090,	996)
	(3100,	1001)
	(3110,	1006)
	(3120,	1017)
	(3130,	1021)
	(3140,	1023)
	(3150,	1028)
	(3160,	1030)
	(3170,	1036)
	(3180,	1039)
	(3190,	1044)
	(3200,	1051)
	(3210,	1052)
	(3220,	1058)
	(3230,	1062)
	(3240,	1064)
	(3250,	1068)
	(3260,	1069)
	(3270,	1072)
	(3280,	1076)
	(3290,	1076)
	(3300,	1083)
	(3310,	1086)
	(3320,	1096)
	(3330,	1099)
	(3340,	1110)
	(3350,	1116)
	(3360,	1120)
	(3370,	1124)
	(3380,	1130)
	(3390,	1131)
	(3400,	1135)
	(3410,	1140)
	(3420,	1145)
	(3430,	1150)
	(3440,	1154)
	(3450,	1164)
	(3460,	1170)
	(3470,	1176)
	(3480,	1181)
	(3490,	1187)
	(3500,	1196)
	(3510,	1202)
	(3520,	1205)
	(3530,	1215)
	(3540,	1217)
	(3550,	1220)
	(3560,	1224)
	(3570,	1233)
	(3580,	1240)
	(3590,	1246)
	(3600,	1250)
	(3610,	1259)
	(3620,	1265)
	(3630,	1268)
	(3640,	1272)
	(3650,	1277)
	(3660,	1280)
	(3670,	1286)
	(3680,	1291)
	(3690,	1298)
	(3700,	1309)
	(3710,	1310)
	(3720,	1315)
	(3730,	1321)
	(3740,	1326)
	(3750,	1329)
	(3760,	1331)
	(3770,	1340)
	(3780,	1345)
	(3790,	1349)
	(3800,	1354)
	(3810,	1363)
	(3820,	1367)
	(3830,	1370)
	(3840,	1375)
	(3850,	1378)
	(3860,	1389)
	(3870,	1397)
	(3880,	1402)
	(3890,	1409)
	(3900,	1415)
	(3910,	1418)
	(3920,	1423)
	(3930,	1424)
	(3940,	1432)
	(3950,	1434)
	(3960,	1435)
	(3970,	1437)
	(3980,	1442)
	(3990,	1445)
	(4000,	1448)
	(4010,	1452)
	(4020,	1458)
	(4030,	1468)
	(4040,	1471)
	(4050,	1473)
	(4060,	1481)
	(4070,	1487)
	(4080,	1493)
	(4090,	1497)
	(4100,	1501)
	(4110,	1502)
	(4120,	1504)
	(4130,	1509)
	(4140,	1513)
	(4150,	1516)
	(4160,	1516)
	(4170,	1521)
	(4180,	1526)
	(4190,	1528)
	(4200,	1536)
	(4210,	1546)
	(4220,	1553)
	(4230,	1555)
	(4240,	1557)
	(4250,	1561)
	(4260,	1562)
	(4270,	1563)
	(4280,	1569)
	(4290,	1573)
	(4300,	1578)
	(4310,	1582)
	(4320,	1587)
	(4330,	1593)
	(4340,	1597)
	(4350,	1601)
	(4360,	1608)
	(4370,	1610)
	(4380,	1615)
	(4390,	1618)
	(4400,	1625)
	(4410,	1628)
	(4420,	1632)
	(4430,	1639)
	(4440,	1648)
	(4450,	1657)
	(4460,	1662)
	(4470,	1666)
	(4480,	1675)
	(4490,	1683)
	(4500,	1686)
	(4510,	1693)
	(4520,	1703)
	(4530,	1708)
	(4540,	1714)
	(4550,	1717)
	(4560,	1725)
	(4570,	1730)
	(4580,	1736)
	(4590,	1739)
	(4600,	1742)
	(4610,	1744)
	(4620,	1751)
	(4630,	1757)
	(4640,	1759)
	(4650,	1763)
	(4660,	1766)
	(4670,	1768)
	(4680,	1770)
	(4690,	1774)
	(4700,	1781)
	(4701,	1781)
	(4702,	1784)
	(4703,	1785)
	(4704,	1785)
	(4705,	1785)
	(4706,	1785)
	(4707,	1785)
	(4708,	1785)
	(4709,	1785)
	(4710,	1785)
	(4711,	1785)
	(4712,	1785)
	(4713,	1785)
	(4714,	1785)
	(4715,	1785)
	(4716,	1785)
	(4717,	1785)
	(4718,	1785)
	(4719,	1785)
	(4720,	1785)
	(4721,	1786)
	(4722,	1786)
	(4723,	1786)
	(4724,	1786)
	(4725,	1786)
	(4726,	1786)
	(4727,	1786)
	(4728,	1786)
	(4729,	1786)
	(4730,	1788)
	(4731,	1788)
	(4732,	1788)
	(4733,	1788)
	(4734,	1788)
	(4735,	1788)
	(4736,	1788)
	(4737,	1788)
	(4738,	1791)
	(4739,	1791)
	(4740,	1791)
	(4741,	1791)
	(4742,	1791)
	(4743,	1791)
	(4744,	1791)
	(4745,	1791)
	(4746,	1791)
	(4747,	1791)
	(4748,	1791)
	(4749,	1791)
	(4750,	1791)
	(4751,	1792)
	(4752,	1792)
	(4753,	1793)
	(4754,	1793)
	(4755,	1793)
	(4756,	1793)
	(4757,	1793)
	(4758,	1793)
	(4759,	1793)
	(4760,	1793)
	(4761,	1794)
	(4762,	1795)
	(4763,	1796)
	(4764,	1796)
	(4765,	1797)
	(4766,	1797)
	(4767,	1797)
	(4768,	1797)
	(4769,	1797)
	(4770,	1798)
	(4771,	1800)
	(4772,	1800)
	(4773,	1800)
	(4774,	1800)
	(4775,	1802)
	(4776,	1803)
	(4777,	1803)
	(4778,	1803)
	(4779,	1803)
	(4780,	1803)
	(4781,	1803)
	(4782,	1803)
	(4783,	1805)
	(4784,	1805)
	(4785,	1810)
	(4786,	1810)
	(4787,	1810)
	(4788,	1812)
	(4789,	1812)
	(4790,	1812)
	(4791,	1813)
	(4792,	1814)
	(4793,	1814)
	(4794,	1817)
	(4795,	1818)
	(4796,	1820)
	(4797,	1820)
	(4798,	1821)
	(4799,	1821)
	(4800,	1821)
	(4801,	1821)
	(4802,	1821)
	(4803,	1821)
	(4804,	1821)
	(4805,	1821)
	(4806,	1821)
	(4807,	1822)
	(4808,	1826)
	(4809,	1830)
	(4810,	1830)
	(4811,	1830)
	(4812,	1830)
	(4813,	1830)
	(4814,	1830)
	(4815,	1830)
	(4816,	1831)
	(4817,	1831)
	(4818,	1831)
	(4819,	1831)
	(4820,	1832)
	(4821,	1833)
	(4822,	1833)
	(4823,	1833)
	(4824,	1833)
	(4825,	1833)
	(4826,	1833)
	(4827,	1833)
	(4828,	1836)
	(4829,	1836)
	(4830,	1837)
	(4831,	1839)
	(4832,	1839)
	(4833,	1839)
	(4834,	1839)
	(4835,	1839)
	(4836,	1839)
	(4837,	1839)
	(4838,	1839)
	(4839,	1845)
	(4840,	1845)
	(4841,	1846)
	(4842,	1847)
	(4843,	1847)
	(4844,	1847)
	(4845,	1848)
	(4846,	1850)
	(4847,	1851)
	(4848,	1851)
	(4849,	1851)
	(4850,	1851)
	(4851,	1857)
	(4852,	1857)
	(4853,	1857)
	(4854,	1859)
	(4855,	1859)
	(4856,	1859)
	(4857,	1859)
	(4858,	1859)
	(4859,	1859)
	(4860,	1860)
	(4861,	1861)
	(4862,	1862)
	(4863,	1863)
	(4864,	1863)
	(4865,	1865)
	(4866,	1865)
	(4867,	1865)
	(4868,	1865)
	(4869,	1866)
	(4870,	1866)
	(4871,	1866)
	(4872,	1866)
	(4873,	1867)
	(4874,	1872)
	(4875,	1875)
	(4876,	1875)
	(4877,	1875)
	(4878,	1876)
	(4879,	1876)
	(4880,	1876)
	(4881,	1876)
	(4882,	1876)
	(4883,	1877)
	(4884,	1879)
	(4885,	1881)
	(4886,	1881)
	(4887,	1882)
	(4888,	1882)
	(4889,	1883)
	(4890,	1884)
	(4891,	1884)
	(4892,	1884)
	(4893,	1884)
	(4894,	1885)
	(4895,	1885)
	(4896,	1885)
	(4897,	1885)
	(4898,	1886)
	(4899,	1886)
	(4900,	1886)
	(4901,	1886)
	(4902,	1886)
	(4903,	1887)
	(4904,	1890)
	(4905,	1890)
	(4906,	1890)
	(4907,	1890)
	(4908,	1890)
	(4909,	1890)
	(4910,	1890)
	(4911,	1890)
	(4912,	1891)
	(4913,	1892)
	(4914,	1893)
	(4915,	1894)
	(4916,	1895)
	(4917,	1895)
	(4918,	1895)
	(4919,	1895)
	(4920,	1895)
	(4921,	1897)
	(4922,	1897)
	(4923,	1898)
	(4924,	1899)
	(4925,	1901)
	(4926,	1903)
	(4927,	1903)
	(4928,	1903)
	(4929,	1903)
	(4930,	1903)
	(4931,	1905)
	(4932,	1905)
	(4933,	1906)
	(4934,	1906)
	(4935,	1906)
	(4936,	1905)
	(4937,	1904)
	(4938,	1905)
	(4939,	1905)
	(4940,	1904)
	(4941,	1904)
	(4942,	1903)
	(4943,	1902)
	(4944,	1901)
	(4945,	1900)
	(4946,	1900)
	(4947,	1899)
	(4948,	1898)
	(4949,	1899)
	(4950,	1898)
	(4951,	1897)
	(4952,	1899)
	(4953,	1898)
	(4954,	1897)
	(4955,	1896)
	(4956,	1895)
	(4957,	1895)
	(4958,	1895)
	(4959,	1894)
	(4960,	1895)
	(4961,	1894)
	(4962,	1893)
	(4963,	1895)
	(4964,	1895)
	(4965,	1894)
	(4966,	1893)
	(4967,	1892)
	(4968,	1891)
	(4969,	1893)
	(4970,	1893)
	(4971,	1894)
	(4972,	1895)
	(4973,	1894)
	(4974,	1893)
	(4975,	1892)
	(4976,	1892)
	(4977,	1891)
	(4978,	1890)
	(4979,	1889)
	(4980,	1888)
	(4981,	1887)
	(4982,	1888)
	(4983,	1887)
	(4984,	1886)
	(4985,	1885)
	(4986,	1884)
	(4987,	1883)
	(4988,	1882)
	(4989,	1882)
	(4990,	1882)
	(4991,	1884)
	(4992,	1886)
	(4993,	1886)
	(4994,	1885)
	(4995,	1884)
	(4996,	1886)
	(4997,	1886)
	(4998,	1885)
	(4999,	1884)
	(5000,	1884)
	(5001,	1883)
	(5002,	1882)
	(5003,	1881)
	(5004,	1880)
	(5005,	1883)
	(5006,	1882)
	(5007,	1882)
	(5008,	1881)
	(5009,	1880)
	(5010,	1880)
	(5011,	1880)
	(5012,	1879)
	(5013,	1878)
	(5014,	1878)
	(5015,	1878)
	(5016,	1884)
	(5017,	1883)
	(5018,	1882)
	(5019,	1881)
	(5020,	1881)
	(5021,	1880)
	(5022,	1882)
	(5023,	1882)
	(5024,	1881)
	(5025,	1882)
	(5026,	1881)
	(5027,	1880)
	(5028,	1881)
	(5029,	1881)
	(5030,	1880)
	(5031,	1879)
	(5032,	1879)
	(5033,	1878)
	(5034,	1878)
	(5035,	1877)
	(5036,	1877)
	(5037,	1876)
	(5038,	1875)
	(5039,	1874)
	(5040,	1873)
	(5041,	1873)
	(5042,	1872)
	(5043,	1872)
	(5044,	1871)
	(5045,	1870)
	(5046,	1870)
	(5047,	1869)
	(5048,	1868)
	(5049,	1867)
	(5050,	1870)
	(5051,	1869)
	(5052,	1872)
	(5053,	1873)
	(5054,	1872)
	(5055,	1871)
	(5056,	1870)
	(5057,	1869)
	(5058,	1868)
	(5059,	1869)
	(5060,	1869)
	(5061,	1868)
	(5062,	1868)
	(5063,	1867)
	(5064,	1866)
	(5065,	1868)
	(5066,	1867)
	(5067,	1867)
	(5068,	1866)
	(5069,	1865)
	(5070,	1864)
	(5071,	1864)
	(5072,	1863)
	(5073,	1863)
	(5074,	1862)
	(5075,	1861)
	(5076,	1860)
	(5077,	1861)
	(5078,	1860)
	(5079,	1859)
	(5080,	1858)
	(5081,	1858)
	(5082,	1858)
	(5083,	1857)
	(5084,	1856)
	(5085,	1856)
	(5086,	1856)
	(5087,	1855)
	(5088,	1854)
	(5089,	1853)
	(5090,	1852)
	(5091,	1851)
	(5092,	1850)
	(5093,	1849)
	(5094,	1850)
	(5095,	1849)
	(5096,	1851)
	(5097,	1851)
	(5098,	1850)
	(5099,	1849)
	(5100,	1849)
	(5110,	1842)
	(5120,	1836)
	(5130,	1829)
	(5140,	1826)
	(5150,	1818)
	(5160,	1812)
	(5170,	1809)
	(5180,	1799)
	(5190,	1795)
	(5200,	1796)
	(5210,	1791)
	(5220,	1788)
	(5230,	1786)
	(5240,	1783)
	(5250,	1780)
	(5260,	1775)
	(5270,	1770)
	(5280,	1769)
	(5290,	1760)
	(5300,	1757)
	(5310,	1754)
	(5320,	1752)
	(5330,	1744)
	(5340,	1737)
	(5350,	1731)
	(5360,	1726)
	(5370,	1717)
	(5380,	1713)
	(5390,	1712)
	(5400,	1707)
	(5410,	1702)
	(5420,	1701)
	(5430,	1698)
	(5440,	1694)
	(5450,	1687)
	(5460,	1683)
	(5470,	1678)
	(5480,	1672)
	(5490,	1669)
	(5500,	1669)
	(5510,	1663)
	(5520,	1657)
	(5530,	1652)
	(5540,	1647)
	(5550,	1641)
	(5560,	1642)
	(5570,	1637)
	(5580,	1635)
	(5590,	1630)
	(5600,	1625)
	(5610,	1619)
	(5620,	1612)
	(5630,	1608)
	(5640,	1607)
	(5650,	1600)
	(5660,	1595)
	(5670,	1592)
	(5680,	1587)
	(5690,	1583)
	(5700,	1584)
	(5710,	1582)
	(5720,	1573)
	(5730,	1566)
	(5740,	1559)
	(5750,	1557)
	(5760,	1553)
	(5770,	1547)
	(5780,	1544)
	(5790,	1547)
	(5800,	1543)
	(5810,	1539)
	(5820,	1530)
	(5830,	1534)
	(5840,	1525)
	(5850,	1521)
	(5860,	1514)
	(5870,	1512)
	(5880,	1507)
	(5890,	1501)
	(5900,	1498)
	(5910,	1493)
	(5920,	1490)
	(5930,	1484)
	(5940,	1474)
	(5950,	1472)
	(5960,	1466)
	(5970,	1459)
	(5980,	1449)
	(5990,	1447)
	(6000,	1442)
	(6010,	1438)
	(6020,	1431)
	(6030,	1426)
	(6040,	1422)
	(6050,	1418)
	(6060,	1411)
	(6070,	1405)
	(6080,	1397)
	(6090,	1389)
	(6100,	1382)
	(6110,	1376)
	(6120,	1370)
	(6130,	1366)
	(6140,	1358)
	(6150,	1353)
	(6160,	1353)
	(6170,	1346)
	(6180,	1341)
	(6190,	1334)
	(6200,	1328)
	(6210,	1331)
	(6220,	1325)
	(6230,	1321)
	(6240,	1316)
	(6250,	1314)
	(6260,	1314)
	(6270,	1307)
	(6280,	1301)
	(6290,	1296)
	(6300,	1289)
	(6310,	1280)
	(6320,	1276)
	(6330,	1270)
	(6340,	1264)
	(6350,	1255)
	(6360,	1246)
	(6370,	1240)
	(6380,	1232)
	(6390,	1224)
	(6400,	1220)
	(6410,	1212)
	(6420,	1205)
	(6430,	1199)
	(6440,	1197)
	(6450,	1193)
	(6460,	1191)
	(6470,	1188)
	(6480,	1181)
	(6490,	1177)
	(6500,	1170)
	(6510,	1167)
	(6520,	1163)
	(6530,	1157)
	(6540,	1153)
	(6550,	1149)
	(6560,	1142)
	(6570,	1141)
	(6580,	1134)
	(6590,	1130)
	(6600,	1125)
	(6610,	1125)
	(6620,	1121)
	(6630,	1116)
	(6640,	1108)
	(6650,	1104)
	(6660,	1099)
	(6670,	1097)
	(6680,	1091)
	(6690,	1094)
	(6700,	1089)
	(6710,	1084)
	(6720,	1078)
	(6730,	1076)
	(6740,	1069)
	(6750,	1067)
	(6760,	1059)
	(6770,	1057)
	(6780,	1058)
	(6790,	1055)
	(6800,	1049)
	(6810,	1044)
	(6820,	1040)
	(6830,	1034)
	(6840,	1025)
	(6850,	1021)
	(6860,	1014)
	(6870,	1008)
	(6880,	1005)
	(6890,	1000)
	(6900,	999)
	(6910,	1004)
	(6920,	1003)
	(6930,	997)
	(6940,	989)
	(6950,	986)
	(6960,	982)
	(6970,	977)
	(6980,	971)
	(6990,	964)
	(7000,	960)
	(7010,	955)
	(7020,	950)
	(7030,	941)
	(7040,	934)
	(7050,	930)
	(7060,	925)
	(7070,	920)
	(7080,	918)
	(7090,	912)
	(7100,	910)
	(7110,	901)
	(7120,	898)
	(7130,	894)
	(7140,	888)
	(7150,	881)
	(7160,	878)
	(7170,	870)
	(7180,	862)
	(7190,	854)
	(7200,	849)
	(7210,	844)
	(7220,	838)
	(7230,	835)
	(7240,	827)
	(7250,	824)
	(7260,	821)
	(7270,	817)
	(7280,	813)
	(7290,	806)
	(7300,	800)
	(7310,	801)
	(7320,	795)
	(7330,	788)
	(7340,	784)
	(7350,	779)
	(7360,	773)
	(7370,	767)
	(7380,	762)
	(7390,	754)
	(7400,	748)
	(7410,	743)
	(7420,	739)
	(7430,	730)
	(7440,	721)
	(7450,	715)
	(7460,	708)
	(7470,	703)
	(7480,	694)
	(7490,	691)
	(7500,	689)
	(7510,	684)
	(7520,	680)
	(7530,	679)
	(7540,	675)
	(7550,	675)
	(7560,	668)
	(7570,	668)
	(7580,	663)
	(7590,	659)
	(7600,	654)
	(7610,	651)
	(7620,	644)
	(7630,	644)
	(7640,	640)
	(7650,	633)
	(7660,	627)
	(7670,	618)
	(7680,	608)
	(7690,	602)
	(7700,	597)
	(7710,	592)
	(7720,	589)
	(7730,	585)
	(7740,	582)
	(7750,	574)
	(7760,	570)
	(7770,	562)
	(7780,	554)
	(7790,	547)
	(7800,	541)
	(7810,	533)
	(7820,	531)
	(7830,	526)
	(7840,	523)
	(7850,	517)
	(7860,	512)
	(7870,	504)
	(7880,	500)
	(7890,	496)
	(7900,	494)
	(7910,	486)
	(7920,	480)
	(7930,	474)
	(7940,	468)
	(7950,	465)
	(7960,	458)
	(7970,	451)
	(7980,	446)
	(7990,	437)
	(8000,	430)
	(8010,	423)
	(8020,	417)
	(8030,	414)
	(8040,	409)
	(8050,	411)
	(8060,	403)
	(8070,	398)
	(8080,	389)
	(8090,	380)
	(8100,	378)
	(8110,	370)
	(8120,	363)
	(8130,	360)
	(8140,	351)
	(8150,	344)
	(8160,	345)
	(8170,	338)
	(8180,	330)
	(8190,	323)
	(8200,	319)
	(8210,	315)
	(8220,	315)
	(8230,	313)
	(8240,	305)
	(8250,	299)
	(8260,	293)
	(8270,	288)
	(8280,	282)
	(8290,	273)
	(8300,	267)
	(8310,	263)
	(8320,	262)
	(8330,	257)
	(8340,	259)
	(8350,	255)
	(8360,	249)
	(8370,	242)
	(8380,	245)
	(8390,	241)
	(8400,	234)
	(8410,	229)
	(8420,	222)
	(8430,	218)
	(8440,	214)
	(8450,	208)
	(8460,	203)
	(8470,	196)
	(8480,	190)
	(8490,	186)
	(8500,	178)
	(8510,	174)
	(8520,	170)
	(8530,	167)
	(8540,	166)
	(8550,	161)
	(8560,	158)
	(8570,	153)
	(8580,	147)
	(8590,	144)
	(8600,	139)
	(8601,	139)
	(8602,	140)
	(8603,	141)
	(8604,	141)
	(8605,	141)
	(8606,	140)
	(8607,	139)
	(8608,	138)
	(8609,	137)
	(8610,	138)
	(8611,	138)
	(8612,	138)
	(8613,	137)
	(8614,	136)
	(8615,	135)
	(8616,	137)
	(8617,	136)
	(8618,	135)
	(8619,	134)
	(8620,	133)
	(8621,	132)
	(8622,	131)
	(8623,	130)
	(8624,	130)
	(8625,	130)
	(8626,	129)
	(8627,	129)
	(8628,	130)
	(8629,	129)
	(8630,	128)
	(8631,	127)
	(8632,	129)
	(8633,	129)
	(8634,	128)
	(8635,	127)
	(8636,	126)
	(8637,	125)
	(8638,	124)
	(8639,	123)
	(8640,	123)
	(8641,	122)
	(8642,	121)
	(8643,	120)
	(8644,	119)
	(8645,	118)
	(8646,	117)
	(8647,	118)
	(8648,	117)
	(8649,	116)
	(8650,	115)
	(8651,	115)
	(8652,	114)
	(8653,	114)
	(8654,	113)
	(8655,	112)
	(8656,	111)
	(8657,	110)
	(8658,	112)
	(8659,	111)
	(8660,	111)
	(8661,	110)
	(8662,	111)
	(8663,	111)
	(8664,	110)
	(8665,	112)
	(8666,	112)
	(8667,	111)
	(8668,	110)
	(8669,	109)
	(8670,	108)
	(8671,	107)
	(8672,	108)
	(8673,	107)
	(8674,	109)
	(8675,	108)
	(8676,	107)
	(8677,	106)
	(8678,	105)
	(8679,	104)
	(8680,	103)
	(8681,	102)
	(8682,	101)
	(8683,	101)
	(8684,	100)
	(8685,	101)
	(8686,	101)
	(8687,	100)
	(8688,	99)
	(8689,	98)
	(8690,	98)
	(8691,	97)
	(8692,	96)
	(8693,	95)
	(8694,	94)
	(8695,	93)
	(8696,	92)
	(8697,	91)
	(8698,	90)
	(8699,	89)
	(8700,	89)
	(8701,	88)
	(8702,	87)
	(8703,	86)
	(8704,	85)
	(8705,	88)
	(8706,	87)
	(8707,	87)
	(8708,	86)
	(8709,	85)
	(8710,	84)
	(8711,	83)
	(8712,	82)
	(8713,	81)
	(8714,	80)
	(8715,	80)
	(8716,	79)
	(8717,	79)
	(8718,	78)
	(8719,	77)
	(8720,	76)
	(8721,	76)
	(8722,	75)
	(8723,	75)
	(8724,	76)
	(8725,	77)
	(8726,	76)
	(8727,	75)
	(8728,	74)
	(8729,	73)
	(8730,	72)
	(8731,	71)
	(8732,	72)
	(8733,	72)
	(8734,	71)
	(8735,	71)
	(8736,	70)
	(8737,	69)
	(8738,	68)
	(8739,	67)
	(8740,	66)
	(8741,	65)
	(8742,	65)
	(8743,	66)
	(8744,	65)
	(8745,	64)
	(8746,	63)
	(8747,	62)
	(8748,	63)
	(8749,	62)
	(8750,	61)
	(8751,	60)
	(8752,	59)
	(8753,	59)
	(8754,	58)
	(8755,	58)
	(8756,	59)
	(8757,	58)
	(8758,	58)
	(8759,	57)
	(8760,	56)
	(8761,	55)
	(8762,	54)
	(8763,	56)
	(8764,	55)
	(8765,	54)
	(8766,	53)
	(8767,	52)
	(8768,	51)
	(8769,	50)
	(8770,	49)
	(8771,	48)
	(8772,	47)
	(8773,	46)
	(8774,	45)
	(8775,	44)
	(8776,	43)
	(8777,	42)
	(8778,	41)
	(8779,	40)
	(8780,	39)
	(8781,	41)
	(8782,	40)
	(8783,	39)
	(8784,	38)
	(8785,	37)
	(8786,	39)
	(8787,	44)
	(8788,	43)
	(8789,	44)
	(8790,	45)
	(8791,	44)
	(8792,	44)
	(8793,	44)
	(8794,	43)
	(8795,	49)
	(8796,	51)
	(8797,	52)
	(8798,	51)
	(8799,	52)
	(8800,	51)
	(8801,	50)
	(8802,	49)
	(8803,	48)
	(8804,	48)
	(8805,	48)
	(8806,	47)
	(8807,	46)
	(8808,	45)
	(8809,	45)
	(8810,	44)
	(8811,	46)
	(8812,	45)
	(8813,	44)
	(8814,	45)
	(8815,	45)
	(8816,	44)
	(8817,	43)
	(8818,	42)
	(8819,	41)
	(8820,	41)
	(8821,	40)
	(8822,	39)
	(8823,	38)
	(8824,	37)
	(8825,	38)
	(8826,	37)
	(8827,	37)
	(8828,	36)
	(8829,	35)
	(8830,	34)
	(8831,	35)
	(8832,	37)
	(8833,	36)
	(8834,	35)
	(8835,	34)
	(8836,	33)
	(8837,	32)
	(8838,	32)
	(8839,	31)
	(8840,	30)
	(8841,	29)
	(8842,	28)
	(8843,	27)
	(8844,	26)
	(8845,	25)
	(8846,	24)
	(8847,	23)
	(8848,	22)
	(8849,	21)
	(8850,	20)
	(8851,	19)
	(8852,	18)
	(8853,	17)
	(8854,	16)
	(8855,	16)
	(8856,	15)
	(8857,	14)
	(8858,	13)
	(8859,	13)
	(8860,	12)
	(8861,	11)
	(8862,	11)
	(8863,	11)
	(8864,	10)
	(8865,	9)
	(8866,	9)
	(8867,	9)
	(8868,	8)
	(8869,	7)
	(8870,	6)
	(8871,	5)
	(8872,	4)
	(8873,	3)
	(8874,	3)
	(8875,	4)
	(8876,	4)
	(8877,	4)
	(8878,	5)
	(8879,	5)
	(8880,	7)
	(8881,	7)
	(8882,	8)
	(8883,	10)
	(8884,	10)
	(8885,	10)
	(8886,	10)
	(8887,	10)
	(8888,	13)
	(8889,	13)
	(8890,	15)
	(8891,	17)
	(8892,	18)
	(8893,	18)
	(8894,	19)
	(8895,	19)
	(8896,	19)
	(8897,	22)
	(8898,	22)
	(8899,	22)
	(8900,	22)
	(8901,	22)
	(8902,	23)
	(8903,	23)
	(8904,	23)
	(8905,	23)
	(8906,	23)
	(8907,	23)
	(8908,	23)
	(8909,	24)
	(8910,	26)
	(8911,	26)
	(8912,	27)
	(8913,	27)
	(8914,	29)
	(8915,	31)
	(8916,	31)
	(8917,	31)
	(8918,	32)
	(8919,	32)
	(8920,	33)
	(8921,	35)
	(8922,	37)
	(8923,	37)
	(8924,	37)
	(8925,	37)
	(8926,	37)
	(8927,	38)
	(8928,	38)
	(8929,	38)
	(8930,	39)
	(8931,	41)
	(8932,	41)
	(8933,	41)
	(8934,	43)
	(8935,	43)
	(8936,	43)
	(8937,	44)
	(8938,	44)
	(8939,	44)
	(8940,	44)
	(8941,	44)
	(8942,	44)
	(8943,	44)
	(8944,	44)
	(8945,	44)
	(8946,	44)
	(8947,	44)
	(8948,	44)
	(8949,	44)
	(8950,	44)
	(8951,	44)
	(8952,	44)
	(8953,	44)
	(8954,	44)
	(8955,	44)
	(8956,	45)
	(8957,	47)
	(8958,	49)
	(8959,	49)
	(8960,	49)
	(8961,	49)
	(8962,	49)
	(8963,	49)
	(8964,	50)
	(8965,	51)
	(8966,	51)
	(8967,	51)
	(8968,	51)
	(8969,	51)
	(8970,	51)
	(8971,	54)
	(8972,	54)
	(8973,	54)
	(8974,	54)
	(8975,	54)
	(8976,	54)
	(8977,	54)
	(8978,	55)
	(8979,	56)
	(8980,	57)
	(8981,	57)
	(8982,	58)
	(8983,	58)
	(8984,	59)
	(8985,	59)
	(8986,	59)
	(8987,	59)
	(8988,	60)
	(8989,	61)
	(8990,	61)
	(8991,	61)
	(8992,	61)
	(8993,	61)
	(8994,	61)
	(8995,	62)
	(8996,	63)
	(8997,	64)
	(8998,	64)
	(8999,	64)
	(9000,	64)
	(9010,	68)
	(9020,	75)
	(9030,	81)
	(9040,	87)
	(9050,	95)
	(9060,	102)
	(9070,	103)
	(9080,	106)
	(9090,	108)
	(9100,	112)
	(9110,	118)
	(9120,	122)
	(9130,	126)
	(9140,	127)
	(9150,	132)
	(9160,	141)
	(9170,	146)
	(9180,	152)
	(9190,	154)
	(9200,	158)
	(9210,	158)
	(9220,	160)
	(9230,	166)
	(9240,	171)
	(9250,	176)
	(9260,	178)
	(9270,	181)
	(9280,	183)
	(9290,	186)
	(9300,	191)
	(9310,	197)
	(9320,	203)
	(9330,	215)
	(9340,	217)
	(9350,	221)
	(9360,	226)
	(9370,	230)
	(9380,	233)
	(9390,	237)
	(9400,	241)
	(9410,	250)
	(9420,	254)
	(9430,	260)
	(9440,	265)
	(9450,	275)
	(9460,	275)
	(9470,	277)
	(9480,	279)
	(9490,	282)
	(9500,	287)
	(9510,	292)
	(9520,	296)
	(9530,	301)
	(9540,	307)
	(9550,	309)
	(9560,	314)
	(9570,	317)
	(9580,	326)
	(9590,	333)
	(9600,	342)
	(9610,	348)
	(9620,	355)
	(9630,	362)
	(9640,	370)
	(9650,	374)
	(9660,	380)
	(9670,	390)
	(9680,	394)
	(9690,	397)
	(9700,	404)
	(9710,	414)
	(9720,	420)
	(9730,	427)
	(9740,	432)
	(9750,	434)
	(9760,	437)
	(9770,	439)
	(9780,	443)
	(9790,	446)
	(9800,	450)
	(9810,	451)
	(9820,	455)
	(9830,	457)
	(9840,	462)
	(9850,	468)
	(9860,	477)
	(9870,	483)
	(9880,	487)
	(9890,	501)
	(9900,	503)
	(9910,	504)
	(9920,	507)
	(9930,	511)
	(9940,	516)
	(9950,	518)
	(9960,	525)
	(9970,	533)
	(9980,	539)
	(9990,	541)
	(10000,	549)
};
\addplot[color=black, mark=none, line width=10pt, smooth] plot coordinates {
	(0,	538)
	(10,	532)
	(20,	524)
	(30,	525)
	(40,	518)
	(50,	514)
	(60,	509)
	(70,	508)
	(80,	505)
	(90,	496)
	(100,	492)
	(110,	487)
	(120,	482)
	(130,	483)
	(140,	478)
	(150,	472)
	(160,	470)
	(170,	464)
	(180,	455)
	(190,	448)
	(200,	442)
	(210,	435)
	(220,	430)
	(230,	429)
	(240,	423)
	(250,	422)
	(260,	416)
	(270,	409)
	(280,	407)
	(290,	401)
	(300,	396)
	(310,	393)
	(320,	387)
	(330,	383)
	(340,	374)
	(350,	372)
	(360,	366)
	(370,	360)
	(380,	356)
	(390,	356)
	(400,	350)
	(410,	351)
	(420,	348)
	(430,	340)
	(440,	332)
	(450,	329)
	(460,	327)
	(470,	325)
	(480,	318)
	(490,	308)
	(500,	302)
	(510,	295)
	(520,	287)
	(530,	280)
	(540,	273)
	(550,	269)
	(560,	267)
	(570,	261)
	(580,	254)
	(590,	248)
	(600,	243)
	(610,	237)
	(620,	228)
	(630,	224)
	(640,	216)
	(650,	213)
	(660,	204)
	(670,	197)
	(680,	189)
	(690,	186)
	(700,	182)
	(710,	175)
	(720,	170)
	(730,	167)
	(740,	161)
	(750,	166)
	(760,	156)
	(770,	148)
	(780,	145)
	(790,	147)
	(800,	141)
	(801,	141)
	(802,	140)
	(803,	140)
	(804,	139)
	(805,	139)
	(806,	139)
	(807,	138)
	(808,	137)
	(809,	138)
	(810,	138)
	(811,	137)
	(812,	136)
	(813,	135)
	(814,	134)
	(815,	133)
	(816,	133)
	(817,	132)
	(818,	131)
	(819,	130)
	(820,	130)
	(821,	133)
	(822,	132)
	(823,	131)
	(824,	133)
	(825,	134)
	(826,	133)
	(827,	132)
	(828,	133)
	(829,	132)
	(830,	132)
	(831,	131)
	(832,	130)
	(833,	131)
	(834,	131)
	(835,	131)
	(836,	130)
	(837,	129)
	(838,	128)
	(839,	127)
	(840,	126)
	(841,	127)
	(842,	126)
	(843,	125)
	(844,	124)
	(845,	123)
	(846,	123)
	(847,	122)
	(848,	122)
	(849,	121)
	(850,	124)
	(851,	123)
	(852,	122)
	(853,	121)
	(854,	120)
	(855,	119)
	(856,	118)
	(857,	117)
	(858,	116)
	(859,	115)
	(860,	114)
	(861,	113)
	(862,	112)
	(863,	112)
	(864,	111)
	(865,	110)
	(866,	109)
	(867,	108)
	(868,	107)
	(869,	106)
	(870,	106)
	(871,	105)
	(872,	104)
	(873,	104)
	(874,	103)
	(875,	102)
	(876,	101)
	(877,	100)
	(878,	99)
	(879,	100)
	(880,	101)
	(881,	101)
	(882,	100)
	(883,	99)
	(884,	98)
	(885,	98)
	(886,	99)
	(887,	98)
	(888,	98)
	(889,	97)
	(890,	97)
	(891,	96)
	(892,	95)
	(893,	95)
	(894,	94)
	(895,	93)
	(896,	92)
	(897,	97)
	(898,	96)
	(899,	97)
	(900,	96)
	(901,	96)
	(902,	95)
	(903,	95)
	(904,	94)
	(905,	93)
	(906,	94)
	(907,	93)
	(908,	93)
	(909,	92)
	(910,	91)
	(911,	90)
	(912,	89)
	(913,	88)
	(914,	87)
	(915,	86)
	(916,	85)
	(917,	84)
	(918,	83)
	(919,	82)
	(920,	82)
	(921,	81)
	(922,	80)
	(923,	79)
	(924,	78)
	(925,	77)
	(926,	76)
	(927,	76)
	(928,	75)
	(929,	75)
	(930,	74)
	(931,	73)
	(932,	72)
	(933,	71)
	(934,	70)
	(935,	69)
	(936,	68)
	(937,	67)
	(938,	66)
	(939,	65)
	(940,	64)
	(941,	63)
	(942,	62)
	(943,	62)
	(944,	61)
	(945,	60)
	(946,	60)
	(947,	61)
	(948,	60)
	(949,	59)
	(950,	58)
	(951,	57)
	(952,	57)
	(953,	56)
	(954,	55)
	(955,	54)
	(956,	53)
	(957,	55)
	(958,	54)
	(959,	53)
	(960,	53)
	(961,	52)
	(962,	51)
	(963,	50)
	(964,	49)
	(965,	48)
	(966,	47)
	(967,	46)
	(968,	45)
	(969,	44)
	(970,	45)
	(971,	45)
	(972,	44)
	(973,	43)
	(974,	42)
	(975,	42)
	(976,	41)
	(977,	40)
	(978,	40)
	(979,	39)
	(980,	38)
	(981,	37)
	(982,	37)
	(983,	36)
	(984,	35)
	(985,	36)
	(986,	39)
	(987,	40)
	(988,	39)
	(989,	38)
	(990,	37)
	(991,	38)
	(992,	37)
	(993,	36)
	(994,	35)
	(995,	34)
	(996,	33)
	(997,	32)
	(998,	31)
	(999,	30)
	(1000,	29)
	(1001,	28)
	(1002,	27)
	(1003,	27)
	(1004,	26)
	(1005,	25)
	(1006,	24)
	(1007,	24)
	(1008,	23)
	(1009,	23)
	(1010,	23)
	(1011,	23)
	(1012,	22)
	(1013,	22)
	(1014,	21)
	(1015,	21)
	(1016,	20)
	(1017,	20)
	(1018,	19)
	(1019,	18)
	(1020,	17)
	(1021,	16)
	(1022,	15)
	(1023,	14)
	(1024,	13)
	(1025,	12)
	(1026,	11)
	(1027,	10)
	(1028,	10)
	(1029,	11)
	(1030,	11)
	(1031,	12)
	(1032,	11)
	(1033,	10)
	(1034,	9)
	(1035,	9)
	(1036,	8)
	(1037,	8)
	(1038,	7)
	(1039,	6)
	(1040,	5)
	(1041,	5)
	(1042,	4)
	(1043,	3)
	(1044,	2)
	(1045,	1)
	(1046,	0)
	(1047,	2)
	(1048,	2)
	(1049,	2)
	(1050,	2)
	(1051,	2)
	(1052,	3)
	(1053,	4)
	(1054,	5)
	(1055,	6)
	(1056,	7)
	(1057,	7)
	(1058,	7)
	(1059,	7)
	(1060,	9)
	(1061,	11)
	(1062,	11)
	(1063,	11)
	(1064,	11)
	(1065,	12)
	(1066,	12)
	(1067,	13)
	(1068,	13)
	(1069,	13)
	(1070,	13)
	(1071,	13)
	(1072,	13)
	(1073,	13)
	(1074,	13)
	(1075,	15)
	(1076,	15)
	(1077,	15)
	(1078,	16)
	(1079,	16)
	(1080,	16)
	(1081,	17)
	(1082,	17)
	(1083,	17)
	(1084,	17)
	(1085,	17)
	(1086,	19)
	(1087,	19)
	(1088,	19)
	(1089,	21)
	(1090,	21)
	(1091,	26)
	(1092,	27)
	(1093,	28)
	(1094,	28)
	(1095,	30)
	(1096,	31)
	(1097,	31)
	(1098,	31)
	(1099,	32)
	(1100,	32)
	(1101,	32)
	(1102,	32)
	(1103,	32)
	(1104,	32)
	(1105,	32)
	(1106,	32)
	(1107,	33)
	(1108,	34)
	(1109,	34)
	(1110,	34)
	(1111,	36)
	(1112,	37)
	(1113,	38)
	(1114,	38)
	(1115,	39)
	(1116,	39)
	(1117,	41)
	(1118,	41)
	(1119,	42)
	(1120,	44)
	(1121,	44)
	(1122,	45)
	(1123,	46)
	(1124,	46)
	(1125,	46)
	(1126,	46)
	(1127,	46)
	(1128,	48)
	(1129,	48)
	(1130,	48)
	(1131,	49)
	(1132,	49)
	(1133,	49)
	(1134,	49)
	(1135,	52)
	(1136,	52)
	(1137,	52)
	(1138,	52)
	(1139,	54)
	(1140,	55)
	(1141,	55)
	(1142,	55)
	(1143,	56)
	(1144,	56)
	(1145,	58)
	(1146,	58)
	(1147,	59)
	(1148,	60)
	(1149,	60)
	(1150,	61)
	(1151,	61)
	(1152,	61)
	(1153,	61)
	(1154,	61)
	(1155,	61)
	(1156,	62)
	(1157,	63)
	(1158,	63)
	(1159,	63)
	(1160,	63)
	(1161,	64)
	(1162,	66)
	(1163,	66)
	(1164,	67)
	(1165,	67)
	(1166,	67)
	(1167,	68)
	(1168,	70)
	(1169,	72)
	(1170,	72)
	(1171,	73)
	(1172,	73)
	(1173,	73)
	(1174,	75)
	(1175,	76)
	(1176,	76)
	(1177,	79)
	(1178,	79)
	(1179,	82)
	(1180,	83)
	(1181,	84)
	(1182,	84)
	(1183,	84)
	(1184,	84)
	(1185,	84)
	(1186,	84)
	(1187,	84)
	(1188,	85)
	(1189,	85)
	(1190,	85)
	(1191,	85)
	(1192,	86)
	(1193,	86)
	(1194,	86)
	(1195,	86)
	(1196,	88)
	(1197,	89)
	(1198,	91)
	(1199,	91)
	(1200,	91)
	(1210,	97)
	(1220,	100)
	(1230,	105)
	(1240,	109)
	(1250,	112)
	(1260,	115)
	(1270,	122)
	(1280,	125)
	(1290,	130)
	(1300,	133)
	(1310,	135)
	(1320,	139)
	(1330,	147)
	(1340,	150)
	(1350,	159)
	(1360,	164)
	(1370,	176)
	(1380,	182)
	(1390,	189)
	(1400,	205)
	(1410,	207)
	(1420,	209)
	(1430,	220)
	(1440,	231)
	(1450,	234)
	(1460,	235)
	(1470,	240)
	(1480,	242)
	(1490,	245)
	(1500,	258)
	(1510,	268)
	(1520,	270)
	(1530,	275)
	(1540,	278)
	(1550,	284)
	(1560,	293)
	(1570,	299)
	(1580,	303)
	(1590,	309)
	(1600,	313)
	(1610,	319)
	(1620,	323)
	(1630,	329)
	(1640,	338)
	(1650,	341)
	(1660,	347)
	(1670,	348)
	(1680,	352)
	(1690,	356)
	(1700,	362)
	(1710,	366)
	(1720,	371)
	(1730,	373)
	(1740,	378)
	(1750,	386)
	(1760,	389)
	(1770,	396)
	(1780,	399)
	(1790,	404)
	(1800,	410)
	(1810,	415)
	(1820,	417)
	(1830,	419)
	(1840,	423)
	(1850,	428)
	(1860,	431)
	(1870,	434)
	(1880,	439)
	(1890,	443)
	(1900,	452)
	(1910,	454)
	(1920,	457)
	(1930,	462)
	(1940,	468)
	(1950,	472)
	(1960,	477)
	(1970,	481)
	(1980,	485)
	(1990,	485)
	(2000,	490)
	(2010,	499)
	(2020,	501)
	(2030,	506)
	(2040,	515)
	(2050,	518)
	(2060,	521)
	(2070,	523)
	(2080,	526)
	(2090,	529)
	(2100,	535)
	(2110,	542)
	(2120,	552)
	(2130,	556)
	(2140,	570)
	(2150,	578)
	(2160,	582)
	(2170,	586)
	(2180,	589)
	(2190,	595)
	(2200,	600)
	(2210,	603)
	(2220,	607)
	(2230,	610)
	(2240,	613)
	(2250,	621)
	(2260,	623)
	(2270,	631)
	(2280,	635)
	(2290,	637)
	(2300,	641)
	(2310,	654)
	(2320,	662)
	(2330,	664)
	(2340,	668)
	(2350,	671)
	(2360,	673)
	(2370,	677)
	(2380,	679)
	(2390,	685)
	(2400,	688)
	(2410,	693)
	(2420,	700)
	(2430,	704)
	(2440,	709)
	(2450,	712)
	(2460,	717)
	(2470,	719)
	(2480,	726)
	(2490,	732)
	(2500,	737)
	(2510,	749)
	(2520,	754)
	(2530,	758)
	(2540,	758)
	(2550,	762)
	(2560,	769)
	(2570,	773)
	(2580,	779)
	(2590,	783)
	(2600,	783)
	(2610,	785)
	(2620,	789)
	(2630,	796)
	(2640,	803)
	(2650,	814)
	(2660,	815)
	(2670,	820)
	(2680,	823)
	(2690,	832)
	(2700,	836)
	(2710,	844)
	(2720,	848)
	(2730,	854)
	(2740,	858)
	(2750,	864)
	(2760,	866)
	(2770,	870)
	(2780,	872)
	(2790,	873)
	(2800,	873)
	(2810,	877)
	(2820,	884)
	(2830,	893)
	(2840,	904)
	(2850,	905)
	(2860,	907)
	(2870,	911)
	(2880,	916)
	(2890,	923)
	(2900,	932)
	(2910,	936)
	(2920,	940)
	(2930,	948)
	(2940,	955)
	(2950,	960)
	(2960,	965)
	(2970,	966)
	(2980,	973)
	(2990,	975)
	(3000,	984)
	(3010,	990)
	(3020,	999)
	(3030,	1004)
	(3040,	1005)
	(3050,	1012)
	(3060,	1016)
	(3070,	1021)
	(3080,	1022)
	(3090,	1025)
	(3100,	1029)
	(3110,	1035)
	(3120,	1040)
	(3130,	1044)
	(3140,	1048)
	(3150,	1052)
	(3160,	1056)
	(3170,	1062)
	(3180,	1062)
	(3190,	1066)
	(3200,	1071)
	(3210,	1075)
	(3220,	1082)
	(3230,	1083)
	(3240,	1091)
	(3250,	1102)
	(3260,	1112)
	(3270,	1116)
	(3280,	1120)
	(3290,	1122)
	(3300,	1125)
	(3310,	1137)
	(3320,	1138)
	(3330,	1142)
	(3340,	1144)
	(3350,	1151)
	(3360,	1156)
	(3370,	1160)
	(3380,	1166)
	(3390,	1175)
	(3400,	1181)
	(3410,	1189)
	(3420,	1193)
	(3430,	1201)
	(3440,	1205)
	(3450,	1208)
	(3460,	1211)
	(3470,	1218)
	(3480,	1229)
	(3490,	1230)
	(3500,	1231)
	(3510,	1236)
	(3520,	1239)
	(3530,	1244)
	(3540,	1250)
	(3550,	1258)
	(3560,	1264)
	(3570,	1270)
	(3580,	1277)
	(3590,	1287)
	(3600,	1293)
	(3610,	1299)
	(3620,	1303)
	(3630,	1307)
	(3640,	1310)
	(3650,	1316)
	(3660,	1320)
	(3670,	1325)
	(3680,	1332)
	(3690,	1338)
	(3700,	1351)
	(3710,	1354)
	(3720,	1361)
	(3730,	1362)
	(3740,	1365)
	(3750,	1374)
	(3760,	1377)
	(3770,	1381)
	(3780,	1389)
	(3790,	1391)
	(3800,	1393)
	(3810,	1403)
	(3820,	1409)
	(3830,	1423)
	(3840,	1427)
	(3850,	1432)
	(3860,	1435)
	(3870,	1442)
	(3880,	1443)
	(3890,	1452)
	(3900,	1459)
	(3910,	1465)
	(3920,	1472)
	(3930,	1477)
	(3940,	1481)
	(3950,	1490)
	(3960,	1493)
	(3970,	1499)
	(3980,	1502)
	(3990,	1510)
	(4000,	1512)
	(4010,	1521)
	(4020,	1526)
	(4030,	1536)
	(4040,	1543)
	(4050,	1546)
	(4060,	1549)
	(4070,	1554)
	(4080,	1559)
	(4090,	1562)
	(4100,	1569)
	(4110,	1575)
	(4120,	1586)
	(4130,	1591)
	(4140,	1594)
	(4150,	1602)
	(4160,	1607)
	(4170,	1610)
	(4180,	1613)
	(4190,	1618)
	(4200,	1629)
	(4210,	1632)
	(4220,	1637)
	(4230,	1642)
	(4240,	1647)
	(4250,	1650)
	(4260,	1654)
	(4270,	1659)
	(4280,	1662)
	(4290,	1665)
	(4300,	1668)
	(4310,	1674)
	(4320,	1676)
	(4330,	1680)
	(4340,	1685)
	(4350,	1688)
	(4360,	1689)
	(4370,	1695)
	(4380,	1700)
	(4390,	1705)
	(4400,	1709)
	(4410,	1718)
	(4420,	1722)
	(4430,	1726)
	(4440,	1734)
	(4450,	1737)
	(4460,	1739)
	(4470,	1745)
	(4480,	1750)
	(4490,	1752)
	(4500,	1753)
	(4510,	1756)
	(4520,	1762)
	(4530,	1767)
	(4540,	1772)
	(4550,	1774)
	(4560,	1774)
	(4570,	1780)
	(4580,	1786)
	(4590,	1789)
	(4600,	1794)
	(4610,	1796)
	(4620,	1802)
	(4630,	1804)
	(4640,	1806)
	(4650,	1809)
	(4660,	1813)
	(4670,	1813)
	(4680,	1816)
	(4690,	1821)
	(4700,	1829)
	(4701,	1829)
	(4702,	1829)
	(4703,	1830)
	(4704,	1831)
	(4705,	1832)
	(4706,	1832)
	(4707,	1832)
	(4708,	1833)
	(4709,	1833)
	(4710,	1834)
	(4711,	1834)
	(4712,	1834)
	(4713,	1834)
	(4714,	1835)
	(4715,	1835)
	(4716,	1836)
	(4717,	1836)
	(4718,	1836)
	(4719,	1836)
	(4720,	1836)
	(4721,	1836)
	(4722,	1836)
	(4723,	1840)
	(4724,	1841)
	(4725,	1841)
	(4726,	1841)
	(4727,	1841)
	(4728,	1842)
	(4729,	1845)
	(4730,	1845)
	(4731,	1845)
	(4732,	1846)
	(4733,	1846)
	(4734,	1851)
	(4735,	1851)
	(4736,	1851)
	(4737,	1852)
	(4738,	1852)
	(4739,	1853)
	(4740,	1853)
	(4741,	1853)
	(4742,	1855)
	(4743,	1856)
	(4744,	1857)
	(4745,	1857)
	(4746,	1857)
	(4747,	1857)
	(4748,	1858)
	(4749,	1858)
	(4750,	1859)
	(4751,	1859)
	(4752,	1859)
	(4753,	1860)
	(4754,	1860)
	(4755,	1860)
	(4756,	1860)
	(4757,	1860)
	(4758,	1860)
	(4759,	1860)
	(4760,	1860)
	(4761,	1860)
	(4762,	1860)
	(4763,	1861)
	(4764,	1864)
	(4765,	1865)
	(4766,	1865)
	(4767,	1867)
	(4768,	1867)
	(4769,	1867)
	(4770,	1867)
	(4771,	1867)
	(4772,	1867)
	(4773,	1867)
	(4774,	1867)
	(4775,	1870)
	(4776,	1871)
	(4777,	1871)
	(4778,	1871)
	(4779,	1871)
	(4780,	1871)
	(4781,	1871)
	(4782,	1873)
	(4783,	1873)
	(4784,	1874)
	(4785,	1874)
	(4786,	1877)
	(4787,	1878)
	(4788,	1878)
	(4789,	1878)
	(4790,	1878)
	(4791,	1878)
	(4792,	1878)
	(4793,	1878)
	(4794,	1880)
	(4795,	1880)
	(4796,	1880)
	(4797,	1882)
	(4798,	1882)
	(4799,	1882)
	(4800,	1882)
	(4801,	1882)
	(4802,	1884)
	(4803,	1884)
	(4804,	1885)
	(4805,	1885)
	(4806,	1887)
	(4807,	1887)
	(4808,	1889)
	(4809,	1889)
	(4810,	1889)
	(4811,	1890)
	(4812,	1890)
	(4813,	1890)
	(4814,	1891)
	(4815,	1892)
	(4816,	1892)
	(4817,	1893)
	(4818,	1893)
	(4819,	1893)
	(4820,	1893)
	(4821,	1894)
	(4822,	1896)
	(4823,	1899)
	(4824,	1899)
	(4825,	1900)
	(4826,	1900)
	(4827,	1902)
	(4828,	1904)
	(4829,	1904)
	(4830,	1904)
	(4831,	1907)
	(4832,	1907)
	(4833,	1908)
	(4834,	1908)
	(4835,	1908)
	(4836,	1908)
	(4837,	1908)
	(4838,	1909)
	(4839,	1912)
	(4840,	1912)
	(4841,	1913)
	(4842,	1914)
	(4843,	1914)
	(4844,	1914)
	(4845,	1914)
	(4846,	1914)
	(4847,	1914)
	(4848,	1914)
	(4849,	1914)
	(4850,	1914)
	(4851,	1914)
	(4852,	1914)
	(4853,	1914)
	(4854,	1914)
	(4855,	1914)
	(4856,	1914)
	(4857,	1914)
	(4858,	1915)
	(4859,	1915)
	(4860,	1915)
	(4861,	1915)
	(4862,	1915)
	(4863,	1916)
	(4864,	1916)
	(4865,	1916)
	(4866,	1917)
	(4867,	1917)
	(4868,	1917)
	(4869,	1917)
	(4870,	1917)
	(4871,	1917)
	(4872,	1917)
	(4873,	1917)
	(4874,	1917)
	(4875,	1917)
	(4876,	1917)
	(4877,	1917)
	(4878,	1917)
	(4879,	1917)
	(4880,	1920)
	(4881,	1920)
	(4882,	1922)
	(4883,	1922)
	(4884,	1922)
	(4885,	1923)
	(4886,	1923)
	(4887,	1923)
	(4888,	1923)
	(4889,	1923)
	(4890,	1923)
	(4891,	1923)
	(4892,	1923)
	(4893,	1923)
	(4894,	1925)
	(4895,	1926)
	(4896,	1926)
	(4897,	1926)
	(4898,	1926)
	(4899,	1926)
	(4900,	1927)
	(4901,	1927)
	(4902,	1927)
	(4903,	1927)
	(4904,	1927)
	(4905,	1929)
	(4906,	1929)
	(4907,	1930)
	(4908,	1930)
	(4909,	1930)
	(4910,	1930)
	(4911,	1930)
	(4912,	1930)
	(4913,	1930)
	(4914,	1930)
	(4915,	1930)
	(4916,	1930)
	(4917,	1930)
	(4918,	1930)
	(4919,	1931)
	(4920,	1931)
	(4921,	1931)
	(4922,	1931)
	(4923,	1931)
	(4924,	1932)
	(4925,	1932)
	(4926,	1933)
	(4927,	1933)
	(4928,	1933)
	(4929,	1934)
	(4930,	1935)
	(4931,	1935)
	(4932,	1936)
	(4933,	1936)
	(4934,	1937)
	(4935,	1937)
	(4936,	1938)
	(4937,	1937)
	(4938,	1938)
	(4939,	1937)
	(4940,	1936)
	(4941,	1935)
	(4942,	1934)
	(4943,	1934)
	(4944,	1933)
	(4945,	1932)
	(4946,	1931)
	(4947,	1930)
	(4948,	1930)
	(4949,	1929)
	(4950,	1928)
	(4951,	1927)
	(4952,	1926)
	(4953,	1925)
	(4954,	1924)
	(4955,	1923)
	(4956,	1923)
	(4957,	1923)
	(4958,	1922)
	(4959,	1922)
	(4960,	1922)
	(4961,	1921)
	(4962,	1921)
	(4963,	1920)
	(4964,	1919)
	(4965,	1918)
	(4966,	1917)
	(4967,	1917)
	(4968,	1917)
	(4969,	1917)
	(4970,	1917)
	(4971,	1916)
	(4972,	1915)
	(4973,	1914)
	(4974,	1913)
	(4975,	1912)
	(4976,	1911)
	(4977,	1912)
	(4978,	1911)
	(4979,	1910)
	(4980,	1909)
	(4981,	1908)
	(4982,	1908)
	(4983,	1907)
	(4984,	1906)
	(4985,	1905)
	(4986,	1904)
	(4987,	1903)
	(4988,	1903)
	(4989,	1903)
	(4990,	1903)
	(4991,	1902)
	(4992,	1901)
	(4993,	1900)
	(4994,	1901)
	(4995,	1900)
	(4996,	1900)
	(4997,	1900)
	(4998,	1900)
	(4999,	1899)
	(5000,	1898)
	(5001,	1897)
	(5002,	1898)
	(5003,	1898)
	(5004,	1897)
	(5005,	1896)
	(5006,	1895)
	(5007,	1894)
	(5008,	1893)
	(5009,	1893)
	(5010,	1893)
	(5011,	1895)
	(5012,	1896)
	(5013,	1895)
	(5014,	1894)
	(5015,	1893)
	(5016,	1894)
	(5017,	1893)
	(5018,	1893)
	(5019,	1892)
	(5020,	1891)
	(5021,	1892)
	(5022,	1891)
	(5023,	1893)
	(5024,	1892)
	(5025,	1891)
	(5026,	1890)
	(5027,	1889)
	(5028,	1889)
	(5029,	1888)
	(5030,	1887)
	(5031,	1886)
	(5032,	1885)
	(5033,	1885)
	(5034,	1884)
	(5035,	1884)
	(5036,	1885)
	(5037,	1884)
	(5038,	1883)
	(5039,	1883)
	(5040,	1882)
	(5041,	1882)
	(5042,	1882)
	(5043,	1882)
	(5044,	1881)
	(5045,	1880)
	(5046,	1880)
	(5047,	1880)
	(5048,	1879)
	(5049,	1879)
	(5050,	1878)
	(5051,	1879)
	(5052,	1878)
	(5053,	1877)
	(5054,	1876)
	(5055,	1876)
	(5056,	1878)
	(5057,	1877)
	(5058,	1876)
	(5059,	1875)
	(5060,	1874)
	(5061,	1873)
	(5062,	1872)
	(5063,	1871)
	(5064,	1870)
	(5065,	1870)
	(5066,	1869)
	(5067,	1869)
	(5068,	1869)
	(5069,	1869)
	(5070,	1872)
	(5071,	1871)
	(5072,	1870)
	(5073,	1869)
	(5074,	1868)
	(5075,	1867)
	(5076,	1866)
	(5077,	1867)
	(5078,	1869)
	(5079,	1868)
	(5080,	1868)
	(5081,	1867)
	(5082,	1867)
	(5083,	1867)
	(5084,	1867)
	(5085,	1867)
	(5086,	1866)
	(5087,	1866)
	(5088,	1866)
	(5089,	1865)
	(5090,	1865)
	(5091,	1864)
	(5092,	1864)
	(5093,	1863)
	(5094,	1862)
	(5095,	1861)
	(5096,	1860)
	(5097,	1862)
	(5098,	1861)
	(5099,	1861)
	(5100,	1860)
	(5110,	1858)
	(5120,	1854)
	(5130,	1849)
	(5140,	1842)
	(5150,	1833)
	(5160,	1834)
	(5170,	1829)
	(5180,	1823)
	(5190,	1821)
	(5200,	1815)
	(5210,	1814)
	(5220,	1813)
	(5230,	1814)
	(5240,	1808)
	(5250,	1802)
	(5260,	1795)
	(5270,	1791)
	(5280,	1782)
	(5290,	1777)
	(5300,	1771)
	(5310,	1765)
	(5320,	1759)
	(5330,	1753)
	(5340,	1747)
	(5350,	1751)
	(5360,	1742)
	(5370,	1734)
	(5380,	1727)
	(5390,	1722)
	(5400,	1719)
	(5410,	1711)
	(5420,	1705)
	(5430,	1701)
	(5440,	1693)
	(5450,	1690)
	(5460,	1686)
	(5470,	1680)
	(5480,	1673)
	(5490,	1668)
	(5500,	1664)
	(5510,	1661)
	(5520,	1661)
	(5530,	1655)
	(5540,	1650)
	(5550,	1646)
	(5560,	1637)
	(5570,	1638)
	(5580,	1630)
	(5590,	1625)
	(5600,	1620)
	(5610,	1611)
	(5620,	1605)
	(5630,	1601)
	(5640,	1597)
	(5650,	1590)
	(5660,	1584)
	(5670,	1579)
	(5680,	1573)
	(5690,	1565)
	(5700,	1559)
	(5710,	1558)
	(5720,	1551)
	(5730,	1546)
	(5740,	1540)
	(5750,	1536)
	(5760,	1530)
	(5770,	1523)
	(5780,	1520)
	(5790,	1512)
	(5800,	1506)
	(5810,	1498)
	(5820,	1492)
	(5830,	1487)
	(5840,	1483)
	(5850,	1477)
	(5860,	1467)
	(5870,	1460)
	(5880,	1456)
	(5890,	1448)
	(5900,	1445)
	(5910,	1438)
	(5920,	1431)
	(5930,	1423)
	(5940,	1420)
	(5950,	1416)
	(5960,	1410)
	(5970,	1403)
	(5980,	1399)
	(5990,	1396)
	(6000,	1389)
	(6010,	1389)
	(6020,	1390)
	(6030,	1383)
	(6040,	1382)
	(6050,	1377)
	(6060,	1369)
	(6070,	1366)
	(6080,	1359)
	(6090,	1353)
	(6100,	1348)
	(6110,	1344)
	(6120,	1342)
	(6130,	1337)
	(6140,	1333)
	(6150,	1330)
	(6160,	1329)
	(6170,	1325)
	(6180,	1318)
	(6190,	1311)
	(6200,	1306)
	(6210,	1298)
	(6220,	1290)
	(6230,	1283)
	(6240,	1277)
	(6250,	1272)
	(6260,	1265)
	(6270,	1261)
	(6280,	1259)
	(6290,	1250)
	(6300,	1241)
	(6310,	1238)
	(6320,	1233)
	(6330,	1227)
	(6340,	1228)
	(6350,	1221)
	(6360,	1215)
	(6370,	1212)
	(6380,	1205)
	(6390,	1199)
	(6400,	1194)
	(6410,	1186)
	(6420,	1183)
	(6430,	1174)
	(6440,	1167)
	(6450,	1160)
	(6460,	1154)
	(6470,	1149)
	(6480,	1146)
	(6490,	1138)
	(6500,	1136)
	(6510,	1134)
	(6520,	1128)
	(6530,	1122)
	(6540,	1118)
	(6550,	1109)
	(6560,	1101)
	(6570,	1095)
	(6580,	1090)
	(6590,	1080)
	(6600,	1074)
	(6610,	1070)
	(6620,	1069)
	(6630,	1066)
	(6640,	1059)
	(6650,	1054)
	(6660,	1046)
	(6670,	1040)
	(6680,	1033)
	(6690,	1027)
	(6700,	1022)
	(6710,	1016)
	(6720,	1011)
	(6730,	1004)
	(6740,	1002)
	(6750,	995)
	(6760,	988)
	(6770,	980)
	(6780,	976)
	(6790,	971)
	(6800,	963)
	(6810,	960)
	(6820,	951)
	(6830,	944)
	(6840,	936)
	(6850,	929)
	(6860,	922)
	(6870,	919)
	(6880,	916)
	(6890,	910)
	(6900,	904)
	(6910,	898)
	(6920,	892)
	(6930,	886)
	(6940,	877)
	(6950,	875)
	(6960,	868)
	(6970,	862)
	(6980,	854)
	(6990,	850)
	(7000,	844)
	(7010,	841)
	(7020,	836)
	(7030,	829)
	(7040,	825)
	(7050,	818)
	(7060,	810)
	(7070,	807)
	(7080,	798)
	(7090,	791)
	(7100,	790)
	(7110,	786)
	(7120,	780)
	(7130,	775)
	(7140,	772)
	(7150,	765)
	(7160,	759)
	(7170,	754)
	(7180,	750)
	(7190,	744)
	(7200,	738)
	(7210,	731)
	(7220,	723)
	(7230,	722)
	(7240,	717)
	(7250,	711)
	(7260,	702)
	(7270,	695)
	(7280,	688)
	(7290,	680)
	(7300,	674)
	(7310,	665)
	(7320,	662)
	(7330,	658)
	(7340,	657)
	(7350,	655)
	(7360,	655)
	(7370,	651)
	(7380,	650)
	(7390,	643)
	(7400,	637)
	(7410,	630)
	(7420,	625)
	(7430,	617)
	(7440,	614)
	(7450,	611)
	(7460,	607)
	(7470,	599)
	(7480,	590)
	(7490,	584)
	(7500,	575)
	(7510,	576)
	(7520,	572)
	(7530,	564)
	(7540,	564)
	(7550,	560)
	(7560,	552)
	(7570,	549)
	(7580,	546)
	(7590,	540)
	(7600,	538)
	(7610,	532)
	(7620,	525)
	(7630,	516)
	(7640,	510)
	(7650,	503)
	(7660,	502)
	(7670,	497)
	(7680,	490)
	(7690,	486)
	(7700,	478)
	(7710,	471)
	(7720,	465)
	(7730,	458)
	(7740,	452)
	(7750,	448)
	(7760,	444)
	(7770,	442)
	(7780,	435)
	(7790,	431)
	(7800,	425)
	(7810,	416)
	(7820,	413)
	(7830,	413)
	(7840,	407)
	(7850,	399)
	(7860,	390)
	(7870,	382)
	(7880,	376)
	(7890,	367)
	(7900,	367)
	(7910,	365)
	(7920,	361)
	(7930,	353)
	(7940,	346)
	(7950,	343)
	(7960,	340)
	(7970,	339)
	(7980,	332)
	(7990,	325)
	(8000,	321)
	(8010,	314)
	(8020,	306)
	(8030,	304)
	(8040,	302)
	(8050,	298)
	(8060,	293)
	(8070,	290)
	(8080,	288)
	(8090,	283)
	(8100,	278)
	(8110,	276)
	(8120,	268)
	(8130,	261)
	(8140,	254)
	(8150,	251)
	(8160,	247)
	(8170,	244)
	(8180,	239)
	(8190,	233)
	(8200,	230)
	(8210,	225)
	(8220,	220)
	(8230,	218)
	(8240,	213)
	(8250,	206)
	(8260,	200)
	(8270,	196)
	(8280,	189)
	(8290,	184)
	(8300,	176)
	(8310,	168)
	(8320,	168)
	(8330,	164)
	(8340,	158)
	(8350,	153)
	(8360,	146)
	(8370,	139)
	(8380,	136)
	(8390,	130)
	(8400,	127)
	(8410,	129)
	(8420,	124)
	(8430,	116)
	(8440,	115)
	(8450,	112)
	(8460,	105)
	(8470,	102)
	(8480,	95)
	(8490,	87)
	(8500,	79)
	(8510,	72)
	(8520,	66)
	(8530,	65)
	(8540,	61)
	(8550,	58)
	(8560,	51)
	(8570,	46)
	(8580,	46)
	(8590,	40)
	(8600,	39)
	(8601,	38)
	(8602,	37)
	(8603,	36)
	(8604,	36)
	(8605,	35)
	(8606,	35)
	(8607,	35)
	(8608,	34)
	(8609,	33)
	(8610,	32)
	(8611,	31)
	(8612,	30)
	(8613,	29)
	(8614,	29)
	(8615,	29)
	(8616,	28)
	(8617,	27)
	(8618,	26)
	(8619,	25)
	(8620,	24)
	(8621,	23)
	(8622,	22)
	(8623,	23)
	(8624,	22)
	(8625,	24)
	(8626,	23)
	(8627,	22)
	(8628,	21)
	(8629,	20)
	(8630,	20)
	(8631,	19)
	(8632,	18)
	(8633,	17)
	(8634,	16)
	(8635,	16)
	(8636,	15)
	(8637,	15)
	(8638,	15)
	(8639,	15)
	(8640,	14)
	(8641,	13)
	(8642,	12)
	(8643,	11)
	(8644,	12)
	(8645,	11)
	(8646,	11)
	(8647,	11)
	(8648,	11)
	(8649,	12)
	(8650,	11)
	(8651,	10)
	(8652,	9)
	(8653,	9)
	(8654,	9)
	(8655,	14)
	(8656,	13)
	(8657,	12)
	(8658,	11)
	(8659,	10)
	(8660,	12)
	(8661,	11)
	(8662,	10)
	(8663,	9)
	(8664,	10)
	(8665,	9)
	(8666,	8)
	(8667,	7)
	(8668,	8)
	(8669,	7)
	(8670,	6)
	(8671,	5)
	(8672,	4)
	(8673,	3)
	(8674,	2)
	(8675,	1)
	(8676,	1)
	(8677,	1)
	(8678,	0)
	(8679,	0)
	(8680,	0)
	(8681,	0)
	(8682,	0)
	(8683,	0)
	(8684,	0)
	(8685,	0)
	(8686,	0)
	(8687,	0)
	(8688,	1)
	(8689,	1)
	(8690,	1)
	(8691,	1)
	(8692,	0)
	(8693,	0)
	(8694,	0)
	(8695,	1)
	(8696,	1)
	(8697,	1)
	(8698,	1)
	(8699,	0)
	(8700,	0)
	(8701,	0)
	(8702,	0)
	(8703,	0)
	(8704,	0)
	(8705,	0)
	(8706,	0)
	(8707,	0)
	(8708,	0)
	(8709,	1)
	(8710,	0)
	(8711,	0)
	(8712,	0)
	(8713,	0)
	(8714,	0)
	(8715,	0)
	(8716,	0)
	(8717,	0)
	(8718,	1)
	(8719,	1)
	(8720,	1)
	(8721,	0)
	(8722,	0)
	(8723,	0)
	(8724,	0)
	(8725,	0)
	(8726,	0)
	(8727,	0)
	(8728,	0)
	(8729,	2)
	(8730,	1)
	(8731,	1)
	(8732,	1)
	(8733,	0)
	(8734,	0)
	(8735,	0)
	(8736,	0)
	(8737,	0)
	(8738,	0)
	(8739,	0)
	(8740,	0)
	(8741,	3)
	(8742,	2)
	(8743,	1)
	(8744,	0)
	(8745,	0)
	(8746,	1)
	(8747,	1)
	(8748,	1)
	(8749,	1)
	(8750,	2)
	(8751,	2)
	(8752,	3)
	(8753,	2)
	(8754,	1)
	(8755,	0)
	(8756,	0)
	(8757,	0)
	(8758,	0)
	(8759,	1)
	(8760,	0)
	(8761,	0)
	(8762,	0)
	(8763,	1)
	(8764,	1)
	(8765,	1)
	(8766,	1)
	(8767,	0)
	(8768,	0)
	(8769,	3)
	(8770,	3)
	(8771,	2)
	(8772,	1)
	(8773,	1)
	(8774,	0)
	(8775,	0)
	(8776,	0)
	(8777,	0)
	(8778,	2)
	(8779,	1)
	(8780,	1)
	(8781,	1)
	(8782,	0)
	(8783,	0)
	(8784,	0)
	(8785,	0)
	(8786,	1)
	(8787,	1)
	(8788,	1)
	(8789,	0)
	(8790,	0)
	(8791,	0)
	(8792,	0)
	(8793,	0)
	(8794,	0)
	(8795,	0)
	(8796,	0)
	(8797,	0)
	(8798,	0)
	(8799,	4)
	(8800,	3)
	(8801,	3)
	(8802,	2)
	(8803,	1)
	(8804,	1)
	(8805,	1)
	(8806,	1)
	(8807,	0)
	(8808,	0)
	(8809,	0)
	(8810,	0)
	(8811,	0)
	(8812,	0)
	(8813,	1)
	(8814,	0)
	(8815,	0)
	(8816,	0)
	(8817,	0)
	(8818,	0)
	(8819,	0)
	(8820,	0)
	(8821,	0)
	(8822,	0)
	(8823,	0)
	(8824,	0)
	(8825,	0)
	(8826,	0)
	(8827,	0)
	(8828,	0)
	(8829,	0)
	(8830,	0)
	(8831,	0)
	(8832,	0)
	(8833,	0)
	(8834,	0)
	(8835,	1)
	(8836,	0)
	(8837,	0)
	(8838,	1)
	(8839,	2)
	(8840,	1)
	(8841,	0)
	(8842,	0)
	(8843,	0)
	(8844,	0)
	(8845,	0)
	(8846,	0)
	(8847,	1)
	(8848,	2)
	(8849,	1)
	(8850,	1)
	(8851,	1)
	(8852,	1)
	(8853,	0)
	(8854,	0)
	(8855,	0)
	(8856,	1)
	(8857,	0)
	(8858,	0)
	(8859,	0)
	(8860,	0)
	(8861,	0)
	(8862,	1)
	(8863,	1)
	(8864,	0)
	(8865,	0)
	(8866,	0)
	(8867,	1)
	(8868,	2)
	(8869,	1)
	(8870,	0)
	(8871,	0)
	(8872,	0)
	(8873,	0)
	(8874,	0)
	(8875,	2)
	(8876,	2)
	(8877,	3)
	(8878,	3)
	(8879,	3)
	(8880,	3)
	(8881,	3)
	(8882,	4)
	(8883,	4)
	(8884,	4)
	(8885,	4)
	(8886,	5)
	(8887,	5)
	(8888,	5)
	(8889,	6)
	(8890,	8)
	(8891,	9)
	(8892,	9)
	(8893,	9)
	(8894,	9)
	(8895,	10)
	(8896,	10)
	(8897,	11)
	(8898,	11)
	(8899,	11)
	(8900,	11)
	(8901,	12)
	(8902,	12)
	(8903,	12)
	(8904,	12)
	(8905,	12)
	(8906,	12)
	(8907,	12)
	(8908,	12)
	(8909,	12)
	(8910,	12)
	(8911,	13)
	(8912,	13)
	(8913,	13)
	(8914,	14)
	(8915,	16)
	(8916,	16)
	(8917,	16)
	(8918,	17)
	(8919,	18)
	(8920,	18)
	(8921,	19)
	(8922,	20)
	(8923,	20)
	(8924,	21)
	(8925,	21)
	(8926,	21)
	(8927,	23)
	(8928,	23)
	(8929,	23)
	(8930,	23)
	(8931,	24)
	(8932,	28)
	(8933,	28)
	(8934,	28)
	(8935,	28)
	(8936,	28)
	(8937,	28)
	(8938,	28)
	(8939,	28)
	(8940,	28)
	(8941,	28)
	(8942,	28)
	(8943,	28)
	(8944,	30)
	(8945,	30)
	(8946,	32)
	(8947,	33)
	(8948,	33)
	(8949,	33)
	(8950,	33)
	(8951,	33)
	(8952,	33)
	(8953,	33)
	(8954,	36)
	(8955,	37)
	(8956,	37)
	(8957,	38)
	(8958,	38)
	(8959,	38)
	(8960,	38)
	(8961,	41)
	(8962,	41)
	(8963,	42)
	(8964,	43)
	(8965,	43)
	(8966,	43)
	(8967,	44)
	(8968,	44)
	(8969,	45)
	(8970,	46)
	(8971,	46)
	(8972,	47)
	(8973,	47)
	(8974,	47)
	(8975,	49)
	(8976,	49)
	(8977,	49)
	(8978,	50)
	(8979,	50)
	(8980,	52)
	(8981,	52)
	(8982,	53)
	(8983,	53)
	(8984,	54)
	(8985,	54)
	(8986,	55)
	(8987,	55)
	(8988,	56)
	(8989,	57)
	(8990,	58)
	(8991,	58)
	(8992,	58)
	(8993,	58)
	(8994,	58)
	(8995,	59)
	(8996,	59)
	(8997,	59)
	(8998,	59)
	(8999,	61)
	(9000,	62)
	(9010,	70)
	(9020,	79)
	(9030,	82)
	(9040,	83)
	(9050,	86)
	(9060,	90)
	(9070,	95)
	(9080,	107)
	(9090,	119)
	(9100,	126)
	(9110,	134)
	(9120,	138)
	(9130,	150)
	(9140,	157)
	(9150,	164)
	(9160,	173)
	(9170,	178)
	(9180,	182)
	(9190,	188)
	(9200,	193)
	(9210,	202)
	(9220,	204)
	(9230,	207)
	(9240,	217)
	(9250,	220)
	(9260,	221)
	(9270,	225)
	(9280,	234)
	(9290,	237)
	(9300,	245)
	(9310,	249)
	(9320,	252)
	(9330,	257)
	(9340,	259)
	(9350,	265)
	(9360,	271)
	(9370,	271)
	(9380,	279)
	(9390,	281)
	(9400,	283)
	(9410,	287)
	(9420,	293)
	(9430,	299)
	(9440,	303)
	(9450,	308)
	(9460,	312)
	(9470,	316)
	(9480,	317)
	(9490,	318)
	(9500,	319)
	(9510,	335)
	(9520,	339)
	(9530,	344)
	(9540,	351)
	(9550,	355)
	(9560,	358)
	(9570,	360)
	(9580,	368)
	(9590,	371)
	(9600,	373)
	(9610,	380)
	(9620,	383)
	(9630,	389)
	(9640,	392)
	(9650,	395)
	(9660,	399)
	(9670,	401)
	(9680,	410)
	(9690,	421)
	(9700,	423)
	(9710,	426)
	(9720,	429)
	(9730,	435)
	(9740,	442)
	(9750,	449)
	(9760,	457)
	(9770,	459)
	(9780,	463)
	(9790,	465)
	(9800,	474)
	(9810,	479)
	(9820,	484)
	(9830,	486)
	(9840,	491)
	(9850,	491)
	(9860,	497)
	(9870,	505)
	(9880,	506)
	(9890,	511)
	(9900,	514)
	(9910,	517)
	(9920,	518)
	(9930,	522)
	(9940,	523)
	(9950,	524)
	(9960,	529)
	(9970,	534)
	(9980,	538)
	(9990,	547)
	(10000,	554)
};

==> fig/realtimezoomdata.tex <==
\addplot[color=black,densely dashdotted] plot coordinates {
	(0,	1407)
	(10,	1412)
	(20,	1417)
	(30,	1425)
	(40,	1433)
	(50,	1438)
	(60,	1454)
	(70,	1454)
	(80,	1460)
	(90,	1464)
	(100,	1472)
	(110,	1477)
	(120,	1481)
	(130,	1486)
	(140,	1493)
	(150,	1494)
	(160,	1496)
	(170,	1500)
	(180,	1505)
	(190,	1513)
	(200,	1520)
	(210,	1528)
	(220,	1531)
	(230,	1539)
	(240,	1547)
	(250,	1552)
	(260,	1560)
	(270,	1564)
	(280,	1568)
	(290,	1571)
	(300,	1572)
	(310,	1574)
	(320,	1584)
	(330,	1585)
	(340,	1592)
	(350,	1594)
	(360,	1601)
	(370,	1603)
	(380,	1607)
	(390,	1613)
	(400,	1615)
	(410,	1618)
	(420,	1622)
	(430,	1625)
	(440,	1626)
	(450,	1632)
	(460,	1637)
	(470,	1642)
	(480,	1652)
	(490,	1656)
	(500,	1661)
	(510,	1664)
	(520,	1669)
	(530,	1671)
	(540,	1683)
	(550,	1689)
	(560,	1690)
	(570,	1695)
	(580,	1699)
	(590,	1704)
	(600,	1708)
	(610,	1709)
	(620,	1716)
	(630,	1725)
	(640,	1731)
	(650,	1737)
	(660,	1742)
	(670,	1746)
	(680,	1751)
	(690,	1757)
	(700,	1766)
	(710,	1775)
	(720,	1782)
	(730,	1792)
	(740,	1797)
	(750,	1803)
	(760,	1806)
	(770,	1814)
	(780,	1816)
	(790,	1819)
	(800,	1824)
	(801,	1824)
	(802,	1827)
	(803,	1827)
	(804,	1827)
	(805,	1827)
	(806,	1828)
	(807,	1828)
	(808,	1828)
	(809,	1828)
	(810,	1828)
	(811,	1828)
	(812,	1828)
	(813,	1828)
	(814,	1828)
	(815,	1828)
	(816,	1828)
	(817,	1829)
	(818,	1829)
	(819,	1829)
	(820,	1829)
	(821,	1829)
	(822,	1829)
	(823,	1829)
	(824,	1830)
	(825,	1830)
	(826,	1830)
	(827,	1830)
	(828,	1830)
	(829,	1830)
	(830,	1831)
	(831,	1833)
	(832,	1833)
	(833,	1834)
	(834,	1834)
	(835,	1834)
	(836,	1834)
	(837,	1834)
	(838,	1834)
	(839,	1837)
	(840,	1837)
	(841,	1837)
	(842,	1838)
	(843,	1839)
	(844,	1839)
	(845,	1840)
	(846,	1840)
	(847,	1840)
	(848,	1840)
	(849,	1840)
	(850,	1840)
	(851,	1841)
	(852,	1842)
	(853,	1842)
	(854,	1842)
	(855,	1844)
	(856,	1845)
	(857,	1845)
	(858,	1846)
	(859,	1847)
	(860,	1847)
	(861,	1847)
	(862,	1847)
	(863,	1847)
	(864,	1847)
	(865,	1848)
	(866,	1848)
	(867,	1849)
	(868,	1852)
	(869,	1853)
	(870,	1853)
	(871,	1853)
	(872,	1853)
	(873,	1853)
	(874,	1853)
	(875,	1853)
	(876,	1853)
	(877,	1853)
	(878,	1853)
	(879,	1853)
	(880,	1853)
	(881,	1853)
	(882,	1853)
	(883,	1853)
	(884,	1853)
	(885,	1853)
	(886,	1853)
	(887,	1853)
	(888,	1853)
	(889,	1853)
	(890,	1853)
	(891,	1853)
	(892,	1853)
	(893,	1854)
	(894,	1854)
	(895,	1854)
	(896,	1854)
	(897,	1854)
	(898,	1854)
	(899,	1855)
	(900,	1855)
	(901,	1856)
	(902,	1856)
	(903,	1856)
	(904,	1856)
	(905,	1856)
	(906,	1856)
	(907,	1857)
	(908,	1857)
	(909,	1858)
	(910,	1858)
	(911,	1861)
	(912,	1862)
	(913,	1862)
	(914,	1862)
	(915,	1862)
	(916,	1862)
	(917,	1863)
	(918,	1863)
	(919,	1863)
	(920,	1863)
	(921,	1865)
	(922,	1865)
	(923,	1867)
	(924,	1867)
	(925,	1869)
	(926,	1869)
	(927,	1870)
	(928,	1870)
	(929,	1871)
	(930,	1872)
	(931,	1872)
	(932,	1872)
	(933,	1872)
	(934,	1872)
	(935,	1872)
	(936,	1872)
	(937,	1873)
	(938,	1874)
	(939,	1874)
	(940,	1875)
	(941,	1875)
	(942,	1877)
	(943,	1877)
	(944,	1877)
	(945,	1877)
	(946,	1877)
	(947,	1877)
	(948,	1879)
	(949,	1879)
	(950,	1879)
	(951,	1880)
	(952,	1880)
	(953,	1880)
	(954,	1880)
	(955,	1880)
	(956,	1880)
	(957,	1880)
	(958,	1881)
	(959,	1881)
	(960,	1883)
	(961,	1884)
	(962,	1884)
	(963,	1884)
	(964,	1886)
	(965,	1886)
	(966,	1887)
	(967,	1888)
	(968,	1888)
	(969,	1888)
	(970,	1888)
	(971,	1888)
	(972,	1889)
	(973,	1890)
	(974,	1890)
	(975,	1890)
	(976,	1890)
	(977,	1890)
	(978,	1890)
	(979,	1890)
	(980,	1890)
	(981,	1895)
	(982,	1895)
	(983,	1896)
	(984,	1896)
	(985,	1897)
	(986,	1897)
	(987,	1899)
	(988,	1899)
	(989,	1899)
	(990,	1899)
	(991,	1899)
	(992,	1899)
	(993,	1900)
	(994,	1900)
	(995,	1900)
	(996,	1901)
	(997,	1902)
	(998,	1903)
	(999,	1903)
	(1000,	1903)
	(1001,	1903)
	(1002,	1903)
	(1003,	1904)
	(1004,	1904)
	(1005,	1905)
	(1006,	1907)
	(1007,	1908)
	(1008,	1908)
	(1009,	1908)
	(1010,	1909)
	(1011,	1909)
	(1012,	1910)
	(1013,	1911)
	(1014,	1912)
	(1015,	1912)
	(1016,	1913)
	(1017,	1914)
	(1018,	1914)
	(1019,	1915)
	(1020,	1917)
	(1021,	1917)
	(1022,	1917)
	(1023,	1919)
	(1024,	1924)
	(1025,	1924)
	(1026,	1924)
	(1027,	1924)
	(1028,	1925)
	(1029,	1925)
	(1030,	1925)
	(1031,	1926)
	(1032,	1926)
	(1033,	1927)
	(1034,	1928)
	(1035,	1930)
	(1036,	1931)
	(1037,	1932)
	(1038,	1932)
	(1039,	1932)
	(1040,	1932)
	(1041,	1934)
	(1042,	1935)
	(1043,	1937)
	(1044,	1937)
	(1045,	1937)
	(1046,	1938)
	(1047,	1938)
	(1048,	1941)
	(1049,	1940)
	(1050,	1939)
	(1051,	1938)
	(1052,	1937)
	(1053,	1937)
	(1054,	1936)
	(1055,	1935)
	(1056,	1934)
	(1057,	1933)
	(1058,	1935)
	(1059,	1934)
	(1060,	1934)
	(1061,	1933)
	(1062,	1932)
	(1063,	1931)
	(1064,	1930)
	(1065,	1929)
	(1066,	1928)
	(1067,	1927)
	(1068,	1926)
	(1069,	1925)
	(1070,	1924)
	(1071,	1924)
	(1072,	1926)
	(1073,	1925)
	(1074,	1925)
	(1075,	1924)
	(1076,	1923)
	(1077,	1922)
	(1078,	1922)
	(1079,	1923)
	(1080,	1922)
	(1081,	1921)
	(1082,	1920)
	(1083,	1919)
	(1084,	1918)
	(1085,	1917)
	(1086,	1916)
	(1087,	1915)
	(1088,	1914)
	(1089,	1913)
	(1090,	1913)
	(1091,	1912)
	(1092,	1912)
	(1093,	1911)
	(1094,	1910)
	(1095,	1909)
	(1096,	1911)
	(1097,	1910)
	(1098,	1909)
	(1099,	1908)
	(1100,	1908)
	(1101,	1908)
	(1102,	1908)
	(1103,	1907)
	(1104,	1907)
	(1105,	1906)
	(1106,	1906)
	(1107,	1906)
	(1108,	1909)
	(1109,	1909)
	(1110,	1908)
	(1111,	1907)
	(1112,	1907)
	(1113,	1906)
	(1114,	1905)
	(1115,	1905)
	(1116,	1904)
	(1117,	1904)
	(1118,	1903)
	(1119,	1902)
	(1120,	1902)
	(1121,	1903)
	(1122,	1904)
	(1123,	1903)
	(1124,	1902)
	(1125,	1902)
	(1126,	1901)
	(1127,	1901)
	(1128,	1900)
	(1129,	1899)
	(1130,	1900)
	(1131,	1899)
	(1132,	1899)
	(1133,	1898)
	(1134,	1897)
	(1135,	1898)
	(1136,	1897)
	(1137,	1897)
	(1138,	1898)
	(1139,	1898)
	(1140,	1899)
	(1141,	1901)
	(1142,	1900)
	(1143,	1899)
	(1144,	1898)
	(1145,	1899)
	(1146,	1901)
	(1147,	1900)
	(1148,	1899)
	(1149,	1898)
	(1150,	1897)
	(1151,	1896)
	(1152,	1895)
	(1153,	1895)
	(1154,	1894)
	(1155,	1893)
	(1156,	1892)
	(1157,	1891)
	(1158,	1891)
	(1159,	1891)
	(1160,	1890)
	(1161,	1890)
	(1162,	1889)
	(1163,	1888)
	(1164,	1889)
	(1165,	1889)
	(1166,	1889)
	(1167,	1888)
	(1168,	1887)
	(1169,	1886)
	(1170,	1885)
	(1171,	1884)
	(1172,	1884)
	(1173,	1884)
	(1174,	1884)
	(1175,	1884)
	(1176,	1883)
	(1177,	1882)
	(1178,	1881)
	(1179,	1880)
	(1180,	1879)
	(1181,	1878)
	(1182,	1877)
	(1183,	1876)
	(1184,	1875)
	(1185,	1875)
	(1186,	1874)
	(1187,	1877)
	(1188,	1876)
	(1189,	1875)
	(1190,	1874)
	(1191,	1874)
	(1192,	1876)
	(1193,	1876)
	(1194,	1875)
	(1195,	1874)
	(1196,	1873)
	(1197,	1874)
	(1198,	1873)
	(1199,	1872)
	(1200,	1871)
	(1210,	1862)
	(1220,	1855)
	(1230,	1848)
	(1240,	1841)
	(1250,	1841)
	(1260,	1835)
	(1270,	1827)
	(1280,	1818)
	(1290,	1820)
	(1300,	1813)
	(1310,	1806)
	(1320,	1804)
	(1330,	1796)
	(1340,	1791)
	(1350,	1785)
	(1360,	1782)
	(1370,	1775)
	(1380,	1773)
	(1390,	1772)
	(1400,	1764)
	(1410,	1758)
	(1420,	1755)
	(1430,	1751)
	(1440,	1749)
	(1450,	1748)
	(1460,	1739)
	(1470,	1733)
	(1480,	1731)
	(1490,	1725)
	(1500,	1718)
	(1510,	1715)
	(1520,	1710)
	(1530,	1705)
	(1540,	1699)
	(1550,	1691)
	(1560,	1682)
	(1570,	1675)
	(1580,	1666)
	(1590,	1659)
	(1600,	1653)
	(1610,	1650)
	(1620,	1646)
	(1630,	1642)
	(1640,	1638)
	(1650,	1631)
	(1660,	1624)
	(1670,	1620)
	(1680,	1617)
	(1690,	1609)
	(1700,	1603)
	(1710,	1598)
	(1720,	1592)
	(1730,	1586)
	(1740,	1590)
	(1750,	1583)
	(1760,	1579)
	(1770,	1573)
	(1780,	1564)
	(1790,	1559)
	(1800,	1558)
	(1810,	1554)
	(1820,	1550)
	(1830,	1547)
	(1840,	1545)
	(1850,	1537)
	(1860,	1528)
	(1870,	1524)
	(1880,	1523)
	(1890,	1517)
	(1900,	1512)
	(1910,	1504)
	(1920,	1497)
	(1930,	1499)
	(1940,	1492)
	(1950,	1483)
	(1960,	1478)
	(1970,	1477)
	(1980,	1472)
	(1990,	1467)
	(2000,	1465)
	(2010,	1457)
	(2020,	1454)
	(2030,	1449)
	(2040,	1442)
	(2050,	1436)
	(2060,	1428)
	(2070,	1422)
	(2080,	1414)
	(2090,	1406)
	(2100,	1399)
	(2110,	1396)
	(2120,	1394)
	(2130,	1391)
	(2140,	1384)
	(2150,	1377)
	(2160,	1371)
	(2170,	1366)
	(2180,	1361)
	(2190,	1358)
	(2200,	1353)
	(2210,	1346)
	(2220,	1341)
	(2230,	1336)
	(2240,	1329)
	(2250,	1322)
	(2260,	1316)
	(2270,	1307)
	(2280,	1306)
	(2290,	1300)
	(2300,	1300)
	(2310,	1295)
	(2320,	1293)
	(2330,	1288)
	(2340,	1282)
	(2350,	1273)
	(2360,	1269)
	(2370,	1267)
	(2380,	1259)
	(2390,	1256)
	(2400,	1250)
	(2410,	1246)
	(2420,	1245)
	(2430,	1240)
	(2440,	1235)
	(2450,	1227)
	(2460,	1222)
	(2470,	1217)
	(2480,	1211)
	(2490,	1203)
	(2500,	1200)
	(2510,	1191)
	(2520,	1183)
	(2530,	1176)
	(2540,	1173)
	(2550,	1164)
	(2560,	1164)
	(2570,	1156)
	(2580,	1151)
	(2590,	1150)
	(2600,	1145)
	(2610,	1137)
	(2620,	1128)
	(2630,	1124)
	(2640,	1122)
	(2650,	1118)
	(2660,	1118)
	(2670,	1114)
	(2680,	1110)
	(2690,	1108)
	(2700,	1103)
	(2710,	1097)
	(2720,	1095)
	(2730,	1090)
	(2740,	1086)
	(2750,	1080)
	(2760,	1074)
	(2770,	1067)
	(2780,	1061)
	(2790,	1060)
	(2800,	1055)
	(2810,	1050)
	(2820,	1043)
	(2830,	1036)
	(2840,	1035)
	(2850,	1030)
	(2860,	1025)
	(2870,	1018)
	(2880,	1012)
	(2890,	1009)
	(2900,	1004)
	(2910,	998)
	(2920,	996)
	(2930,	989)
	(2940,	982)
	(2950,	975)
	(2960,	966)
	(2970,	958)
	(2980,	954)
	(2990,	950)
	(3000,	949)
	(3010,	948)
	(3020,	940)
	(3030,	934)
	(3040,	932)
	(3050,	925)
	(3060,	916)
	(3070,	912)
	(3080,	905)
	(3090,	898)
	(3100,	893)
	(3110,	888)
	(3120,	882)
	(3130,	881)
	(3140,	876)
	(3150,	873)
	(3160,	867)
	(3170,	863)
	(3180,	854)
	(3190,	847)
	(3200,	842)
	(3210,	841)
	(3220,	835)
	(3230,	828)
	(3240,	823)
	(3250,	818)
	(3260,	812)
	(3270,	804)
	(3280,	796)
	(3290,	793)
	(3300,	787)
	(3310,	781)
	(3320,	778)
	(3330,	772)
	(3340,	768)
	(3350,	761)
	(3360,	755)
	(3370,	749)
	(3380,	745)
	(3390,	743)
	(3400,	736)
	(3410,	733)
	(3420,	733)
	(3430,	730)
	(3440,	721)
	(3450,	711)
	(3460,	703)
	(3470,	694)
	(3480,	690)
	(3490,	693)
	(3500,	685)
	(3510,	677)
	(3520,	668)
	(3530,	663)
	(3540,	658)
	(3550,	650)
	(3560,	644)
	(3570,	641)
	(3580,	639)
	(3590,	633)
	(3600,	626)
	(3610,	623)
	(3620,	617)
	(3630,	611)
	(3640,	603)
	(3650,	594)
	(3660,	586)
	(3670,	580)
	(3680,	574)
	(3690,	569)
	(3700,	563)
	(3710,	554)
	(3720,	550)
	(3730,	546)
	(3740,	542)
	(3750,	533)
	(3760,	534)
	(3770,	525)
	(3780,	520)
	(3790,	513)
	(3800,	504)
	(3810,	506)
	(3820,	497)
	(3830,	490)
	(3840,	486)
	(3850,	481)
	(3860,	471)
	(3870,	464)
	(3880,	460)
	(3890,	462)
	(3900,	454)
	(3910,	451)
	(3920,	447)
	(3930,	445)
	(3940,	438)
	(3950,	434)
	(3960,	428)
	(3970,	422)
	(3980,	416)
	(3990,	408)
	(4000,	405)
	(4010,	399)
	(4020,	394)
	(4030,	397)
	(4040,	388)
	(4050,	384)
	(4060,	379)
	(4070,	373)
	(4080,	367)
	(4090,	365)
	(4100,	358)
	(4110,	355)
	(4120,	351)
	(4130,	345)
	(4140,	345)
	(4150,	347)
	(4160,	340)
	(4170,	341)
	(4180,	334)
	(4190,	327)
	(4200,	320)
	(4210,	317)
	(4220,	311)
	(4230,	314)
	(4240,	305)
	(4250,	298)
	(4260,	292)
	(4270,	286)
	(4280,	280)
	(4290,	273)
	(4300,	266)
	(4310,	263)
	(4320,	263)
	(4330,	258)
	(4340,	254)
	(4350,	247)
	(4360,	243)
	(4370,	238)
	(4380,	234)
	(4390,	226)
	(4400,	222)
	(4410,	213)
	(4420,	212)
	(4430,	209)
	(4440,	201)
	(4450,	193)
	(4460,	192)
	(4470,	187)
	(4480,	183)
	(4490,	183)
	(4500,	176)
	(4510,	171)
	(4520,	165)
	(4530,	159)
	(4540,	157)
	(4550,	151)
	(4560,	145)
	(4570,	141)
	(4580,	136)
	(4590,	128)
	(4600,	122)
	(4610,	117)
	(4620,	113)
	(4630,	106)
	(4640,	102)
	(4650,	95)
	(4660,	89)
	(4670,	85)
	(4680,	81)
	(4690,	72)
	(4700,	66)
	(4701,	66)
	(4702,	65)
	(4703,	66)
	(4704,	65)
	(4705,	64)
	(4706,	63)
	(4707,	62)
	(4708,	61)
	(4709,	61)
	(4710,	62)
	(4711,	62)
	(4712,	61)
	(4713,	61)
	(4714,	61)
	(4715,	60)
	(4716,	59)
	(4717,	58)
	(4718,	57)
	(4719,	57)
	(4720,	56)
	(4721,	55)
	(4722,	54)
	(4723,	57)
	(4724,	57)
	(4725,	57)
	(4726,	57)
	(4727,	57)
	(4728,	56)
	(4729,	55)
	(4730,	54)
	(4731,	53)
	(4732,	52)
	(4733,	53)
	(4734,	52)
	(4735,	52)
	(4736,	52)
	(4737,	51)
	(4738,	50)
	(4739,	49)
	(4740,	48)
	(4741,	47)
	(4742,	46)
	(4743,	48)
	(4744,	47)
	(4745,	46)
	(4746,	45)
	(4747,	44)
	(4748,	43)
	(4749,	42)
	(4750,	42)
	(4751,	41)
	(4752,	41)
	(4753,	40)
	(4754,	40)
	(4755,	40)
	(4756,	40)
	(4757,	40)
	(4758,	39)
	(4759,	39)
	(4760,	39)
	(4761,	38)
	(4762,	37)
	(4763,	36)
	(4764,	35)
	(4765,	35)
	(4766,	34)
	(4767,	34)
	(4768,	35)
	(4769,	34)
	(4770,	33)
	(4771,	34)
	(4772,	34)
	(4773,	33)
	(4774,	35)
	(4775,	35)
	(4776,	34)
	(4777,	35)
	(4778,	35)
	(4779,	34)
	(4780,	33)
	(4781,	34)
	(4782,	33)
	(4783,	32)
	(4784,	32)
	(4785,	32)
	(4786,	31)
	(4787,	30)
	(4788,	29)
	(4789,	30)
	(4790,	31)
	(4791,	31)
	(4792,	30)
	(4793,	30)
	(4794,	29)
	(4795,	28)
	(4796,	27)
	(4797,	26)
	(4798,	25)
	(4799,	24)
	(4800,	23)
	(4801,	22)
	(4802,	21)
	(4803,	20)
	(4804,	19)
	(4805,	18)
	(4806,	17)
	(4807,	16)
	(4808,	15)
	(4809,	14)
	(4810,	13)
	(4811,	12)
	(4812,	12)
	(4813,	11)
	(4814,	11)
	(4815,	10)
	(4816,	9)
	(4817,	9)
	(4818,	9)
	(4819,	8)
	(4820,	7)
	(4821,	7)
	(4822,	6)
	(4823,	5)
	(4824,	4)
	(4825,	3)
	(4826,	5)
	(4827,	5)
	(4828,	4)
	(4829,	3)
	(4830,	2)
	(4831,	1)
	(4832,	1)
	(4833,	1)
	(4834,	2)
	(4835,	1)
	(4836,	2)
	(4837,	3)
	(4838,	2)
	(4839,	1)
	(4840,	0)
	(4841,	0)
	(4842,	0)
	(4843,	0)
	(4844,	0)
	(4845,	0)
	(4846,	1)
	(4847,	0)
	(4848,	0)
	(4849,	0)
	(4850,	0)
	(4851,	0)
	(4852,	0)
	(4853,	0)
	(4854,	0)
	(4855,	0)
	(4856,	0)
	(4857,	2)
	(4858,	1)
	(4859,	0)
	(4860,	0)
	(4861,	0)
	(4862,	0)
	(4863,	0)
	(4864,	0)
	(4865,	0)
	(4866,	0)
	(4867,	0)
	(4868,	2)
	(4869,	1)
	(4870,	1)
	(4871,	0)
	(4872,	0)
	(4873,	0)
	(4874,	0)
	(4875,	0)
	(4876,	0)
	(4877,	0)
	(4878,	0)
	(4879,	1)
	(4880,	3)
	(4881,	2)
	(4882,	2)
	(4883,	3)
	(4884,	2)
	(4885,	2)
	(4886,	1)
	(4887,	0)
	(4888,	0)
	(4889,	0)
	(4890,	0)
	(4891,	0)
	(4892,	0)
	(4893,	0)
	(4894,	0)
	(4895,	0)
	(4896,	1)
	(4897,	0)
	(4898,	0)
	(4899,	0)
	(4900,	1)
	(4901,	0)
	(4902,	0)
	(4903,	0)
	(4904,	2)
	(4905,	1)
	(4906,	1)
	(4907,	0)
	(4908,	0)
	(4909,	0)
	(4910,	0)
	(4911,	0)
	(4912,	2)
	(4913,	1)
	(4914,	0)
	(4915,	0)
	(4916,	0)
	(4917,	0)
	(4918,	0)
	(4919,	0)
	(4920,	0)
	(4921,	2)
	(4922,	1)
	(4923,	0)
	(4924,	0)
	(4925,	0)
	(4926,	0)
	(4927,	0)
	(4928,	1)
	(4929,	0)
	(4930,	0)
	(4931,	0)
	(4932,	0)
	(4933,	0)
	(4934,	0)
	(4935,	1)
	(4936,	2)
	(4937,	2)
	(4938,	2)
	(4939,	2)
	(4940,	4)
	(4941,	4)
	(4942,	5)
	(4943,	5)
	(4944,	5)
	(4945,	6)
	(4946,	6)
	(4947,	6)
	(4948,	7)
	(4949,	8)
	(4950,	9)
	(4951,	9)
	(4952,	9)
	(4953,	9)
	(4954,	11)
	(4955,	14)
	(4956,	15)
	(4957,	16)
	(4958,	16)
	(4959,	19)
	(4960,	20)
	(4961,	21)
	(4962,	21)
	(4963,	24)
	(4964,	26)
	(4965,	26)
	(4966,	26)
	(4967,	27)
	(4968,	27)
	(4969,	27)
	(4970,	27)
	(4971,	28)
	(4972,	30)
	(4973,	30)
	(4974,	30)
	(4975,	30)
	(4976,	30)
	(4977,	30)
	(4978,	30)
	(4979,	30)
	(4980,	30)
	(4981,	30)
	(4982,	30)
	(4983,	30)
	(4984,	31)
	(4985,	31)
	(4986,	31)
	(4987,	32)
	(4988,	32)
	(4989,	32)
	(4990,	32)
	(4991,	32)
	(4992,	32)
	(4993,	32)
	(4994,	33)
	(4995,	33)
	(4996,	33)
	(4997,	33)
	(4998,	35)
	(4999,	38)
	(5000,	39)
	(5001,	39)
	(5002,	39)
	(5003,	40)
	(5004,	40)
	(5005,	40)
	(5006,	41)
	(5007,	41)
	(5008,	42)
	(5009,	42)
	(5010,	42)
	(5011,	42)
	(5012,	42)
	(5013,	42)
	(5014,	42)
	(5015,	42)
	(5016,	42)
	(5017,	43)
	(5018,	43)
	(5019,	43)
	(5020,	43)
	(5021,	43)
	(5022,	43)
	(5023,	46)
	(5024,	46)
	(5025,	47)
	(5026,	47)
	(5027,	47)
	(5028,	47)
	(5029,	47)
	(5030,	47)
	(5031,	47)
	(5032,	47)
	(5033,	50)
	(5034,	52)
	(5035,	54)
	(5036,	54)
	(5037,	58)
	(5038,	58)
	(5039,	58)
	(5040,	58)
	(5041,	58)
	(5042,	58)
	(5043,	58)
	(5044,	58)
	(5045,	58)
	(5046,	60)
	(5047,	62)
	(5048,	62)
	(5049,	62)
	(5050,	62)
	(5051,	62)
	(5052,	62)
	(5053,	62)
	(5054,	62)
	(5055,	62)
	(5056,	66)
	(5057,	69)
	(5058,	69)
	(5059,	69)
	(5060,	69)
	(5061,	70)
	(5062,	70)
	(5063,	70)
	(5064,	70)
	(5065,	70)
	(5066,	70)
	(5067,	71)
	(5068,	71)
	(5069,	73)
	(5070,	75)
	(5071,	75)
	(5072,	75)
	(5073,	76)
	(5074,	76)
	(5075,	76)
	(5076,	76)
	(5077,	76)
	(5078,	76)
	(5079,	76)
	(5080,	76)
	(5081,	76)
	(5082,	76)
	(5083,	76)
	(5084,	76)
	(5085,	78)
	(5086,	79)
	(5087,	79)
	(5088,	80)
	(5089,	80)
	(5090,	80)
	(5091,	81)
	(5092,	83)
	(5093,	83)
	(5094,	83)
	(5095,	83)
	(5096,	83)
	(5097,	83)
	(5098,	83)
	(5099,	84)
	(5100,	84)
	(5110,	86)
	(5120,	92)
	(5130,	95)
	(5140,	105)
	(5150,	106)
	(5160,	109)
	(5170,	116)
	(5180,	123)
	(5190,	127)
	(5200,	130)
	(5210,	131)
	(5220,	138)
	(5230,	143)
	(5240,	146)
	(5250,	152)
	(5260,	161)
	(5270,	171)
	(5280,	171)
	(5290,	176)
	(5300,	186)
	(5310,	195)
	(5320,	199)
	(5330,	204)
	(5340,	211)
	(5350,	219)
	(5360,	227)
	(5370,	229)
	(5380,	230)
	(5390,	233)
	(5400,	240)
	(5410,	241)
	(5420,	249)
	(5430,	251)
	(5440,	253)
	(5450,	259)
	(5460,	263)
	(5470,	272)
	(5480,	278)
	(5490,	285)
	(5500,	289)
	(5510,	289)
	(5520,	294)
	(5530,	299)
	(5540,	307)
	(5550,	307)
	(5560,	311)
	(5570,	316)
	(5580,	320)
	(5590,	332)
	(5600,	334)
	(5610,	341)
	(5620,	347)
	(5630,	352)
	(5640,	354)
	(5650,	358)
	(5660,	358)
	(5670,	366)
	(5680,	370)
	(5690,	370)
	(5700,	375)
	(5710,	383)
	(5720,	389)
	(5730,	395)
	(5740,	401)
	(5750,	406)
	(5760,	412)
	(5770,	421)
	(5780,	424)
	(5790,	426)
	(5800,	432)
	(5810,	439)
	(5820,	441)
	(5830,	442)
	(5840,	444)
	(5850,	456)
	(5860,	460)
	(5870,	461)
	(5880,	471)
	(5890,	474)
	(5900,	477)
	(5910,	479)
	(5920,	481)
	(5930,	488)
	(5940,	490)
	(5950,	493)
	(5960,	500)
	(5970,	506)
	(5980,	511)
	(5990,	514)
	(6000,	518)
	(6010,	524)
	(6020,	526)
	(6030,	529)
	(6040,	534)
	(6050,	540)
	(6060,	547)
	(6070,	550)
	(6080,	551)
	(6090,	557)
	(6100,	560)
	(6110,	567)
	(6120,	571)
	(6130,	573)
	(6140,	577)
	(6150,	581)
	(6160,	586)
	(6170,	600)
	(6180,	609)
	(6190,	620)
	(6200,	624)
	(6210,	632)
	(6220,	637)
	(6230,	639)
	(6240,	643)
	(6250,	648)
	(6260,	656)
	(6270,	661)
	(6280,	664)
	(6290,	670)
	(6300,	673)
	(6310,	676)
	(6320,	685)
	(6330,	690)
	(6340,	693)
	(6350,	697)
	(6360,	704)
	(6370,	706)
	(6380,	711)
	(6390,	714)
	(6400,	717)
	(6410,	718)
	(6420,	723)
	(6430,	732)
	(6440,	733)
	(6450,	740)
	(6460,	742)
	(6470,	746)
	(6480,	750)
	(6490,	753)
	(6500,	758)
	(6510,	767)
	(6520,	775)
	(6530,	781)
	(6540,	783)
	(6550,	785)
	(6560,	787)
	(6570,	792)
	(6580,	801)
	(6590,	807)
	(6600,	810)
	(6610,	814)
	(6620,	819)
	(6630,	827)
	(6640,	831)
	(6650,	835)
	(6660,	838)
	(6670,	845)
	(6680,	849)
	(6690,	853)
	(6700,	858)
	(6710,	861)
	(6720,	864)
	(6730,	867)
	(6740,	869)
	(6750,	877)
	(6760,	886)
	(6770,	894)
	(6780,	894)
	(6790,	898)
	(6800,	899)
	(6810,	902)
	(6820,	909)
	(6830,	911)
	(6840,	918)
	(6850,	925)
	(6860,	929)
	(6870,	933)
	(6880,	939)
	(6890,	946)
	(6900,	953)
	(6910,	958)
	(6920,	969)
	(6930,	973)
	(6940,	976)
	(6950,	977)
	(6960,	986)
	(6970,	992)
	(6980,	999)
	(6990,	1002)
	(7000,	1008)
	(7010,	1011)
	(7020,	1016)
	(7030,	1020)
	(7040,	1025)
	(7050,	1030)
	(7060,	1035)
	(7070,	1037)
	(7080,	1041)
	(7090,	1046)
	(7100,	1061)
	(7110,	1063)
	(7120,	1074)
	(7130,	1080)
	(7140,	1085)
	(7150,	1088)
	(7160,	1095)
	(7170,	1107)
	(7180,	1109)
	(7190,	1115)
	(7200,	1116)
	(7210,	1124)
	(7220,	1126)
	(7230,	1139)
	(7240,	1152)
	(7250,	1159)
	(7260,	1162)
	(7270,	1169)
	(7280,	1171)
	(7290,	1177)
	(7300,	1181)
	(7310,	1184)
	(7320,	1186)
	(7330,	1189)
	(7340,	1195)
	(7350,	1196)
	(7360,	1204)
	(7370,	1209)
	(7380,	1213)
	(7390,	1221)
	(7400,	1221)
	(7410,	1224)
	(7420,	1228)
	(7430,	1231)
	(7440,	1247)
	(7450,	1250)
	(7460,	1251)
	(7470,	1252)
	(7480,	1258)
	(7490,	1269)
	(7500,	1275)
	(7510,	1283)
	(7520,	1286)
	(7530,	1289)
	(7540,	1294)
	(7550,	1303)
	(7560,	1304)
	(7570,	1307)
	(7580,	1311)
	(7590,	1320)
	(7600,	1328)
	(7610,	1333)
	(7620,	1343)
	(7630,	1346)
	(7640,	1348)
	(7650,	1355)
	(7660,	1359)
	(7670,	1370)
	(7680,	1377)
	(7690,	1380)
	(7700,	1386)
	(7710,	1394)
	(7720,	1400)
	(7730,	1404)
	(7740,	1410)
	(7750,	1417)
	(7760,	1422)
	(7770,	1429)
	(7780,	1432)
	(7790,	1435)
	(7800,	1440)
	(7810,	1448)
	(7820,	1452)
	(7830,	1458)
	(7840,	1459)
	(7850,	1465)
	(7860,	1471)
	(7870,	1475)
	(7880,	1480)
	(7890,	1482)
	(7900,	1483)
	(7910,	1491)
	(7920,	1501)
	(7930,	1509)
	(7940,	1516)
	(7950,	1527)
	(7960,	1529)
	(7970,	1534)
	(7980,	1551)
	(7990,	1561)
	(8000,	1573)
	(8010,	1577)
	(8020,	1579)
	(8030,	1584)
	(8040,	1589)
	(8050,	1594)
	(8060,	1597)
	(8070,	1601)
	(8080,	1606)
	(8090,	1609)
	(8100,	1614)
	(8110,	1619)
	(8120,	1623)
	(8130,	1630)
	(8140,	1642)
	(8150,	1644)
	(8160,	1647)
	(8170,	1654)
	(8180,	1661)
	(8190,	1666)
	(8200,	1672)
	(8210,	1675)
	(8220,	1677)
	(8230,	1690)
	(8240,	1692)
	(8250,	1699)
	(8260,	1704)
	(8270,	1710)
	(8280,	1718)
	(8290,	1723)
	(8300,	1724)
	(8310,	1727)
	(8320,	1729)
	(8330,	1734)
	(8340,	1741)
	(8350,	1747)
	(8360,	1757)
	(8370,	1758)
	(8380,	1761)
	(8390,	1765)
	(8400,	1769)
	(8410,	1775)
	(8420,	1783)
	(8430,	1784)
	(8440,	1790)
	(8450,	1794)
	(8460,	1795)
	(8470,	1802)
	(8480,	1804)
	(8490,	1806)
	(8500,	1814)
	(8510,	1819)
	(8520,	1822)
	(8530,	1827)
	(8540,	1831)
	(8550,	1833)
	(8560,	1836)
	(8570,	1837)
	(8580,	1842)
	(8590,	1855)
	(8600,	1859)
	(8601,	1859)
	(8602,	1859)
	(8603,	1859)
	(8604,	1859)
	(8605,	1859)
	(8606,	1859)
	(8607,	1859)
	(8608,	1860)
	(8609,	1860)
	(8610,	1861)
	(8611,	1861)
	(8612,	1861)
	(8613,	1861)
	(8614,	1861)
	(8615,	1861)
	(8616,	1861)
	(8617,	1861)
	(8618,	1861)
	(8619,	1861)
	(8620,	1862)
	(8621,	1862)
	(8622,	1862)
	(8623,	1863)
	(8624,	1863)
	(8625,	1863)
	(8626,	1864)
	(8627,	1865)
	(8628,	1865)
	(8629,	1870)
	(8630,	1870)
	(8631,	1871)
	(8632,	1873)
	(8633,	1874)
	(8634,	1874)
	(8635,	1874)
	(8636,	1877)
	(8637,	1877)
	(8638,	1877)
	(8639,	1877)
	(8640,	1877)
	(8641,	1878)
	(8642,	1878)
	(8643,	1878)
	(8644,	1878)
	(8645,	1878)
	(8646,	1878)
	(8647,	1878)
	(8648,	1878)
	(8649,	1878)
	(8650,	1878)
	(8651,	1878)
	(8652,	1878)
	(8653,	1878)
	(8654,	1879)
	(8655,	1880)
	(8656,	1881)
	(8657,	1881)
	(8658,	1881)
	(8659,	1881)
	(8660,	1881)
	(8661,	1881)
	(8662,	1881)
	(8663,	1881)
	(8664,	1881)
	(8665,	1882)
	(8666,	1882)
	(8667,	1882)
	(8668,	1882)
	(8669,	1882)
	(8670,	1882)
	(8671,	1882)
	(8672,	1882)
	(8673,	1882)
	(8674,	1882)
	(8675,	1882)
	(8676,	1882)
	(8677,	1882)
	(8678,	1883)
	(8679,	1883)
	(8680,	1883)
	(8681,	1883)
	(8682,	1884)
	(8683,	1885)
	(8684,	1885)
	(8685,	1886)
	(8686,	1886)
	(8687,	1886)
	(8688,	1886)
	(8689,	1888)
	(8690,	1890)
	(8691,	1890)
	(8692,	1890)
	(8693,	1890)
	(8694,	1891)
	(8695,	1891)
	(8696,	1891)
	(8697,	1892)
	(8698,	1897)
	(8699,	1899)
	(8700,	1899)
	(8701,	1900)
	(8702,	1901)
	(8703,	1901)
	(8704,	1901)
	(8705,	1901)
	(8706,	1901)
	(8707,	1901)
	(8708,	1902)
	(8709,	1904)
	(8710,	1905)
	(8711,	1907)
	(8712,	1909)
	(8713,	1909)
	(8714,	1909)
	(8715,	1910)
	(8716,	1910)
	(8717,	1911)
	(8718,	1912)
	(8719,	1912)
	(8720,	1915)
	(8721,	1915)
	(8722,	1916)
	(8723,	1916)
	(8724,	1916)
	(8725,	1916)
	(8726,	1916)
	(8727,	1916)
	(8728,	1916)
	(8729,	1918)
	(8730,	1918)
	(8731,	1920)
	(8732,	1920)
	(8733,	1920)
	(8734,	1920)
	(8735,	1920)
	(8736,	1920)
	(8737,	1920)
	(8738,	1920)
	(8739,	1920)
	(8740,	1920)
	(8741,	1921)
	(8742,	1921)
	(8743,	1921)
	(8744,	1921)
	(8745,	1922)
	(8746,	1922)
	(8747,	1922)
	(8748,	1922)
	(8749,	1922)
	(8750,	1922)
	(8751,	1925)
	(8752,	1925)
	(8753,	1925)
	(8754,	1928)
	(8755,	1928)
	(8756,	1931)
	(8757,	1931)
	(8758,	1933)
	(8759,	1934)
	(8760,	1934)
	(8761,	1934)
	(8762,	1934)
	(8763,	1934)
	(8764,	1936)
	(8765,	1938)
	(8766,	1938)
	(8767,	1938)
	(8768,	1938)
	(8769,	1938)
	(8770,	1939)
	(8771,	1940)
	(8772,	1940)
	(8773,	1941)
	(8774,	1941)
	(8775,	1942)
	(8776,	1942)
	(8777,	1942)
	(8778,	1942)
	(8779,	1942)
	(8780,	1942)
	(8781,	1942)
	(8782,	1942)
	(8783,	1942)
	(8784,	1942)
	(8785,	1942)
	(8786,	1942)
	(8787,	1942)
	(8788,	1942)
	(8789,	1942)
	(8790,	1942)
	(8791,	1942)
	(8792,	1943)
	(8793,	1947)
	(8794,	1947)
	(8795,	1947)
	(8796,	1947)
	(8797,	1949)
	(8798,	1950)
	(8799,	1950)
	(8800,	1950)
	(8801,	1950)
	(8802,	1950)
	(8803,	1950)
	(8804,	1950)
	(8805,	1950)
	(8806,	1950)
	(8807,	1950)
	(8808,	1950)
	(8809,	1950)
	(8810,	1950)
	(8811,	1950)
	(8812,	1950)
	(8813,	1950)
	(8814,	1950)
	(8815,	1950)
	(8816,	1951)
	(8817,	1951)
	(8818,	1956)
	(8819,	1958)
	(8820,	1958)
	(8821,	1958)
	(8822,	1958)
	(8823,	1958)
	(8824,	1958)
	(8825,	1958)
	(8826,	1961)
	(8827,	1962)
	(8828,	1962)
	(8829,	1964)
	(8830,	1965)
	(8831,	1965)
	(8832,	1965)
	(8833,	1965)
	(8834,	1965)
	(8835,	1965)
	(8836,	1965)
	(8837,	1966)
	(8838,	1966)
	(8839,	1966)
	(8840,	1966)
	(8841,	1966)
	(8842,	1966)
	(8843,	1966)
	(8844,	1968)
	(8845,	1969)
	(8846,	1969)
	(8847,	1969)
	(8848,	1969)
	(8849,	1972)
	(8850,	1972)
	(8851,	1978)
	(8852,	1978)
	(8853,	1979)
	(8854,	1979)
	(8855,	1981)
	(8856,	1981)
	(8857,	1981)
	(8858,	1982)
	(8859,	1983)
	(8860,	1983)
	(8861,	1983)
	(8862,	1983)
	(8863,	1983)
	(8864,	1983)
	(8865,	1984)
	(8866,	1984)
	(8867,	1984)
	(8868,	1985)
	(8869,	1988)
	(8870,	1989)
	(8871,	1991)
	(8872,	1991)
	(8873,	1991)
	(8874,	1991)
	(8875,	1990)
	(8876,	1989)
	(8877,	1988)
	(8878,	1988)
	(8879,	1987)
	(8880,	1986)
	(8881,	1987)
	(8882,	1986)
	(8883,	1986)
	(8884,	1985)
	(8885,	1984)
	(8886,	1983)
	(8887,	1982)
	(8888,	1981)
	(8889,	1982)
	(8890,	1982)
	(8891,	1983)
	(8892,	1982)
	(8893,	1982)
	(8894,	1981)
	(8895,	1980)
	(8896,	1981)
	(8897,	1980)
	(8898,	1979)
	(8899,	1979)
	(8900,	1978)
	(8901,	1978)
	(8902,	1979)
	(8903,	1978)
	(8904,	1978)
	(8905,	1978)
	(8906,	1978)
	(8907,	1978)
	(8908,	1977)
	(8909,	1976)
	(8910,	1975)
	(8911,	1974)
	(8912,	1973)
	(8913,	1972)
	(8914,	1971)
	(8915,	1971)
	(8916,	1972)
	(8917,	1972)
	(8918,	1971)
	(8919,	1970)
	(8920,	1971)
	(8921,	1970)
	(8922,	1969)
	(8923,	1970)
	(8924,	1969)
	(8925,	1969)
	(8926,	1968)
	(8927,	1967)
	(8928,	1968)
	(8929,	1967)
	(8930,	1966)
	(8931,	1965)
	(8932,	1968)
	(8933,	1967)
	(8934,	1966)
	(8935,	1965)
	(8936,	1965)
	(8937,	1964)
	(8938,	1964)
	(8939,	1963)
	(8940,	1963)
	(8941,	1962)
	(8942,	1961)
	(8943,	1960)
	(8944,	1959)
	(8945,	1959)
	(8946,	1958)
	(8947,	1957)
	(8948,	1957)
	(8949,	1956)
	(8950,	1955)
	(8951,	1954)
	(8952,	1954)
	(8953,	1953)
	(8954,	1952)
	(8955,	1951)
	(8956,	1950)
	(8957,	1951)
	(8958,	1951)
	(8959,	1950)
	(8960,	1950)
	(8961,	1950)
	(8962,	1949)
	(8963,	1948)
	(8964,	1947)
	(8965,	1946)
	(8966,	1948)
	(8967,	1947)
	(8968,	1946)
	(8969,	1945)
	(8970,	1947)
	(8971,	1946)
	(8972,	1946)
	(8973,	1945)
	(8974,	1944)
	(8975,	1944)
	(8976,	1943)
	(8977,	1942)
	(8978,	1941)
	(8979,	1940)
	(8980,	1939)
	(8981,	1938)
	(8982,	1937)
	(8983,	1938)
	(8984,	1938)
	(8985,	1938)
	(8986,	1938)
	(8987,	1937)
	(8988,	1937)
	(8989,	1936)
	(8990,	1935)
	(8991,	1936)
	(8992,	1935)
	(8993,	1935)
	(8994,	1935)
	(8995,	1934)
	(8996,	1933)
	(8997,	1933)
	(8998,	1932)
	(8999,	1931)
	(9000,	1930)
	(9010,	1928)
	(9020,	1919)
	(9030,	1914)
	(9040,	1912)
	(9050,	1903)
	(9060,	1901)
	(9070,	1895)
	(9080,	1895)
	(9090,	1887)
	(9100,	1880)
	(9110,	1872)
	(9120,	1864)
	(9130,	1857)
	(9140,	1853)
	(9150,	1851)
	(9160,	1845)
	(9170,	1840)
	(9180,	1834)
	(9190,	1830)
	(9200,	1825)
	(9210,	1819)
	(9220,	1816)
	(9230,	1808)
	(9240,	1807)
	(9250,	1798)
	(9260,	1794)
	(9270,	1792)
	(9280,	1784)
	(9290,	1779)
	(9300,	1774)
	(9310,	1771)
	(9320,	1767)
	(9330,	1765)
	(9340,	1759)
	(9350,	1753)
	(9360,	1752)
	(9370,	1748)
	(9380,	1744)
	(9390,	1738)
	(9400,	1732)
	(9410,	1724)
	(9420,	1717)
	(9430,	1711)
	(9440,	1702)
	(9450,	1696)
	(9460,	1691)
	(9470,	1687)
	(9480,	1683)
	(9490,	1677)
	(9500,	1671)
	(9510,	1665)
	(9520,	1665)
	(9530,	1665)
	(9540,	1661)
	(9550,	1656)
	(9560,	1650)
	(9570,	1653)
	(9580,	1649)
	(9590,	1646)
	(9600,	1643)
	(9610,	1639)
	(9620,	1634)
	(9630,	1634)
	(9640,	1631)
	(9650,	1624)
	(9660,	1615)
	(9670,	1609)
	(9680,	1606)
	(9690,	1606)
	(9700,	1607)
	(9710,	1599)
	(9720,	1591)
	(9730,	1586)
	(9740,	1581)
	(9750,	1571)
	(9760,	1568)
	(9770,	1562)
	(9780,	1557)
	(9790,	1551)
	(9800,	1546)
	(9810,	1544)
	(9820,	1537)
	(9830,	1530)
	(9840,	1525)
	(9850,	1522)
	(9860,	1513)
	(9870,	1507)
	(9880,	1500)
	(9890,	1497)
	(9900,	1495)
	(9910,	1491)
	(9920,	1484)
	(9930,	1477)
	(9940,	1471)
	(9950,	1463)
	(9960,	1456)
	(9970,	1449)
	(9980,	1444)
	(9990,	1438)
	(10000,	1430)
};
\addplot[color=gray,densely dashdotted] plot coordinates {
	(0,	1539)
	(10,	1543)
	(20,	1548)
	(30,	1553)
	(40,	1554)
	(50,	1554)
	(60,	1557)
	(70,	1562)
	(80,	1569)
	(90,	1579)
	(100,	1585)
	(110,	1591)
	(120,	1595)
	(130,	1600)
	(140,	1610)
	(150,	1612)
	(160,	1614)
	(170,	1624)
	(180,	1635)
	(190,	1636)
	(200,	1638)
	(210,	1641)
	(220,	1646)
	(230,	1653)
	(240,	1655)
	(250,	1661)
	(260,	1663)
	(270,	1667)
	(280,	1671)
	(290,	1679)
	(300,	1683)
	(310,	1692)
	(320,	1698)
	(330,	1702)
	(340,	1714)
	(350,	1719)
	(360,	1720)
	(370,	1724)
	(380,	1727)
	(390,	1731)
	(400,	1738)
	(410,	1744)
	(420,	1749)
	(430,	1753)
	(440,	1759)
	(450,	1762)
	(460,	1768)
	(470,	1769)
	(480,	1771)
	(490,	1778)
	(500,	1780)
	(510,	1783)
	(520,	1785)
	(530,	1789)
	(540,	1793)
	(550,	1799)
	(560,	1802)
	(570,	1811)
	(580,	1821)
	(590,	1822)
	(600,	1823)
	(610,	1825)
	(620,	1827)
	(630,	1835)
	(640,	1836)
	(650,	1838)
	(660,	1844)
	(670,	1851)
	(680,	1856)
	(690,	1856)
	(700,	1861)
	(710,	1866)
	(720,	1869)
	(730,	1877)
	(740,	1883)
	(750,	1888)
	(760,	1894)
	(770,	1898)
	(780,	1898)
	(790,	1910)
	(800,	1912)
	(801,	1912)
	(802,	1912)
	(803,	1912)
	(804,	1913)
	(805,	1913)
	(806,	1915)
	(807,	1915)
	(808,	1915)
	(809,	1915)
	(810,	1915)
	(811,	1916)
	(812,	1916)
	(813,	1916)
	(814,	1916)
	(815,	1916)
	(816,	1916)
	(817,	1917)
	(818,	1917)
	(819,	1920)
	(820,	1920)
	(821,	1920)
	(822,	1922)
	(823,	1922)
	(824,	1922)
	(825,	1922)
	(826,	1924)
	(827,	1925)
	(828,	1928)
	(829,	1928)
	(830,	1928)
	(831,	1928)
	(832,	1929)
	(833,	1930)
	(834,	1931)
	(835,	1931)
	(836,	1931)
	(837,	1932)
	(838,	1932)
	(839,	1932)
	(840,	1933)
	(841,	1933)
	(842,	1933)
	(843,	1934)
	(844,	1935)
	(845,	1936)
	(846,	1936)
	(847,	1936)
	(848,	1937)
	(849,	1937)
	(850,	1937)
	(851,	1937)
	(852,	1938)
	(853,	1938)
	(854,	1938)
	(855,	1939)
	(856,	1939)
	(857,	1939)
	(858,	1940)
	(859,	1941)
	(860,	1941)
	(861,	1942)
	(862,	1942)
	(863,	1943)
	(864,	1943)
	(865,	1943)
	(866,	1943)
	(867,	1943)
	(868,	1943)
	(869,	1944)
	(870,	1944)
	(871,	1945)
	(872,	1945)
	(873,	1946)
	(874,	1946)
	(875,	1946)
	(876,	1946)
	(877,	1946)
	(878,	1946)
	(879,	1946)
	(880,	1946)
	(881,	1947)
	(882,	1951)
	(883,	1951)
	(884,	1951)
	(885,	1952)
	(886,	1953)
	(887,	1954)
	(888,	1955)
	(889,	1956)
	(890,	1956)
	(891,	1957)
	(892,	1958)
	(893,	1959)
	(894,	1959)
	(895,	1959)
	(896,	1959)
	(897,	1959)
	(898,	1959)
	(899,	1959)
	(900,	1959)
	(901,	1959)
	(902,	1961)
	(903,	1964)
	(904,	1964)
	(905,	1965)
	(906,	1965)
	(907,	1965)
	(908,	1966)
	(909,	1966)
	(910,	1966)
	(911,	1966)
	(912,	1966)
	(913,	1966)
	(914,	1967)
	(915,	1968)
	(916,	1968)
	(917,	1968)
	(918,	1968)
	(919,	1968)
	(920,	1970)
	(921,	1972)
	(922,	1973)
	(923,	1973)
	(924,	1973)
	(925,	1973)
	(926,	1973)
	(927,	1974)
	(928,	1974)
	(929,	1974)
	(930,	1974)
	(931,	1975)
	(932,	1975)
	(933,	1975)
	(934,	1975)
	(935,	1976)
	(936,	1976)
	(937,	1976)
	(938,	1977)
	(939,	1979)
	(940,	1982)
	(941,	1982)
	(942,	1982)
	(943,	1983)
	(944,	1983)
	(945,	1983)
	(946,	1985)
	(947,	1985)
	(948,	1985)
	(949,	1985)
	(950,	1986)
	(951,	1986)
	(952,	1986)
	(953,	1987)
	(954,	1987)
	(955,	1987)
	(956,	1988)
	(957,	1988)
	(958,	1988)
	(959,	1988)
	(960,	1988)
	(961,	1988)
	(962,	1989)
	(963,	1989)
	(964,	1989)
	(965,	1989)
	(966,	1990)
	(967,	1990)
	(968,	1992)
	(969,	1993)
	(970,	1994)
	(971,	1994)
	(972,	1996)
	(973,	1996)
	(974,	1996)
	(975,	1996)
	(976,	1996)
	(977,	1996)
	(978,	1997)
	(979,	1999)
	(980,	1999)
	(981,	1999)
	(982,	1999)
	(983,	1999)
	(984,	2000)
	(985,	2000)
	(986,	2000)
	(987,	2000)
	(988,	2001)
	(989,	2001)
	(990,	2001)
	(991,	2002)
	(992,	2002)
	(993,	2002)
	(994,	2004)
	(995,	2004)
	(996,	2005)
	(997,	2005)
	(998,	2005)
	(999,	2006)
	(1000,	2006)
	(1001,	2006)
	(1002,	2006)
	(1003,	2006)
	(1004,	2006)
	(1005,	2006)
	(1006,	2006)
	(1007,	2006)
	(1008,	2006)
	(1009,	2007)
	(1010,	2007)
	(1011,	2007)
	(1012,	2007)
	(1013,	2008)
	(1014,	2009)
	(1015,	2010)
	(1016,	2010)
	(1017,	2012)
	(1018,	2012)
	(1019,	2012)
	(1020,	2015)
	(1021,	2015)
	(1022,	2015)
	(1023,	2017)
	(1024,	2019)
	(1025,	2020)
	(1026,	2020)
	(1027,	2020)
	(1028,	2020)
	(1029,	2020)
	(1030,	2020)
	(1031,	2020)
	(1032,	2020)
	(1033,	2021)
	(1034,	2021)
	(1035,	2021)
	(1036,	2021)
	(1037,	2022)
	(1038,	2022)
	(1039,	2023)
	(1040,	2023)
	(1041,	2023)
	(1042,	2023)
	(1043,	2023)
	(1044,	2023)
	(1045,	2024)
	(1046,	2024)
	(1047,	2026)
	(1048,	2026)
	(1049,	2025)
	(1050,	2026)
	(1051,	2025)
	(1052,	2024)
	(1053,	2023)
	(1054,	2022)
	(1055,	2021)
	(1056,	2022)
	(1057,	2021)
	(1058,	2020)
	(1059,	2019)
	(1060,	2018)
	(1061,	2020)
	(1062,	2019)
	(1063,	2020)
	(1064,	2019)
	(1065,	2018)
	(1066,	2021)
	(1067,	2020)
	(1068,	2019)
	(1069,	2018)
	(1070,	2017)
	(1071,	2016)
	(1072,	2016)
	(1073,	2015)
	(1074,	2014)
	(1075,	2015)
	(1076,	2014)
	(1077,	2016)
	(1078,	2015)
	(1079,	2014)
	(1080,	2013)
	(1081,	2012)
	(1082,	2011)
	(1083,	2010)
	(1084,	2009)
	(1085,	2008)
	(1086,	2008)
	(1087,	2007)
	(1088,	2006)
	(1089,	2005)
	(1090,	2004)
	(1091,	2003)
	(1092,	2002)
	(1093,	2001)
	(1094,	2000)
	(1095,	1999)
	(1096,	1998)
	(1097,	1997)
	(1098,	1997)
	(1099,	1997)
	(1100,	1996)
	(1101,	1995)
	(1102,	1994)
	(1103,	1993)
	(1104,	1992)
	(1105,	1991)
	(1106,	1990)
	(1107,	1989)
	(1108,	1988)
	(1109,	1987)
	(1110,	1987)
	(1111,	1986)
	(1112,	1987)
	(1113,	1987)
	(1114,	1987)
	(1115,	1986)
	(1116,	1985)
	(1117,	1986)
	(1118,	1986)
	(1119,	1985)
	(1120,	1984)
	(1121,	1983)
	(1122,	1983)
	(1123,	1984)
	(1124,	1983)
	(1125,	1983)
	(1126,	1982)
	(1127,	1981)
	(1128,	1980)
	(1129,	1979)
	(1130,	1980)
	(1131,	1979)
	(1132,	1978)
	(1133,	1977)
	(1134,	1976)
	(1135,	1975)
	(1136,	1974)
	(1137,	1974)
	(1138,	1975)
	(1139,	1975)
	(1140,	1974)
	(1141,	1973)
	(1142,	1972)
	(1143,	1971)
	(1144,	1970)
	(1145,	1969)
	(1146,	1968)
	(1147,	1967)
	(1148,	1966)
	(1149,	1965)
	(1150,	1965)
	(1151,	1964)
	(1152,	1965)
	(1153,	1965)
	(1154,	1964)
	(1155,	1963)
	(1156,	1963)
	(1157,	1962)
	(1158,	1962)
	(1159,	1961)
	(1160,	1961)
	(1161,	1960)
	(1162,	1960)
	(1163,	1959)
	(1164,	1958)
	(1165,	1957)
	(1166,	1957)
	(1167,	1958)
	(1168,	1958)
	(1169,	1958)
	(1170,	1959)
	(1171,	1958)
	(1172,	1957)
	(1173,	1956)
	(1174,	1956)
	(1175,	1955)
	(1176,	1954)
	(1177,	1953)
	(1178,	1952)
	(1179,	1951)
	(1180,	1950)
	(1181,	1949)
	(1182,	1949)
	(1183,	1953)
	(1184,	1952)
	(1185,	1954)
	(1186,	1954)
	(1187,	1953)
	(1188,	1956)
	(1189,	1958)
	(1190,	1957)
	(1191,	1956)
	(1192,	1955)
	(1193,	1955)
	(1194,	1954)
	(1195,	1953)
	(1196,	1952)
	(1197,	1951)
	(1198,	1950)
	(1199,	1950)
	(1200,	1951)
	(1210,	1947)
	(1220,	1939)
	(1230,	1930)
	(1240,	1925)
	(1250,	1923)
	(1260,	1921)
	(1270,	1919)
	(1280,	1913)
	(1290,	1907)
	(1300,	1901)
	(1310,	1904)
	(1320,	1898)
	(1330,	1896)
	(1340,	1890)
	(1350,	1886)
	(1360,	1878)
	(1370,	1875)
	(1380,	1872)
	(1390,	1863)
	(1400,	1860)
	(1410,	1856)
	(1420,	1853)
	(1430,	1850)
	(1440,	1843)
	(1450,	1840)
	(1460,	1832)
	(1470,	1824)
	(1480,	1817)
	(1490,	1812)
	(1500,	1805)
	(1510,	1803)
	(1520,	1798)
	(1530,	1792)
	(1540,	1790)
	(1550,	1782)
	(1560,	1780)
	(1570,	1773)
	(1580,	1767)
	(1590,	1766)
	(1600,	1761)
	(1610,	1753)
	(1620,	1749)
	(1630,	1742)
	(1640,	1735)
	(1650,	1733)
	(1660,	1727)
	(1670,	1722)
	(1680,	1719)
	(1690,	1716)
	(1700,	1711)
	(1710,	1705)
	(1720,	1697)
	(1730,	1694)
	(1740,	1685)
	(1750,	1678)
	(1760,	1671)
	(1770,	1663)
	(1780,	1655)
	(1790,	1650)
	(1800,	1644)
	(1810,	1641)
	(1820,	1635)
	(1830,	1630)
	(1840,	1627)
	(1850,	1622)
	(1860,	1615)
	(1870,	1612)
	(1880,	1605)
	(1890,	1598)
	(1900,	1591)
	(1910,	1587)
	(1920,	1581)
	(1930,	1574)
	(1940,	1569)
	(1950,	1567)
	(1960,	1564)
	(1970,	1562)
	(1980,	1552)
	(1990,	1545)
	(2000,	1536)
	(2010,	1527)
	(2020,	1524)
	(2030,	1520)
	(2040,	1512)
	(2050,	1504)
	(2060,	1496)
	(2070,	1497)
	(2080,	1489)
	(2090,	1484)
	(2100,	1477)
	(2110,	1472)
	(2120,	1465)
	(2130,	1457)
	(2140,	1449)
	(2150,	1445)
	(2160,	1440)
	(2170,	1436)
	(2180,	1436)
	(2190,	1434)
	(2200,	1432)
	(2210,	1424)
	(2220,	1418)
	(2230,	1409)
	(2240,	1407)
	(2250,	1405)
	(2260,	1397)
	(2270,	1389)
	(2280,	1383)
	(2290,	1375)
	(2300,	1374)
	(2310,	1366)
	(2320,	1363)
	(2330,	1358)
	(2340,	1352)
	(2350,	1346)
	(2360,	1342)
	(2370,	1337)
	(2380,	1335)
	(2390,	1331)
	(2400,	1326)
	(2410,	1324)
	(2420,	1318)
	(2430,	1321)
	(2440,	1313)
	(2450,	1303)
	(2460,	1298)
	(2470,	1293)
	(2480,	1287)
	(2490,	1281)
	(2500,	1275)
	(2510,	1269)
	(2520,	1270)
	(2530,	1263)
	(2540,	1255)
	(2550,	1249)
	(2560,	1240)
	(2570,	1232)
	(2580,	1225)
	(2590,	1218)
	(2600,	1217)
	(2610,	1212)
	(2620,	1205)
	(2630,	1201)
	(2640,	1193)
	(2650,	1188)
	(2660,	1178)
	(2670,	1174)
	(2680,	1175)
	(2690,	1169)
	(2700,	1161)
	(2710,	1165)
	(2720,	1158)
	(2730,	1155)
	(2740,	1150)
	(2750,	1144)
	(2760,	1137)
	(2770,	1134)
	(2780,	1131)
	(2790,	1123)
	(2800,	1118)
	(2810,	1108)
	(2820,	1104)
	(2830,	1096)
	(2840,	1092)
	(2850,	1084)
	(2860,	1079)
	(2870,	1074)
	(2880,	1073)
	(2890,	1070)
	(2900,	1060)
	(2910,	1058)
	(2920,	1055)
	(2930,	1049)
	(2940,	1045)
	(2950,	1038)
	(2960,	1034)
	(2970,	1031)
	(2980,	1024)
	(2990,	1018)
	(3000,	1012)
	(3010,	1004)
	(3020,	1002)
	(3030,	996)
	(3040,	993)
	(3050,	987)
	(3060,	984)
	(3070,	987)
	(3080,	987)
	(3090,	981)
	(3100,	971)
	(3110,	963)
	(3120,	955)
	(3130,	952)
	(3140,	947)
	(3150,	941)
	(3160,	931)
	(3170,	924)
	(3180,	920)
	(3190,	913)
	(3200,	906)
	(3210,	899)
	(3220,	890)
	(3230,	883)
	(3240,	874)
	(3250,	872)
	(3260,	866)
	(3270,	860)
	(3280,	853)
	(3290,	855)
	(3300,	847)
	(3310,	844)
	(3320,	838)
	(3330,	835)
	(3340,	829)
	(3350,	823)
	(3360,	815)
	(3370,	810)
	(3380,	804)
	(3390,	800)
	(3400,	794)
	(3410,	787)
	(3420,	782)
	(3430,	775)
	(3440,	770)
	(3450,	770)
	(3460,	764)
	(3470,	761)
	(3480,	754)
	(3490,	749)
	(3500,	745)
	(3510,	742)
	(3520,	736)
	(3530,	733)
	(3540,	726)
	(3550,	724)
	(3560,	716)
	(3570,	710)
	(3580,	709)
	(3590,	711)
	(3600,	708)
	(3610,	704)
	(3620,	703)
	(3630,	694)
	(3640,	689)
	(3650,	686)
	(3660,	679)
	(3670,	670)
	(3680,	663)
	(3690,	657)
	(3700,	649)
	(3710,	644)
	(3720,	639)
	(3730,	637)
	(3740,	629)
	(3750,	623)
	(3760,	617)
	(3770,	608)
	(3780,	601)
	(3790,	597)
	(3800,	593)
	(3810,	586)
	(3820,	579)
	(3830,	572)
	(3840,	567)
	(3850,	561)
	(3860,	556)
	(3870,	551)
	(3880,	544)
	(3890,	537)
	(3900,	533)
	(3910,	526)
	(3920,	518)
	(3930,	509)
	(3940,	504)
	(3950,	500)
	(3960,	497)
	(3970,	489)
	(3980,	480)
	(3990,	472)
	(4000,	469)
	(4010,	465)
	(4020,	458)
	(4030,	455)
	(4040,	447)
	(4050,	442)
	(4060,	438)
	(4070,	432)
	(4080,	424)
	(4090,	423)
	(4100,	417)
	(4110,	410)
	(4120,	408)
	(4130,	405)
	(4140,	402)
	(4150,	400)
	(4160,	395)
	(4170,	391)
	(4180,	382)
	(4190,	376)
	(4200,	370)
	(4210,	366)
	(4220,	365)
	(4230,	364)
	(4240,	363)
	(4250,	355)
	(4260,	350)
	(4270,	343)
	(4280,	340)
	(4290,	331)
	(4300,	324)
	(4310,	318)
	(4320,	310)
	(4330,	305)
	(4340,	308)
	(4350,	302)
	(4360,	296)
	(4370,	291)
	(4380,	284)
	(4390,	278)
	(4400,	279)
	(4410,	274)
	(4420,	271)
	(4430,	267)
	(4440,	259)
	(4450,	253)
	(4460,	245)
	(4470,	242)
	(4480,	240)
	(4490,	236)
	(4500,	234)
	(4510,	224)
	(4520,	220)
	(4530,	214)
	(4540,	204)
	(4550,	195)
	(4560,	191)
	(4570,	186)
	(4580,	181)
	(4590,	177)
	(4600,	174)
	(4610,	172)
	(4620,	166)
	(4630,	159)
	(4640,	154)
	(4650,	147)
	(4660,	139)
	(4670,	132)
	(4680,	137)
	(4690,	132)
	(4700,	125)
	(4701,	124)
	(4702,	123)
	(4703,	123)
	(4704,	122)
	(4705,	123)
	(4706,	122)
	(4707,	121)
	(4708,	120)
	(4709,	120)
	(4710,	123)
	(4711,	122)
	(4712,	121)
	(4713,	120)
	(4714,	120)
	(4715,	121)
	(4716,	120)
	(4717,	119)
	(4718,	118)
	(4719,	118)
	(4720,	117)
	(4721,	116)
	(4722,	115)
	(4723,	115)
	(4724,	114)
	(4725,	113)
	(4726,	112)
	(4727,	111)
	(4728,	111)
	(4729,	110)
	(4730,	111)
	(4731,	110)
	(4732,	111)
	(4733,	110)
	(4734,	110)
	(4735,	109)
	(4736,	108)
	(4737,	107)
	(4738,	106)
	(4739,	105)
	(4740,	104)
	(4741,	106)
	(4742,	106)
	(4743,	105)
	(4744,	108)
	(4745,	107)
	(4746,	106)
	(4747,	105)
	(4748,	104)
	(4749,	103)
	(4750,	102)
	(4751,	105)
	(4752,	105)
	(4753,	104)
	(4754,	106)
	(4755,	106)
	(4756,	108)
	(4757,	107)
	(4758,	107)
	(4759,	106)
	(4760,	105)
	(4761,	109)
	(4762,	108)
	(4763,	107)
	(4764,	106)
	(4765,	106)
	(4766,	105)
	(4767,	105)
	(4768,	104)
	(4769,	103)
	(4770,	103)
	(4771,	102)
	(4772,	101)
	(4773,	100)
	(4774,	99)
	(4775,	99)
	(4776,	99)
	(4777,	98)
	(4778,	97)
	(4779,	98)
	(4780,	98)
	(4781,	97)
	(4782,	96)
	(4783,	95)
	(4784,	94)
	(4785,	94)
	(4786,	94)
	(4787,	93)
	(4788,	92)
	(4789,	92)
	(4790,	92)
	(4791,	91)
	(4792,	92)
	(4793,	91)
	(4794,	90)
	(4795,	90)
	(4796,	91)
	(4797,	91)
	(4798,	90)
	(4799,	89)
	(4800,	90)
	(4801,	90)
	(4802,	89)
	(4803,	89)
	(4804,	88)
	(4805,	87)
	(4806,	88)
	(4807,	87)
	(4808,	86)
	(4809,	85)
	(4810,	85)
	(4811,	84)
	(4812,	83)
	(4813,	82)
	(4814,	81)
	(4815,	81)
	(4816,	81)
	(4817,	80)
	(4818,	79)
	(4819,	78)
	(4820,	77)
	(4821,	76)
	(4822,	75)
	(4823,	75)
	(4824,	74)
	(4825,	74)
	(4826,	73)
	(4827,	72)
	(4828,	73)
	(4829,	72)
	(4830,	71)
	(4831,	70)
	(4832,	70)
	(4833,	69)
	(4834,	68)
	(4835,	68)
	(4836,	67)
	(4837,	66)
	(4838,	65)
	(4839,	64)
	(4840,	63)
	(4841,	62)
	(4842,	61)
	(4843,	61)
	(4844,	60)
	(4845,	59)
	(4846,	58)
	(4847,	58)
	(4848,	57)
	(4849,	59)
	(4850,	58)
	(4851,	57)
	(4852,	56)
	(4853,	55)
	(4854,	54)
	(4855,	54)
	(4856,	53)
	(4857,	52)
	(4858,	51)
	(4859,	50)
	(4860,	49)
	(4861,	48)
	(4862,	47)
	(4863,	46)
	(4864,	45)
	(4865,	44)
	(4866,	43)
	(4867,	42)
	(4868,	41)
	(4869,	40)
	(4870,	39)
	(4871,	38)
	(4872,	37)
	(4873,	36)
	(4874,	35)
	(4875,	34)
	(4876,	33)
	(4877,	34)
	(4878,	34)
	(4879,	33)
	(4880,	32)
	(4881,	31)
	(4882,	30)
	(4883,	29)
	(4884,	28)
	(4885,	30)
	(4886,	29)
	(4887,	28)
	(4888,	27)
	(4889,	26)
	(4890,	25)
	(4891,	24)
	(4892,	23)
	(4893,	23)
	(4894,	22)
	(4895,	21)
	(4896,	20)
	(4897,	19)
	(4898,	18)
	(4899,	17)
	(4900,	17)
	(4901,	16)
	(4902,	15)
	(4903,	14)
	(4904,	13)
	(4905,	12)
	(4906,	11)
	(4907,	10)
	(4908,	11)
	(4909,	10)
	(4910,	9)
	(4911,	8)
	(4912,	8)
	(4913,	10)
	(4914,	9)
	(4915,	8)
	(4916,	7)
	(4917,	6)
	(4918,	5)
	(4919,	5)
	(4920,	5)
	(4921,	5)
	(4922,	4)
	(4923,	3)
	(4924,	4)
	(4925,	4)
	(4926,	5)
	(4927,	4)
	(4928,	3)
	(4929,	2)
	(4930,	2)
	(4931,	2)
	(4932,	2)
	(4933,	1)
	(4934,	0)
	(4935,	0)
	(4936,	2)
	(4937,	2)
	(4938,	3)
	(4939,	3)
	(4940,	3)
	(4941,	4)
	(4942,	5)
	(4943,	5)
	(4944,	5)
	(4945,	7)
	(4946,	7)
	(4947,	8)
	(4948,	10)
	(4949,	10)
	(4950,	10)
	(4951,	10)
	(4952,	11)
	(4953,	11)
	(4954,	11)
	(4955,	12)
	(4956,	12)
	(4957,	12)
	(4958,	12)
	(4959,	12)
	(4960,	12)
	(4961,	12)
	(4962,	12)
	(4963,	14)
	(4964,	15)
	(4965,	15)
	(4966,	15)
	(4967,	17)
	(4968,	22)
	(4969,	23)
	(4970,	25)
	(4971,	25)
	(4972,	26)
	(4973,	26)
	(4974,	28)
	(4975,	31)
	(4976,	31)
	(4977,	31)
	(4978,	31)
	(4979,	31)
	(4980,	31)
	(4981,	31)
	(4982,	31)
	(4983,	32)
	(4984,	32)
	(4985,	32)
	(4986,	32)
	(4987,	32)
	(4988,	35)
	(4989,	35)
	(4990,	35)
	(4991,	35)
	(4992,	35)
	(4993,	36)
	(4994,	37)
	(4995,	37)
	(4996,	37)
	(4997,	37)
	(4998,	37)
	(4999,	37)
	(5000,	40)
	(5001,	40)
	(5002,	42)
	(5003,	42)
	(5004,	42)
	(5005,	42)
	(5006,	43)
	(5007,	43)
	(5008,	43)
	(5009,	43)
	(5010,	46)
	(5011,	46)
	(5012,	46)
	(5013,	46)
	(5014,	47)
	(5015,	48)
	(5016,	49)
	(5017,	50)
	(5018,	50)
	(5019,	52)
	(5020,	52)
	(5021,	53)
	(5022,	53)
	(5023,	54)
	(5024,	54)
	(5025,	55)
	(5026,	55)
	(5027,	55)
	(5028,	55)
	(5029,	55)
	(5030,	55)
	(5031,	55)
	(5032,	56)
	(5033,	57)
	(5034,	57)
	(5035,	57)
	(5036,	58)
	(5037,	58)
	(5038,	59)
	(5039,	59)
	(5040,	59)
	(5041,	60)
	(5042,	60)
	(5043,	61)
	(5044,	61)
	(5045,	61)
	(5046,	62)
	(5047,	62)
	(5048,	64)
	(5049,	65)
	(5050,	66)
	(5051,	67)
	(5052,	68)
	(5053,	68)
	(5054,	68)
	(5055,	68)
	(5056,	69)
	(5057,	70)
	(5058,	71)
	(5059,	72)
	(5060,	73)
	(5061,	73)
	(5062,	73)
	(5063,	74)
	(5064,	74)
	(5065,	75)
	(5066,	75)
	(5067,	75)
	(5068,	75)
	(5069,	77)
	(5070,	78)
	(5071,	78)
	(5072,	79)
	(5073,	79)
	(5074,	80)
	(5075,	80)
	(5076,	80)
	(5077,	80)
	(5078,	80)
	(5079,	80)
	(5080,	80)
	(5081,	81)
	(5082,	81)
	(5083,	81)
	(5084,	81)
	(5085,	81)
	(5086,	81)
	(5087,	82)
	(5088,	82)
	(5089,	82)
	(5090,	82)
	(5091,	82)
	(5092,	82)
	(5093,	85)
	(5094,	85)
	(5095,	86)
	(5096,	86)
	(5097,	87)
	(5098,	89)
	(5099,	89)
	(5100,	89)
	(5110,	99)
	(5120,	103)
	(5130,	111)
	(5140,	120)
	(5150,	125)
	(5160,	131)
	(5170,	136)
	(5180,	147)
	(5190,	150)
	(5200,	157)
	(5210,	160)
	(5220,	163)
	(5230,	170)
	(5240,	172)
	(5250,	175)
	(5260,	179)
	(5270,	183)
	(5280,	188)
	(5290,	196)
	(5300,	203)
	(5310,	209)
	(5320,	218)
	(5330,	222)
	(5340,	225)
	(5350,	233)
	(5360,	237)
	(5370,	242)
	(5380,	248)
	(5390,	251)
	(5400,	257)
	(5410,	261)
	(5420,	263)
	(5430,	267)
	(5440,	270)
	(5450,	273)
	(5460,	277)
	(5470,	285)
	(5480,	293)
	(5490,	299)
	(5500,	306)
	(5510,	309)
	(5520,	315)
	(5530,	320)
	(5540,	325)
	(5550,	328)
	(5560,	329)
	(5570,	338)
	(5580,	343)
	(5590,	350)
	(5600,	355)
	(5610,	361)
	(5620,	369)
	(5630,	372)
	(5640,	379)
	(5650,	381)
	(5660,	393)
	(5670,	396)
	(5680,	401)
	(5690,	408)
	(5700,	411)
	(5710,	414)
	(5720,	417)
	(5730,	423)
	(5740,	425)
	(5750,	433)
	(5760,	436)
	(5770,	441)
	(5780,	445)
	(5790,	453)
	(5800,	460)
	(5810,	460)
	(5820,	469)
	(5830,	476)
	(5840,	484)
	(5850,	491)
	(5860,	494)
	(5870,	497)
	(5880,	505)
	(5890,	508)
	(5900,	512)
	(5910,	515)
	(5920,	519)
	(5930,	524)
	(5940,	527)
	(5950,	531)
	(5960,	533)
	(5970,	538)
	(5980,	545)
	(5990,	547)
	(6000,	549)
	(6010,	558)
	(6020,	569)
	(6030,	572)
	(6040,	579)
	(6050,	584)
	(6060,	589)
	(6070,	593)
	(6080,	597)
	(6090,	599)
	(6100,	604)
	(6110,	607)
	(6120,	613)
	(6130,	615)
	(6140,	621)
	(6150,	629)
	(6160,	633)
	(6170,	641)
	(6180,	642)
	(6190,	647)
	(6200,	652)
	(6210,	659)
	(6220,	674)
	(6230,	682)
	(6240,	686)
	(6250,	697)
	(6260,	698)
	(6270,	707)
	(6280,	714)
	(6290,	719)
	(6300,	730)
	(6310,	734)
	(6320,	745)
	(6330,	753)
	(6340,	759)
	(6350,	762)
	(6360,	762)
	(6370,	770)
	(6380,	775)
	(6390,	779)
	(6400,	784)
	(6410,	787)
	(6420,	791)
	(6430,	796)
	(6440,	797)
	(6450,	802)
	(6460,	805)
	(6470,	809)
	(6480,	811)
	(6490,	815)
	(6500,	816)
	(6510,	823)
	(6520,	825)
	(6530,	831)
	(6540,	842)
	(6550,	844)
	(6560,	848)
	(6570,	852)
	(6580,	857)
	(6590,	860)
	(6600,	860)
	(6610,	868)
	(6620,	875)
	(6630,	876)
	(6640,	881)
	(6650,	885)
	(6660,	891)
	(6670,	899)
	(6680,	905)
	(6690,	910)
	(6700,	912)
	(6710,	923)
	(6720,	927)
	(6730,	928)
	(6740,	931)
	(6750,	934)
	(6760,	939)
	(6770,	942)
	(6780,	947)
	(6790,	951)
	(6800,	957)
	(6810,	962)
	(6820,	964)
	(6830,	965)
	(6840,	968)
	(6850,	975)
	(6860,	980)
	(6870,	982)
	(6880,	989)
	(6890,	993)
	(6900,	997)
	(6910,	997)
	(6920,	998)
	(6930,	1000)
	(6940,	1005)
	(6950,	1010)
	(6960,	1016)
	(6970,	1018)
	(6980,	1021)
	(6990,	1025)
	(7000,	1030)
	(7010,	1035)
	(7020,	1044)
	(7030,	1046)
	(7040,	1053)
	(7050,	1055)
	(7060,	1058)
	(7070,	1066)
	(7080,	1075)
	(7090,	1079)
	(7100,	1083)
	(7110,	1088)
	(7120,	1090)
	(7130,	1095)
	(7140,	1104)
	(7150,	1108)
	(7160,	1114)
	(7170,	1120)
	(7180,	1127)
	(7190,	1135)
	(7200,	1140)
	(7210,	1145)
	(7220,	1155)
	(7230,	1158)
	(7240,	1164)
	(7250,	1171)
	(7260,	1177)
	(7270,	1184)
	(7280,	1187)
	(7290,	1191)
	(7300,	1196)
	(7310,	1202)
	(7320,	1206)
	(7330,	1211)
	(7340,	1214)
	(7350,	1217)
	(7360,	1222)
	(7370,	1229)
	(7380,	1232)
	(7390,	1242)
	(7400,	1246)
	(7410,	1253)
	(7420,	1264)
	(7430,	1265)
	(7440,	1272)
	(7450,	1273)
	(7460,	1276)
	(7470,	1281)
	(7480,	1287)
	(7490,	1293)
	(7500,	1295)
	(7510,	1300)
	(7520,	1302)
	(7530,	1316)
	(7540,	1322)
	(7550,	1328)
	(7560,	1334)
	(7570,	1340)
	(7580,	1347)
	(7590,	1356)
	(7600,	1363)
	(7610,	1366)
	(7620,	1371)
	(7630,	1380)
	(7640,	1384)
	(7650,	1388)
	(7660,	1393)
	(7670,	1397)
	(7680,	1398)
	(7690,	1401)
	(7700,	1404)
	(7710,	1409)
	(7720,	1416)
	(7730,	1418)
	(7740,	1424)
	(7750,	1427)
	(7760,	1428)
	(7770,	1429)
	(7780,	1432)
	(7790,	1433)
	(7800,	1440)
	(7810,	1442)
	(7820,	1447)
	(7830,	1450)
	(7840,	1454)
	(7850,	1460)
	(7860,	1462)
	(7870,	1468)
	(7880,	1474)
	(7890,	1475)
	(7900,	1478)
	(7910,	1483)
	(7920,	1487)
	(7930,	1491)
	(7940,	1496)
	(7950,	1500)
	(7960,	1505)
	(7970,	1507)
	(7980,	1511)
	(7990,	1517)
	(8000,	1519)
	(8010,	1525)
	(8020,	1527)
	(8030,	1531)
	(8040,	1539)
	(8050,	1542)
	(8060,	1550)
	(8070,	1557)
	(8080,	1563)
	(8090,	1571)
	(8100,	1576)
	(8110,	1584)
	(8120,	1588)
	(8130,	1596)
	(8140,	1602)
	(8150,	1612)
	(8160,	1626)
	(8170,	1629)
	(8180,	1632)
	(8190,	1639)
	(8200,	1644)
	(8210,	1649)
	(8220,	1653)
	(8230,	1655)
	(8240,	1658)
	(8250,	1660)
	(8260,	1664)
	(8270,	1666)
	(8280,	1674)
	(8290,	1682)
	(8300,	1684)
	(8310,	1692)
	(8320,	1701)
	(8330,	1707)
	(8340,	1709)
	(8350,	1714)
	(8360,	1718)
	(8370,	1723)
	(8380,	1728)
	(8390,	1731)
	(8400,	1736)
	(8410,	1742)
	(8420,	1745)
	(8430,	1746)
	(8440,	1749)
	(8450,	1755)
	(8460,	1765)
	(8470,	1772)
	(8480,	1775)
	(8490,	1775)
	(8500,	1780)
	(8510,	1784)
	(8520,	1788)
	(8530,	1794)
	(8540,	1802)
	(8550,	1805)
	(8560,	1813)
	(8570,	1818)
	(8580,	1825)
	(8590,	1826)
	(8600,	1841)
	(8601,	1842)
	(8602,	1843)
	(8603,	1845)
	(8604,	1846)
	(8605,	1846)
	(8606,	1846)
	(8607,	1847)
	(8608,	1847)
	(8609,	1847)
	(8610,	1848)
	(8611,	1849)
	(8612,	1849)
	(8613,	1851)
	(8614,	1851)
	(8615,	1851)
	(8616,	1852)
	(8617,	1852)
	(8618,	1852)
	(8619,	1853)
	(8620,	1853)
	(8621,	1853)
	(8622,	1854)
	(8623,	1855)
	(8624,	1855)
	(8625,	1858)
	(8626,	1858)
	(8627,	1858)
	(8628,	1858)
	(8629,	1859)
	(8630,	1859)
	(8631,	1859)
	(8632,	1859)
	(8633,	1859)
	(8634,	1863)
	(8635,	1863)
	(8636,	1863)
	(8637,	1863)
	(8638,	1863)
	(8639,	1863)
	(8640,	1863)
	(8641,	1863)
	(8642,	1863)
	(8643,	1864)
	(8644,	1865)
	(8645,	1865)
	(8646,	1865)
	(8647,	1865)
	(8648,	1866)
	(8649,	1866)
	(8650,	1866)
	(8651,	1867)
	(8652,	1867)
	(8653,	1867)
	(8654,	1867)
	(8655,	1867)
	(8656,	1867)
	(8657,	1867)
	(8658,	1867)
	(8659,	1867)
	(8660,	1867)
	(8661,	1867)
	(8662,	1867)
	(8663,	1867)
	(8664,	1867)
	(8665,	1870)
	(8666,	1870)
	(8667,	1870)
	(8668,	1871)
	(8669,	1871)
	(8670,	1871)
	(8671,	1871)
	(8672,	1871)
	(8673,	1875)
	(8674,	1875)
	(8675,	1875)
	(8676,	1875)
	(8677,	1875)
	(8678,	1877)
	(8679,	1878)
	(8680,	1880)
	(8681,	1880)
	(8682,	1880)
	(8683,	1880)
	(8684,	1881)
	(8685,	1881)
	(8686,	1881)
	(8687,	1881)
	(8688,	1881)
	(8689,	1881)
	(8690,	1882)
	(8691,	1883)
	(8692,	1883)
	(8693,	1883)
	(8694,	1883)
	(8695,	1883)
	(8696,	1883)
	(8697,	1884)
	(8698,	1884)
	(8699,	1889)
	(8700,	1889)
	(8701,	1889)
	(8702,	1889)
	(8703,	1889)
	(8704,	1889)
	(8705,	1889)
	(8706,	1891)
	(8707,	1892)
	(8708,	1892)
	(8709,	1892)
	(8710,	1894)
	(8711,	1895)
	(8712,	1897)
	(8713,	1897)
	(8714,	1897)
	(8715,	1897)
	(8716,	1898)
	(8717,	1900)
	(8718,	1900)
	(8719,	1900)
	(8720,	1901)
	(8721,	1902)
	(8722,	1902)
	(8723,	1903)
	(8724,	1903)
	(8725,	1904)
	(8726,	1904)
	(8727,	1904)
	(8728,	1904)
	(8729,	1904)
	(8730,	1904)
	(8731,	1906)
	(8732,	1906)
	(8733,	1906)
	(8734,	1906)
	(8735,	1906)
	(8736,	1906)
	(8737,	1906)
	(8738,	1906)
	(8739,	1906)
	(8740,	1906)
	(8741,	1906)
	(8742,	1906)
	(8743,	1907)
	(8744,	1907)
	(8745,	1909)
	(8746,	1910)
	(8747,	1910)
	(8748,	1911)
	(8749,	1912)
	(8750,	1912)
	(8751,	1913)
	(8752,	1913)
	(8753,	1913)
	(8754,	1914)
	(8755,	1914)
	(8756,	1919)
	(8757,	1919)
	(8758,	1919)
	(8759,	1919)
	(8760,	1919)
	(8761,	1921)
	(8762,	1921)
	(8763,	1923)
	(8764,	1924)
	(8765,	1924)
	(8766,	1924)
	(8767,	1924)
	(8768,	1924)
	(8769,	1924)
	(8770,	1924)
	(8771,	1926)
	(8772,	1932)
	(8773,	1932)
	(8774,	1932)
	(8775,	1932)
	(8776,	1932)
	(8777,	1934)
	(8778,	1935)
	(8779,	1936)
	(8780,	1936)
	(8781,	1938)
	(8782,	1938)
	(8783,	1938)
	(8784,	1938)
	(8785,	1938)
	(8786,	1938)
	(8787,	1938)
	(8788,	1939)
	(8789,	1939)
	(8790,	1939)
	(8791,	1939)
	(8792,	1939)
	(8793,	1939)
	(8794,	1939)
	(8795,	1939)
	(8796,	1939)
	(8797,	1940)
	(8798,	1940)
	(8799,	1941)
	(8800,	1941)
	(8801,	1942)
	(8802,	1942)
	(8803,	1943)
	(8804,	1943)
	(8805,	1943)
	(8806,	1945)
	(8807,	1945)
	(8808,	1946)
	(8809,	1946)
	(8810,	1946)
	(8811,	1946)
	(8812,	1946)
	(8813,	1948)
	(8814,	1950)
	(8815,	1950)
	(8816,	1951)
	(8817,	1951)
	(8818,	1952)
	(8819,	1954)
	(8820,	1954)
	(8821,	1954)
	(8822,	1954)
	(8823,	1954)
	(8824,	1954)
	(8825,	1954)
	(8826,	1957)
	(8827,	1957)
	(8828,	1959)
	(8829,	1959)
	(8830,	1959)
	(8831,	1959)
	(8832,	1960)
	(8833,	1960)
	(8834,	1960)
	(8835,	1960)
	(8836,	1960)
	(8837,	1960)
	(8838,	1962)
	(8839,	1963)
	(8840,	1963)
	(8841,	1964)
	(8842,	1965)
	(8843,	1965)
	(8844,	1965)
	(8845,	1965)
	(8846,	1966)
	(8847,	1966)
	(8848,	1966)
	(8849,	1967)
	(8850,	1967)
	(8851,	1967)
	(8852,	1968)
	(8853,	1968)
	(8854,	1968)
	(8855,	1974)
	(8856,	1974)
	(8857,	1974)
	(8858,	1974)
	(8859,	1975)
	(8860,	1975)
	(8861,	1975)
	(8862,	1975)
	(8863,	1975)
	(8864,	1976)
	(8865,	1977)
	(8866,	1977)
	(8867,	1977)
	(8868,	1977)
	(8869,	1978)
	(8870,	1978)
	(8871,	1980)
	(8872,	1980)
	(8873,	1980)
	(8874,	1980)
	(8875,	1980)
	(8876,	1979)
	(8877,	1978)
	(8878,	1977)
	(8879,	1976)
	(8880,	1975)
	(8881,	1974)
	(8882,	1973)
	(8883,	1972)
	(8884,	1971)
	(8885,	1970)
	(8886,	1972)
	(8887,	1971)
	(8888,	1970)
	(8889,	1969)
	(8890,	1968)
	(8891,	1969)
	(8892,	1969)
	(8893,	1968)
	(8894,	1968)
	(8895,	1967)
	(8896,	1966)
	(8897,	1965)
	(8898,	1964)
	(8899,	1963)
	(8900,	1962)
	(8901,	1961)
	(8902,	1960)
	(8903,	1959)
	(8904,	1961)
	(8905,	1960)
	(8906,	1959)
	(8907,	1960)
	(8908,	1963)
	(8909,	1966)
	(8910,	1965)
	(8911,	1964)
	(8912,	1964)
	(8913,	1968)
	(8914,	1967)
	(8915,	1967)
	(8916,	1966)
	(8917,	1965)
	(8918,	1964)
	(8919,	1963)
	(8920,	1962)
	(8921,	1961)
	(8922,	1960)
	(8923,	1959)
	(8924,	1959)
	(8925,	1958)
	(8926,	1957)
	(8927,	1956)
	(8928,	1956)
	(8929,	1957)
	(8930,	1956)
	(8931,	1958)
	(8932,	1959)
	(8933,	1960)
	(8934,	1960)
	(8935,	1959)
	(8936,	1958)
	(8937,	1957)
	(8938,	1960)
	(8939,	1960)
	(8940,	1961)
	(8941,	1961)
	(8942,	1960)
	(8943,	1962)
	(8944,	1961)
	(8945,	1960)
	(8946,	1959)
	(8947,	1958)
	(8948,	1957)
	(8949,	1957)
	(8950,	1956)
	(8951,	1956)
	(8952,	1955)
	(8953,	1954)
	(8954,	1953)
	(8955,	1952)
	(8956,	1951)
	(8957,	1950)
	(8958,	1949)
	(8959,	1948)
	(8960,	1947)
	(8961,	1946)
	(8962,	1945)
	(8963,	1945)
	(8964,	1944)
	(8965,	1943)
	(8966,	1942)
	(8967,	1941)
	(8968,	1940)
	(8969,	1939)
	(8970,	1939)
	(8971,	1938)
	(8972,	1937)
	(8973,	1936)
	(8974,	1935)
	(8975,	1935)
	(8976,	1936)
	(8977,	1935)
	(8978,	1934)
	(8979,	1933)
	(8980,	1932)
	(8981,	1931)
	(8982,	1930)
	(8983,	1929)
	(8984,	1928)
	(8985,	1928)
	(8986,	1929)
	(8987,	1928)
	(8988,	1927)
	(8989,	1926)
	(8990,	1926)
	(8991,	1925)
	(8992,	1925)
	(8993,	1924)
	(8994,	1923)
	(8995,	1922)
	(8996,	1922)
	(8997,	1922)
	(8998,	1922)
	(8999,	1921)
	(9000,	1921)
	(9010,	1915)
	(9020,	1906)
	(9030,	1899)
	(9040,	1893)
	(9050,	1891)
	(9060,	1884)
	(9070,	1882)
	(9080,	1875)
	(9090,	1867)
	(9100,	1860)
	(9110,	1856)
	(9120,	1856)
	(9130,	1849)
	(9140,	1842)
	(9150,	1836)
	(9160,	1830)
	(9170,	1825)
	(9180,	1818)
	(9190,	1814)
	(9200,	1816)
	(9210,	1812)
	(9220,	1806)
	(9230,	1800)
	(9240,	1795)
	(9250,	1789)
	(9260,	1782)
	(9270,	1778)
	(9280,	1772)
	(9290,	1768)
	(9300,	1762)
	(9310,	1757)
	(9320,	1750)
	(9330,	1741)
	(9340,	1736)
	(9350,	1732)
	(9360,	1727)
	(9370,	1720)
	(9380,	1722)
	(9390,	1716)
	(9400,	1712)
	(9410,	1705)
	(9420,	1700)
	(9430,	1693)
	(9440,	1685)
	(9450,	1680)
	(9460,	1673)
	(9470,	1663)
	(9480,	1655)
	(9490,	1652)
	(9500,	1645)
	(9510,	1637)
	(9520,	1629)
	(9530,	1624)
	(9540,	1623)
	(9550,	1618)
	(9560,	1608)
	(9570,	1602)
	(9580,	1594)
	(9590,	1590)
	(9600,	1584)
	(9610,	1588)
	(9620,	1581)
	(9630,	1574)
	(9640,	1576)
	(9650,	1574)
	(9660,	1571)
	(9670,	1564)
	(9680,	1556)
	(9690,	1553)
	(9700,	1550)
	(9710,	1544)
	(9720,	1543)
	(9730,	1541)
	(9740,	1535)
	(9750,	1530)
	(9760,	1527)
	(9770,	1524)
	(9780,	1519)
	(9790,	1511)
	(9800,	1507)
	(9810,	1505)
	(9820,	1506)
	(9830,	1505)
	(9840,	1504)
	(9850,	1501)
	(9860,	1494)
	(9870,	1489)
	(9880,	1487)
	(9890,	1480)
	(9900,	1475)
	(9910,	1469)
	(9920,	1465)
	(9930,	1460)
	(9940,	1456)
	(9950,	1448)
	(9960,	1443)
	(9970,	1439)
	(9980,	1439)
	(9990,	1433)
	(10000,	1427)
};
\addplot[color=black] plot coordinates {
	(0,	456)
	(10,	451)
	(20,	445)
	(30,	440)
	(40,	436)
	(50,	431)
	(60,	425)
	(70,	424)
	(80,	419)
	(90,	411)
	(100,	408)
	(110,	407)
	(120,	403)
	(130,	398)
	(140,	389)
	(150,	380)
	(160,	377)
	(170,	372)
	(180,	373)
	(190,	371)
	(200,	365)
	(210,	360)
	(220,	353)
	(230,	346)
	(240,	342)
	(250,	335)
	(260,	330)
	(270,	327)
	(280,	321)
	(290,	316)
	(300,	310)
	(310,	302)
	(320,	297)
	(330,	295)
	(340,	293)
	(350,	287)
	(360,	281)
	(370,	277)
	(380,	271)
	(390,	264)
	(400,	259)
	(410,	254)
	(420,	248)
	(430,	242)
	(440,	244)
	(450,	237)
	(460,	232)
	(470,	224)
	(480,	219)
	(490,	220)
	(500,	220)
	(510,	216)
	(520,	206)
	(530,	204)
	(540,	196)
	(550,	193)
	(560,	187)
	(570,	182)
	(580,	177)
	(590,	172)
	(600,	163)
	(610,	160)
	(620,	156)
	(630,	152)
	(640,	146)
	(650,	137)
	(660,	128)
	(670,	124)
	(680,	119)
	(690,	115)
	(700,	112)
	(710,	110)
	(720,	106)
	(730,	96)
	(740,	95)
	(750,	90)
	(760,	81)
	(770,	79)
	(780,	74)
	(790,	69)
	(800,	66)
	(801,	67)
	(802,	67)
	(803,	67)
	(804,	66)
	(805,	65)
	(806,	64)
	(807,	63)
	(808,	64)
	(809,	63)
	(810,	65)
	(811,	66)
	(812,	66)
	(813,	65)
	(814,	64)
	(815,	63)
	(816,	62)
	(817,	61)
	(818,	60)
	(819,	59)
	(820,	58)
	(821,	57)
	(822,	56)
	(823,	56)
	(824,	57)
	(825,	57)
	(826,	56)
	(827,	55)
	(828,	55)
	(829,	57)
	(830,	56)
	(831,	55)
	(832,	54)
	(833,	53)
	(834,	52)
	(835,	51)
	(836,	50)
	(837,	50)
	(838,	49)
	(839,	50)
	(840,	49)
	(841,	49)
	(842,	50)
	(843,	50)
	(844,	49)
	(845,	51)
	(846,	50)
	(847,	49)
	(848,	48)
	(849,	47)
	(850,	46)
	(851,	47)
	(852,	46)
	(853,	46)
	(854,	48)
	(855,	47)
	(856,	46)
	(857,	45)
	(858,	44)
	(859,	43)
	(860,	42)
	(861,	41)
	(862,	40)
	(863,	39)
	(864,	38)
	(865,	37)
	(866,	36)
	(867,	35)
	(868,	35)
	(869,	34)
	(870,	34)
	(871,	33)
	(872,	32)
	(873,	32)
	(874,	31)
	(875,	31)
	(876,	33)
	(877,	33)
	(878,	32)
	(879,	31)
	(880,	32)
	(881,	31)
	(882,	30)
	(883,	30)
	(884,	29)
	(885,	30)
	(886,	30)
	(887,	29)
	(888,	28)
	(889,	27)
	(890,	26)
	(891,	25)
	(892,	24)
	(893,	24)
	(894,	23)
	(895,	22)
	(896,	21)
	(897,	20)
	(898,	19)
	(899,	19)
	(900,	18)
	(901,	17)
	(902,	16)
	(903,	15)
	(904,	15)
	(905,	14)
	(906,	13)
	(907,	12)
	(908,	11)
	(909,	11)
	(910,	11)
	(911,	12)
	(912,	11)
	(913,	10)
	(914,	9)
	(915,	8)
	(916,	8)
	(917,	7)
	(918,	8)
	(919,	8)
	(920,	7)
	(921,	8)
	(922,	7)
	(923,	6)
	(924,	5)
	(925,	4)
	(926,	4)
	(927,	3)
	(928,	4)
	(929,	3)
	(930,	3)
	(931,	2)
	(932,	2)
	(933,	1)
	(934,	0)
	(935,	0)
	(936,	0)
	(937,	0)
	(938,	1)
	(939,	0)
	(940,	0)
	(941,	0)
	(942,	0)
	(943,	1)
	(944,	1)
	(945,	2)
	(946,	1)
	(947,	1)
	(948,	1)
	(949,	2)
	(950,	1)
	(951,	0)
	(952,	0)
	(953,	0)
	(954,	0)
	(955,	0)
	(956,	0)
	(957,	0)
	(958,	0)
	(959,	0)
	(960,	0)
	(961,	0)
	(962,	0)
	(963,	0)
	(964,	0)
	(965,	0)
	(966,	0)
	(967,	0)
	(968,	0)
	(969,	0)
	(970,	1)
	(971,	1)
	(972,	1)
	(973,	1)
	(974,	1)
	(975,	0)
	(976,	1)
	(977,	0)
	(978,	0)
	(979,	0)
	(980,	0)
	(981,	0)
	(982,	0)
	(983,	1)
	(984,	0)
	(985,	0)
	(986,	0)
	(987,	0)
	(988,	1)
	(989,	1)
	(990,	0)
	(991,	2)
	(992,	1)
	(993,	2)
	(994,	1)
	(995,	1)
	(996,	0)
	(997,	0)
	(998,	1)
	(999,	2)
	(1000,	2)
	(1001,	3)
	(1002,	2)
	(1003,	1)
	(1004,	1)
	(1005,	0)
	(1006,	0)
	(1007,	0)
	(1008,	2)
	(1009,	1)
	(1010,	1)
	(1011,	0)
	(1012,	0)
	(1013,	1)
	(1014,	0)
	(1015,	0)
	(1016,	0)
	(1017,	0)
	(1018,	0)
	(1019,	0)
	(1020,	1)
	(1021,	1)
	(1022,	0)
	(1023,	0)
	(1024,	0)
	(1025,	0)
	(1026,	1)
	(1027,	0)
	(1028,	0)
	(1029,	0)
	(1030,	0)
	(1031,	0)
	(1032,	0)
	(1033,	0)
	(1034,	0)
	(1035,	0)
	(1036,	0)
	(1037,	0)
	(1038,	1)
	(1039,	0)
	(1040,	0)
	(1041,	1)
	(1042,	1)
	(1043,	0)
	(1044,	1)
	(1045,	0)
	(1046,	0)
	(1047,	0)
	(1048,	3)
	(1049,	3)
	(1050,	4)
	(1051,	5)
	(1052,	5)
	(1053,	5)
	(1054,	5)
	(1055,	5)
	(1056,	6)
	(1057,	6)
	(1058,	6)
	(1059,	6)
	(1060,	7)
	(1061,	8)
	(1062,	8)
	(1063,	8)
	(1064,	8)
	(1065,	8)
	(1066,	9)
	(1067,	9)
	(1068,	9)
	(1069,	9)
	(1070,	10)
	(1071,	10)
	(1072,	11)
	(1073,	11)
	(1074,	11)
	(1075,	11)
	(1076,	11)
	(1077,	13)
	(1078,	16)
	(1079,	16)
	(1080,	16)
	(1081,	16)
	(1082,	18)
	(1083,	18)
	(1084,	18)
	(1085,	18)
	(1086,	18)
	(1087,	19)
	(1088,	19)
	(1089,	20)
	(1090,	20)
	(1091,	20)
	(1092,	21)
	(1093,	21)
	(1094,	21)
	(1095,	22)
	(1096,	22)
	(1097,	22)
	(1098,	22)
	(1099,	22)
	(1100,	22)
	(1101,	23)
	(1102,	24)
	(1103,	24)
	(1104,	24)
	(1105,	25)
	(1106,	25)
	(1107,	25)
	(1108,	25)
	(1109,	27)
	(1110,	28)
	(1111,	29)
	(1112,	29)
	(1113,	29)
	(1114,	29)
	(1115,	30)
	(1116,	30)
	(1117,	30)
	(1118,	30)
	(1119,	30)
	(1120,	30)
	(1121,	30)
	(1122,	30)
	(1123,	30)
	(1124,	30)
	(1125,	30)
	(1126,	30)
	(1127,	30)
	(1128,	30)
	(1129,	31)
	(1130,	31)
	(1131,	31)
	(1132,	31)
	(1133,	31)
	(1134,	31)
	(1135,	33)
	(1136,	33)
	(1137,	35)
	(1138,	36)
	(1139,	36)
	(1140,	36)
	(1141,	36)
	(1142,	37)
	(1143,	37)
	(1144,	37)
	(1145,	38)
	(1146,	38)
	(1147,	38)
	(1148,	38)
	(1149,	41)
	(1150,	41)
	(1151,	41)
	(1152,	41)
	(1153,	41)
	(1154,	44)
	(1155,	45)
	(1156,	45)
	(1157,	45)
	(1158,	45)
	(1159,	45)
	(1160,	47)
	(1161,	47)
	(1162,	48)
	(1163,	48)
	(1164,	48)
	(1165,	49)
	(1166,	49)
	(1167,	49)
	(1168,	49)
	(1169,	49)
	(1170,	49)
	(1171,	49)
	(1172,	49)
	(1173,	51)
	(1174,	51)
	(1175,	51)
	(1176,	51)
	(1177,	51)
	(1178,	51)
	(1179,	51)
	(1180,	51)
	(1181,	51)
	(1182,	51)
	(1183,	51)
	(1184,	51)
	(1185,	51)
	(1186,	51)
	(1187,	51)
	(1188,	51)
	(1189,	52)
	(1190,	52)
	(1191,	56)
	(1192,	57)
	(1193,	58)
	(1194,	59)
	(1195,	60)
	(1196,	61)
	(1197,	61)
	(1198,	62)
	(1199,	62)
	(1200,	62)
	(1210,	64)
	(1220,	69)
	(1230,	72)
	(1240,	75)
	(1250,	80)
	(1260,	86)
	(1270,	93)
	(1280,	98)
	(1290,	103)
	(1300,	104)
	(1310,	109)
	(1320,	113)
	(1330,	116)
	(1340,	119)
	(1350,	124)
	(1360,	128)
	(1370,	131)
	(1380,	133)
	(1390,	137)
	(1400,	141)
	(1410,	147)
	(1420,	153)
	(1430,	156)
	(1440,	161)
	(1450,	169)
	(1460,	172)
	(1470,	180)
	(1480,	186)
	(1490,	195)
	(1500,	200)
	(1510,	209)
	(1520,	216)
	(1530,	220)
	(1540,	228)
	(1550,	236)
	(1560,	243)
	(1570,	249)
	(1580,	252)
	(1590,	254)
	(1600,	261)
	(1610,	265)
	(1620,	271)
	(1630,	275)
	(1640,	276)
	(1650,	282)
	(1660,	292)
	(1670,	296)
	(1680,	303)
	(1690,	310)
	(1700,	315)
	(1710,	318)
	(1720,	322)
	(1730,	335)
	(1740,	337)
	(1750,	341)
	(1760,	351)
	(1770,	354)
	(1780,	360)
	(1790,	368)
	(1800,	382)
	(1810,	385)
	(1820,	389)
	(1830,	392)
	(1840,	394)
	(1850,	398)
	(1860,	403)
	(1870,	405)
	(1880,	406)
	(1890,	413)
	(1900,	419)
	(1910,	426)
	(1920,	427)
	(1930,	432)
	(1940,	437)
	(1950,	445)
	(1960,	452)
	(1970,	456)
	(1980,	464)
	(1990,	468)
	(2000,	473)
	(2010,	475)
	(2020,	482)
	(2030,	484)
	(2040,	488)
	(2050,	493)
	(2060,	499)
	(2070,	503)
	(2080,	505)
	(2090,	507)
	(2100,	512)
	(2110,	518)
	(2120,	528)
	(2130,	531)
	(2140,	533)
	(2150,	538)
	(2160,	546)
	(2170,	551)
	(2180,	560)
	(2190,	565)
	(2200,	568)
	(2210,	577)
	(2220,	585)
	(2230,	593)
	(2240,	599)
	(2250,	604)
	(2260,	610)
	(2270,	616)
	(2280,	619)
	(2290,	623)
	(2300,	626)
	(2310,	632)
	(2320,	634)
	(2330,	638)
	(2340,	640)
	(2350,	644)
	(2360,	647)
	(2370,	648)
	(2380,	654)
	(2390,	660)
	(2400,	667)
	(2410,	673)
	(2420,	689)
	(2430,	693)
	(2440,	697)
	(2450,	708)
	(2460,	714)
	(2470,	721)
	(2480,	725)
	(2490,	731)
	(2500,	735)
	(2510,	740)
	(2520,	745)
	(2530,	747)
	(2540,	752)
	(2550,	753)
	(2560,	757)
	(2570,	760)
	(2580,	761)
	(2590,	767)
	(2600,	774)
	(2610,	783)
	(2620,	787)
	(2630,	792)
	(2640,	795)
	(2650,	795)
	(2660,	801)
	(2670,	801)
	(2680,	807)
	(2690,	812)
	(2700,	812)
	(2710,	817)
	(2720,	819)
	(2730,	826)
	(2740,	831)
	(2750,	832)
	(2760,	837)
	(2770,	845)
	(2780,	849)
	(2790,	854)
	(2800,	861)
	(2810,	872)
	(2820,	877)
	(2830,	881)
	(2840,	884)
	(2850,	887)
	(2860,	890)
	(2870,	894)
	(2880,	901)
	(2890,	904)
	(2900,	909)
	(2910,	914)
	(2920,	921)
	(2930,	930)
	(2940,	939)
	(2950,	944)
	(2960,	946)
	(2970,	948)
	(2980,	951)
	(2990,	952)
	(3000,	956)
	(3010,	964)
	(3020,	968)
	(3030,	973)
	(3040,	979)
	(3050,	982)
	(3060,	987)
	(3070,	993)
	(3080,	993)
	(3090,	996)
	(3100,	1001)
	(3110,	1006)
	(3120,	1017)
	(3130,	1021)
	(3140,	1023)
	(3150,	1028)
	(3160,	1030)
	(3170,	1036)
	(3180,	1039)
	(3190,	1044)
	(3200,	1051)
	(3210,	1052)
	(3220,	1058)
	(3230,	1062)
	(3240,	1064)
	(3250,	1068)
	(3260,	1069)
	(3270,	1072)
	(3280,	1076)
	(3290,	1076)
	(3300,	1083)
	(3310,	1086)
	(3320,	1096)
	(3330,	1099)
	(3340,	1110)
	(3350,	1116)
	(3360,	1120)
	(3370,	1124)
	(3380,	1130)
	(3390,	1131)
	(3400,	1135)
	(3410,	1140)
	(3420,	1145)
	(3430,	1150)
	(3440,	1154)
	(3450,	1164)
	(3460,	1170)
	(3470,	1176)
	(3480,	1181)
	(3490,	1187)
	(3500,	1196)
	(3510,	1202)
	(3520,	1205)
	(3530,	1215)
	(3540,	1217)
	(3550,	1220)
	(3560,	1224)
	(3570,	1233)
	(3580,	1240)
	(3590,	1246)
	(3600,	1250)
	(3610,	1259)
	(3620,	1265)
	(3630,	1268)
	(3640,	1272)
	(3650,	1277)
	(3660,	1280)
	(3670,	1286)
	(3680,	1291)
	(3690,	1298)
	(3700,	1309)
	(3710,	1310)
	(3720,	1315)
	(3730,	1321)
	(3740,	1326)
	(3750,	1329)
	(3760,	1331)
	(3770,	1340)
	(3780,	1345)
	(3790,	1349)
	(3800,	1354)
	(3810,	1363)
	(3820,	1367)
	(3830,	1370)
	(3840,	1375)
	(3850,	1378)
	(3860,	1389)
	(3870,	1397)
	(3880,	1402)
	(3890,	1409)
	(3900,	1415)
	(3910,	1418)
	(3920,	1423)
	(3930,	1424)
	(3940,	1432)
	(3950,	1434)
	(3960,	1435)
	(3970,	1437)
	(3980,	1442)
	(3990,	1445)
	(4000,	1448)
	(4010,	1452)
	(4020,	1458)
	(4030,	1468)
	(4040,	1471)
	(4050,	1473)
	(4060,	1481)
	(4070,	1487)
	(4080,	1493)
	(4090,	1497)
	(4100,	1501)
	(4110,	1502)
	(4120,	1504)
	(4130,	1509)
	(4140,	1513)
	(4150,	1516)
	(4160,	1516)
	(4170,	1521)
	(4180,	1526)
	(4190,	1528)
	(4200,	1536)
	(4210,	1546)
	(4220,	1553)
	(4230,	1555)
	(4240,	1557)
	(4250,	1561)
	(4260,	1562)
	(4270,	1563)
	(4280,	1569)
	(4290,	1573)
	(4300,	1578)
	(4310,	1582)
	(4320,	1587)
	(4330,	1593)
	(4340,	1597)
	(4350,	1601)
	(4360,	1608)
	(4370,	1610)
	(4380,	1615)
	(4390,	1618)
	(4400,	1625)
	(4410,	1628)
	(4420,	1632)
	(4430,	1639)
	(4440,	1648)
	(4450,	1657)
	(4460,	1662)
	(4470,	1666)
	(4480,	1675)
	(4490,	1683)
	(4500,	1686)
	(4510,	1693)
	(4520,	1703)
	(4530,	1708)
	(4540,	1714)
	(4550,	1717)
	(4560,	1725)
	(4570,	1730)
	(4580,	1736)
	(4590,	1739)
	(4600,	1742)
	(4610,	1744)
	(4620,	1751)
	(4630,	1757)
	(4640,	1759)
	(4650,	1763)
	(4660,	1766)
	(4670,	1768)
	(4680,	1770)
	(4690,	1774)
	(4700,	1781)
	(4701,	1781)
	(4702,	1784)
	(4703,	1785)
	(4704,	1785)
	(4705,	1785)
	(4706,	1785)
	(4707,	1785)
	(4708,	1785)
	(4709,	1785)
	(4710,	1785)
	(4711,	1785)
	(4712,	1785)
	(4713,	1785)
	(4714,	1785)
	(4715,	1785)
	(4716,	1785)
	(4717,	1785)
	(4718,	1785)
	(4719,	1785)
	(4720,	1785)
	(4721,	1786)
	(4722,	1786)
	(4723,	1786)
	(4724,	1786)
	(4725,	1786)
	(4726,	1786)
	(4727,	1786)
	(4728,	1786)
	(4729,	1786)
	(4730,	1788)
	(4731,	1788)
	(4732,	1788)
	(4733,	1788)
	(4734,	1788)
	(4735,	1788)
	(4736,	1788)
	(4737,	1788)
	(4738,	1791)
	(4739,	1791)
	(4740,	1791)
	(4741,	1791)
	(4742,	1791)
	(4743,	1791)
	(4744,	1791)
	(4745,	1791)
	(4746,	1791)
	(4747,	1791)
	(4748,	1791)
	(4749,	1791)
	(4750,	1791)
	(4751,	1792)
	(4752,	1792)
	(4753,	1793)
	(4754,	1793)
	(4755,	1793)
	(4756,	1793)
	(4757,	1793)
	(4758,	1793)
	(4759,	1793)
	(4760,	1793)
	(4761,	1794)
	(4762,	1795)
	(4763,	1796)
	(4764,	1796)
	(4765,	1797)
	(4766,	1797)
	(4767,	1797)
	(4768,	1797)
	(4769,	1797)
	(4770,	1798)
	(4771,	1800)
	(4772,	1800)
	(4773,	1800)
	(4774,	1800)
	(4775,	1802)
	(4776,	1803)
	(4777,	1803)
	(4778,	1803)
	(4779,	1803)
	(4780,	1803)
	(4781,	1803)
	(4782,	1803)
	(4783,	1805)
	(4784,	1805)
	(4785,	1810)
	(4786,	1810)
	(4787,	1810)
	(4788,	1812)
	(4789,	1812)
	(4790,	1812)
	(4791,	1813)
	(4792,	1814)
	(4793,	1814)
	(4794,	1817)
	(4795,	1818)
	(4796,	1820)
	(4797,	1820)
	(4798,	1821)
	(4799,	1821)
	(4800,	1821)
	(4801,	1821)
	(4802,	1821)
	(4803,	1821)
	(4804,	1821)
	(4805,	1821)
	(4806,	1821)
	(4807,	1822)
	(4808,	1826)
	(4809,	1830)
	(4810,	1830)
	(4811,	1830)
	(4812,	1830)
	(4813,	1830)
	(4814,	1830)
	(4815,	1830)
	(4816,	1831)
	(4817,	1831)
	(4818,	1831)
	(4819,	1831)
	(4820,	1832)
	(4821,	1833)
	(4822,	1833)
	(4823,	1833)
	(4824,	1833)
	(4825,	1833)
	(4826,	1833)
	(4827,	1833)
	(4828,	1836)
	(4829,	1836)
	(4830,	1837)
	(4831,	1839)
	(4832,	1839)
	(4833,	1839)
	(4834,	1839)
	(4835,	1839)
	(4836,	1839)
	(4837,	1839)
	(4838,	1839)
	(4839,	1845)
	(4840,	1845)
	(4841,	1846)
	(4842,	1847)
	(4843,	1847)
	(4844,	1847)
	(4845,	1848)
	(4846,	1850)
	(4847,	1851)
	(4848,	1851)
	(4849,	1851)
	(4850,	1851)
	(4851,	1857)
	(4852,	1857)
	(4853,	1857)
	(4854,	1859)
	(4855,	1859)
	(4856,	1859)
	(4857,	1859)
	(4858,	1859)
	(4859,	1859)
	(4860,	1860)
	(4861,	1861)
	(4862,	1862)
	(4863,	1863)
	(4864,	1863)
	(4865,	1865)
	(4866,	1865)
	(4867,	1865)
	(4868,	1865)
	(4869,	1866)
	(4870,	1866)
	(4871,	1866)
	(4872,	1866)
	(4873,	1867)
	(4874,	1872)
	(4875,	1875)
	(4876,	1875)
	(4877,	1875)
	(4878,	1876)
	(4879,	1876)
	(4880,	1876)
	(4881,	1876)
	(4882,	1876)
	(4883,	1877)
	(4884,	1879)
	(4885,	1881)
	(4886,	1881)
	(4887,	1882)
	(4888,	1882)
	(4889,	1883)
	(4890,	1884)
	(4891,	1884)
	(4892,	1884)
	(4893,	1884)
	(4894,	1885)
	(4895,	1885)
	(4896,	1885)
	(4897,	1885)
	(4898,	1886)
	(4899,	1886)
	(4900,	1886)
	(4901,	1886)
	(4902,	1886)
	(4903,	1887)
	(4904,	1890)
	(4905,	1890)
	(4906,	1890)
	(4907,	1890)
	(4908,	1890)
	(4909,	1890)
	(4910,	1890)
	(4911,	1890)
	(4912,	1891)
	(4913,	1892)
	(4914,	1893)
	(4915,	1894)
	(4916,	1895)
	(4917,	1895)
	(4918,	1895)
	(4919,	1895)
	(4920,	1895)
	(4921,	1897)
	(4922,	1897)
	(4923,	1898)
	(4924,	1899)
	(4925,	1901)
	(4926,	1903)
	(4927,	1903)
	(4928,	1903)
	(4929,	1903)
	(4930,	1903)
	(4931,	1905)
	(4932,	1905)
	(4933,	1906)
	(4934,	1906)
	(4935,	1906)
	(4936,	1905)
	(4937,	1904)
	(4938,	1905)
	(4939,	1905)
	(4940,	1904)
	(4941,	1904)
	(4942,	1903)
	(4943,	1902)
	(4944,	1901)
	(4945,	1900)
	(4946,	1900)
	(4947,	1899)
	(4948,	1898)
	(4949,	1899)
	(4950,	1898)
	(4951,	1897)
	(4952,	1899)
	(4953,	1898)
	(4954,	1897)
	(4955,	1896)
	(4956,	1895)
	(4957,	1895)
	(4958,	1895)
	(4959,	1894)
	(4960,	1895)
	(4961,	1894)
	(4962,	1893)
	(4963,	1895)
	(4964,	1895)
	(4965,	1894)
	(4966,	1893)
	(4967,	1892)
	(4968,	1891)
	(4969,	1893)
	(4970,	1893)
	(4971,	1894)
	(4972,	1895)
	(4973,	1894)
	(4974,	1893)
	(4975,	1892)
	(4976,	1892)
	(4977,	1891)
	(4978,	1890)
	(4979,	1889)
	(4980,	1888)
	(4981,	1887)
	(4982,	1888)
	(4983,	1887)
	(4984,	1886)
	(4985,	1885)
	(4986,	1884)
	(4987,	1883)
	(4988,	1882)
	(4989,	1882)
	(4990,	1882)
	(4991,	1884)
	(4992,	1886)
	(4993,	1886)
	(4994,	1885)
	(4995,	1884)
	(4996,	1886)
	(4997,	1886)
	(4998,	1885)
	(4999,	1884)
	(5000,	1884)
	(5001,	1883)
	(5002,	1882)
	(5003,	1881)
	(5004,	1880)
	(5005,	1883)
	(5006,	1882)
	(5007,	1882)
	(5008,	1881)
	(5009,	1880)
	(5010,	1880)
	(5011,	1880)
	(5012,	1879)
	(5013,	1878)
	(5014,	1878)
	(5015,	1878)
	(5016,	1884)
	(5017,	1883)
	(5018,	1882)
	(5019,	1881)
	(5020,	1881)
	(5021,	1880)
	(5022,	1882)
	(5023,	1882)
	(5024,	1881)
	(5025,	1882)
	(5026,	1881)
	(5027,	1880)
	(5028,	1881)
	(5029,	1881)
	(5030,	1880)
	(5031,	1879)
	(5032,	1879)
	(5033,	1878)
	(5034,	1878)
	(5035,	1877)
	(5036,	1877)
	(5037,	1876)
	(5038,	1875)
	(5039,	1874)
	(5040,	1873)
	(5041,	1873)
	(5042,	1872)
	(5043,	1872)
	(5044,	1871)
	(5045,	1870)
	(5046,	1870)
	(5047,	1869)
	(5048,	1868)
	(5049,	1867)
	(5050,	1870)
	(5051,	1869)
	(5052,	1872)
	(5053,	1873)
	(5054,	1872)
	(5055,	1871)
	(5056,	1870)
	(5057,	1869)
	(5058,	1868)
	(5059,	1869)
	(5060,	1869)
	(5061,	1868)
	(5062,	1868)
	(5063,	1867)
	(5064,	1866)
	(5065,	1868)
	(5066,	1867)
	(5067,	1867)
	(5068,	1866)
	(5069,	1865)
	(5070,	1864)
	(5071,	1864)
	(5072,	1863)
	(5073,	1863)
	(5074,	1862)
	(5075,	1861)
	(5076,	1860)
	(5077,	1861)
	(5078,	1860)
	(5079,	1859)
	(5080,	1858)
	(5081,	1858)
	(5082,	1858)
	(5083,	1857)
	(5084,	1856)
	(5085,	1856)
	(5086,	1856)
	(5087,	1855)
	(5088,	1854)
	(5089,	1853)
	(5090,	1852)
	(5091,	1851)
	(5092,	1850)
	(5093,	1849)
	(5094,	1850)
	(5095,	1849)
	(5096,	1851)
	(5097,	1851)
	(5098,	1850)
	(5099,	1849)
	(5100,	1849)
	(5110,	1842)
	(5120,	1836)
	(5130,	1829)
	(5140,	1826)
	(5150,	1818)
	(5160,	1812)
	(5170,	1809)
	(5180,	1799)
	(5190,	1795)
	(5200,	1796)
	(5210,	1791)
	(5220,	1788)
	(5230,	1786)
	(5240,	1783)
	(5250,	1780)
	(5260,	1775)
	(5270,	1770)
	(5280,	1769)
	(5290,	1760)
	(5300,	1757)
	(5310,	1754)
	(5320,	1752)
	(5330,	1744)
	(5340,	1737)
	(5350,	1731)
	(5360,	1726)
	(5370,	1717)
	(5380,	1713)
	(5390,	1712)
	(5400,	1707)
	(5410,	1702)
	(5420,	1701)
	(5430,	1698)
	(5440,	1694)
	(5450,	1687)
	(5460,	1683)
	(5470,	1678)
	(5480,	1672)
	(5490,	1669)
	(5500,	1669)
	(5510,	1663)
	(5520,	1657)
	(5530,	1652)
	(5540,	1647)
	(5550,	1641)
	(5560,	1642)
	(5570,	1637)
	(5580,	1635)
	(5590,	1630)
	(5600,	1625)
	(5610,	1619)
	(5620,	1612)
	(5630,	1608)
	(5640,	1607)
	(5650,	1600)
	(5660,	1595)
	(5670,	1592)
	(5680,	1587)
	(5690,	1583)
	(5700,	1584)
	(5710,	1582)
	(5720,	1573)
	(5730,	1566)
	(5740,	1559)
	(5750,	1557)
	(5760,	1553)
	(5770,	1547)
	(5780,	1544)
	(5790,	1547)
	(5800,	1543)
	(5810,	1539)
	(5820,	1530)
	(5830,	1534)
	(5840,	1525)
	(5850,	1521)
	(5860,	1514)
	(5870,	1512)
	(5880,	1507)
	(5890,	1501)
	(5900,	1498)
	(5910,	1493)
	(5920,	1490)
	(5930,	1484)
	(5940,	1474)
	(5950,	1472)
	(5960,	1466)
	(5970,	1459)
	(5980,	1449)
	(5990,	1447)
	(6000,	1442)
	(6010,	1438)
	(6020,	1431)
	(6030,	1426)
	(6040,	1422)
	(6050,	1418)
	(6060,	1411)
	(6070,	1405)
	(6080,	1397)
	(6090,	1389)
	(6100,	1382)
	(6110,	1376)
	(6120,	1370)
	(6130,	1366)
	(6140,	1358)
	(6150,	1353)
	(6160,	1353)
	(6170,	1346)
	(6180,	1341)
	(6190,	1334)
	(6200,	1328)
	(6210,	1331)
	(6220,	1325)
	(6230,	1321)
	(6240,	1316)
	(6250,	1314)
	(6260,	1314)
	(6270,	1307)
	(6280,	1301)
	(6290,	1296)
	(6300,	1289)
	(6310,	1280)
	(6320,	1276)
	(6330,	1270)
	(6340,	1264)
	(6350,	1255)
	(6360,	1246)
	(6370,	1240)
	(6380,	1232)
	(6390,	1224)
	(6400,	1220)
	(6410,	1212)
	(6420,	1205)
	(6430,	1199)
	(6440,	1197)
	(6450,	1193)
	(6460,	1191)
	(6470,	1188)
	(6480,	1181)
	(6490,	1177)
	(6500,	1170)
	(6510,	1167)
	(6520,	1163)
	(6530,	1157)
	(6540,	1153)
	(6550,	1149)
	(6560,	1142)
	(6570,	1141)
	(6580,	1134)
	(6590,	1130)
	(6600,	1125)
	(6610,	1125)
	(6620,	1121)
	(6630,	1116)
	(6640,	1108)
	(6650,	1104)
	(6660,	1099)
	(6670,	1097)
	(6680,	1091)
	(6690,	1094)
	(6700,	1089)
	(6710,	1084)
	(6720,	1078)
	(6730,	1076)
	(6740,	1069)
	(6750,	1067)
	(6760,	1059)
	(6770,	1057)
	(6780,	1058)
	(6790,	1055)
	(6800,	1049)
	(6810,	1044)
	(6820,	1040)
	(6830,	1034)
	(6840,	1025)
	(6850,	1021)
	(6860,	1014)
	(6870,	1008)
	(6880,	1005)
	(6890,	1000)
	(6900,	999)
	(6910,	1004)
	(6920,	1003)
	(6930,	997)
	(6940,	989)
	(6950,	986)
	(6960,	982)
	(6970,	977)
	(6980,	971)
	(6990,	964)
	(7000,	960)
	(7010,	955)
	(7020,	950)
	(7030,	941)
	(7040,	934)
	(7050,	930)
	(7060,	925)
	(7070,	920)
	(7080,	918)
	(7090,	912)
	(7100,	910)
	(7110,	901)
	(7120,	898)
	(7130,	894)
	(7140,	888)
	(7150,	881)
	(7160,	878)
	(7170,	870)
	(7180,	862)
	(7190,	854)
	(7200,	849)
	(7210,	844)
	(7220,	838)
	(7230,	835)
	(7240,	827)
	(7250,	824)
	(7260,	821)
	(7270,	817)
	(7280,	813)
	(7290,	806)
	(7300,	800)
	(7310,	801)
	(7320,	795)
	(7330,	788)
	(7340,	784)
	(7350,	779)
	(7360,	773)
	(7370,	767)
	(7380,	762)
	(7390,	754)
	(7400,	748)
	(7410,	743)
	(7420,	739)
	(7430,	730)
	(7440,	721)
	(7450,	715)
	(7460,	708)
	(7470,	703)
	(7480,	694)
	(7490,	691)
	(7500,	689)
	(7510,	684)
	(7520,	680)
	(7530,	679)
	(7540,	675)
	(7550,	675)
	(7560,	668)
	(7570,	668)
	(7580,	663)
	(7590,	659)
	(7600,	654)
	(7610,	651)
	(7620,	644)
	(7630,	644)
	(7640,	640)
	(7650,	633)
	(7660,	627)
	(7670,	618)
	(7680,	608)
	(7690,	602)
	(7700,	597)
	(7710,	592)
	(7720,	589)
	(7730,	585)
	(7740,	582)
	(7750,	574)
	(7760,	570)
	(7770,	562)
	(7780,	554)
	(7790,	547)
	(7800,	541)
	(7810,	533)
	(7820,	531)
	(7830,	526)
	(7840,	523)
	(7850,	517)
	(7860,	512)
	(7870,	504)
	(7880,	500)
	(7890,	496)
	(7900,	494)
	(7910,	486)
	(7920,	480)
	(7930,	474)
	(7940,	468)
	(7950,	465)
	(7960,	458)
	(7970,	451)
	(7980,	446)
	(7990,	437)
	(8000,	430)
	(8010,	423)
	(8020,	417)
	(8030,	414)
	(8040,	409)
	(8050,	411)
	(8060,	403)
	(8070,	398)
	(8080,	389)
	(8090,	380)
	(8100,	378)
	(8110,	370)
	(8120,	363)
	(8130,	360)
	(8140,	351)
	(8150,	344)
	(8160,	345)
	(8170,	338)
	(8180,	330)
	(8190,	323)
	(8200,	319)
	(8210,	315)
	(8220,	315)
	(8230,	313)
	(8240,	305)
	(8250,	299)
	(8260,	293)
	(8270,	288)
	(8280,	282)
	(8290,	273)
	(8300,	267)
	(8310,	263)
	(8320,	262)
	(8330,	257)
	(8340,	259)
	(8350,	255)
	(8360,	249)
	(8370,	242)
	(8380,	245)
	(8390,	241)
	(8400,	234)
	(8410,	229)
	(8420,	222)
	(8430,	218)
	(8440,	214)
	(8450,	208)
	(8460,	203)
	(8470,	196)
	(8480,	190)
	(8490,	186)
	(8500,	178)
	(8510,	174)
	(8520,	170)
	(8530,	167)
	(8540,	166)
	(8550,	161)
	(8560,	158)
	(8570,	153)
	(8580,	147)
	(8590,	144)
	(8600,	139)
	(8601,	139)
	(8602,	140)
	(8603,	141)
	(8604,	141)
	(8605,	141)
	(8606,	140)
	(8607,	139)
	(8608,	138)
	(8609,	137)
	(8610,	138)
	(8611,	138)
	(8612,	138)
	(8613,	137)
	(8614,	136)
	(8615,	135)
	(8616,	137)
	(8617,	136)
	(8618,	135)
	(8619,	134)
	(8620,	133)
	(8621,	132)
	(8622,	131)
	(8623,	130)
	(8624,	130)
	(8625,	130)
	(8626,	129)
	(8627,	129)
	(8628,	130)
	(8629,	129)
	(8630,	128)
	(8631,	127)
	(8632,	129)
	(8633,	129)
	(8634,	128)
	(8635,	127)
	(8636,	126)
	(8637,	125)
	(8638,	124)
	(8639,	123)
	(8640,	123)
	(8641,	122)
	(8642,	121)
	(8643,	120)
	(8644,	119)
	(8645,	118)
	(8646,	117)
	(8647,	118)
	(8648,	117)
	(8649,	116)
	(8650,	115)
	(8651,	115)
	(8652,	114)
	(8653,	114)
	(8654,	113)
	(8655,	112)
	(8656,	111)
	(8657,	110)
	(8658,	112)
	(8659,	111)
	(8660,	111)
	(8661,	110)
	(8662,	111)
	(8663,	111)
	(8664,	110)
	(8665,	112)
	(8666,	112)
	(8667,	111)
	(8668,	110)
	(8669,	109)
	(8670,	108)
	(8671,	107)
	(8672,	108)
	(8673,	107)
	(8674,	109)
	(8675,	108)
	(8676,	107)
	(8677,	106)
	(8678,	105)
	(8679,	104)
	(8680,	103)
	(8681,	102)
	(8682,	101)
	(8683,	101)
	(8684,	100)
	(8685,	101)
	(8686,	101)
	(8687,	100)
	(8688,	99)
	(8689,	98)
	(8690,	98)
	(8691,	97)
	(8692,	96)
	(8693,	95)
	(8694,	94)
	(8695,	93)
	(8696,	92)
	(8697,	91)
	(8698,	90)
	(8699,	89)
	(8700,	89)
	(8701,	88)
	(8702,	87)
	(8703,	86)
	(8704,	85)
	(8705,	88)
	(8706,	87)
	(8707,	87)
	(8708,	86)
	(8709,	85)
	(8710,	84)
	(8711,	83)
	(8712,	82)
	(8713,	81)
	(8714,	80)
	(8715,	80)
	(8716,	79)
	(8717,	79)
	(8718,	78)
	(8719,	77)
	(8720,	76)
	(8721,	76)
	(8722,	75)
	(8723,	75)
	(8724,	76)
	(8725,	77)
	(8726,	76)
	(8727,	75)
	(8728,	74)
	(8729,	73)
	(8730,	72)
	(8731,	71)
	(8732,	72)
	(8733,	72)
	(8734,	71)
	(8735,	71)
	(8736,	70)
	(8737,	69)
	(8738,	68)
	(8739,	67)
	(8740,	66)
	(8741,	65)
	(8742,	65)
	(8743,	66)
	(8744,	65)
	(8745,	64)
	(8746,	63)
	(8747,	62)
	(8748,	63)
	(8749,	62)
	(8750,	61)
	(8751,	60)
	(8752,	59)
	(8753,	59)
	(8754,	58)
	(8755,	58)
	(8756,	59)
	(8757,	58)
	(8758,	58)
	(8759,	57)
	(8760,	56)
	(8761,	55)
	(8762,	54)
	(8763,	56)
	(8764,	55)
	(8765,	54)
	(8766,	53)
	(8767,	52)
	(8768,	51)
	(8769,	50)
	(8770,	49)
	(8771,	48)
	(8772,	47)
	(8773,	46)
	(8774,	45)
	(8775,	44)
	(8776,	43)
	(8777,	42)
	(8778,	41)
	(8779,	40)
	(8780,	39)
	(8781,	41)
	(8782,	40)
	(8783,	39)
	(8784,	38)
	(8785,	37)
	(8786,	39)
	(8787,	44)
	(8788,	43)
	(8789,	44)
	(8790,	45)
	(8791,	44)
	(8792,	44)
	(8793,	44)
	(8794,	43)
	(8795,	49)
	(8796,	51)
	(8797,	52)
	(8798,	51)
	(8799,	52)
	(8800,	51)
	(8801,	50)
	(8802,	49)
	(8803,	48)
	(8804,	48)
	(8805,	48)
	(8806,	47)
	(8807,	46)
	(8808,	45)
	(8809,	45)
	(8810,	44)
	(8811,	46)
	(8812,	45)
	(8813,	44)
	(8814,	45)
	(8815,	45)
	(8816,	44)
	(8817,	43)
	(8818,	42)
	(8819,	41)
	(8820,	41)
	(8821,	40)
	(8822,	39)
	(8823,	38)
	(8824,	37)
	(8825,	38)
	(8826,	37)
	(8827,	37)
	(8828,	36)
	(8829,	35)
	(8830,	34)
	(8831,	35)
	(8832,	37)
	(8833,	36)
	(8834,	35)
	(8835,	34)
	(8836,	33)
	(8837,	32)
	(8838,	32)
	(8839,	31)
	(8840,	30)
	(8841,	29)
	(8842,	28)
	(8843,	27)
	(8844,	26)
	(8845,	25)
	(8846,	24)
	(8847,	23)
	(8848,	22)
	(8849,	21)
	(8850,	20)
	(8851,	19)
	(8852,	18)
	(8853,	17)
	(8854,	16)
	(8855,	16)
	(8856,	15)
	(8857,	14)
	(8858,	13)
	(8859,	13)
	(8860,	12)
	(8861,	11)
	(8862,	11)
	(8863,	11)
	(8864,	10)
	(8865,	9)
	(8866,	9)
	(8867,	9)
	(8868,	8)
	(8869,	7)
	(8870,	6)
	(8871,	5)
	(8872,	4)
	(8873,	3)
	(8874,	3)
	(8875,	4)
	(8876,	4)
	(8877,	4)
	(8878,	5)
	(8879,	5)
	(8880,	7)
	(8881,	7)
	(8882,	8)
	(8883,	10)
	(8884,	10)
	(8885,	10)
	(8886,	10)
	(8887,	10)
	(8888,	13)
	(8889,	13)
	(8890,	15)
	(8891,	17)
	(8892,	18)
	(8893,	18)
	(8894,	19)
	(8895,	19)
	(8896,	19)
	(8897,	22)
	(8898,	22)
	(8899,	22)
	(8900,	22)
	(8901,	22)
	(8902,	23)
	(8903,	23)
	(8904,	23)
	(8905,	23)
	(8906,	23)
	(8907,	23)
	(8908,	23)
	(8909,	24)
	(8910,	26)
	(8911,	26)
	(8912,	27)
	(8913,	27)
	(8914,	29)
	(8915,	31)
	(8916,	31)
	(8917,	31)
	(8918,	32)
	(8919,	32)
	(8920,	33)
	(8921,	35)
	(8922,	37)
	(8923,	37)
	(8924,	37)
	(8925,	37)
	(8926,	37)
	(8927,	38)
	(8928,	38)
	(8929,	38)
	(8930,	39)
	(8931,	41)
	(8932,	41)
	(8933,	41)
	(8934,	43)
	(8935,	43)
	(8936,	43)
	(8937,	44)
	(8938,	44)
	(8939,	44)
	(8940,	44)
	(8941,	44)
	(8942,	44)
	(8943,	44)
	(8944,	44)
	(8945,	44)
	(8946,	44)
	(8947,	44)
	(8948,	44)
	(8949,	44)
	(8950,	44)
	(8951,	44)
	(8952,	44)
	(8953,	44)
	(8954,	44)
	(8955,	44)
	(8956,	45)
	(8957,	47)
	(8958,	49)
	(8959,	49)
	(8960,	49)
	(8961,	49)
	(8962,	49)
	(8963,	49)
	(8964,	50)
	(8965,	51)
	(8966,	51)
	(8967,	51)
	(8968,	51)
	(8969,	51)
	(8970,	51)
	(8971,	54)
	(8972,	54)
	(8973,	54)
	(8974,	54)
	(8975,	54)
	(8976,	54)
	(8977,	54)
	(8978,	55)
	(8979,	56)
	(8980,	57)
	(8981,	57)
	(8982,	58)
	(8983,	58)
	(8984,	59)
	(8985,	59)
	(8986,	59)
	(8987,	59)
	(8988,	60)
	(8989,	61)
	(8990,	61)
	(8991,	61)
	(8992,	61)
	(8993,	61)
	(8994,	61)
	(8995,	62)
	(8996,	63)
	(8997,	64)
	(8998,	64)
	(8999,	64)
	(9000,	64)
	(9010,	68)
	(9020,	75)
	(9030,	81)
	(9040,	87)
	(9050,	95)
	(9060,	102)
	(9070,	103)
	(9080,	106)
	(9090,	108)
	(9100,	112)
	(9110,	118)
	(9120,	122)
	(9130,	126)
	(9140,	127)
	(9150,	132)
	(9160,	141)
	(9170,	146)
	(9180,	152)
	(9190,	154)
	(9200,	158)
	(9210,	158)
	(9220,	160)
	(9230,	166)
	(9240,	171)
	(9250,	176)
	(9260,	178)
	(9270,	181)
	(9280,	183)
	(9290,	186)
	(9300,	191)
	(9310,	197)
	(9320,	203)
	(9330,	215)
	(9340,	217)
	(9350,	221)
	(9360,	226)
	(9370,	230)
	(9380,	233)
	(9390,	237)
	(9400,	241)
	(9410,	250)
	(9420,	254)
	(9430,	260)
	(9440,	265)
	(9450,	275)
	(9460,	275)
	(9470,	277)
	(9480,	279)
	(9490,	282)
	(9500,	287)
	(9510,	292)
	(9520,	296)
	(9530,	301)
	(9540,	307)
	(9550,	309)
	(9560,	314)
	(9570,	317)
	(9580,	326)
	(9590,	333)
	(9600,	342)
	(9610,	348)
	(9620,	355)
	(9630,	362)
	(9640,	370)
	(9650,	374)
	(9660,	380)
	(9670,	390)
	(9680,	394)
	(9690,	397)
	(9700,	404)
	(9710,	414)
	(9720,	420)
	(9730,	427)
	(9740,	432)
	(9750,	434)
	(9760,	437)
	(9770,	439)
	(9780,	443)
	(9790,	446)
	(9800,	450)
	(9810,	451)
	(9820,	455)
	(9830,	457)
	(9840,	462)
	(9850,	468)
	(9860,	477)
	(9870,	483)
	(9880,	487)
	(9890,	501)
	(9900,	503)
	(9910,	504)
	(9920,	507)
	(9930,	511)
	(9940,	516)
	(9950,	518)
	(9960,	525)
	(9970,	533)
	(9980,	539)
	(9990,	541)
	(10000,	549)
};
\addplot[color=gray] plot coordinates {
	(0,	538)
	(10,	532)
	(20,	524)
	(30,	525)
	(40,	518)
	(50,	514)
	(60,	509)
	(70,	508)
	(80,	505)
	(90,	496)
	(100,	492)
	(110,	487)
	(120,	482)
	(130,	483)
	(140,	478)
	(150,	472)
	(160,	470)
	(170,	464)
	(180,	455)
	(190,	448)
	(200,	442)
	(210,	435)
	(220,	430)
	(230,	429)
	(240,	423)
	(250,	422)
	(260,	416)
	(270,	409)
	(280,	407)
	(290,	401)
	(300,	396)
	(310,	393)
	(320,	387)
	(330,	383)
	(340,	374)
	(350,	372)
	(360,	366)
	(370,	360)
	(380,	356)
	(390,	356)
	(400,	350)
	(410,	351)
	(420,	348)
	(430,	340)
	(440,	332)
	(450,	329)
	(460,	327)
	(470,	325)
	(480,	318)
	(490,	308)
	(500,	302)
	(510,	295)
	(520,	287)
	(530,	280)
	(540,	273)
	(550,	269)
	(560,	267)
	(570,	261)
	(580,	254)
	(590,	248)
	(600,	243)
	(610,	237)
	(620,	228)
	(630,	224)
	(640,	216)
	(650,	213)
	(660,	204)
	(670,	197)
	(680,	189)
	(690,	186)
	(700,	182)
	(710,	175)
	(720,	170)
	(730,	167)
	(740,	161)
	(750,	166)
	(760,	156)
	(770,	148)
	(780,	145)
	(790,	147)
	(800,	141)
	(801,	141)
	(802,	140)
	(803,	140)
	(804,	139)
	(805,	139)
	(806,	139)
	(807,	138)
	(808,	137)
	(809,	138)
	(810,	138)
	(811,	137)
	(812,	136)
	(813,	135)
	(814,	134)
	(815,	133)
	(816,	133)
	(817,	132)
	(818,	131)
	(819,	130)
	(820,	130)
	(821,	133)
	(822,	132)
	(823,	131)
	(824,	133)
	(825,	134)
	(826,	133)
	(827,	132)
	(828,	133)
	(829,	132)
	(830,	132)
	(831,	131)
	(832,	130)
	(833,	131)
	(834,	131)
	(835,	131)
	(836,	130)
	(837,	129)
	(838,	128)
	(839,	127)
	(840,	126)
	(841,	127)
	(842,	126)
	(843,	125)
	(844,	124)
	(845,	123)
	(846,	123)
	(847,	122)
	(848,	122)
	(849,	121)
	(850,	124)
	(851,	123)
	(852,	122)
	(853,	121)
	(854,	120)
	(855,	119)
	(856,	118)
	(857,	117)
	(858,	116)
	(859,	115)
	(860,	114)
	(861,	113)
	(862,	112)
	(863,	112)
	(864,	111)
	(865,	110)
	(866,	109)
	(867,	108)
	(868,	107)
	(869,	106)
	(870,	106)
	(871,	105)
	(872,	104)
	(873,	104)
	(874,	103)
	(875,	102)
	(876,	101)
	(877,	100)
	(878,	99)
	(879,	100)
	(880,	101)
	(881,	101)
	(882,	100)
	(883,	99)
	(884,	98)
	(885,	98)
	(886,	99)
	(887,	98)
	(888,	98)
	(889,	97)
	(890,	97)
	(891,	96)
	(892,	95)
	(893,	95)
	(894,	94)
	(895,	93)
	(896,	92)
	(897,	97)
	(898,	96)
	(899,	97)
	(900,	96)
	(901,	96)
	(902,	95)
	(903,	95)
	(904,	94)
	(905,	93)
	(906,	94)
	(907,	93)
	(908,	93)
	(909,	92)
	(910,	91)
	(911,	90)
	(912,	89)
	(913,	88)
	(914,	87)
	(915,	86)
	(916,	85)
	(917,	84)
	(918,	83)
	(919,	82)
	(920,	82)
	(921,	81)
	(922,	80)
	(923,	79)
	(924,	78)
	(925,	77)
	(926,	76)
	(927,	76)
	(928,	75)
	(929,	75)
	(930,	74)
	(931,	73)
	(932,	72)
	(933,	71)
	(934,	70)
	(935,	69)
	(936,	68)
	(937,	67)
	(938,	66)
	(939,	65)
	(940,	64)
	(941,	63)
	(942,	62)
	(943,	62)
	(944,	61)
	(945,	60)
	(946,	60)
	(947,	61)
	(948,	60)
	(949,	59)
	(950,	58)
	(951,	57)
	(952,	57)
	(953,	56)
	(954,	55)
	(955,	54)
	(956,	53)
	(957,	55)
	(958,	54)
	(959,	53)
	(960,	53)
	(961,	52)
	(962,	51)
	(963,	50)
	(964,	49)
	(965,	48)
	(966,	47)
	(967,	46)
	(968,	45)
	(969,	44)
	(970,	45)
	(971,	45)
	(972,	44)
	(973,	43)
	(974,	42)
	(975,	42)
	(976,	41)
	(977,	40)
	(978,	40)
	(979,	39)
	(980,	38)
	(981,	37)
	(982,	37)
	(983,	36)
	(984,	35)
	(985,	36)
	(986,	39)
	(987,	40)
	(988,	39)
	(989,	38)
	(990,	37)
	(991,	38)
	(992,	37)
	(993,	36)
	(994,	35)
	(995,	34)
	(996,	33)
	(997,	32)
	(998,	31)
	(999,	30)
	(1000,	29)
	(1001,	28)
	(1002,	27)
	(1003,	27)
	(1004,	26)
	(1005,	25)
	(1006,	24)
	(1007,	24)
	(1008,	23)
	(1009,	23)
	(1010,	23)
	(1011,	23)
	(1012,	22)
	(1013,	22)
	(1014,	21)
	(1015,	21)
	(1016,	20)
	(1017,	20)
	(1018,	19)
	(1019,	18)
	(1020,	17)
	(1021,	16)
	(1022,	15)
	(1023,	14)
	(1024,	13)
	(1025,	12)
	(1026,	11)
	(1027,	10)
	(1028,	10)
	(1029,	11)
	(1030,	11)
	(1031,	12)
	(1032,	11)
	(1033,	10)
	(1034,	9)
	(1035,	9)
	(1036,	8)
	(1037,	8)
	(1038,	7)
	(1039,	6)
	(1040,	5)
	(1041,	5)
	(1042,	4)
	(1043,	3)
	(1044,	2)
	(1045,	1)
	(1046,	0)
	(1047,	2)
	(1048,	2)
	(1049,	2)
	(1050,	2)
	(1051,	2)
	(1052,	3)
	(1053,	4)
	(1054,	5)
	(1055,	6)
	(1056,	7)
	(1057,	7)
	(1058,	7)
	(1059,	7)
	(1060,	9)
	(1061,	11)
	(1062,	11)
	(1063,	11)
	(1064,	11)
	(1065,	12)
	(1066,	12)
	(1067,	13)
	(1068,	13)
	(1069,	13)
	(1070,	13)
	(1071,	13)
	(1072,	13)
	(1073,	13)
	(1074,	13)
	(1075,	15)
	(1076,	15)
	(1077,	15)
	(1078,	16)
	(1079,	16)
	(1080,	16)
	(1081,	17)
	(1082,	17)
	(1083,	17)
	(1084,	17)
	(1085,	17)
	(1086,	19)
	(1087,	19)
	(1088,	19)
	(1089,	21)
	(1090,	21)
	(1091,	26)
	(1092,	27)
	(1093,	28)
	(1094,	28)
	(1095,	30)
	(1096,	31)
	(1097,	31)
	(1098,	31)
	(1099,	32)
	(1100,	32)
	(1101,	32)
	(1102,	32)
	(1103,	32)
	(1104,	32)
	(1105,	32)
	(1106,	32)
	(1107,	33)
	(1108,	34)
	(1109,	34)
	(1110,	34)
	(1111,	36)
	(1112,	37)
	(1113,	38)
	(1114,	38)
	(1115,	39)
	(1116,	39)
	(1117,	41)
	(1118,	41)
	(1119,	42)
	(1120,	44)
	(1121,	44)
	(1122,	45)
	(1123,	46)
	(1124,	46)
	(1125,	46)
	(1126,	46)
	(1127,	46)
	(1128,	48)
	(1129,	48)
	(1130,	48)
	(1131,	49)
	(1132,	49)
	(1133,	49)
	(1134,	49)
	(1135,	52)
	(1136,	52)
	(1137,	52)
	(1138,	52)
	(1139,	54)
	(1140,	55)
	(1141,	55)
	(1142,	55)
	(1143,	56)
	(1144,	56)
	(1145,	58)
	(1146,	58)
	(1147,	59)
	(1148,	60)
	(1149,	60)
	(1150,	61)
	(1151,	61)
	(1152,	61)
	(1153,	61)
	(1154,	61)
	(1155,	61)
	(1156,	62)
	(1157,	63)
	(1158,	63)
	(1159,	63)
	(1160,	63)
	(1161,	64)
	(1162,	66)
	(1163,	66)
	(1164,	67)
	(1165,	67)
	(1166,	67)
	(1167,	68)
	(1168,	70)
	(1169,	72)
	(1170,	72)
	(1171,	73)
	(1172,	73)
	(1173,	73)
	(1174,	75)
	(1175,	76)
	(1176,	76)
	(1177,	79)
	(1178,	79)
	(1179,	82)
	(1180,	83)
	(1181,	84)
	(1182,	84)
	(1183,	84)
	(1184,	84)
	(1185,	84)
	(1186,	84)
	(1187,	84)
	(1188,	85)
	(1189,	85)
	(1190,	85)
	(1191,	85)
	(1192,	86)
	(1193,	86)
	(1194,	86)
	(1195,	86)
	(1196,	88)
	(1197,	89)
	(1198,	91)
	(1199,	91)
	(1200,	91)
	(1210,	97)
	(1220,	100)
	(1230,	105)
	(1240,	109)
	(1250,	112)
	(1260,	115)
	(1270,	122)
	(1280,	125)
	(1290,	130)
	(1300,	133)
	(1310,	135)
	(1320,	139)
	(1330,	147)
	(1340,	150)
	(1350,	159)
	(1360,	164)
	(1370,	176)
	(1380,	182)
	(1390,	189)
	(1400,	205)
	(1410,	207)
	(1420,	209)
	(1430,	220)
	(1440,	231)
	(1450,	234)
	(1460,	235)
	(1470,	240)
	(1480,	242)
	(1490,	245)
	(1500,	258)
	(1510,	268)
	(1520,	270)
	(1530,	275)
	(1540,	278)
	(1550,	284)
	(1560,	293)
	(1570,	299)
	(1580,	303)
	(1590,	309)
	(1600,	313)
	(1610,	319)
	(1620,	323)
	(1630,	329)
	(1640,	338)
	(1650,	341)
	(1660,	347)
	(1670,	348)
	(1680,	352)
	(1690,	356)
	(1700,	362)
	(1710,	366)
	(1720,	371)
	(1730,	373)
	(1740,	378)
	(1750,	386)
	(1760,	389)
	(1770,	396)
	(1780,	399)
	(1790,	404)
	(1800,	410)
	(1810,	415)
	(1820,	417)
	(1830,	419)
	(1840,	423)
	(1850,	428)
	(1860,	431)
	(1870,	434)
	(1880,	439)
	(1890,	443)
	(1900,	452)
	(1910,	454)
	(1920,	457)
	(1930,	462)
	(1940,	468)
	(1950,	472)
	(1960,	477)
	(1970,	481)
	(1980,	485)
	(1990,	485)
	(2000,	490)
	(2010,	499)
	(2020,	501)
	(2030,	506)
	(2040,	515)
	(2050,	518)
	(2060,	521)
	(2070,	523)
	(2080,	526)
	(2090,	529)
	(2100,	535)
	(2110,	542)
	(2120,	552)
	(2130,	556)
	(2140,	570)
	(2150,	578)
	(2160,	582)
	(2170,	586)
	(2180,	589)
	(2190,	595)
	(2200,	600)
	(2210,	603)
	(2220,	607)
	(2230,	610)
	(2240,	613)
	(2250,	621)
	(2260,	623)
	(2270,	631)
	(2280,	635)
	(2290,	637)
	(2300,	641)
	(2310,	654)
	(2320,	662)
	(2330,	664)
	(2340,	668)
	(2350,	671)
	(2360,	673)
	(2370,	677)
	(2380,	679)
	(2390,	685)
	(2400,	688)
	(2410,	693)
	(2420,	700)
	(2430,	704)
	(2440,	709)
	(2450,	712)
	(2460,	717)
	(2470,	719)
	(2480,	726)
	(2490,	732)
	(2500,	737)
	(2510,	749)
	(2520,	754)
	(2530,	758)
	(2540,	758)
	(2550,	762)
	(2560,	769)
	(2570,	773)
	(2580,	779)
	(2590,	783)
	(2600,	783)
	(2610,	785)
	(2620,	789)
	(2630,	796)
	(2640,	803)
	(2650,	814)
	(2660,	815)
	(2670,	820)
	(2680,	823)
	(2690,	832)
	(2700,	836)
	(2710,	844)
	(2720,	848)
	(2730,	854)
	(2740,	858)
	(2750,	864)
	(2760,	866)
	(2770,	870)
	(2780,	872)
	(2790,	873)
	(2800,	873)
	(2810,	877)
	(2820,	884)
	(2830,	893)
	(2840,	904)
	(2850,	905)
	(2860,	907)
	(2870,	911)
	(2880,	916)
	(2890,	923)
	(2900,	932)
	(2910,	936)
	(2920,	940)
	(2930,	948)
	(2940,	955)
	(2950,	960)
	(2960,	965)
	(2970,	966)
	(2980,	973)
	(2990,	975)
	(3000,	984)
	(3010,	990)
	(3020,	999)
	(3030,	1004)
	(3040,	1005)
	(3050,	1012)
	(3060,	1016)
	(3070,	1021)
	(3080,	1022)
	(3090,	1025)
	(3100,	1029)
	(3110,	1035)
	(3120,	1040)
	(3130,	1044)
	(3140,	1048)
	(3150,	1052)
	(3160,	1056)
	(3170,	1062)
	(3180,	1062)
	(3190,	1066)
	(3200,	1071)
	(3210,	1075)
	(3220,	1082)
	(3230,	1083)
	(3240,	1091)
	(3250,	1102)
	(3260,	1112)
	(3270,	1116)
	(3280,	1120)
	(3290,	1122)
	(3300,	1125)
	(3310,	1137)
	(3320,	1138)
	(3330,	1142)
	(3340,	1144)
	(3350,	1151)
	(3360,	1156)
	(3370,	1160)
	(3380,	1166)
	(3390,	1175)
	(3400,	1181)
	(3410,	1189)
	(3420,	1193)
	(3430,	1201)
	(3440,	1205)
	(3450,	1208)
	(3460,	1211)
	(3470,	1218)
	(3480,	1229)
	(3490,	1230)
	(3500,	1231)
	(3510,	1236)
	(3520,	1239)
	(3530,	1244)
	(3540,	1250)
	(3550,	1258)
	(3560,	1264)
	(3570,	1270)
	(3580,	1277)
	(3590,	1287)
	(3600,	1293)
	(3610,	1299)
	(3620,	1303)
	(3630,	1307)
	(3640,	1310)
	(3650,	1316)
	(3660,	1320)
	(3670,	1325)
	(3680,	1332)
	(3690,	1338)
	(3700,	1351)
	(3710,	1354)
	(3720,	1361)
	(3730,	1362)
	(3740,	1365)
	(3750,	1374)
	(3760,	1377)
	(3770,	1381)
	(3780,	1389)
	(3790,	1391)
	(3800,	1393)
	(3810,	1403)
	(3820,	1409)
	(3830,	1423)
	(3840,	1427)
	(3850,	1432)
	(3860,	1435)
	(3870,	1442)
	(3880,	1443)
	(3890,	1452)
	(3900,	1459)
	(3910,	1465)
	(3920,	1472)
	(3930,	1477)
	(3940,	1481)
	(3950,	1490)
	(3960,	1493)
	(3970,	1499)
	(3980,	1502)
	(3990,	1510)
	(4000,	1512)
	(4010,	1521)
	(4020,	1526)
	(4030,	1536)
	(4040,	1543)
	(4050,	1546)
	(4060,	1549)
	(4070,	1554)
	(4080,	1559)
	(4090,	1562)
	(4100,	1569)
	(4110,	1575)
	(4120,	1586)
	(4130,	1591)
	(4140,	1594)
	(4150,	1602)
	(4160,	1607)
	(4170,	1610)
	(4180,	1613)
	(4190,	1618)
	(4200,	1629)
	(4210,	1632)
	(4220,	1637)
	(4230,	1642)
	(4240,	1647)
	(4250,	1650)
	(4260,	1654)
	(4270,	1659)
	(4280,	1662)
	(4290,	1665)
	(4300,	1668)
	(4310,	1674)
	(4320,	1676)
	(4330,	1680)
	(4340,	1685)
	(4350,	1688)
	(4360,	1689)
	(4370,	1695)
	(4380,	1700)
	(4390,	1705)
	(4400,	1709)
	(4410,	1718)
	(4420,	1722)
	(4430,	1726)
	(4440,	1734)
	(4450,	1737)
	(4460,	1739)
	(4470,	1745)
	(4480,	1750)
	(4490,	1752)
	(4500,	1753)
	(4510,	1756)
	(4520,	1762)
	(4530,	1767)
	(4540,	1772)
	(4550,	1774)
	(4560,	1774)
	(4570,	1780)
	(4580,	1786)
	(4590,	1789)
	(4600,	1794)
	(4610,	1796)
	(4620,	1802)
	(4630,	1804)
	(4640,	1806)
	(4650,	1809)
	(4660,	1813)
	(4670,	1813)
	(4680,	1816)
	(4690,	1821)
	(4700,	1829)
	(4701,	1829)
	(4702,	1829)
	(4703,	1830)
	(4704,	1831)
	(4705,	1832)
	(4706,	1832)
	(4707,	1832)
	(4708,	1833)
	(4709,	1833)
	(4710,	1834)
	(4711,	1834)
	(4712,	1834)
	(4713,	1834)
	(4714,	1835)
	(4715,	1835)
	(4716,	1836)
	(4717,	1836)
	(4718,	1836)
	(4719,	1836)
	(4720,	1836)
	(4721,	1836)
	(4722,	1836)
	(4723,	1840)
	(4724,	1841)
	(4725,	1841)
	(4726,	1841)
	(4727,	1841)
	(4728,	1842)
	(4729,	1845)
	(4730,	1845)
	(4731,	1845)
	(4732,	1846)
	(4733,	1846)
	(4734,	1851)
	(4735,	1851)
	(4736,	1851)
	(4737,	1852)
	(4738,	1852)
	(4739,	1853)
	(4740,	1853)
	(4741,	1853)
	(4742,	1855)
	(4743,	1856)
	(4744,	1857)
	(4745,	1857)
	(4746,	1857)
	(4747,	1857)
	(4748,	1858)
	(4749,	1858)
	(4750,	1859)
	(4751,	1859)
	(4752,	1859)
	(4753,	1860)
	(4754,	1860)
	(4755,	1860)
	(4756,	1860)
	(4757,	1860)
	(4758,	1860)
	(4759,	1860)
	(4760,	1860)
	(4761,	1860)
	(4762,	1860)
	(4763,	1861)
	(4764,	1864)
	(4765,	1865)
	(4766,	1865)
	(4767,	1867)
	(4768,	1867)
	(4769,	1867)
	(4770,	1867)
	(4771,	1867)
	(4772,	1867)
	(4773,	1867)
	(4774,	1867)
	(4775,	1870)
	(4776,	1871)
	(4777,	1871)
	(4778,	1871)
	(4779,	1871)
	(4780,	1871)
	(4781,	1871)
	(4782,	1873)
	(4783,	1873)
	(4784,	1874)
	(4785,	1874)
	(4786,	1877)
	(4787,	1878)
	(4788,	1878)
	(4789,	1878)
	(4790,	1878)
	(4791,	1878)
	(4792,	1878)
	(4793,	1878)
	(4794,	1880)
	(4795,	1880)
	(4796,	1880)
	(4797,	1882)
	(4798,	1882)
	(4799,	1882)
	(4800,	1882)
	(4801,	1882)
	(4802,	1884)
	(4803,	1884)
	(4804,	1885)
	(4805,	1885)
	(4806,	1887)
	(4807,	1887)
	(4808,	1889)
	(4809,	1889)
	(4810,	1889)
	(4811,	1890)
	(4812,	1890)
	(4813,	1890)
	(4814,	1891)
	(4815,	1892)
	(4816,	1892)
	(4817,	1893)
	(4818,	1893)
	(4819,	1893)
	(4820,	1893)
	(4821,	1894)
	(4822,	1896)
	(4823,	1899)
	(4824,	1899)
	(4825,	1900)
	(4826,	1900)
	(4827,	1902)
	(4828,	1904)
	(4829,	1904)
	(4830,	1904)
	(4831,	1907)
	(4832,	1907)
	(4833,	1908)
	(4834,	1908)
	(4835,	1908)
	(4836,	1908)
	(4837,	1908)
	(4838,	1909)
	(4839,	1912)
	(4840,	1912)
	(4841,	1913)
	(4842,	1914)
	(4843,	1914)
	(4844,	1914)
	(4845,	1914)
	(4846,	1914)
	(4847,	1914)
	(4848,	1914)
	(4849,	1914)
	(4850,	1914)
	(4851,	1914)
	(4852,	1914)
	(4853,	1914)
	(4854,	1914)
	(4855,	1914)
	(4856,	1914)
	(4857,	1914)
	(4858,	1915)
	(4859,	1915)
	(4860,	1915)
	(4861,	1915)
	(4862,	1915)
	(4863,	1916)
	(4864,	1916)
	(4865,	1916)
	(4866,	1917)
	(4867,	1917)
	(4868,	1917)
	(4869,	1917)
	(4870,	1917)
	(4871,	1917)
	(4872,	1917)
	(4873,	1917)
	(4874,	1917)
	(4875,	1917)
	(4876,	1917)
	(4877,	1917)
	(4878,	1917)
	(4879,	1917)
	(4880,	1920)
	(4881,	1920)
	(4882,	1922)
	(4883,	1922)
	(4884,	1922)
	(4885,	1923)
	(4886,	1923)
	(4887,	1923)
	(4888,	1923)
	(4889,	1923)
	(4890,	1923)
	(4891,	1923)
	(4892,	1923)
	(4893,	1923)
	(4894,	1925)
	(4895,	1926)
	(4896,	1926)
	(4897,	1926)
	(4898,	1926)
	(4899,	1926)
	(4900,	1927)
	(4901,	1927)
	(4902,	1927)
	(4903,	1927)
	(4904,	1927)
	(4905,	1929)
	(4906,	1929)
	(4907,	1930)
	(4908,	1930)
	(4909,	1930)
	(4910,	1930)
	(4911,	1930)
	(4912,	1930)
	(4913,	1930)
	(4914,	1930)
	(4915,	1930)
	(4916,	1930)
	(4917,	1930)
	(4918,	1930)
	(4919,	1931)
	(4920,	1931)
	(4921,	1931)
	(4922,	1931)
	(4923,	1931)
	(4924,	1932)
	(4925,	1932)
	(4926,	1933)
	(4927,	1933)
	(4928,	1933)
	(4929,	1934)
	(4930,	1935)
	(4931,	1935)
	(4932,	1936)
	(4933,	1936)
	(4934,	1937)
	(4935,	1937)
	(4936,	1938)
	(4937,	1937)
	(4938,	1938)
	(4939,	1937)
	(4940,	1936)
	(4941,	1935)
	(4942,	1934)
	(4943,	1934)
	(4944,	1933)
	(4945,	1932)
	(4946,	1931)
	(4947,	1930)
	(4948,	1930)
	(4949,	1929)
	(4950,	1928)
	(4951,	1927)
	(4952,	1926)
	(4953,	1925)
	(4954,	1924)
	(4955,	1923)
	(4956,	1923)
	(4957,	1923)
	(4958,	1922)
	(4959,	1922)
	(4960,	1922)
	(4961,	1921)
	(4962,	1921)
	(4963,	1920)
	(4964,	1919)
	(4965,	1918)
	(4966,	1917)
	(4967,	1917)
	(4968,	1917)
	(4969,	1917)
	(4970,	1917)
	(4971,	1916)
	(4972,	1915)
	(4973,	1914)
	(4974,	1913)
	(4975,	1912)
	(4976,	1911)
	(4977,	1912)
	(4978,	1911)
	(4979,	1910)
	(4980,	1909)
	(4981,	1908)
	(4982,	1908)
	(4983,	1907)
	(4984,	1906)
	(4985,	1905)
	(4986,	1904)
	(4987,	1903)
	(4988,	1903)
	(4989,	1903)
	(4990,	1903)
	(4991,	1902)
	(4992,	1901)
	(4993,	1900)
	(4994,	1901)
	(4995,	1900)
	(4996,	1900)
	(4997,	1900)
	(4998,	1900)
	(4999,	1899)
	(5000,	1898)
	(5001,	1897)
	(5002,	1898)
	(5003,	1898)
	(5004,	1897)
	(5005,	1896)
	(5006,	1895)
	(5007,	1894)
	(5008,	1893)
	(5009,	1893)
	(5010,	1893)
	(5011,	1895)
	(5012,	1896)
	(5013,	1895)
	(5014,	1894)
	(5015,	1893)
	(5016,	1894)
	(5017,	1893)
	(5018,	1893)
	(5019,	1892)
	(5020,	1891)
	(5021,	1892)
	(5022,	1891)
	(5023,	1893)
	(5024,	1892)
	(5025,	1891)
	(5026,	1890)
	(5027,	1889)
	(5028,	1889)
	(5029,	1888)
	(5030,	1887)
	(5031,	1886)
	(5032,	1885)
	(5033,	1885)
	(5034,	1884)
	(5035,	1884)
	(5036,	1885)
	(5037,	1884)
	(5038,	1883)
	(5039,	1883)
	(5040,	1882)
	(5041,	1882)
	(5042,	1882)
	(5043,	1882)
	(5044,	1881)
	(5045,	1880)
	(5046,	1880)
	(5047,	1880)
	(5048,	1879)
	(5049,	1879)
	(5050,	1878)
	(5051,	1879)
	(5052,	1878)
	(5053,	1877)
	(5054,	1876)
	(5055,	1876)
	(5056,	1878)
	(5057,	1877)
	(5058,	1876)
	(5059,	1875)
	(5060,	1874)
	(5061,	1873)
	(5062,	1872)
	(5063,	1871)
	(5064,	1870)
	(5065,	1870)
	(5066,	1869)
	(5067,	1869)
	(5068,	1869)
	(5069,	1869)
	(5070,	1872)
	(5071,	1871)
	(5072,	1870)
	(5073,	1869)
	(5074,	1868)
	(5075,	1867)
	(5076,	1866)
	(5077,	1867)
	(5078,	1869)
	(5079,	1868)
	(5080,	1868)
	(5081,	1867)
	(5082,	1867)
	(5083,	1867)
	(5084,	1867)
	(5085,	1867)
	(5086,	1866)
	(5087,	1866)
	(5088,	1866)
	(5089,	1865)
	(5090,	1865)
	(5091,	1864)
	(5092,	1864)
	(5093,	1863)
	(5094,	1862)
	(5095,	1861)
	(5096,	1860)
	(5097,	1862)
	(5098,	1861)
	(5099,	1861)
	(5100,	1860)
	(5110,	1858)
	(5120,	1854)
	(5130,	1849)
	(5140,	1842)
	(5150,	1833)
	(5160,	1834)
	(5170,	1829)
	(5180,	1823)
	(5190,	1821)
	(5200,	1815)
	(5210,	1814)
	(5220,	1813)
	(5230,	1814)
	(5240,	1808)
	(5250,	1802)
	(5260,	1795)
	(5270,	1791)
	(5280,	1782)
	(5290,	1777)
	(5300,	1771)
	(5310,	1765)
	(5320,	1759)
	(5330,	1753)
	(5340,	1747)
	(5350,	1751)
	(5360,	1742)
	(5370,	1734)
	(5380,	1727)
	(5390,	1722)
	(5400,	1719)
	(5410,	1711)
	(5420,	1705)
	(5430,	1701)
	(5440,	1693)
	(5450,	1690)
	(5460,	1686)
	(5470,	1680)
	(5480,	1673)
	(5490,	1668)
	(5500,	1664)
	(5510,	1661)
	(5520,	1661)
	(5530,	1655)
	(5540,	1650)
	(5550,	1646)
	(5560,	1637)
	(5570,	1638)
	(5580,	1630)
	(5590,	1625)
	(5600,	1620)
	(5610,	1611)
	(5620,	1605)
	(5630,	1601)
	(5640,	1597)
	(5650,	1590)
	(5660,	1584)
	(5670,	1579)
	(5680,	1573)
	(5690,	1565)
	(5700,	1559)
	(5710,	1558)
	(5720,	1551)
	(5730,	1546)
	(5740,	1540)
	(5750,	1536)
	(5760,	1530)
	(5770,	1523)
	(5780,	1520)
	(5790,	1512)
	(5800,	1506)
	(5810,	1498)
	(5820,	1492)
	(5830,	1487)
	(5840,	1483)
	(5850,	1477)
	(5860,	1467)
	(5870,	1460)
	(5880,	1456)
	(5890,	1448)
	(5900,	1445)
	(5910,	1438)
	(5920,	1431)
	(5930,	1423)
	(5940,	1420)
	(5950,	1416)
	(5960,	1410)
	(5970,	1403)
	(5980,	1399)
	(5990,	1396)
	(6000,	1389)
	(6010,	1389)
	(6020,	1390)
	(6030,	1383)
	(6040,	1382)
	(6050,	1377)
	(6060,	1369)
	(6070,	1366)
	(6080,	1359)
	(6090,	1353)
	(6100,	1348)
	(6110,	1344)
	(6120,	1342)
	(6130,	1337)
	(6140,	1333)
	(6150,	1330)
	(6160,	1329)
	(6170,	1325)
	(6180,	1318)
	(6190,	1311)
	(6200,	1306)
	(6210,	1298)
	(6220,	1290)
	(6230,	1283)
	(6240,	1277)
	(6250,	1272)
	(6260,	1265)
	(6270,	1261)
	(6280,	1259)
	(6290,	1250)
	(6300,	1241)
	(6310,	1238)
	(6320,	1233)
	(6330,	1227)
	(6340,	1228)
	(6350,	1221)
	(6360,	1215)
	(6370,	1212)
	(6380,	1205)
	(6390,	1199)
	(6400,	1194)
	(6410,	1186)
	(6420,	1183)
	(6430,	1174)
	(6440,	1167)
	(6450,	1160)
	(6460,	1154)
	(6470,	1149)
	(6480,	1146)
	(6490,	1138)
	(6500,	1136)
	(6510,	1134)
	(6520,	1128)
	(6530,	1122)
	(6540,	1118)
	(6550,	1109)
	(6560,	1101)
	(6570,	1095)
	(6580,	1090)
	(6590,	1080)
	(6600,	1074)
	(6610,	1070)
	(6620,	1069)
	(6630,	1066)
	(6640,	1059)
	(6650,	1054)
	(6660,	1046)
	(6670,	1040)
	(6680,	1033)
	(6690,	1027)
	(6700,	1022)
	(6710,	1016)
	(6720,	1011)
	(6730,	1004)
	(6740,	1002)
	(6750,	995)
	(6760,	988)
	(6770,	980)
	(6780,	976)
	(6790,	971)
	(6800,	963)
	(6810,	960)
	(6820,	951)
	(6830,	944)
	(6840,	936)
	(6850,	929)
	(6860,	922)
	(6870,	919)
	(6880,	916)
	(6890,	910)
	(6900,	904)
	(6910,	898)
	(6920,	892)
	(6930,	886)
	(6940,	877)
	(6950,	875)
	(6960,	868)
	(6970,	862)
	(6980,	854)
	(6990,	850)
	(7000,	844)
	(7010,	841)
	(7020,	836)
	(7030,	829)
	(7040,	825)
	(7050,	818)
	(7060,	810)
	(7070,	807)
	(7080,	798)
	(7090,	791)
	(7100,	790)
	(7110,	786)
	(7120,	780)
	(7130,	775)
	(7140,	772)
	(7150,	765)
	(7160,	759)
	(7170,	754)
	(7180,	750)
	(7190,	744)
	(7200,	738)
	(7210,	731)
	(7220,	723)
	(7230,	722)
	(7240,	717)
	(7250,	711)
	(7260,	702)
	(7270,	695)
	(7280,	688)
	(7290,	680)
	(7300,	674)
	(7310,	665)
	(7320,	662)
	(7330,	658)
	(7340,	657)
	(7350,	655)
	(7360,	655)
	(7370,	651)
	(7380,	650)
	(7390,	643)
	(7400,	637)
	(7410,	630)
	(7420,	625)
	(7430,	617)
	(7440,	614)
	(7450,	611)
	(7460,	607)
	(7470,	599)
	(7480,	590)
	(7490,	584)
	(7500,	575)
	(7510,	576)
	(7520,	572)
	(7530,	564)
	(7540,	564)
	(7550,	560)
	(7560,	552)
	(7570,	549)
	(7580,	546)
	(7590,	540)
	(7600,	538)
	(7610,	532)
	(7620,	525)
	(7630,	516)
	(7640,	510)
	(7650,	503)
	(7660,	502)
	(7670,	497)
	(7680,	490)
	(7690,	486)
	(7700,	478)
	(7710,	471)
	(7720,	465)
	(7730,	458)
	(7740,	452)
	(7750,	448)
	(7760,	444)
	(7770,	442)
	(7780,	435)
	(7790,	431)
	(7800,	425)
	(7810,	416)
	(7820,	413)
	(7830,	413)
	(7840,	407)
	(7850,	399)
	(7860,	390)
	(7870,	382)
	(7880,	376)
	(7890,	367)
	(7900,	367)
	(7910,	365)
	(7920,	361)
	(7930,	353)
	(7940,	346)
	(7950,	343)
	(7960,	340)
	(7970,	339)
	(7980,	332)
	(7990,	325)
	(8000,	321)
	(8010,	314)
	(8020,	306)
	(8030,	304)
	(8040,	302)
	(8050,	298)
	(8060,	293)
	(8070,	290)
	(8080,	288)
	(8090,	283)
	(8100,	278)
	(8110,	276)
	(8120,	268)
	(8130,	261)
	(8140,	254)
	(8150,	251)
	(8160,	247)
	(8170,	244)
	(8180,	239)
	(8190,	233)
	(8200,	230)
	(8210,	225)
	(8220,	220)
	(8230,	218)
	(8240,	213)
	(8250,	206)
	(8260,	200)
	(8270,	196)
	(8280,	189)
	(8290,	184)
	(8300,	176)
	(8310,	168)
	(8320,	168)
	(8330,	164)
	(8340,	158)
	(8350,	153)
	(8360,	146)
	(8370,	139)
	(8380,	136)
	(8390,	130)
	(8400,	127)
	(8410,	129)
	(8420,	124)
	(8430,	116)
	(8440,	115)
	(8450,	112)
	(8460,	105)
	(8470,	102)
	(8480,	95)
	(8490,	87)
	(8500,	79)
	(8510,	72)
	(8520,	66)
	(8530,	65)
	(8540,	61)
	(8550,	58)
	(8560,	51)
	(8570,	46)
	(8580,	46)
	(8590,	40)
	(8600,	39)
	(8601,	38)
	(8602,	37)
	(8603,	36)
	(8604,	36)
	(8605,	35)
	(8606,	35)
	(8607,	35)
	(8608,	34)
	(8609,	33)
	(8610,	32)
	(8611,	31)
	(8612,	30)
	(8613,	29)
	(8614,	29)
	(8615,	29)
	(8616,	28)
	(8617,	27)
	(8618,	26)
	(8619,	25)
	(8620,	24)
	(8621,	23)
	(8622,	22)
	(8623,	23)
	(8624,	22)
	(8625,	24)
	(8626,	23)
	(8627,	22)
	(8628,	21)
	(8629,	20)
	(8630,	20)
	(8631,	19)
	(8632,	18)
	(8633,	17)
	(8634,	16)
	(8635,	16)
	(8636,	15)
	(8637,	15)
	(8638,	15)
	(8639,	15)
	(8640,	14)
	(8641,	13)
	(8642,	12)
	(8643,	11)
	(8644,	12)
	(8645,	11)
	(8646,	11)
	(8647,	11)
	(8648,	11)
	(8649,	12)
	(8650,	11)
	(8651,	10)
	(8652,	9)
	(8653,	9)
	(8654,	9)
	(8655,	14)
	(8656,	13)
	(8657,	12)
	(8658,	11)
	(8659,	10)
	(8660,	12)
	(8661,	11)
	(8662,	10)
	(8663,	9)
	(8664,	10)
	(8665,	9)
	(8666,	8)
	(8667,	7)
	(8668,	8)
	(8669,	7)
	(8670,	6)
	(8671,	5)
	(8672,	4)
	(8673,	3)
	(8674,	2)
	(8675,	1)
	(8676,	1)
	(8677,	1)
	(8678,	0)
	(8679,	0)
	(8680,	0)
	(8681,	0)
	(8682,	0)
	(8683,	0)
	(8684,	0)
	(8685,	0)
	(8686,	0)
	(8687,	0)
	(8688,	1)
	(8689,	1)
	(8690,	1)
	(8691,	1)
	(8692,	0)
	(8693,	0)
	(8694,	0)
	(8695,	1)
	(8696,	1)
	(8697,	1)
	(8698,	1)
	(8699,	0)
	(8700,	0)
	(8701,	0)
	(8702,	0)
	(8703,	0)
	(8704,	0)
	(8705,	0)
	(8706,	0)
	(8707,	0)
	(8708,	0)
	(8709,	1)
	(8710,	0)
	(8711,	0)
	(8712,	0)
	(8713,	0)
	(8714,	0)
	(8715,	0)
	(8716,	0)
	(8717,	0)
	(8718,	1)
	(8719,	1)
	(8720,	1)
	(8721,	0)
	(8722,	0)
	(8723,	0)
	(8724,	0)
	(8725,	0)
	(8726,	0)
	(8727,	0)
	(8728,	0)
	(8729,	2)
	(8730,	1)
	(8731,	1)
	(8732,	1)
	(8733,	0)
	(8734,	0)
	(8735,	0)
	(8736,	0)
	(8737,	0)
	(8738,	0)
	(8739,	0)
	(8740,	0)
	(8741,	3)
	(8742,	2)
	(8743,	1)
	(8744,	0)
	(8745,	0)
	(8746,	1)
	(8747,	1)
	(8748,	1)
	(8749,	1)
	(8750,	2)
	(8751,	2)
	(8752,	3)
	(8753,	2)
	(8754,	1)
	(8755,	0)
	(8756,	0)
	(8757,	0)
	(8758,	0)
	(8759,	1)
	(8760,	0)
	(8761,	0)
	(8762,	0)
	(8763,	1)
	(8764,	1)
	(8765,	1)
	(8766,	1)
	(8767,	0)
	(8768,	0)
	(8769,	3)
	(8770,	3)
	(8771,	2)
	(8772,	1)
	(8773,	1)
	(8774,	0)
	(8775,	0)
	(8776,	0)
	(8777,	0)
	(8778,	2)
	(8779,	1)
	(8780,	1)
	(8781,	1)
	(8782,	0)
	(8783,	0)
	(8784,	0)
	(8785,	0)
	(8786,	1)
	(8787,	1)
	(8788,	1)
	(8789,	0)
	(8790,	0)
	(8791,	0)
	(8792,	0)
	(8793,	0)
	(8794,	0)
	(8795,	0)
	(8796,	0)
	(8797,	0)
	(8798,	0)
	(8799,	4)
	(8800,	3)
	(8801,	3)
	(8802,	2)
	(8803,	1)
	(8804,	1)
	(8805,	1)
	(8806,	1)
	(8807,	0)
	(8808,	0)
	(8809,	0)
	(8810,	0)
	(8811,	0)
	(8812,	0)
	(8813,	1)
	(8814,	0)
	(8815,	0)
	(8816,	0)
	(8817,	0)
	(8818,	0)
	(8819,	0)
	(8820,	0)
	(8821,	0)
	(8822,	0)
	(8823,	0)
	(8824,	0)
	(8825,	0)
	(8826,	0)
	(8827,	0)
	(8828,	0)
	(8829,	0)
	(8830,	0)
	(8831,	0)
	(8832,	0)
	(8833,	0)
	(8834,	0)
	(8835,	1)
	(8836,	0)
	(8837,	0)
	(8838,	1)
	(8839,	2)
	(8840,	1)
	(8841,	0)
	(8842,	0)
	(8843,	0)
	(8844,	0)
	(8845,	0)
	(8846,	0)
	(8847,	1)
	(8848,	2)
	(8849,	1)
	(8850,	1)
	(8851,	1)
	(8852,	1)
	(8853,	0)
	(8854,	0)
	(8855,	0)
	(8856,	1)
	(8857,	0)
	(8858,	0)
	(8859,	0)
	(8860,	0)
	(8861,	0)
	(8862,	1)
	(8863,	1)
	(8864,	0)
	(8865,	0)
	(8866,	0)
	(8867,	1)
	(8868,	2)
	(8869,	1)
	(8870,	0)
	(8871,	0)
	(8872,	0)
	(8873,	0)
	(8874,	0)
	(8875,	2)
	(8876,	2)
	(8877,	3)
	(8878,	3)
	(8879,	3)
	(8880,	3)
	(8881,	3)
	(8882,	4)
	(8883,	4)
	(8884,	4)
	(8885,	4)
	(8886,	5)
	(8887,	5)
	(8888,	5)
	(8889,	6)
	(8890,	8)
	(8891,	9)
	(8892,	9)
	(8893,	9)
	(8894,	9)
	(8895,	10)
	(8896,	10)
	(8897,	11)
	(8898,	11)
	(8899,	11)
	(8900,	11)
	(8901,	12)
	(8902,	12)
	(8903,	12)
	(8904,	12)
	(8905,	12)
	(8906,	12)
	(8907,	12)
	(8908,	12)
	(8909,	12)
	(8910,	12)
	(8911,	13)
	(8912,	13)
	(8913,	13)
	(8914,	14)
	(8915,	16)
	(8916,	16)
	(8917,	16)
	(8918,	17)
	(8919,	18)
	(8920,	18)
	(8921,	19)
	(8922,	20)
	(8923,	20)
	(8924,	21)
	(8925,	21)
	(8926,	21)
	(8927,	23)
	(8928,	23)
	(8929,	23)
	(8930,	23)
	(8931,	24)
	(8932,	28)
	(8933,	28)
	(8934,	28)
	(8935,	28)
	(8936,	28)
	(8937,	28)
	(8938,	28)
	(8939,	28)
	(8940,	28)
	(8941,	28)
	(8942,	28)
	(8943,	28)
	(8944,	30)
	(8945,	30)
	(8946,	32)
	(8947,	33)
	(8948,	33)
	(8949,	33)
	(8950,	33)
	(8951,	33)
	(8952,	33)
	(8953,	33)
	(8954,	36)
	(8955,	37)
	(8956,	37)
	(8957,	38)
	(8958,	38)
	(8959,	38)
	(8960,	38)
	(8961,	41)
	(8962,	41)
	(8963,	42)
	(8964,	43)
	(8965,	43)
	(8966,	43)
	(8967,	44)
	(8968,	44)
	(8969,	45)
	(8970,	46)
	(8971,	46)
	(8972,	47)
	(8973,	47)
	(8974,	47)
	(8975,	49)
	(8976,	49)
	(8977,	49)
	(8978,	50)
	(8979,	50)
	(8980,	52)
	(8981,	52)
	(8982,	53)
	(8983,	53)
	(8984,	54)
	(8985,	54)
	(8986,	55)
	(8987,	55)
	(8988,	56)
	(8989,	57)
	(8990,	58)
	(8991,	58)
	(8992,	58)
	(8993,	58)
	(8994,	58)
	(8995,	59)
	(8996,	59)
	(8997,	59)
	(8998,	59)
	(8999,	61)
	(9000,	62)
	(9010,	70)
	(9020,	79)
	(9030,	82)
	(9040,	83)
	(9050,	86)
	(9060,	90)
	(9070,	95)
	(9080,	107)
	(9090,	119)
	(9100,	126)
	(9110,	134)
	(9120,	138)
	(9130,	150)
	(9140,	157)
	(9150,	164)
	(9160,	173)
	(9170,	178)
	(9180,	182)
	(9190,	188)
	(9200,	193)
	(9210,	202)
	(9220,	204)
	(9230,	207)
	(9240,	217)
	(9250,	220)
	(9260,	221)
	(9270,	225)
	(9280,	234)
	(9290,	237)
	(9300,	245)
	(9310,	249)
	(9320,	252)
	(9330,	257)
	(9340,	259)
	(9350,	265)
	(9360,	271)
	(9370,	271)
	(9380,	279)
	(9390,	281)
	(9400,	283)
	(9410,	287)
	(9420,	293)
	(9430,	299)
	(9440,	303)
	(9450,	308)
	(9460,	312)
	(9470,	316)
	(9480,	317)
	(9490,	318)
	(9500,	319)
	(9510,	335)
	(9520,	339)
	(9530,	344)
	(9540,	351)
	(9550,	355)
	(9560,	358)
	(9570,	360)
	(9580,	368)
	(9590,	371)
	(9600,	373)
	(9610,	380)
	(9620,	383)
	(9630,	389)
	(9640,	392)
	(9650,	395)
	(9660,	399)
	(9670,	401)
	(9680,	410)
	(9690,	421)
	(9700,	423)
	(9710,	426)
	(9720,	429)
	(9730,	435)
	(9740,	442)
	(9750,	449)
	(9760,	457)
	(9770,	459)
	(9780,	463)
	(9790,	465)
	(9800,	474)
	(9810,	479)
	(9820,	484)
	(9830,	486)
	(9840,	491)
	(9850,	491)
	(9860,	497)
	(9870,	505)
	(9880,	506)
	(9890,	511)
	(9900,	514)
	(9910,	517)
	(9920,	518)
	(9930,	522)
	(9940,	523)
	(9950,	524)
	(9960,	529)
	(9970,	534)
	(9980,	538)
	(9990,	547)
	(10000,	554)
};

==> fig/spy1.tex <==
\addplot[color=black] plot coordinates {
	(803,	67)
	(807,	63)
	(811,	66)
	(815,	63)
	(819,	59)
	(823,	56)
	(827,	55)
	(831,	55)
	(835,	51)
	(839,	50)
	(843,	50)
	(847,	49)
	(851,	47)
	(855,	47)
	(859,	43)
	(863,	39)
	(867,	35)
	(871,	33)
	(875,	31)
	(879,	31)
	(883,	30)
	(887,	29)
	(891,	25)
	(895,	22)
	(899,	19)
	(903,	15)
	(907,	12)
	(911,	12)
	(915,	8)
	(919,	8)
	(923,	6)
	(927,	3)
	(931,	2)
	(935,	0)
	(939,	0)
	(943,	1)
	(947,	1)
	(951,	0)
	(955,	0)
	(959,	0)
	(963,	0)
	(967,	0)
	(971,	1)
	(975,	0)
	(979,	0)
	(983,	1)
	(987,	0)
	(991,	2)
	(995,	1)
	(999,	2)
	(1003,	1)
	(1007,	0)
	(1011,	0)
	(1015,	0)
	(1019,	0)
	(1023,	0)
	(1027,	0)
	(1031,	0)
	(1035,	0)
	(1039,	0)
	(1043,	0)
	(1047,	0)
	(1051,	5)
	(1055,	5)
	(1059,	6)
	(1063,	8)
	(1067,	9)
	(1071,	10)
	(1075,	11)
	(1079,	16)
	(1083,	18)
	(1087,	19)
	(1091,	20)
	(1095,	22)
	(1099,	22)
	(1103,	24)
	(1107,	25)
	(1111,	29)
	(1115,	30)
	(1119,	30)
	(1123,	30)
	(1127,	30)
	(1131,	31)
	(1135,	33)
	(1139,	36)
	(1143,	37)
	(1147,	38)
	(1151,	41)
	(1155,	45)
	(1159,	45)
	(1163,	48)
	(1167,	49)
	(1171,	49)
	(1175,	51)
	(1179,	51)
	(1183,	51)
	(1187,	51)
	(1191,	56)
	(1195,	60)
	(1199,	62)
};
\addplot[color=gray] plot coordinates {
	(802,	140)
	(806,	139)
	(810,	138)
	(814,	134)
	(818,	131)
	(822,	132)
	(826,	133)
	(830,	132)
	(834,	131)
	(838,	128)
	(842,	126)
	(846,	123)
	(850,	124)
	(854,	120)
	(858,	116)
	(862,	112)
	(866,	109)
	(870,	106)
	(874,	103)
	(878,	99)
	(882,	100)
	(886,	99)
	(890,	97)
	(894,	94)
	(898,	96)
	(902,	95)
	(906,	94)
	(910,	91)
	(914,	87)
	(918,	83)
	(922,	80)
	(926,	76)
	(930,	74)
	(934,	70)
	(938,	66)
	(942,	62)
	(946,	60)
	(950,	58)
	(954,	55)
	(958,	54)
	(962,	51)
	(966,	47)
	(970,	45)
	(974,	42)
	(978,	40)
	(982,	37)
	(986,	39)
	(990,	37)
	(994,	35)
	(998,	31)
	(1002,	27)
	(1006,	24)
	(1010,	23)
	(1014,	21)
	(1018,	19)
	(1022,	15)
	(1026,	11)
	(1030,	11)
	(1034,	9)
	(1038,	7)
	(1042,	4)
	(1046,	0)
	(1050,	2)
	(1054,	5)
	(1058,	7)
	(1062,	11)
	(1066,	12)
	(1070,	13)
	(1074,	13)
	(1078,	16)
	(1082,	17)
	(1086,	19)
	(1090,	21)
	(1094,	28)
	(1098,	31)
	(1102,	32)
	(1106,	32)
	(1110,	34)
	(1114,	38)
	(1118,	41)
	(1122,	45)
	(1126,	46)
	(1130,	48)
	(1134,	49)
	(1138,	52)
	(1142,	55)
	(1146,	58)
	(1150,	61)
	(1154,	61)
	(1158,	63)
	(1162,	66)
	(1166,	67)
	(1170,	72)
	(1174,	75)
	(1178,	79)
	(1182,	84)
	(1186,	84)
	(1190,	85)
	(1194,	86)
	(1198,	91)
};

==> fig/spy2.tex <==
\addplot[color=black,densely dashdotted] plot coordinates {
	(4703,	66)
	(4707,	62)
	(4711,	62)
	(4715,	60)
	(4719,	57)
	(4723,	57)
	(4727,	57)
	(4731,	53)
	(4735,	52)
	(4739,	49)
	(4743,	48)
	(4747,	44)
	(4751,	41)
	(4755,	40)
	(4759,	39)
	(4763,	36)
	(4767,	34)
	(4771,	34)
	(4775,	35)
	(4779,	34)
	(4783,	32)
	(4787,	30)
	(4791,	31)
	(4795,	28)
	(4799,	24)
	(4803,	20)
	(4807,	16)
	(4811,	12)
	(4815,	10)
	(4819,	8)
	(4823,	5)
	(4827,	5)
	(4831,	1)
	(4835,	1)
	(4839,	1)
	(4843,	0)
	(4847,	0)
	(4851,	0)
	(4855,	0)
	(4859,	0)
	(4863,	0)
	(4867,	0)
	(4871,	0)
	(4875,	0)
	(4879,	1)
	(4883,	3)
	(4887,	0)
	(4891,	0)
	(4895,	0)
	(4899,	0)
	(4903,	0)
	(4907,	0)
	(4911,	0)
	(4915,	0)
	(4919,	0)
	(4923,	0)
	(4927,	0)
	(4931,	0)
	(4935,	1)
	(4939,	2)
	(4943,	5)
	(4947,	6)
	(4951,	9)
	(4955,	14)
	(4959,	19)
	(4963,	24)
	(4967,	27)
	(4971,	28)
	(4975,	30)
	(4979,	30)
	(4983,	30)
	(4987,	32)
	(4991,	32)
	(4995,	33)
	(4999,	38)
	(5003,	40)
	(5007,	41)
	(5011,	42)
	(5015,	42)
	(5019,	43)
	(5023,	46)
	(5027,	47)
	(5031,	47)
	(5035,	54)
	(5039,	58)
	(5043,	58)
	(5047,	62)
	(5051,	62)
	(5055,	62)
	(5059,	69)
	(5063,	70)
	(5067,	71)
	(5071,	75)
	(5075,	76)
	(5079,	76)
	(5083,	76)
	(5087,	79)
	(5091,	81)
	(5095,	83)
	(5099,	84)
};
\addplot[color=gray,densely dashdotted] plot coordinates {
	(4702,	123)
	(4706,	122)
	(4710,	123)
	(4714,	120)
	(4718,	118)
	(4722,	115)
	(4726,	112)
	(4730,	111)
	(4734,	110)
	(4738,	106)
	(4742,	106)
	(4746,	106)
	(4750,	102)
	(4754,	106)
	(4758,	107)
	(4762,	108)
	(4766,	105)
	(4770,	103)
	(4774,	99)
	(4778,	97)
	(4782,	96)
	(4786,	94)
	(4790,	92)
	(4794,	90)
	(4798,	90)
	(4802,	89)
	(4806,	88)
	(4810,	85)
	(4814,	81)
	(4818,	79)
	(4822,	75)
	(4826,	73)
	(4830,	71)
	(4834,	68)
	(4838,	65)
	(4842,	61)
	(4846,	58)
	(4850,	58)
	(4854,	54)
	(4858,	51)
	(4862,	47)
	(4866,	43)
	(4870,	39)
	(4874,	35)
	(4878,	34)
	(4882,	30)
	(4886,	29)
	(4890,	25)
	(4894,	22)
	(4898,	18)
	(4902,	15)
	(4906,	11)
	(4910,	9)
	(4914,	9)
	(4918,	5)
	(4922,	4)
	(4926,	5)
	(4930,	2)
	(4934,	0)
	(4938,	3)
	(4942,	5)
	(4946,	7)
	(4950,	10)
	(4954,	11)
	(4958,	12)
	(4962,	12)
	(4966,	15)
	(4970,	25)
	(4974,	28)
	(4978,	31)
	(4982,	31)
	(4986,	32)
	(4990,	35)
	(4994,	37)
	(4998,	37)
	(5002,	42)
	(5006,	43)
	(5010,	46)
	(5014,	47)
	(5018,	50)
	(5022,	53)
	(5026,	55)
	(5030,	55)
	(5034,	57)
	(5038,	59)
	(5042,	60)
	(5046,	62)
	(5050,	66)
	(5054,	68)
	(5058,	71)
	(5062,	73)
	(5066,	75)
	(5070,	78)
	(5074,	80)
	(5078,	80)
	(5082,	81)
	(5086,	81)
	(5090,	82)
	(5094,	85)
	(5098,	89)
};


==> fig/spy3.tex <==
\addplot[color=black] plot coordinates {
	(8603,	141)
	(8607,	139)
	(8611,	138)
	(8615,	135)
	(8619,	134)
	(8623,	130)
	(8627,	129)
	(8631,	127)
	(8635,	127)
	(8639,	123)
	(8643,	120)
	(8647,	118)
	(8651,	115)
	(8655,	112)
	(8659,	111)
	(8663,	111)
	(8667,	111)
	(8671,	107)
	(8675,	108)
	(8679,	104)
	(8683,	101)
	(8687,	100)
	(8691,	97)
	(8695,	93)
	(8699,	89)
	(8703,	86)
	(8707,	87)
	(8711,	83)
	(8715,	80)
	(8719,	77)
	(8723,	75)
	(8727,	75)
	(8731,	71)
	(8735,	71)
	(8739,	67)
	(8743,	66)
	(8747,	62)
	(8751,	60)
	(8755,	58)
	(8759,	57)
	(8763,	56)
	(8767,	52)
	(8771,	48)
	(8775,	44)
	(8779,	40)
	(8783,	39)
	(8787,	44)
	(8791,	44)
	(8795,	49)
	(8799,	52)
	(8803,	48)
	(8807,	46)
	(8811,	46)
	(8815,	45)
	(8819,	41)
	(8823,	38)
	(8827,	37)
	(8831,	35)
	(8835,	34)
	(8839,	31)
	(8843,	27)
	(8847,	23)
	(8851,	19)
	(8855,	16)
	(8859,	13)
	(8863,	11)
	(8867,	9)
	(8871,	5)
	(8875,	4)
	(8879,	5)
	(8883,	10)
	(8887,	10)
	(8891,	17)
	(8895,	19)
	(8899,	22)
	(8903,	23)
	(8907,	23)
	(8911,	26)
	(8915,	31)
	(8919,	32)
	(8923,	37)
	(8927,	38)
	(8931,	41)
	(8935,	43)
	(8939,	44)
	(8943,	44)
	(8947,	44)
	(8951,	44)
	(8955,	44)
	(8959,	49)
	(8963,	49)
	(8967,	51)
	(8971,	54)
	(8975,	54)
	(8979,	56)
	(8983,	58)
	(8987,	59)
	(8991,	61)
	(8995,	62)
	(8999,	64)
};
\addplot[color=gray] plot coordinates {
	(8602,	37)
	(8606,	35)
	(8610,	32)
	(8614,	29)
	(8618,	26)
	(8622,	22)
	(8626,	23)
	(8630,	20)
	(8634,	16)
	(8638,	15)
	(8642,	12)
	(8646,	11)
	(8650,	11)
	(8654,	9)
	(8658,	11)
	(8662,	10)
	(8666,	8)
	(8670,	6)
	(8674,	2)
	(8678,	0)
	(8682,	0)
	(8686,	0)
	(8690,	1)
	(8694,	0)
	(8698,	1)
	(8702,	0)
	(8706,	0)
	(8710,	0)
	(8714,	0)
	(8718,	1)
	(8722,	0)
	(8726,	0)
	(8730,	1)
	(8734,	0)
	(8738,	0)
	(8742,	2)
	(8746,	1)
	(8750,	2)
	(8754,	1)
	(8758,	0)
	(8762,	0)
	(8766,	1)
	(8770,	3)
	(8774,	0)
	(8778,	2)
	(8782,	0)
	(8786,	1)
	(8790,	0)
	(8794,	0)
	(8798,	0)
	(8802,	2)
	(8806,	1)
	(8810,	0)
	(8814,	0)
	(8818,	0)
	(8822,	0)
	(8826,	0)
	(8830,	0)
	(8834,	0)
	(8838,	1)
	(8842,	0)
	(8846,	0)
	(8850,	1)
	(8854,	0)
	(8858,	0)
	(8862,	1)
	(8866,	0)
	(8870,	0)
	(8874,	0)
	(8878,	3)
	(8882,	4)
	(8886,	5)
	(8890,	8)
	(8894,	9)
	(8898,	11)
	(8902,	12)
	(8906,	12)
	(8910,	12)
	(8914,	14)
	(8918,	17)
	(8922,	20)
	(8926,	21)
	(8930,	23)
	(8934,	28)
	(8938,	28)
	(8942,	28)
	(8946,	32)
	(8950,	33)
	(8954,	36)
	(8958,	38)
	(8962,	41)
	(8966,	43)
	(8970,	46)
	(8974,	47)
	(8978,	50)
	(8982,	53)
	(8986,	55)
	(8990,	58)
	(8994,	58)
	(8998,	59)
};

==> fig/thinned.tex <==
\addplot[color=black,densely dashdotted] plot coordinates {
	(30,	1425)
	(70,	1454)
	(110,	1477)
	(150,	1494)
	(190,	1513)
	(230,	1539)
	(270,	1564)
	(310,	1574)
	(350,	1594)
	(390,	1613)
	(430,	1625)
	(470,	1642)
	(510,	1664)
	(550,	1689)
	(590,	1704)
	(630,	1725)
	(670,	1746)
	(710,	1775)
	(750,	1803)
	(790,	1819)
	(803,	1827)
	(807,	1828)
	(811,	1828)
	(815,	1828)
	(819,	1829)
	(823,	1829)
	(827,	1830)
	(831,	1833)
	(835,	1834)
	(839,	1837)
	(843,	1839)
	(847,	1840)
	(851,	1841)
	(855,	1844)
	(859,	1847)
	(863,	1847)
	(867,	1849)
	(871,	1853)
	(875,	1853)
	(879,	1853)
	(883,	1853)
	(887,	1853)
	(891,	1853)
	(895,	1854)
	(899,	1855)
	(903,	1856)
	(907,	1857)
	(911,	1861)
	(915,	1862)
	(919,	1863)
	(923,	1867)
	(927,	1870)
	(931,	1872)
	(935,	1872)
	(939,	1874)
	(943,	1877)
	(947,	1877)
	(951,	1880)
	(955,	1880)
	(959,	1881)
	(963,	1884)
	(967,	1888)
	(971,	1888)
	(975,	1890)
	(979,	1890)
	(983,	1896)
	(987,	1899)
	(991,	1899)
	(995,	1900)
	(999,	1903)
	(1003,	1904)
	(1007,	1908)
	(1011,	1909)
	(1015,	1912)
	(1019,	1915)
	(1023,	1919)
	(1027,	1924)
	(1031,	1926)
	(1035,	1930)
	(1039,	1932)
	(1043,	1937)
	(1047,	1938)
	(1051,	1938)
	(1055,	1935)
	(1059,	1934)
	(1063,	1931)
	(1067,	1927)
	(1071,	1924)
	(1075,	1924)
	(1079,	1923)
	(1083,	1919)
	(1087,	1915)
	(1091,	1912)
	(1095,	1909)
	(1099,	1908)
	(1103,	1907)
	(1107,	1906)
	(1111,	1907)
	(1115,	1905)
	(1119,	1902)
	(1123,	1903)
	(1127,	1901)
	(1131,	1899)
	(1135,	1898)
	(1139,	1898)
	(1143,	1899)
	(1147,	1900)
	(1151,	1896)
	(1155,	1893)
	(1159,	1891)
	(1163,	1888)
	(1167,	1888)
	(1171,	1884)
	(1175,	1884)
	(1179,	1880)
	(1183,	1876)
	(1187,	1877)
	(1191,	1874)
	(1195,	1874)
	(1199,	1872)
	(1230,	1848)
	(1270,	1827)
	(1310,	1806)
	(1350,	1785)
	(1390,	1772)
	(1430,	1751)
	(1470,	1733)
	(1510,	1715)
	(1550,	1691)
	(1590,	1659)
	(1630,	1642)
	(1670,	1620)
	(1710,	1598)
	(1750,	1583)
	(1790,	1559)
	(1830,	1547)
	(1870,	1524)
	(1910,	1504)
	(1950,	1483)
	(1990,	1467)
	(2030,	1449)
	(2070,	1422)
	(2110,	1396)
	(2150,	1377)
	(2190,	1358)
	(2230,	1336)
	(2270,	1307)
	(2310,	1295)
	(2350,	1273)
	(2390,	1256)
	(2430,	1240)
	(2470,	1217)
	(2510,	1191)
	(2550,	1164)
	(2590,	1150)
	(2630,	1124)
	(2670,	1114)
	(2710,	1097)
	(2750,	1080)
	(2790,	1060)
	(2830,	1036)
	(2870,	1018)
	(2910,	998)
	(2950,	975)
	(2990,	950)
	(3030,	934)
	(3070,	912)
	(3110,	888)
	(3150,	873)
	(3190,	847)
	(3230,	828)
	(3270,	804)
	(3310,	781)
	(3350,	761)
	(3390,	743)
	(3430,	730)
	(3470,	694)
	(3510,	677)
	(3550,	650)
	(3590,	633)
	(3630,	611)
	(3670,	580)
	(3710,	554)
	(3750,	533)
	(3790,	513)
	(3830,	490)
	(3870,	464)
	(3910,	451)
	(3950,	434)
	(3990,	408)
	(4030,	397)
	(4070,	373)
	(4110,	355)
	(4150,	347)
	(4190,	327)
	(4230,	314)
	(4270,	286)
	(4310,	263)
	(4350,	247)
	(4390,	226)
	(4430,	209)
	(4470,	187)
	(4510,	171)
	(4550,	151)
	(4590,	128)
	(4630,	106)
	(4670,	85)
	(4701,	66)
	(4705,	64)
	(4709,	61)
	(4713,	61)
	(4717,	58)
	(4721,	55)
	(4725,	57)
	(4729,	55)
	(4733,	53)
	(4737,	51)
	(4741,	47)
	(4745,	46)
	(4749,	42)
	(4753,	40)
	(4757,	40)
	(4761,	38)
	(4765,	35)
	(4769,	34)
	(4773,	33)
	(4777,	35)
	(4781,	34)
	(4785,	32)
	(4789,	30)
	(4793,	30)
	(4797,	26)
	(4801,	22)
	(4805,	18)
	(4809,	14)
	(4813,	11)
	(4817,	9)
	(4821,	7)
	(4825,	3)
	(4829,	3)
	(4833,	1)
	(4837,	3)
	(4841,	0)
	(4845,	0)
	(4849,	0)
	(4853,	0)
	(4857,	2)
	(4861,	0)
	(4865,	0)
	(4869,	1)
	(4873,	0)
	(4877,	0)
	(4881,	2)
	(4885,	2)
	(4889,	0)
	(4893,	0)
	(4897,	0)
	(4901,	0)
	(4905,	1)
	(4909,	0)
	(4913,	1)
	(4917,	0)
	(4921,	2)
	(4925,	0)
	(4929,	0)
	(4933,	0)
	(4937,	2)
	(4941,	4)
	(4945,	6)
	(4949,	8)
	(4953,	9)
	(4957,	16)
	(4961,	21)
	(4965,	26)
	(4969,	27)
	(4973,	30)
	(4977,	30)
	(4981,	30)
	(4985,	31)
	(4989,	32)
	(4993,	32)
	(4997,	33)
	(5001,	39)
	(5005,	40)
	(5009,	42)
	(5013,	42)
	(5017,	43)
	(5021,	43)
	(5025,	47)
	(5029,	47)
	(5033,	50)
	(5037,	58)
	(5041,	58)
	(5045,	58)
	(5049,	62)
	(5053,	62)
	(5057,	69)
	(5061,	70)
	(5065,	70)
	(5069,	73)
	(5073,	76)
	(5077,	76)
	(5081,	76)
	(5085,	78)
	(5089,	80)
	(5093,	83)
	(5097,	83)
	(5110,	86)
	(5150,	106)
	(5190,	127)
	(5230,	143)
	(5270,	171)
	(5310,	195)
	(5350,	219)
	(5390,	233)
	(5430,	251)
	(5470,	272)
	(5510,	289)
	(5550,	307)
	(5590,	332)
	(5630,	352)
	(5670,	366)
	(5710,	383)
	(5750,	406)
	(5790,	426)
	(5830,	442)
	(5870,	461)
	(5910,	479)
	(5950,	493)
	(5990,	514)
	(6030,	529)
	(6070,	550)
	(6110,	567)
	(6150,	581)
	(6190,	620)
	(6230,	639)
	(6270,	661)
	(6310,	676)
	(6350,	697)
	(6390,	714)
	(6430,	732)
	(6470,	746)
	(6510,	767)
	(6550,	785)
	(6590,	807)
	(6630,	827)
	(6670,	845)
	(6710,	861)
	(6750,	877)
	(6790,	898)
	(6830,	911)
	(6870,	933)
	(6910,	958)
	(6950,	977)
	(6990,	1002)
	(7030,	1020)
	(7070,	1037)
	(7110,	1063)
	(7150,	1088)
	(7190,	1115)
	(7230,	1139)
	(7270,	1169)
	(7310,	1184)
	(7350,	1196)
	(7390,	1221)
	(7430,	1231)
	(7470,	1252)
	(7510,	1283)
	(7550,	1303)
	(7590,	1320)
	(7630,	1346)
	(7670,	1370)
	(7710,	1394)
	(7750,	1417)
	(7790,	1435)
	(7830,	1458)
	(7870,	1475)
	(7910,	1491)
	(7950,	1527)
	(7990,	1561)
	(8030,	1584)
	(8070,	1601)
	(8110,	1619)
	(8150,	1644)
	(8190,	1666)
	(8230,	1690)
	(8270,	1710)
	(8310,	1727)
	(8350,	1747)
	(8390,	1765)
	(8430,	1784)
	(8470,	1802)
	(8510,	1819)
	(8550,	1833)
	(8590,	1855)
	(8603,	1859)
	(8607,	1859)
	(8611,	1861)
	(8615,	1861)
	(8619,	1861)
	(8623,	1863)
	(8627,	1865)
	(8631,	1871)
	(8635,	1874)
	(8639,	1877)
	(8643,	1878)
	(8647,	1878)
	(8651,	1878)
	(8655,	1880)
	(8659,	1881)
	(8663,	1881)
	(8667,	1882)
	(8671,	1882)
	(8675,	1882)
	(8679,	1883)
	(8683,	1885)
	(8687,	1886)
	(8691,	1890)
	(8695,	1891)
	(8699,	1899)
	(8703,	1901)
	(8707,	1901)
	(8711,	1907)
	(8715,	1910)
	(8719,	1912)
	(8723,	1916)
	(8727,	1916)
	(8731,	1920)
	(8735,	1920)
	(8739,	1920)
	(8743,	1921)
	(8747,	1922)
	(8751,	1925)
	(8755,	1928)
	(8759,	1934)
	(8763,	1934)
	(8767,	1938)
	(8771,	1940)
	(8775,	1942)
	(8779,	1942)
	(8783,	1942)
	(8787,	1942)
	(8791,	1942)
	(8795,	1947)
	(8799,	1950)
	(8803,	1950)
	(8807,	1950)
	(8811,	1950)
	(8815,	1950)
	(8819,	1958)
	(8823,	1958)
	(8827,	1962)
	(8831,	1965)
	(8835,	1965)
	(8839,	1966)
	(8843,	1966)
	(8847,	1969)
	(8851,	1978)
	(8855,	1981)
	(8859,	1983)
	(8863,	1983)
	(8867,	1984)
	(8871,	1991)
	(8875,	1990)
	(8879,	1987)
	(8883,	1986)
	(8887,	1982)
	(8891,	1983)
	(8895,	1980)
	(8899,	1979)
	(8903,	1978)
	(8907,	1978)
	(8911,	1974)
	(8915,	1971)
	(8919,	1970)
	(8923,	1970)
	(8927,	1967)
	(8931,	1965)
	(8935,	1965)
	(8939,	1963)
	(8943,	1960)
	(8947,	1957)
	(8951,	1954)
	(8955,	1951)
	(8959,	1950)
	(8963,	1948)
	(8967,	1947)
	(8971,	1946)
	(8975,	1944)
	(8979,	1940)
	(8983,	1938)
	(8987,	1937)
	(8991,	1936)
	(8995,	1934)
	(8999,	1931)
	(9030,	1914)
	(9070,	1895)
	(9110,	1872)
	(9150,	1851)
	(9190,	1830)
	(9230,	1808)
	(9270,	1792)
	(9310,	1771)
	(9350,	1753)
	(9390,	1738)
	(9430,	1711)
	(9470,	1687)
	(9510,	1665)
	(9550,	1656)
	(9590,	1646)
	(9630,	1634)
	(9670,	1609)
	(9710,	1599)
	(9750,	1571)
	(9790,	1551)
	(9830,	1530)
	(9870,	1507)
	(9910,	1491)
	(9950,	1463)
	(9990,	1438)
};
\addplot[color=gray,densely dashdotted] plot coordinates {
	(20,	1548)
	(60,	1557)
	(100,	1585)
	(140,	1610)
	(180,	1635)
	(220,	1646)
	(260,	1663)
	(300,	1683)
	(340,	1714)
	(380,	1727)
	(420,	1749)
	(460,	1768)
	(500,	1780)
	(540,	1793)
	(580,	1821)
	(620,	1827)
	(660,	1844)
	(700,	1861)
	(740,	1883)
	(780,	1898)
	(802,	1912)
	(806,	1915)
	(810,	1915)
	(814,	1916)
	(818,	1917)
	(822,	1922)
	(826,	1924)
	(830,	1928)
	(834,	1931)
	(838,	1932)
	(842,	1933)
	(846,	1936)
	(850,	1937)
	(854,	1938)
	(858,	1940)
	(862,	1942)
	(866,	1943)
	(870,	1944)
	(874,	1946)
	(878,	1946)
	(882,	1951)
	(886,	1953)
	(890,	1956)
	(894,	1959)
	(898,	1959)
	(902,	1961)
	(906,	1965)
	(910,	1966)
	(914,	1967)
	(918,	1968)
	(922,	1973)
	(926,	1973)
	(930,	1974)
	(934,	1975)
	(938,	1977)
	(942,	1982)
	(946,	1985)
	(950,	1986)
	(954,	1987)
	(958,	1988)
	(962,	1989)
	(966,	1990)
	(970,	1994)
	(974,	1996)
	(978,	1997)
	(982,	1999)
	(986,	2000)
	(990,	2001)
	(994,	2004)
	(998,	2005)
	(1002,	2006)
	(1006,	2006)
	(1010,	2007)
	(1014,	2009)
	(1018,	2012)
	(1022,	2015)
	(1026,	2020)
	(1030,	2020)
	(1034,	2021)
	(1038,	2022)
	(1042,	2023)
	(1046,	2024)
	(1050,	2026)
	(1054,	2022)
	(1058,	2020)
	(1062,	2019)
	(1066,	2021)
	(1070,	2017)
	(1074,	2014)
	(1078,	2015)
	(1082,	2011)
	(1086,	2008)
	(1090,	2004)
	(1094,	2000)
	(1098,	1997)
	(1102,	1994)
	(1106,	1990)
	(1110,	1987)
	(1114,	1987)
	(1118,	1986)
	(1122,	1983)
	(1126,	1982)
	(1130,	1980)
	(1134,	1976)
	(1138,	1975)
	(1142,	1972)
	(1146,	1968)
	(1150,	1965)
	(1154,	1964)
	(1158,	1962)
	(1162,	1960)
	(1166,	1957)
	(1170,	1959)
	(1174,	1956)
	(1178,	1952)
	(1182,	1949)
	(1186,	1954)
	(1190,	1957)
	(1194,	1954)
	(1198,	1950)
	(1220,	1939)
	(1260,	1921)
	(1300,	1901)
	(1340,	1890)
	(1380,	1872)
	(1420,	1853)
	(1460,	1832)
	(1500,	1805)
	(1540,	1790)
	(1580,	1767)
	(1620,	1749)
	(1660,	1727)
	(1700,	1711)
	(1740,	1685)
	(1780,	1655)
	(1820,	1635)
	(1860,	1615)
	(1900,	1591)
	(1940,	1569)
	(1980,	1552)
	(2020,	1524)
	(2060,	1496)
	(2100,	1477)
	(2140,	1449)
	(2180,	1436)
	(2220,	1418)
	(2260,	1397)
	(2300,	1374)
	(2340,	1352)
	(2380,	1335)
	(2420,	1318)
	(2460,	1298)
	(2500,	1275)
	(2540,	1255)
	(2580,	1225)
	(2620,	1205)
	(2660,	1178)
	(2700,	1161)
	(2740,	1150)
	(2780,	1131)
	(2820,	1104)
	(2860,	1079)
	(2900,	1060)
	(2940,	1045)
	(2980,	1024)
	(3020,	1002)
	(3060,	984)
	(3100,	971)
	(3140,	947)
	(3180,	920)
	(3220,	890)
	(3260,	866)
	(3300,	847)
	(3340,	829)
	(3380,	804)
	(3420,	782)
	(3460,	764)
	(3500,	745)
	(3540,	726)
	(3580,	709)
	(3620,	703)
	(3660,	679)
	(3700,	649)
	(3740,	629)
	(3780,	601)
	(3820,	579)
	(3860,	556)
	(3900,	533)
	(3940,	504)
	(3980,	480)
	(4020,	458)
	(4060,	438)
	(4100,	417)
	(4140,	402)
	(4180,	382)
	(4220,	365)
	(4260,	350)
	(4300,	324)
	(4340,	308)
	(4380,	284)
	(4420,	271)
	(4460,	245)
	(4500,	234)
	(4540,	204)
	(4580,	181)
	(4620,	166)
	(4660,	139)
	(4700,	125)
	(4704,	122)
	(4708,	120)
	(4712,	121)
	(4716,	120)
	(4720,	117)
	(4724,	114)
	(4728,	111)
	(4732,	111)
	(4736,	108)
	(4740,	104)
	(4744,	108)
	(4748,	104)
	(4752,	105)
	(4756,	108)
	(4760,	105)
	(4764,	106)
	(4768,	104)
	(4772,	101)
	(4776,	99)
	(4780,	98)
	(4784,	94)
	(4788,	92)
	(4792,	92)
	(4796,	91)
	(4800,	90)
	(4804,	88)
	(4808,	86)
	(4812,	83)
	(4816,	81)
	(4820,	77)
	(4824,	74)
	(4828,	73)
	(4832,	70)
	(4836,	67)
	(4840,	63)
	(4844,	60)
	(4848,	57)
	(4852,	56)
	(4856,	53)
	(4860,	49)
	(4864,	45)
	(4868,	41)
	(4872,	37)
	(4876,	33)
	(4880,	32)
	(4884,	28)
	(4888,	27)
	(4892,	23)
	(4896,	20)
	(4900,	17)
	(4904,	13)
	(4908,	11)
	(4912,	8)
	(4916,	7)
	(4920,	5)
	(4924,	4)
	(4928,	3)
	(4932,	2)
	(4936,	2)
	(4940,	3)
	(4944,	5)
	(4948,	10)
	(4952,	11)
	(4956,	12)
	(4960,	12)
	(4964,	15)
	(4968,	22)
	(4972,	26)
	(4976,	31)
	(4980,	31)
	(4984,	32)
	(4988,	35)
	(4992,	35)
	(4996,	37)
	(5000,	40)
	(5004,	42)
	(5008,	43)
	(5012,	46)
	(5016,	49)
	(5020,	52)
	(5024,	54)
	(5028,	55)
	(5032,	56)
	(5036,	58)
	(5040,	59)
	(5044,	61)
	(5048,	64)
	(5052,	68)
	(5056,	69)
	(5060,	73)
	(5064,	74)
	(5068,	75)
	(5072,	79)
	(5076,	80)
	(5080,	80)
	(5084,	81)
	(5088,	82)
	(5092,	82)
	(5096,	86)
	(5100,	89)
	(5140,	120)
	(5180,	147)
	(5220,	163)
	(5260,	179)
	(5300,	203)
	(5340,	225)
	(5380,	248)
	(5420,	263)
	(5460,	277)
	(5500,	306)
	(5540,	325)
	(5580,	343)
	(5620,	369)
	(5660,	393)
	(5700,	411)
	(5740,	425)
	(5780,	445)
	(5820,	469)
	(5860,	494)
	(5900,	512)
	(5940,	527)
	(5980,	545)
	(6020,	569)
	(6060,	589)
	(6100,	604)
	(6140,	621)
	(6180,	642)
	(6220,	674)
	(6260,	698)
	(6300,	730)
	(6340,	759)
	(6380,	775)
	(6420,	791)
	(6460,	805)
	(6500,	816)
	(6540,	842)
	(6580,	857)
	(6620,	875)
	(6660,	891)
	(6700,	912)
	(6740,	931)
	(6780,	947)
	(6820,	964)
	(6860,	980)
	(6900,	997)
	(6940,	1005)
	(6980,	1021)
	(7020,	1044)
	(7060,	1058)
	(7100,	1083)
	(7140,	1104)
	(7180,	1127)
	(7220,	1155)
	(7260,	1177)
	(7300,	1196)
	(7340,	1214)
	(7380,	1232)
	(7420,	1264)
	(7460,	1276)
	(7500,	1295)
	(7540,	1322)
	(7580,	1347)
	(7620,	1371)
	(7660,	1393)
	(7700,	1404)
	(7740,	1424)
	(7780,	1432)
	(7820,	1447)
	(7860,	1462)
	(7900,	1478)
	(7940,	1496)
	(7980,	1511)
	(8020,	1527)
	(8060,	1550)
	(8100,	1576)
	(8140,	1602)
	(8180,	1632)
	(8220,	1653)
	(8260,	1664)
	(8300,	1684)
	(8340,	1709)
	(8380,	1728)
	(8420,	1745)
	(8460,	1765)
	(8500,	1780)
	(8540,	1802)
	(8580,	1825)
	(8602,	1843)
	(8606,	1846)
	(8610,	1848)
	(8614,	1851)
	(8618,	1852)
	(8622,	1854)
	(8626,	1858)
	(8630,	1859)
	(8634,	1863)
	(8638,	1863)
	(8642,	1863)
	(8646,	1865)
	(8650,	1866)
	(8654,	1867)
	(8658,	1867)
	(8662,	1867)
	(8666,	1870)
	(8670,	1871)
	(8674,	1875)
	(8678,	1877)
	(8682,	1880)
	(8686,	1881)
	(8690,	1882)
	(8694,	1883)
	(8698,	1884)
	(8702,	1889)
	(8706,	1891)
	(8710,	1894)
	(8714,	1897)
	(8718,	1900)
	(8722,	1902)
	(8726,	1904)
	(8730,	1904)
	(8734,	1906)
	(8738,	1906)
	(8742,	1906)
	(8746,	1910)
	(8750,	1912)
	(8754,	1914)
	(8758,	1919)
	(8762,	1921)
	(8766,	1924)
	(8770,	1924)
	(8774,	1932)
	(8778,	1935)
	(8782,	1938)
	(8786,	1938)
	(8790,	1939)
	(8794,	1939)
	(8798,	1940)
	(8802,	1942)
	(8806,	1945)
	(8810,	1946)
	(8814,	1950)
	(8818,	1952)
	(8822,	1954)
	(8826,	1957)
	(8830,	1959)
	(8834,	1960)
	(8838,	1962)
	(8842,	1965)
	(8846,	1966)
	(8850,	1967)
	(8854,	1968)
	(8858,	1974)
	(8862,	1975)
	(8866,	1977)
	(8870,	1978)
	(8874,	1980)
	(8878,	1977)
	(8882,	1973)
	(8886,	1972)
	(8890,	1968)
	(8894,	1968)
	(8898,	1964)
	(8902,	1960)
	(8906,	1959)
	(8910,	1965)
	(8914,	1967)
	(8918,	1964)
	(8922,	1960)
	(8926,	1957)
	(8930,	1956)
	(8934,	1960)
	(8938,	1960)
	(8942,	1960)
	(8946,	1959)
	(8950,	1956)
	(8954,	1953)
	(8958,	1949)
	(8962,	1945)
	(8966,	1942)
	(8970,	1939)
	(8974,	1935)
	(8978,	1934)
	(8982,	1930)
	(8986,	1929)
	(8990,	1926)
	(8994,	1923)
	(8998,	1922)
	(9020,	1906)
	(9060,	1884)
	(9100,	1860)
	(9140,	1842)
	(9180,	1818)
	(9220,	1806)
	(9260,	1782)
	(9300,	1762)
	(9340,	1736)
	(9380,	1722)
	(9420,	1700)
	(9460,	1673)
	(9500,	1645)
	(9540,	1623)
	(9580,	1594)
	(9620,	1581)
	(9660,	1571)
	(9700,	1550)
	(9740,	1535)
	(9780,	1519)
	(9820,	1506)
	(9860,	1494)
	(9900,	1475)
	(9940,	1456)
	(9980,	1439)
};
\addplot[color=black] plot coordinates {
	(10,	451)
	(50,	431)
	(90,	411)
	(130,	398)
	(170,	372)
	(210,	360)
	(250,	335)
	(290,	316)
	(330,	295)
	(370,	277)
	(410,	254)
	(450,	237)
	(490,	220)
	(530,	204)
	(570,	182)
	(610,	160)
	(650,	137)
	(690,	115)
	(730,	96)
	(770,	79)
	(801,	67)
	(805,	65)
	(809,	63)
	(813,	65)
	(817,	61)
	(821,	57)
	(825,	57)
	(829,	57)
	(833,	53)
	(837,	50)
	(841,	49)
	(845,	51)
	(849,	47)
	(853,	46)
	(857,	45)
	(861,	41)
	(865,	37)
	(869,	34)
	(873,	32)
	(877,	33)
	(881,	31)
	(885,	30)
	(889,	27)
	(893,	24)
	(897,	20)
	(901,	17)
	(905,	14)
	(909,	11)
	(913,	10)
	(917,	7)
	(921,	8)
	(925,	4)
	(929,	3)
	(933,	1)
	(937,	0)
	(941,	0)
	(945,	2)
	(949,	2)
	(953,	0)
	(957,	0)
	(961,	0)
	(965,	0)
	(969,	0)
	(973,	1)
	(977,	0)
	(981,	0)
	(985,	0)
	(989,	1)
	(993,	2)
	(997,	0)
	(1001,	3)
	(1005,	0)
	(1009,	1)
	(1013,	1)
	(1017,	0)
	(1021,	1)
	(1025,	0)
	(1029,	0)
	(1033,	0)
	(1037,	0)
	(1041,	1)
	(1045,	0)
	(1049,	3)
	(1053,	5)
	(1057,	6)
	(1061,	8)
	(1065,	8)
	(1069,	9)
	(1073,	11)
	(1077,	13)
	(1081,	16)
	(1085,	18)
	(1089,	20)
	(1093,	21)
	(1097,	22)
	(1101,	23)
	(1105,	25)
	(1109,	27)
	(1113,	29)
	(1117,	30)
	(1121,	30)
	(1125,	30)
	(1129,	31)
	(1133,	31)
	(1137,	35)
	(1141,	36)
	(1145,	38)
	(1149,	41)
	(1153,	41)
	(1157,	45)
	(1161,	47)
	(1165,	49)
	(1169,	49)
	(1173,	51)
	(1177,	51)
	(1181,	51)
	(1185,	51)
	(1189,	52)
	(1193,	58)
	(1197,	61)
	(1210,	64)
	(1250,	80)
	(1290,	103)
	(1330,	116)
	(1370,	131)
	(1410,	147)
	(1450,	169)
	(1490,	195)
	(1530,	220)
	(1570,	249)
	(1610,	265)
	(1650,	282)
	(1690,	310)
	(1730,	335)
	(1770,	354)
	(1810,	385)
	(1850,	398)
	(1890,	413)
	(1930,	432)
	(1970,	456)
	(2010,	475)
	(2050,	493)
	(2090,	507)
	(2130,	531)
	(2170,	551)
	(2210,	577)
	(2250,	604)
	(2290,	623)
	(2330,	638)
	(2370,	648)
	(2410,	673)
	(2450,	708)
	(2490,	731)
	(2530,	747)
	(2570,	760)
	(2610,	783)
	(2650,	795)
	(2690,	812)
	(2730,	826)
	(2770,	845)
	(2810,	872)
	(2850,	887)
	(2890,	904)
	(2930,	930)
	(2970,	948)
	(3010,	964)
	(3050,	982)
	(3090,	996)
	(3130,	1021)
	(3170,	1036)
	(3210,	1052)
	(3250,	1068)
	(3290,	1076)
	(3330,	1099)
	(3370,	1124)
	(3410,	1140)
	(3450,	1164)
	(3490,	1187)
	(3530,	1215)
	(3570,	1233)
	(3610,	1259)
	(3650,	1277)
	(3690,	1298)
	(3730,	1321)
	(3770,	1340)
	(3810,	1363)
	(3850,	1378)
	(3890,	1409)
	(3930,	1424)
	(3970,	1437)
	(4010,	1452)
	(4050,	1473)
	(4090,	1497)
	(4130,	1509)
	(4170,	1521)
	(4210,	1546)
	(4250,	1561)
	(4290,	1573)
	(4330,	1593)
	(4370,	1610)
	(4410,	1628)
	(4450,	1657)
	(4490,	1683)
	(4530,	1708)
	(4570,	1730)
	(4610,	1744)
	(4650,	1763)
	(4690,	1774)
	(4703,	1785)
	(4707,	1785)
	(4711,	1785)
	(4715,	1785)
	(4719,	1785)
	(4723,	1786)
	(4727,	1786)
	(4731,	1788)
	(4735,	1788)
	(4739,	1791)
	(4743,	1791)
	(4747,	1791)
	(4751,	1792)
	(4755,	1793)
	(4759,	1793)
	(4763,	1796)
	(4767,	1797)
	(4771,	1800)
	(4775,	1802)
	(4779,	1803)
	(4783,	1805)
	(4787,	1810)
	(4791,	1813)
	(4795,	1818)
	(4799,	1821)
	(4803,	1821)
	(4807,	1822)
	(4811,	1830)
	(4815,	1830)
	(4819,	1831)
	(4823,	1833)
	(4827,	1833)
	(4831,	1839)
	(4835,	1839)
	(4839,	1845)
	(4843,	1847)
	(4847,	1851)
	(4851,	1857)
	(4855,	1859)
	(4859,	1859)
	(4863,	1863)
	(4867,	1865)
	(4871,	1866)
	(4875,	1875)
	(4879,	1876)
	(4883,	1877)
	(4887,	1882)
	(4891,	1884)
	(4895,	1885)
	(4899,	1886)
	(4903,	1887)
	(4907,	1890)
	(4911,	1890)
	(4915,	1894)
	(4919,	1895)
	(4923,	1898)
	(4927,	1903)
	(4931,	1905)
	(4935,	1906)
	(4939,	1905)
	(4943,	1902)
	(4947,	1899)
	(4951,	1897)
	(4955,	1896)
	(4959,	1894)
	(4963,	1895)
	(4967,	1892)
	(4971,	1894)
	(4975,	1892)
	(4979,	1889)
	(4983,	1887)
	(4987,	1883)
	(4991,	1884)
	(4995,	1884)
	(4999,	1884)
	(5003,	1881)
	(5007,	1882)
	(5011,	1880)
	(5015,	1878)
	(5019,	1881)
	(5023,	1882)
	(5027,	1880)
	(5031,	1879)
	(5035,	1877)
	(5039,	1874)
	(5043,	1872)
	(5047,	1869)
	(5051,	1869)
	(5055,	1871)
	(5059,	1869)
	(5063,	1867)
	(5067,	1867)
	(5071,	1864)
	(5075,	1861)
	(5079,	1859)
	(5083,	1857)
	(5087,	1855)
	(5091,	1851)
	(5095,	1849)
	(5099,	1849)
	(5130,	1829)
	(5170,	1809)
	(5210,	1791)
	(5250,	1780)
	(5290,	1760)
	(5330,	1744)
	(5370,	1717)
	(5410,	1702)
	(5450,	1687)
	(5490,	1669)
	(5530,	1652)
	(5570,	1637)
	(5610,	1619)
	(5650,	1600)
	(5690,	1583)
	(5730,	1566)
	(5770,	1547)
	(5810,	1539)
	(5850,	1521)
	(5890,	1501)
	(5930,	1484)
	(5970,	1459)
	(6010,	1438)
	(6050,	1418)
	(6090,	1389)
	(6130,	1366)
	(6170,	1346)
	(6210,	1331)
	(6250,	1314)
	(6290,	1296)
	(6330,	1270)
	(6370,	1240)
	(6410,	1212)
	(6450,	1193)
	(6490,	1177)
	(6530,	1157)
	(6570,	1141)
	(6610,	1125)
	(6650,	1104)
	(6690,	1094)
	(6730,	1076)
	(6770,	1057)
	(6810,	1044)
	(6850,	1021)
	(6890,	1000)
	(6930,	997)
	(6970,	977)
	(7010,	955)
	(7050,	930)
	(7090,	912)
	(7130,	894)
	(7170,	870)
	(7210,	844)
	(7250,	824)
	(7290,	806)
	(7330,	788)
	(7370,	767)
	(7410,	743)
	(7450,	715)
	(7490,	691)
	(7530,	679)
	(7570,	668)
	(7610,	651)
	(7650,	633)
	(7690,	602)
	(7730,	585)
	(7770,	562)
	(7810,	533)
	(7850,	517)
	(7890,	496)
	(7930,	474)
	(7970,	451)
	(8010,	423)
	(8050,	411)
	(8090,	380)
	(8130,	360)
	(8170,	338)
	(8210,	315)
	(8250,	299)
	(8290,	273)
	(8330,	257)
	(8370,	242)
	(8410,	229)
	(8450,	208)
	(8490,	186)
	(8530,	167)
	(8570,	153)
	(8601,	139)
	(8605,	141)
	(8609,	137)
	(8613,	137)
	(8617,	136)
	(8621,	132)
	(8625,	130)
	(8629,	129)
	(8633,	129)
	(8637,	125)
	(8641,	122)
	(8645,	118)
	(8649,	116)
	(8653,	114)
	(8657,	110)
	(8661,	110)
	(8665,	112)
	(8669,	109)
	(8673,	107)
	(8677,	106)
	(8681,	102)
	(8685,	101)
	(8689,	98)
	(8693,	95)
	(8697,	91)
	(8701,	88)
	(8705,	88)
	(8709,	85)
	(8713,	81)
	(8717,	79)
	(8721,	76)
	(8725,	77)
	(8729,	73)
	(8733,	72)
	(8737,	69)
	(8741,	65)
	(8745,	64)
	(8749,	62)
	(8753,	59)
	(8757,	58)
	(8761,	55)
	(8765,	54)
	(8769,	50)
	(8773,	46)
	(8777,	42)
	(8781,	41)
	(8785,	37)
	(8789,	44)
	(8793,	44)
	(8797,	52)
	(8801,	50)
	(8805,	48)
	(8809,	45)
	(8813,	44)
	(8817,	43)
	(8821,	40)
	(8825,	38)
	(8829,	35)
	(8833,	36)
	(8837,	32)
	(8841,	29)
	(8845,	25)
	(8849,	21)
	(8853,	17)
	(8857,	14)
	(8861,	11)
	(8865,	9)
	(8869,	7)
	(8873,	3)
	(8877,	4)
	(8881,	7)
	(8885,	10)
	(8889,	13)
	(8893,	18)
	(8897,	22)
	(8901,	22)
	(8905,	23)
	(8909,	24)
	(8913,	27)
	(8917,	31)
	(8921,	35)
	(8925,	37)
	(8929,	38)
	(8933,	41)
	(8937,	44)
	(8941,	44)
	(8945,	44)
	(8949,	44)
	(8953,	44)
	(8957,	47)
	(8961,	49)
	(8965,	51)
	(8969,	51)
	(8973,	54)
	(8977,	54)
	(8981,	57)
	(8985,	59)
	(8989,	61)
	(8993,	61)
	(8997,	64)
	(9010,	68)
	(9050,	95)
	(9090,	108)
	(9130,	126)
	(9170,	146)
	(9210,	158)
	(9250,	176)
	(9290,	186)
	(9330,	215)
	(9370,	230)
	(9410,	250)
	(9450,	275)
	(9490,	282)
	(9530,	301)
	(9570,	317)
	(9610,	348)
	(9650,	374)
	(9690,	397)
	(9730,	427)
	(9770,	439)
	(9810,	451)
	(9850,	468)
	(9890,	501)
	(9930,	511)
	(9970,	533)
};
\addplot[color=gray] plot coordinates {
	(0,	538)
	(40,	518)
	(80,	505)
	(120,	482)
	(160,	470)
	(200,	442)
	(240,	423)
	(280,	407)
	(320,	387)
	(360,	366)
	(400,	350)
	(440,	332)
	(480,	318)
	(520,	287)
	(560,	267)
	(600,	243)
	(640,	216)
	(680,	189)
	(720,	170)
	(760,	156)
	(800,	141)
	(804,	139)
	(808,	137)
	(812,	136)
	(816,	133)
	(820,	130)
	(824,	133)
	(828,	133)
	(832,	130)
	(836,	130)
	(840,	126)
	(844,	124)
	(848,	122)
	(852,	122)
	(856,	118)
	(860,	114)
	(864,	111)
	(868,	107)
	(872,	104)
	(876,	101)
	(880,	101)
	(884,	98)
	(888,	98)
	(892,	95)
	(896,	92)
	(900,	96)
	(904,	94)
	(908,	93)
	(912,	89)
	(916,	85)
	(920,	82)
	(924,	78)
	(928,	75)
	(932,	72)
	(936,	68)
	(940,	64)
	(944,	61)
	(948,	60)
	(952,	57)
	(956,	53)
	(960,	53)
	(964,	49)
	(968,	45)
	(972,	44)
	(976,	41)
	(980,	38)
	(984,	35)
	(988,	39)
	(992,	37)
	(996,	33)
	(1000,	29)
	(1004,	26)
	(1008,	23)
	(1012,	22)
	(1016,	20)
	(1020,	17)
	(1024,	13)
	(1028,	10)
	(1032,	11)
	(1036,	8)
	(1040,	5)
	(1044,	2)
	(1048,	2)
	(1052,	3)
	(1056,	7)
	(1060,	9)
	(1064,	11)
	(1068,	13)
	(1072,	13)
	(1076,	15)
	(1080,	16)
	(1084,	17)
	(1088,	19)
	(1092,	27)
	(1096,	31)
	(1100,	32)
	(1104,	32)
	(1108,	34)
	(1112,	37)
	(1116,	39)
	(1120,	44)
	(1124,	46)
	(1128,	48)
	(1132,	49)
	(1136,	52)
	(1140,	55)
	(1144,	56)
	(1148,	60)
	(1152,	61)
	(1156,	62)
	(1160,	63)
	(1164,	67)
	(1168,	70)
	(1172,	73)
	(1176,	76)
	(1180,	83)
	(1184,	84)
	(1188,	85)
	(1192,	86)
	(1196,	88)
	(1200,	91)
	(1240,	109)
	(1280,	125)
	(1320,	139)
	(1360,	164)
	(1400,	205)
	(1440,	231)
	(1480,	242)
	(1520,	270)
	(1560,	293)
	(1600,	313)
	(1640,	338)
	(1680,	352)
	(1720,	371)
	(1760,	389)
	(1800,	410)
	(1840,	423)
	(1880,	439)
	(1920,	457)
	(1960,	477)
	(2000,	490)
	(2040,	515)
	(2080,	526)
	(2120,	552)
	(2160,	582)
	(2200,	600)
	(2240,	613)
	(2280,	635)
	(2320,	662)
	(2360,	673)
	(2400,	688)
	(2440,	709)
	(2480,	726)
	(2520,	754)
	(2560,	769)
	(2600,	783)
	(2640,	803)
	(2680,	823)
	(2720,	848)
	(2760,	866)
	(2800,	873)
	(2840,	904)
	(2880,	916)
	(2920,	940)
	(2960,	965)
	(3000,	984)
	(3040,	1005)
	(3080,	1022)
	(3120,	1040)
	(3160,	1056)
	(3200,	1071)
	(3240,	1091)
	(3280,	1120)
	(3320,	1138)
	(3360,	1156)
	(3400,	1181)
	(3440,	1205)
	(3480,	1229)
	(3520,	1239)
	(3560,	1264)
	(3600,	1293)
	(3640,	1310)
	(3680,	1332)
	(3720,	1361)
	(3760,	1377)
	(3800,	1393)
	(3840,	1427)
	(3880,	1443)
	(3920,	1472)
	(3960,	1493)
	(4000,	1512)
	(4040,	1543)
	(4080,	1559)
	(4120,	1586)
	(4160,	1607)
	(4200,	1629)
	(4240,	1647)
	(4280,	1662)
	(4320,	1676)
	(4360,	1689)
	(4400,	1709)
	(4440,	1734)
	(4480,	1750)
	(4520,	1762)
	(4560,	1774)
	(4600,	1794)
	(4640,	1806)
	(4680,	1816)
	(4702,	1829)
	(4706,	1832)
	(4710,	1834)
	(4714,	1835)
	(4718,	1836)
	(4722,	1836)
	(4726,	1841)
	(4730,	1845)
	(4734,	1851)
	(4738,	1852)
	(4742,	1855)
	(4746,	1857)
	(4750,	1859)
	(4754,	1860)
	(4758,	1860)
	(4762,	1860)
	(4766,	1865)
	(4770,	1867)
	(4774,	1867)
	(4778,	1871)
	(4782,	1873)
	(4786,	1877)
	(4790,	1878)
	(4794,	1880)
	(4798,	1882)
	(4802,	1884)
	(4806,	1887)
	(4810,	1889)
	(4814,	1891)
	(4818,	1893)
	(4822,	1896)
	(4826,	1900)
	(4830,	1904)
	(4834,	1908)
	(4838,	1909)
	(4842,	1914)
	(4846,	1914)
	(4850,	1914)
	(4854,	1914)
	(4858,	1915)
	(4862,	1915)
	(4866,	1917)
	(4870,	1917)
	(4874,	1917)
	(4878,	1917)
	(4882,	1922)
	(4886,	1923)
	(4890,	1923)
	(4894,	1925)
	(4898,	1926)
	(4902,	1927)
	(4906,	1929)
	(4910,	1930)
	(4914,	1930)
	(4918,	1930)
	(4922,	1931)
	(4926,	1933)
	(4930,	1935)
	(4934,	1937)
	(4938,	1938)
	(4942,	1934)
	(4946,	1931)
	(4950,	1928)
	(4954,	1924)
	(4958,	1922)
	(4962,	1921)
	(4966,	1917)
	(4970,	1917)
	(4974,	1913)
	(4978,	1911)
	(4982,	1908)
	(4986,	1904)
	(4990,	1903)
	(4994,	1901)
	(4998,	1900)
	(5002,	1898)
	(5006,	1895)
	(5010,	1893)
	(5014,	1894)
	(5018,	1893)
	(5022,	1891)
	(5026,	1890)
	(5030,	1887)
	(5034,	1884)
	(5038,	1883)
	(5042,	1882)
	(5046,	1880)
	(5050,	1878)
	(5054,	1876)
	(5058,	1876)
	(5062,	1872)
	(5066,	1869)
	(5070,	1872)
	(5074,	1868)
	(5078,	1869)
	(5082,	1867)
	(5086,	1866)
	(5090,	1865)
	(5094,	1862)
	(5098,	1861)
	(5120,	1854)
	(5160,	1834)
	(5200,	1815)
	(5240,	1808)
	(5280,	1782)
	(5320,	1759)
	(5360,	1742)
	(5400,	1719)
	(5440,	1693)
	(5480,	1673)
	(5520,	1661)
	(5560,	1637)
	(5600,	1620)
	(5640,	1597)
	(5680,	1573)
	(5720,	1551)
	(5760,	1530)
	(5800,	1506)
	(5840,	1483)
	(5880,	1456)
	(5920,	1431)
	(5960,	1410)
	(6000,	1389)
	(6040,	1382)
	(6080,	1359)
	(6120,	1342)
	(6160,	1329)
	(6200,	1306)
	(6240,	1277)
	(6280,	1259)
	(6320,	1233)
	(6360,	1215)
	(6400,	1194)
	(6440,	1167)
	(6480,	1146)
	(6520,	1128)
	(6560,	1101)
	(6600,	1074)
	(6640,	1059)
	(6680,	1033)
	(6720,	1011)
	(6760,	988)
	(6800,	963)
	(6840,	936)
	(6880,	916)
	(6920,	892)
	(6960,	868)
	(7000,	844)
	(7040,	825)
	(7080,	798)
	(7120,	780)
	(7160,	759)
	(7200,	738)
	(7240,	717)
	(7280,	688)
	(7320,	662)
	(7360,	655)
	(7400,	637)
	(7440,	614)
	(7480,	590)
	(7520,	572)
	(7560,	552)
	(7600,	538)
	(7640,	510)
	(7680,	490)
	(7720,	465)
	(7760,	444)
	(7800,	425)
	(7840,	407)
	(7880,	376)
	(7920,	361)
	(7960,	340)
	(8000,	321)
	(8040,	302)
	(8080,	288)
	(8120,	268)
	(8160,	247)
	(8200,	230)
	(8240,	213)
	(8280,	189)
	(8320,	168)
	(8360,	146)
	(8400,	127)
	(8440,	115)
	(8480,	95)
	(8520,	66)
	(8560,	51)
	(8600,	39)
	(8604,	36)
	(8608,	34)
	(8612,	30)
	(8616,	28)
	(8620,	24)
	(8624,	22)
	(8628,	21)
	(8632,	18)
	(8636,	15)
	(8640,	14)
	(8644,	12)
	(8648,	11)
	(8652,	9)
	(8656,	13)
	(8660,	12)
	(8664,	10)
	(8668,	8)
	(8672,	4)
	(8676,	1)
	(8680,	0)
	(8684,	0)
	(8688,	1)
	(8692,	0)
	(8696,	1)
	(8700,	0)
	(8704,	0)
	(8708,	0)
	(8712,	0)
	(8716,	0)
	(8720,	1)
	(8724,	0)
	(8728,	0)
	(8732,	1)
	(8736,	0)
	(8740,	0)
	(8744,	0)
	(8748,	1)
	(8752,	3)
	(8756,	0)
	(8760,	0)
	(8764,	1)
	(8768,	0)
	(8772,	1)
	(8776,	0)
	(8780,	1)
	(8784,	0)
	(8788,	1)
	(8792,	0)
	(8796,	0)
	(8800,	3)
	(8804,	1)
	(8808,	0)
	(8812,	0)
	(8816,	0)
	(8820,	0)
	(8824,	0)
	(8828,	0)
	(8832,	0)
	(8836,	0)
	(8840,	1)
	(8844,	0)
	(8848,	2)
	(8852,	1)
	(8856,	1)
	(8860,	0)
	(8864,	0)
	(8868,	2)
	(8872,	0)
	(8876,	2)
	(8880,	3)
	(8884,	4)
	(8888,	5)
	(8892,	9)
	(8896,	10)
	(8900,	11)
	(8904,	12)
	(8908,	12)
	(8912,	13)
	(8916,	16)
	(8920,	18)
	(8924,	21)
	(8928,	23)
	(8932,	28)
	(8936,	28)
	(8940,	28)
	(8944,	30)
	(8948,	33)
	(8952,	33)
	(8956,	37)
	(8960,	38)
	(8964,	43)
	(8968,	44)
	(8972,	47)
	(8976,	49)
	(8980,	52)
	(8984,	54)
	(8988,	56)
	(8992,	58)
	(8996,	59)
	(9000,	62)
	(9040,	83)
	(9080,	107)
	(9120,	138)
	(9160,	173)
	(9200,	193)
	(9240,	217)
	(9280,	234)
	(9320,	252)
	(9360,	271)
	(9400,	283)
	(9440,	303)
	(9480,	317)
	(9520,	339)
	(9560,	358)
	(9600,	373)
	(9640,	392)
	(9680,	410)
	(9720,	429)
	(9760,	457)
	(9800,	474)
	(9840,	491)
	(9880,	506)
	(9920,	518)
	(9960,	529)
	(10000,	554)
};

==> fig/zoom1.tex <==
\addplot[color=green, mark=none, line width=10pt, smooth] plot coordinates {
	(800,	66)
	(801,	67)
	(802,	67)
	(803,	67)
	(804,	66)
	(805,	65)
	(806,	64)
	(807,	63)
	(808,	64)
	(809,	63)
	(810,	65)
	(811,	66)
	(812,	66)
	(813,	65)
	(814,	64)
	(815,	63)
	(816,	62)
	(817,	61)
	(818,	60)
	(819,	59)
	(820,	58)
	(821,	57)
	(822,	56)
	(823,	56)
	(824,	57)
	(825,	57)
	(826,	56)
	(827,	55)
	(828,	55)
	(829,	57)
	(830,	56)
	(831,	55)
	(832,	54)
	(833,	53)
	(834,	52)
	(835,	51)
	(836,	50)
	(837,	50)
	(838,	49)
	(839,	50)
	(840,	49)
	(841,	49)
	(842,	50)
	(843,	50)
	(844,	49)
	(845,	51)
	(846,	50)
	(847,	49)
	(848,	48)
	(849,	47)
	(850,	46)
	(851,	47)
	(852,	46)
	(853,	46)
	(854,	48)
	(855,	47)
	(856,	46)
	(857,	45)
	(858,	44)
	(859,	43)
	(860,	42)
	(861,	41)
	(862,	40)
	(863,	39)
	(864,	38)
	(865,	37)
	(866,	36)
	(867,	35)
	(868,	35)
	(869,	34)
	(870,	34)
	(871,	33)
	(872,	32)
	(873,	32)
	(874,	31)
	(875,	31)
	(876,	33)
	(877,	33)
	(878,	32)
	(879,	31)
	(880,	32)
	(881,	31)
	(882,	30)
	(883,	30)
	(884,	29)
	(885,	30)
	(886,	30)
	(887,	29)
	(888,	28)
	(889,	27)
	(890,	26)
	(891,	25)
	(892,	24)
	(893,	24)
	(894,	23)
	(895,	22)
	(896,	21)
	(897,	20)
	(898,	19)
	(899,	19)
	(900,	18)
	(901,	17)
	(902,	16)
	(903,	15)
	(904,	15)
	(905,	14)
	(906,	13)
	(907,	12)
	(908,	11)
	(909,	11)
	(910,	11)
	(911,	12)
	(912,	11)
	(913,	10)
	(914,	9)
	(915,	8)
	(916,	8)
	(917,	7)
	(918,	8)
	(919,	8)
	(920,	7)
	(921,	8)
	(922,	7)
	(923,	6)
	(924,	5)
	(925,	4)
	(926,	4)
	(927,	3)
	(928,	4)
	(929,	3)
	(930,	3)
	(931,	2)
	(932,	2)
	(933,	1)
	(934,	0)
	(935,	0)
	(936,	0)
	(937,	0)
	(938,	1)
	(939,	0)
	(940,	0)
	(941,	0)
	(942,	0)
	(943,	1)
	(944,	1)
	(945,	2)
	(946,	1)
	(947,	1)
	(948,	1)
	(949,	2)
	(950,	1)
	(951,	0)
	(952,	0)
	(953,	0)
	(954,	0)
	(955,	0)
	(956,	0)
	(957,	0)
	(958,	0)
	(959,	0)
	(960,	0)
	(961,	0)
	(962,	0)
	(963,	0)
	(964,	0)
	(965,	0)
	(966,	0)
	(967,	0)
	(968,	0)
	(969,	0)
	(970,	1)
	(971,	1)
	(972,	1)
	(973,	1)
	(974,	1)
	(975,	0)
	(976,	1)
	(977,	0)
	(978,	0)
	(979,	0)
	(980,	0)
	(981,	0)
	(982,	0)
	(983,	1)
	(984,	0)
	(985,	0)
	(986,	0)
	(987,	0)
	(988,	1)
	(989,	1)
	(990,	0)
	(991,	2)
	(992,	1)
	(993,	2)
	(994,	1)
	(995,	1)
	(996,	0)
	(997,	0)
	(998,	1)
	(999,	2)
	(1000,	2)
	(1001,	3)
	(1002,	2)
	(1003,	1)
	(1004,	1)
	(1005,	0)
	(1006,	0)
	(1007,	0)
	(1008,	2)
	(1009,	1)
	(1010,	1)
	(1011,	0)
	(1012,	0)
	(1013,	1)
	(1014,	0)
	(1015,	0)
	(1016,	0)
	(1017,	0)
	(1018,	0)
	(1019,	0)
	(1020,	1)
	(1021,	1)
	(1022,	0)
	(1023,	0)
	(1024,	0)
	(1025,	0)
	(1026,	1)
	(1027,	0)
	(1028,	0)
	(1029,	0)
	(1030,	0)
	(1031,	0)
	(1032,	0)
	(1033,	0)
	(1034,	0)
	(1035,	0)
	(1036,	0)
	(1037,	0)
	(1038,	1)
	(1039,	0)
	(1040,	0)
	(1041,	1)
	(1042,	1)
	(1043,	0)
	(1044,	1)
	(1045,	0)
	(1046,	0)
	(1047,	0)
	(1048,	3)
	(1049,	3)
	(1050,	4)
	(1051,	5)
	(1052,	5)
	(1053,	5)
	(1054,	5)
	(1055,	5)
	(1056,	6)
	(1057,	6)
	(1058,	6)
	(1059,	6)
	(1060,	7)
	(1061,	8)
	(1062,	8)
	(1063,	8)
	(1064,	8)
	(1065,	8)
	(1066,	9)
	(1067,	9)
	(1068,	9)
	(1069,	9)
	(1070,	10)
	(1071,	10)
	(1072,	11)
	(1073,	11)
	(1074,	11)
	(1075,	11)
	(1076,	11)
	(1077,	13)
	(1078,	16)
	(1079,	16)
	(1080,	16)
	(1081,	16)
	(1082,	18)
	(1083,	18)
	(1084,	18)
	(1085,	18)
	(1086,	18)
	(1087,	19)
	(1088,	19)
	(1089,	20)
	(1090,	20)
	(1091,	20)
	(1092,	21)
	(1093,	21)
	(1094,	21)
	(1095,	22)
	(1096,	22)
	(1097,	22)
	(1098,	22)
	(1099,	22)
	(1100,	22)
	(1101,	23)
	(1102,	24)
	(1103,	24)
	(1104,	24)
	(1105,	25)
	(1106,	25)
	(1107,	25)
	(1108,	25)
	(1109,	27)
	(1110,	28)
	(1111,	29)
	(1112,	29)
	(1113,	29)
	(1114,	29)
	(1115,	30)
	(1116,	30)
	(1117,	30)
	(1118,	30)
	(1119,	30)
	(1120,	30)
	(1121,	30)
	(1122,	30)
	(1123,	30)
	(1124,	30)
	(1125,	30)
	(1126,	30)
	(1127,	30)
	(1128,	30)
	(1129,	31)
	(1130,	31)
	(1131,	31)
	(1132,	31)
	(1133,	31)
	(1134,	31)
	(1135,	33)
	(1136,	33)
	(1137,	35)
	(1138,	36)
	(1139,	36)
	(1140,	36)
	(1141,	36)
	(1142,	37)
	(1143,	37)
	(1144,	37)
	(1145,	38)
	(1146,	38)
	(1147,	38)
	(1148,	38)
	(1149,	41)
	(1150,	41)
	(1151,	41)
	(1152,	41)
	(1153,	41)
	(1154,	44)
	(1155,	45)
	(1156,	45)
	(1157,	45)
	(1158,	45)
	(1159,	45)
	(1160,	47)
	(1161,	47)
	(1162,	48)
	(1163,	48)
	(1164,	48)
	(1165,	49)
	(1166,	49)
	(1167,	49)
	(1168,	49)
	(1169,	49)
	(1170,	49)
	(1171,	49)
	(1172,	49)
	(1173,	51)
	(1174,	51)
	(1175,	51)
	(1176,	51)
	(1177,	51)
	(1178,	51)
	(1179,	51)
	(1180,	51)
	(1181,	51)
	(1182,	51)
	(1183,	51)
	(1184,	51)
	(1185,	51)
	(1186,	51)
	(1187,	51)
	(1188,	51)
	(1189,	52)
	(1190,	52)
	(1191,	56)
	(1192,	57)
	(1193,	58)
	(1194,	59)
	(1195,	60)
	(1196,	61)
	(1197,	61)
	(1198,	62)
	(1199,	62)
	(1200,	62)
};
\addplot[color=black, mark=none, line width=10pt, smooth] plot coordinates {
	(800,	141)
	(801,	141)
	(802,	140)
	(803,	140)
	(804,	139)
	(805,	139)
	(806,	139)
	(807,	138)
	(808,	137)
	(809,	138)
	(810,	138)
	(811,	137)
	(812,	136)
	(813,	135)
	(814,	134)
	(815,	133)
	(816,	133)
	(817,	132)
	(818,	131)
	(819,	130)
	(820,	130)
	(821,	133)
	(822,	132)
	(823,	131)
	(824,	133)
	(825,	134)
	(826,	133)
	(827,	132)
	(828,	133)
	(829,	132)
	(830,	132)
	(831,	131)
	(832,	130)
	(833,	131)
	(834,	131)
	(835,	131)
	(836,	130)
	(837,	129)
	(838,	128)
	(839,	127)
	(840,	126)
	(841,	127)
	(842,	126)
	(843,	125)
	(844,	124)
	(845,	123)
	(846,	123)
	(847,	122)
	(848,	122)
	(849,	121)
	(850,	124)
	(851,	123)
	(852,	122)
	(853,	121)
	(854,	120)
	(855,	119)
	(856,	118)
	(857,	117)
	(858,	116)
	(859,	115)
	(860,	114)
	(861,	113)
	(862,	112)
	(863,	112)
	(864,	111)
	(865,	110)
	(866,	109)
	(867,	108)
	(868,	107)
	(869,	106)
	(870,	106)
	(871,	105)
	(872,	104)
	(873,	104)
	(874,	103)
	(875,	102)
	(876,	101)
	(877,	100)
	(878,	99)
	(879,	100)
	(880,	101)
	(881,	101)
	(882,	100)
	(883,	99)
	(884,	98)
	(885,	98)
	(886,	99)
	(887,	98)
	(888,	98)
	(889,	97)
	(890,	97)
	(891,	96)
	(892,	95)
	(893,	95)
	(894,	94)
	(895,	93)
	(896,	92)
	(897,	97)
	(898,	96)
	(899,	97)
	(900,	96)
	(901,	96)
	(902,	95)
	(903,	95)
	(904,	94)
	(905,	93)
	(906,	94)
	(907,	93)
	(908,	93)
	(909,	92)
	(910,	91)
	(911,	90)
	(912,	89)
	(913,	88)
	(914,	87)
	(915,	86)
	(916,	85)
	(917,	84)
	(918,	83)
	(919,	82)
	(920,	82)
	(921,	81)
	(922,	80)
	(923,	79)
	(924,	78)
	(925,	77)
	(926,	76)
	(927,	76)
	(928,	75)
	(929,	75)
	(930,	74)
	(931,	73)
	(932,	72)
	(933,	71)
	(934,	70)
	(935,	69)
	(936,	68)
	(937,	67)
	(938,	66)
	(939,	65)
	(940,	64)
	(941,	63)
	(942,	62)
	(943,	62)
	(944,	61)
	(945,	60)
	(946,	60)
	(947,	61)
	(948,	60)
	(949,	59)
	(950,	58)
	(951,	57)
	(952,	57)
	(953,	56)
	(954,	55)
	(955,	54)
	(956,	53)
	(957,	55)
	(958,	54)
	(959,	53)
	(960,	53)
	(961,	52)
	(962,	51)
	(963,	50)
	(964,	49)
	(965,	48)
	(966,	47)
	(967,	46)
	(968,	45)
	(969,	44)
	(970,	45)
	(971,	45)
	(972,	44)
	(973,	43)
	(974,	42)
	(975,	42)
	(976,	41)
	(977,	40)
	(978,	40)
	(979,	39)
	(980,	38)
	(981,	37)
	(982,	37)
	(983,	36)
	(984,	35)
	(985,	36)
	(986,	39)
	(987,	40)
	(988,	39)
	(989,	38)
	(990,	37)
	(991,	38)
	(992,	37)
	(993,	36)
	(994,	35)
	(995,	34)
	(996,	33)
	(997,	32)
	(998,	31)
	(999,	30)
	(1000,	29)
	(1001,	28)
	(1002,	27)
	(1003,	27)
	(1004,	26)
	(1005,	25)
	(1006,	24)
	(1007,	24)
	(1008,	23)
	(1009,	23)
	(1010,	23)
	(1011,	23)
	(1012,	22)
	(1013,	22)
	(1014,	21)
	(1015,	21)
	(1016,	20)
	(1017,	20)
	(1018,	19)
	(1019,	18)
	(1020,	17)
	(1021,	16)
	(1022,	15)
	(1023,	14)
	(1024,	13)
	(1025,	12)
	(1026,	11)
	(1027,	10)
	(1028,	10)
	(1029,	11)
	(1030,	11)
	(1031,	12)
	(1032,	11)
	(1033,	10)
	(1034,	9)
	(1035,	9)
	(1036,	8)
	(1037,	8)
	(1038,	7)
	(1039,	6)
	(1040,	5)
	(1041,	5)
	(1042,	4)
	(1043,	3)
	(1044,	2)
	(1045,	1)
	(1046,	0)
	(1047,	2)
	(1048,	2)
	(1049,	2)
	(1050,	2)
	(1051,	2)
	(1052,	3)
	(1053,	4)
	(1054,	5)
	(1055,	6)
	(1056,	7)
	(1057,	7)
	(1058,	7)
	(1059,	7)
	(1060,	9)
	(1061,	11)
	(1062,	11)
	(1063,	11)
	(1064,	11)
	(1065,	12)
	(1066,	12)
	(1067,	13)
	(1068,	13)
	(1069,	13)
	(1070,	13)
	(1071,	13)
	(1072,	13)
	(1073,	13)
	(1074,	13)
	(1075,	15)
	(1076,	15)
	(1077,	15)
	(1078,	16)
	(1079,	16)
	(1080,	16)
	(1081,	17)
	(1082,	17)
	(1083,	17)
	(1084,	17)
	(1085,	17)
	(1086,	19)
	(1087,	19)
	(1088,	19)
	(1089,	21)
	(1090,	21)
	(1091,	26)
	(1092,	27)
	(1093,	28)
	(1094,	28)
	(1095,	30)
	(1096,	31)
	(1097,	31)
	(1098,	31)
	(1099,	32)
	(1100,	32)
	(1101,	32)
	(1102,	32)
	(1103,	32)
	(1104,	32)
	(1105,	32)
	(1106,	32)
	(1107,	33)
	(1108,	34)
	(1109,	34)
	(1110,	34)
	(1111,	36)
	(1112,	37)
	(1113,	38)
	(1114,	38)
	(1115,	39)
	(1116,	39)
	(1117,	41)
	(1118,	41)
	(1119,	42)
	(1120,	44)
	(1121,	44)
	(1122,	45)
	(1123,	46)
	(1124,	46)
	(1125,	46)
	(1126,	46)
	(1127,	46)
	(1128,	48)
	(1129,	48)
	(1130,	48)
	(1131,	49)
	(1132,	49)
	(1133,	49)
	(1134,	49)
	(1135,	52)
	(1136,	52)
	(1137,	52)
	(1138,	52)
	(1139,	54)
	(1140,	55)
	(1141,	55)
	(1142,	55)
	(1143,	56)
	(1144,	56)
	(1145,	58)
	(1146,	58)
	(1147,	59)
	(1148,	60)
	(1149,	60)
	(1150,	61)
	(1151,	61)
	(1152,	61)
	(1153,	61)
	(1154,	61)
	(1155,	61)
	(1156,	62)
	(1157,	63)
	(1158,	63)
	(1159,	63)
	(1160,	63)
	(1161,	64)
	(1162,	66)
	(1163,	66)
	(1164,	67)
	(1165,	67)
	(1166,	67)
	(1167,	68)
	(1168,	70)
	(1169,	72)
	(1170,	72)
	(1171,	73)
	(1172,	73)
	(1173,	73)
	(1174,	75)
	(1175,	76)
	(1176,	76)
	(1177,	79)
	(1178,	79)
	(1179,	82)
	(1180,	83)
	(1181,	84)
	(1182,	84)
	(1183,	84)
	(1184,	84)
	(1185,	84)
	(1186,	84)
	(1187,	84)
	(1188,	85)
	(1189,	85)
	(1190,	85)
	(1191,	85)
	(1192,	86)
	(1193,	86)
	(1194,	86)
	(1195,	86)
	(1196,	88)
	(1197,	89)
	(1198,	91)
	(1199,	91)
	(1200,	91)
};

==> fig/zoom2.tex <==
\addplot[color=red, mark=none, line width=10pt, smooth] plot coordinates {
	(4700,	66)
	(4701,	66)
	(4702,	65)
	(4703,	66)
	(4704,	65)
	(4705,	64)
	(4706,	63)
	(4707,	62)
	(4708,	61)
	(4709,	61)
	(4710,	62)
	(4711,	62)
	(4712,	61)
	(4713,	61)
	(4714,	61)
	(4715,	60)
	(4716,	59)
	(4717,	58)
	(4718,	57)
	(4719,	57)
	(4720,	56)
	(4721,	55)
	(4722,	54)
	(4723,	57)
	(4724,	57)
	(4725,	57)
	(4726,	57)
	(4727,	57)
	(4728,	56)
	(4729,	55)
	(4730,	54)
	(4731,	53)
	(4732,	52)
	(4733,	53)
	(4734,	52)
	(4735,	52)
	(4736,	52)
	(4737,	51)
	(4738,	50)
	(4739,	49)
	(4740,	48)
	(4741,	47)
	(4742,	46)
	(4743,	48)
	(4744,	47)
	(4745,	46)
	(4746,	45)
	(4747,	44)
	(4748,	43)
	(4749,	42)
	(4750,	42)
	(4751,	41)
	(4752,	41)
	(4753,	40)
	(4754,	40)
	(4755,	40)
	(4756,	40)
	(4757,	40)
	(4758,	39)
	(4759,	39)
	(4760,	39)
	(4761,	38)
	(4762,	37)
	(4763,	36)
	(4764,	35)
	(4765,	35)
	(4766,	34)
	(4767,	34)
	(4768,	35)
	(4769,	34)
	(4770,	33)
	(4771,	34)
	(4772,	34)
	(4773,	33)
	(4774,	35)
	(4775,	35)
	(4776,	34)
	(4777,	35)
	(4778,	35)
	(4779,	34)
	(4780,	33)
	(4781,	34)
	(4782,	33)
	(4783,	32)
	(4784,	32)
	(4785,	32)
	(4786,	31)
	(4787,	30)
	(4788,	29)
	(4789,	30)
	(4790,	31)
	(4791,	31)
	(4792,	30)
	(4793,	30)
	(4794,	29)
	(4795,	28)
	(4796,	27)
	(4797,	26)
	(4798,	25)
	(4799,	24)
	(4800,	23)
	(4801,	22)
	(4802,	21)
	(4803,	20)
	(4804,	19)
	(4805,	18)
	(4806,	17)
	(4807,	16)
	(4808,	15)
	(4809,	14)
	(4810,	13)
	(4811,	12)
	(4812,	12)
	(4813,	11)
	(4814,	11)
	(4815,	10)
	(4816,	9)
	(4817,	9)
	(4818,	9)
	(4819,	8)
	(4820,	7)
	(4821,	7)
	(4822,	6)
	(4823,	5)
	(4824,	4)
	(4825,	3)
	(4826,	5)
	(4827,	5)
	(4828,	4)
	(4829,	3)
	(4830,	2)
	(4831,	1)
	(4832,	1)
	(4833,	1)
	(4834,	2)
	(4835,	1)
	(4836,	2)
	(4837,	3)
	(4838,	2)
	(4839,	1)
	(4840,	0)
	(4841,	0)
	(4842,	0)
	(4843,	0)
	(4844,	0)
	(4845,	0)
	(4846,	1)
	(4847,	0)
	(4848,	0)
	(4849,	0)
	(4850,	0)
	(4851,	0)
	(4852,	0)
	(4853,	0)
	(4854,	0)
	(4855,	0)
	(4856,	0)
	(4857,	2)
	(4858,	1)
	(4859,	0)
	(4860,	0)
	(4861,	0)
	(4862,	0)
	(4863,	0)
	(4864,	0)
	(4865,	0)
	(4866,	0)
	(4867,	0)
	(4868,	2)
	(4869,	1)
	(4870,	1)
	(4871,	0)
	(4872,	0)
	(4873,	0)
	(4874,	0)
	(4875,	0)
	(4876,	0)
	(4877,	0)
	(4878,	0)
	(4879,	1)
	(4880,	3)
	(4881,	2)
	(4882,	2)
	(4883,	3)
	(4884,	2)
	(4885,	2)
	(4886,	1)
	(4887,	0)
	(4888,	0)
	(4889,	0)
	(4890,	0)
	(4891,	0)
	(4892,	0)
	(4893,	0)
	(4894,	0)
	(4895,	0)
	(4896,	1)
	(4897,	0)
	(4898,	0)
	(4899,	0)
	(4900,	1)
	(4901,	0)
	(4902,	0)
	(4903,	0)
	(4904,	2)
	(4905,	1)
	(4906,	1)
	(4907,	0)
	(4908,	0)
	(4909,	0)
	(4910,	0)
	(4911,	0)
	(4912,	2)
	(4913,	1)
	(4914,	0)
	(4915,	0)
	(4916,	0)
	(4917,	0)
	(4918,	0)
	(4919,	0)
	(4920,	0)
	(4921,	2)
	(4922,	1)
	(4923,	0)
	(4924,	0)
	(4925,	0)
	(4926,	0)
	(4927,	0)
	(4928,	1)
	(4929,	0)
	(4930,	0)
	(4931,	0)
	(4932,	0)
	(4933,	0)
	(4934,	0)
	(4935,	1)
	(4936,	2)
	(4937,	2)
	(4938,	2)
	(4939,	2)
	(4940,	4)
	(4941,	4)
	(4942,	5)
	(4943,	5)
	(4944,	5)
	(4945,	6)
	(4946,	6)
	(4947,	6)
	(4948,	7)
	(4949,	8)
	(4950,	9)
	(4951,	9)
	(4952,	9)
	(4953,	9)
	(4954,	11)
	(4955,	14)
	(4956,	15)
	(4957,	16)
	(4958,	16)
	(4959,	19)
	(4960,	20)
	(4961,	21)
	(4962,	21)
	(4963,	24)
	(4964,	26)
	(4965,	26)
	(4966,	26)
	(4967,	27)
	(4968,	27)
	(4969,	27)
	(4970,	27)
	(4971,	28)
	(4972,	30)
	(4973,	30)
	(4974,	30)
	(4975,	30)
	(4976,	30)
	(4977,	30)
	(4978,	30)
	(4979,	30)
	(4980,	30)
	(4981,	30)
	(4982,	30)
	(4983,	30)
	(4984,	31)
	(4985,	31)
	(4986,	31)
	(4987,	32)
	(4988,	32)
	(4989,	32)
	(4990,	32)
	(4991,	32)
	(4992,	32)
	(4993,	32)
	(4994,	33)
	(4995,	33)
	(4996,	33)
	(4997,	33)
	(4998,	35)
	(4999,	38)
	(5000,	39)
	(5001,	39)
	(5002,	39)
	(5003,	40)
	(5004,	40)
	(5005,	40)
	(5006,	41)
	(5007,	41)
	(5008,	42)
	(5009,	42)
	(5010,	42)
	(5011,	42)
	(5012,	42)
	(5013,	42)
	(5014,	42)
	(5015,	42)
	(5016,	42)
	(5017,	43)
	(5018,	43)
	(5019,	43)
	(5020,	43)
	(5021,	43)
	(5022,	43)
	(5023,	46)
	(5024,	46)
	(5025,	47)
	(5026,	47)
	(5027,	47)
	(5028,	47)
	(5029,	47)
	(5030,	47)
	(5031,	47)
	(5032,	47)
	(5033,	50)
	(5034,	52)
	(5035,	54)
	(5036,	54)
	(5037,	58)
	(5038,	58)
	(5039,	58)
	(5040,	58)
	(5041,	58)
	(5042,	58)
	(5043,	58)
	(5044,	58)
	(5045,	58)
	(5046,	60)
	(5047,	62)
	(5048,	62)
	(5049,	62)
	(5050,	62)
	(5051,	62)
	(5052,	62)
	(5053,	62)
	(5054,	62)
	(5055,	62)
	(5056,	66)
	(5057,	69)
	(5058,	69)
	(5059,	69)
	(5060,	69)
	(5061,	70)
	(5062,	70)
	(5063,	70)
	(5064,	70)
	(5065,	70)
	(5066,	70)
	(5067,	71)
	(5068,	71)
	(5069,	73)
	(5070,	75)
	(5071,	75)
	(5072,	75)
	(5073,	76)
	(5074,	76)
	(5075,	76)
	(5076,	76)
	(5077,	76)
	(5078,	76)
	(5079,	76)
	(5080,	76)
	(5081,	76)
	(5082,	76)
	(5083,	76)
	(5084,	76)
	(5085,	78)
	(5086,	79)
	(5087,	79)
	(5088,	80)
	(5089,	80)
	(5090,	80)
	(5091,	81)
	(5092,	83)
	(5093,	83)
	(5094,	83)
	(5095,	83)
	(5096,	83)
	(5097,	83)
	(5098,	83)
	(5099,	84)
	(5100,	84)
};
\addplot[color=blue, mark=none, line width=10pt, smooth] plot coordinates {
	(4700,	125)
	(4701,	124)
	(4702,	123)
	(4703,	123)
	(4704,	122)
	(4705,	123)
	(4706,	122)
	(4707,	121)
	(4708,	120)
	(4709,	120)
	(4710,	123)
	(4711,	122)
	(4712,	121)
	(4713,	120)
	(4714,	120)
	(4715,	121)
	(4716,	120)
	(4717,	119)
	(4718,	118)
	(4719,	118)
	(4720,	117)
	(4721,	116)
	(4722,	115)
	(4723,	115)
	(4724,	114)
	(4725,	113)
	(4726,	112)
	(4727,	111)
	(4728,	111)
	(4729,	110)
	(4730,	111)
	(4731,	110)
	(4732,	111)
	(4733,	110)
	(4734,	110)
	(4735,	109)
	(4736,	108)
	(4737,	107)
	(4738,	106)
	(4739,	105)
	(4740,	104)
	(4741,	106)
	(4742,	106)
	(4743,	105)
	(4744,	108)
	(4745,	107)
	(4746,	106)
	(4747,	105)
	(4748,	104)
	(4749,	103)
	(4750,	102)
	(4751,	105)
	(4752,	105)
	(4753,	104)
	(4754,	106)
	(4755,	106)
	(4756,	108)
	(4757,	107)
	(4758,	107)
	(4759,	106)
	(4760,	105)
	(4761,	109)
	(4762,	108)
	(4763,	107)
	(4764,	106)
	(4765,	106)
	(4766,	105)
	(4767,	105)
	(4768,	104)
	(4769,	103)
	(4770,	103)
	(4771,	102)
	(4772,	101)
	(4773,	100)
	(4774,	99)
	(4775,	99)
	(4776,	99)
	(4777,	98)
	(4778,	97)
	(4779,	98)
	(4780,	98)
	(4781,	97)
	(4782,	96)
	(4783,	95)
	(4784,	94)
	(4785,	94)
	(4786,	94)
	(4787,	93)
	(4788,	92)
	(4789,	92)
	(4790,	92)
	(4791,	91)
	(4792,	92)
	(4793,	91)
	(4794,	90)
	(4795,	90)
	(4796,	91)
	(4797,	91)
	(4798,	90)
	(4799,	89)
	(4800,	90)
	(4801,	90)
	(4802,	89)
	(4803,	89)
	(4804,	88)
	(4805,	87)
	(4806,	88)
	(4807,	87)
	(4808,	86)
	(4809,	85)
	(4810,	85)
	(4811,	84)
	(4812,	83)
	(4813,	82)
	(4814,	81)
	(4815,	81)
	(4816,	81)
	(4817,	80)
	(4818,	79)
	(4819,	78)
	(4820,	77)
	(4821,	76)
	(4822,	75)
	(4823,	75)
	(4824,	74)
	(4825,	74)
	(4826,	73)
	(4827,	72)
	(4828,	73)
	(4829,	72)
	(4830,	71)
	(4831,	70)
	(4832,	70)
	(4833,	69)
	(4834,	68)
	(4835,	68)
	(4836,	67)
	(4837,	66)
	(4838,	65)
	(4839,	64)
	(4840,	63)
	(4841,	62)
	(4842,	61)
	(4843,	61)
	(4844,	60)
	(4845,	59)
	(4846,	58)
	(4847,	58)
	(4848,	57)
	(4849,	59)
	(4850,	58)
	(4851,	57)
	(4852,	56)
	(4853,	55)
	(4854,	54)
	(4855,	54)
	(4856,	53)
	(4857,	52)
	(4858,	51)
	(4859,	50)
	(4860,	49)
	(4861,	48)
	(4862,	47)
	(4863,	46)
	(4864,	45)
	(4865,	44)
	(4866,	43)
	(4867,	42)
	(4868,	41)
	(4869,	40)
	(4870,	39)
	(4871,	38)
	(4872,	37)
	(4873,	36)
	(4874,	35)
	(4875,	34)
	(4876,	33)
	(4877,	34)
	(4878,	34)
	(4879,	33)
	(4880,	32)
	(4881,	31)
	(4882,	30)
	(4883,	29)
	(4884,	28)
	(4885,	30)
	(4886,	29)
	(4887,	28)
	(4888,	27)
	(4889,	26)
	(4890,	25)
	(4891,	24)
	(4892,	23)
	(4893,	23)
	(4894,	22)
	(4895,	21)
	(4896,	20)
	(4897,	19)
	(4898,	18)
	(4899,	17)
	(4900,	17)
	(4901,	16)
	(4902,	15)
	(4903,	14)
	(4904,	13)
	(4905,	12)
	(4906,	11)
	(4907,	10)
	(4908,	11)
	(4909,	10)
	(4910,	9)
	(4911,	8)
	(4912,	8)
	(4913,	10)
	(4914,	9)
	(4915,	8)
	(4916,	7)
	(4917,	6)
	(4918,	5)
	(4919,	5)
	(4920,	5)
	(4921,	5)
	(4922,	4)
	(4923,	3)
	(4924,	4)
	(4925,	4)
	(4926,	5)
	(4927,	4)
	(4928,	3)
	(4929,	2)
	(4930,	2)
	(4931,	2)
	(4932,	2)
	(4933,	1)
	(4934,	0)
	(4935,	0)
	(4936,	2)
	(4937,	2)
	(4938,	3)
	(4939,	3)
	(4940,	3)
	(4941,	4)
	(4942,	5)
	(4943,	5)
	(4944,	5)
	(4945,	7)
	(4946,	7)
	(4947,	8)
	(4948,	10)
	(4949,	10)
	(4950,	10)
	(4951,	10)
	(4952,	11)
	(4953,	11)
	(4954,	11)
	(4955,	12)
	(4956,	12)
	(4957,	12)
	(4958,	12)
	(4959,	12)
	(4960,	12)
	(4961,	12)
	(4962,	12)
	(4963,	14)
	(4964,	15)
	(4965,	15)
	(4966,	15)
	(4967,	17)
	(4968,	22)
	(4969,	23)
	(4970,	25)
	(4971,	25)
	(4972,	26)
	(4973,	26)
	(4974,	28)
	(4975,	31)
	(4976,	31)
	(4977,	31)
	(4978,	31)
	(4979,	31)
	(4980,	31)
	(4981,	31)
	(4982,	31)
	(4983,	32)
	(4984,	32)
	(4985,	32)
	(4986,	32)
	(4987,	32)
	(4988,	35)
	(4989,	35)
	(4990,	35)
	(4991,	35)
	(4992,	35)
	(4993,	36)
	(4994,	37)
	(4995,	37)
	(4996,	37)
	(4997,	37)
	(4998,	37)
	(4999,	37)
	(5000,	40)
	(5001,	40)
	(5002,	42)
	(5003,	42)
	(5004,	42)
	(5005,	42)
	(5006,	43)
	(5007,	43)
	(5008,	43)
	(5009,	43)
	(5010,	46)
	(5011,	46)
	(5012,	46)
	(5013,	46)
	(5014,	47)
	(5015,	48)
	(5016,	49)
	(5017,	50)
	(5018,	50)
	(5019,	52)
	(5020,	52)
	(5021,	53)
	(5022,	53)
	(5023,	54)
	(5024,	54)
	(5025,	55)
	(5026,	55)
	(5027,	55)
	(5028,	55)
	(5029,	55)
	(5030,	55)
	(5031,	55)
	(5032,	56)
	(5033,	57)
	(5034,	57)
	(5035,	57)
	(5036,	58)
	(5037,	58)
	(5038,	59)
	(5039,	59)
	(5040,	59)
	(5041,	60)
	(5042,	60)
	(5043,	61)
	(5044,	61)
	(5045,	61)
	(5046,	62)
	(5047,	62)
	(5048,	64)
	(5049,	65)
	(5050,	66)
	(5051,	67)
	(5052,	68)
	(5053,	68)
	(5054,	68)
	(5055,	68)
	(5056,	69)
	(5057,	70)
	(5058,	71)
	(5059,	72)
	(5060,	73)
	(5061,	73)
	(5062,	73)
	(5063,	74)
	(5064,	74)
	(5065,	75)
	(5066,	75)
	(5067,	75)
	(5068,	75)
	(5069,	77)
	(5070,	78)
	(5071,	78)
	(5072,	79)
	(5073,	79)
	(5074,	80)
	(5075,	80)
	(5076,	80)
	(5077,	80)
	(5078,	80)
	(5079,	80)
	(5080,	80)
	(5081,	81)
	(5082,	81)
	(5083,	81)
	(5084,	81)
	(5085,	81)
	(5086,	81)
	(5087,	82)
	(5088,	82)
	(5089,	82)
	(5090,	82)
	(5091,	82)
	(5092,	82)
	(5093,	85)
	(5094,	85)
	(5095,	86)
	(5096,	86)
	(5097,	87)
	(5098,	89)
	(5099,	89)
	(5100,	89)
};

==> fig/zoom3.tex <==
\addplot[color=green, mark=none, line width=10pt, smooth] plot coordinates {
	(8600,	139)
	(8601,	139)
	(8602,	140)
	(8603,	141)
	(8604,	141)
	(8605,	141)
	(8606,	140)
	(8607,	139)
	(8608,	138)
	(8609,	137)
	(8610,	138)
	(8611,	138)
	(8612,	138)
	(8613,	137)
	(8614,	136)
	(8615,	135)
	(8616,	137)
	(8617,	136)
	(8618,	135)
	(8619,	134)
	(8620,	133)
	(8621,	132)
	(8622,	131)
	(8623,	130)
	(8624,	130)
	(8625,	130)
	(8626,	129)
	(8627,	129)
	(8628,	130)
	(8629,	129)
	(8630,	128)
	(8631,	127)
	(8632,	129)
	(8633,	129)
	(8634,	128)
	(8635,	127)
	(8636,	126)
	(8637,	125)
	(8638,	124)
	(8639,	123)
	(8640,	123)
	(8641,	122)
	(8642,	121)
	(8643,	120)
	(8644,	119)
	(8645,	118)
	(8646,	117)
	(8647,	118)
	(8648,	117)
	(8649,	116)
	(8650,	115)
	(8651,	115)
	(8652,	114)
	(8653,	114)
	(8654,	113)
	(8655,	112)
	(8656,	111)
	(8657,	110)
	(8658,	112)
	(8659,	111)
	(8660,	111)
	(8661,	110)
	(8662,	111)
	(8663,	111)
	(8664,	110)
	(8665,	112)
	(8666,	112)
	(8667,	111)
	(8668,	110)
	(8669,	109)
	(8670,	108)
	(8671,	107)
	(8672,	108)
	(8673,	107)
	(8674,	109)
	(8675,	108)
	(8676,	107)
	(8677,	106)
	(8678,	105)
	(8679,	104)
	(8680,	103)
	(8681,	102)
	(8682,	101)
	(8683,	101)
	(8684,	100)
	(8685,	101)
	(8686,	101)
	(8687,	100)
	(8688,	99)
	(8689,	98)
	(8690,	98)
	(8691,	97)
	(8692,	96)
	(8693,	95)
	(8694,	94)
	(8695,	93)
	(8696,	92)
	(8697,	91)
	(8698,	90)
	(8699,	89)
	(8700,	89)
	(8701,	88)
	(8702,	87)
	(8703,	86)
	(8704,	85)
	(8705,	88)
	(8706,	87)
	(8707,	87)
	(8708,	86)
	(8709,	85)
	(8710,	84)
	(8711,	83)
	(8712,	82)
	(8713,	81)
	(8714,	80)
	(8715,	80)
	(8716,	79)
	(8717,	79)
	(8718,	78)
	(8719,	77)
	(8720,	76)
	(8721,	76)
	(8722,	75)
	(8723,	75)
	(8724,	76)
	(8725,	77)
	(8726,	76)
	(8727,	75)
	(8728,	74)
	(8729,	73)
	(8730,	72)
	(8731,	71)
	(8732,	72)
	(8733,	72)
	(8734,	71)
	(8735,	71)
	(8736,	70)
	(8737,	69)
	(8738,	68)
	(8739,	67)
	(8740,	66)
	(8741,	65)
	(8742,	65)
	(8743,	66)
	(8744,	65)
	(8745,	64)
	(8746,	63)
	(8747,	62)
	(8748,	63)
	(8749,	62)
	(8750,	61)
	(8751,	60)
	(8752,	59)
	(8753,	59)
	(8754,	58)
	(8755,	58)
	(8756,	59)
	(8757,	58)
	(8758,	58)
	(8759,	57)
	(8760,	56)
	(8761,	55)
	(8762,	54)
	(8763,	56)
	(8764,	55)
	(8765,	54)
	(8766,	53)
	(8767,	52)
	(8768,	51)
	(8769,	50)
	(8770,	49)
	(8771,	48)
	(8772,	47)
	(8773,	46)
	(8774,	45)
	(8775,	44)
	(8776,	43)
	(8777,	42)
	(8778,	41)
	(8779,	40)
	(8780,	39)
	(8781,	41)
	(8782,	40)
	(8783,	39)
	(8784,	38)
	(8785,	37)
	(8786,	39)
	(8787,	44)
	(8788,	43)
	(8789,	44)
	(8790,	45)
	(8791,	44)
	(8792,	44)
	(8793,	44)
	(8794,	43)
	(8795,	49)
	(8796,	51)
	(8797,	52)
	(8798,	51)
	(8799,	52)
	(8800,	51)
	(8801,	50)
	(8802,	49)
	(8803,	48)
	(8804,	48)
	(8805,	48)
	(8806,	47)
	(8807,	46)
	(8808,	45)
	(8809,	45)
	(8810,	44)
	(8811,	46)
	(8812,	45)
	(8813,	44)
	(8814,	45)
	(8815,	45)
	(8816,	44)
	(8817,	43)
	(8818,	42)
	(8819,	41)
	(8820,	41)
	(8821,	40)
	(8822,	39)
	(8823,	38)
	(8824,	37)
	(8825,	38)
	(8826,	37)
	(8827,	37)
	(8828,	36)
	(8829,	35)
	(8830,	34)
	(8831,	35)
	(8832,	37)
	(8833,	36)
	(8834,	35)
	(8835,	34)
	(8836,	33)
	(8837,	32)
	(8838,	32)
	(8839,	31)
	(8840,	30)
	(8841,	29)
	(8842,	28)
	(8843,	27)
	(8844,	26)
	(8845,	25)
	(8846,	24)
	(8847,	23)
	(8848,	22)
	(8849,	21)
	(8850,	20)
	(8851,	19)
	(8852,	18)
	(8853,	17)
	(8854,	16)
	(8855,	16)
	(8856,	15)
	(8857,	14)
	(8858,	13)
	(8859,	13)
	(8860,	12)
	(8861,	11)
	(8862,	11)
	(8863,	11)
	(8864,	10)
	(8865,	9)
	(8866,	9)
	(8867,	9)
	(8868,	8)
	(8869,	7)
	(8870,	6)
	(8871,	5)
	(8872,	4)
	(8873,	3)
	(8874,	3)
	(8875,	4)
	(8876,	4)
	(8877,	4)
	(8878,	5)
	(8879,	5)
	(8880,	7)
	(8881,	7)
	(8882,	8)
	(8883,	10)
	(8884,	10)
	(8885,	10)
	(8886,	10)
	(8887,	10)
	(8888,	13)
	(8889,	13)
	(8890,	15)
	(8891,	17)
	(8892,	18)
	(8893,	18)
	(8894,	19)
	(8895,	19)
	(8896,	19)
	(8897,	22)
	(8898,	22)
	(8899,	22)
	(8900,	22)
	(8901,	22)
	(8902,	23)
	(8903,	23)
	(8904,	23)
	(8905,	23)
	(8906,	23)
	(8907,	23)
	(8908,	23)
	(8909,	24)
	(8910,	26)
	(8911,	26)
	(8912,	27)
	(8913,	27)
	(8914,	29)
	(8915,	31)
	(8916,	31)
	(8917,	31)
	(8918,	32)
	(8919,	32)
	(8920,	33)
	(8921,	35)
	(8922,	37)
	(8923,	37)
	(8924,	37)
	(8925,	37)
	(8926,	37)
	(8927,	38)
	(8928,	38)
	(8929,	38)
	(8930,	39)
	(8931,	41)
	(8932,	41)
	(8933,	41)
	(8934,	43)
	(8935,	43)
	(8936,	43)
	(8937,	44)
	(8938,	44)
	(8939,	44)
	(8940,	44)
	(8941,	44)
	(8942,	44)
	(8943,	44)
	(8944,	44)
	(8945,	44)
	(8946,	44)
	(8947,	44)
	(8948,	44)
	(8949,	44)
	(8950,	44)
	(8951,	44)
	(8952,	44)
	(8953,	44)
	(8954,	44)
	(8955,	44)
	(8956,	45)
	(8957,	47)
	(8958,	49)
	(8959,	49)
	(8960,	49)
	(8961,	49)
	(8962,	49)
	(8963,	49)
	(8964,	50)
	(8965,	51)
	(8966,	51)
	(8967,	51)
	(8968,	51)
	(8969,	51)
	(8970,	51)
	(8971,	54)
	(8972,	54)
	(8973,	54)
	(8974,	54)
	(8975,	54)
	(8976,	54)
	(8977,	54)
	(8978,	55)
	(8979,	56)
	(8980,	57)
	(8981,	57)
	(8982,	58)
	(8983,	58)
	(8984,	59)
	(8985,	59)
	(8986,	59)
	(8987,	59)
	(8988,	60)
	(8989,	61)
	(8990,	61)
	(8991,	61)
	(8992,	61)
	(8993,	61)
	(8994,	61)
	(8995,	62)
	(8996,	63)
	(8997,	64)
	(8998,	64)
	(8999,	64)
	(9000,	64)
};
\addplot[color=black, mark=none, line width=10pt, smooth] plot coordinates {
	(8600,	39)
	(8601,	38)
	(8602,	37)
	(8603,	36)
	(8604,	36)
	(8605,	35)
	(8606,	35)
	(8607,	35)
	(8608,	34)
	(8609,	33)
	(8610,	32)
	(8611,	31)
	(8612,	30)
	(8613,	29)
	(8614,	29)
	(8615,	29)
	(8616,	28)
	(8617,	27)
	(8618,	26)
	(8619,	25)
	(8620,	24)
	(8621,	23)
	(8622,	22)
	(8623,	23)
	(8624,	22)
	(8625,	24)
	(8626,	23)
	(8627,	22)
	(8628,	21)
	(8629,	20)
	(8630,	20)
	(8631,	19)
	(8632,	18)
	(8633,	17)
	(8634,	16)
	(8635,	16)
	(8636,	15)
	(8637,	15)
	(8638,	15)
	(8639,	15)
	(8640,	14)
	(8641,	13)
	(8642,	12)
	(8643,	11)
	(8644,	12)
	(8645,	11)
	(8646,	11)
	(8647,	11)
	(8648,	11)
	(8649,	12)
	(8650,	11)
	(8651,	10)
	(8652,	9)
	(8653,	9)
	(8654,	9)
	(8655,	14)
	(8656,	13)
	(8657,	12)
	(8658,	11)
	(8659,	10)
	(8660,	12)
	(8661,	11)
	(8662,	10)
	(8663,	9)
	(8664,	10)
	(8665,	9)
	(8666,	8)
	(8667,	7)
	(8668,	8)
	(8669,	7)
	(8670,	6)
	(8671,	5)
	(8672,	4)
	(8673,	3)
	(8674,	2)
	(8675,	1)
	(8676,	1)
	(8677,	1)
	(8678,	0)
	(8679,	0)
	(8680,	0)
	(8681,	0)
	(8682,	0)
	(8683,	0)
	(8684,	0)
	(8685,	0)
	(8686,	0)
	(8687,	0)
	(8688,	1)
	(8689,	1)
	(8690,	1)
	(8691,	1)
	(8692,	0)
	(8693,	0)
	(8694,	0)
	(8695,	1)
	(8696,	1)
	(8697,	1)
	(8698,	1)
	(8699,	0)
	(8700,	0)
	(8701,	0)
	(8702,	0)
	(8703,	0)
	(8704,	0)
	(8705,	0)
	(8706,	0)
	(8707,	0)
	(8708,	0)
	(8709,	1)
	(8710,	0)
	(8711,	0)
	(8712,	0)
	(8713,	0)
	(8714,	0)
	(8715,	0)
	(8716,	0)
	(8717,	0)
	(8718,	1)
	(8719,	1)
	(8720,	1)
	(8721,	0)
	(8722,	0)
	(8723,	0)
	(8724,	0)
	(8725,	0)
	(8726,	0)
	(8727,	0)
	(8728,	0)
	(8729,	2)
	(8730,	1)
	(8731,	1)
	(8732,	1)
	(8733,	0)
	(8734,	0)
	(8735,	0)
	(8736,	0)
	(8737,	0)
	(8738,	0)
	(8739,	0)
	(8740,	0)
	(8741,	3)
	(8742,	2)
	(8743,	1)
	(8744,	0)
	(8745,	0)
	(8746,	1)
	(8747,	1)
	(8748,	1)
	(8749,	1)
	(8750,	2)
	(8751,	2)
	(8752,	3)
	(8753,	2)
	(8754,	1)
	(8755,	0)
	(8756,	0)
	(8757,	0)
	(8758,	0)
	(8759,	1)
	(8760,	0)
	(8761,	0)
	(8762,	0)
	(8763,	1)
	(8764,	1)
	(8765,	1)
	(8766,	1)
	(8767,	0)
	(8768,	0)
	(8769,	3)
	(8770,	3)
	(8771,	2)
	(8772,	1)
	(8773,	1)
	(8774,	0)
	(8775,	0)
	(8776,	0)
	(8777,	0)
	(8778,	2)
	(8779,	1)
	(8780,	1)
	(8781,	1)
	(8782,	0)
	(8783,	0)
	(8784,	0)
	(8785,	0)
	(8786,	1)
	(8787,	1)
	(8788,	1)
	(8789,	0)
	(8790,	0)
	(8791,	0)
	(8792,	0)
	(8793,	0)
	(8794,	0)
	(8795,	0)
	(8796,	0)
	(8797,	0)
	(8798,	0)
	(8799,	4)
	(8800,	3)
	(8801,	3)
	(8802,	2)
	(8803,	1)
	(8804,	1)
	(8805,	1)
	(8806,	1)
	(8807,	0)
	(8808,	0)
	(8809,	0)
	(8810,	0)
	(8811,	0)
	(8812,	0)
	(8813,	1)
	(8814,	0)
	(8815,	0)
	(8816,	0)
	(8817,	0)
	(8818,	0)
	(8819,	0)
	(8820,	0)
	(8821,	0)
	(8822,	0)
	(8823,	0)
	(8824,	0)
	(8825,	0)
	(8826,	0)
	(8827,	0)
	(8828,	0)
	(8829,	0)
	(8830,	0)
	(8831,	0)
	(8832,	0)
	(8833,	0)
	(8834,	0)
	(8835,	1)
	(8836,	0)
	(8837,	0)
	(8838,	1)
	(8839,	2)
	(8840,	1)
	(8841,	0)
	(8842,	0)
	(8843,	0)
	(8844,	0)
	(8845,	0)
	(8846,	0)
	(8847,	1)
	(8848,	2)
	(8849,	1)
	(8850,	1)
	(8851,	1)
	(8852,	1)
	(8853,	0)
	(8854,	0)
	(8855,	0)
	(8856,	1)
	(8857,	0)
	(8858,	0)
	(8859,	0)
	(8860,	0)
	(8861,	0)
	(8862,	1)
	(8863,	1)
	(8864,	0)
	(8865,	0)
	(8866,	0)
	(8867,	1)
	(8868,	2)
	(8869,	1)
	(8870,	0)
	(8871,	0)
	(8872,	0)
	(8873,	0)
	(8874,	0)
	(8875,	2)
	(8876,	2)
	(8877,	3)
	(8878,	3)
	(8879,	3)
	(8880,	3)
	(8881,	3)
	(8882,	4)
	(8883,	4)
	(8884,	4)
	(8885,	4)
	(8886,	5)
	(8887,	5)
	(8888,	5)
	(8889,	6)
	(8890,	8)
	(8891,	9)
	(8892,	9)
	(8893,	9)
	(8894,	9)
	(8895,	10)
	(8896,	10)
	(8897,	11)
	(8898,	11)
	(8899,	11)
	(8900,	11)
	(8901,	12)
	(8902,	12)
	(8903,	12)
	(8904,	12)
	(8905,	12)
	(8906,	12)
	(8907,	12)
	(8908,	12)
	(8909,	12)
	(8910,	12)
	(8911,	13)
	(8912,	13)
	(8913,	13)
	(8914,	14)
	(8915,	16)
	(8916,	16)
	(8917,	16)
	(8918,	17)
	(8919,	18)
	(8920,	18)
	(8921,	19)
	(8922,	20)
	(8923,	20)
	(8924,	21)
	(8925,	21)
	(8926,	21)
	(8927,	23)
	(8928,	23)
	(8929,	23)
	(8930,	23)
	(8931,	24)
	(8932,	28)
	(8933,	28)
	(8934,	28)
	(8935,	28)
	(8936,	28)
	(8937,	28)
	(8938,	28)
	(8939,	28)
	(8940,	28)
	(8941,	28)
	(8942,	28)
	(8943,	28)
	(8944,	30)
	(8945,	30)
	(8946,	32)
	(8947,	33)
	(8948,	33)
	(8949,	33)
	(8950,	33)
	(8951,	33)
	(8952,	33)
	(8953,	33)
	(8954,	36)
	(8955,	37)
	(8956,	37)
	(8957,	38)
	(8958,	38)
	(8959,	38)
	(8960,	38)
	(8961,	41)
	(8962,	41)
	(8963,	42)
	(8964,	43)
	(8965,	43)
	(8966,	43)
	(8967,	44)
	(8968,	44)
	(8969,	45)
	(8970,	46)
	(8971,	46)
	(8972,	47)
	(8973,	47)
	(8974,	47)
	(8975,	49)
	(8976,	49)
	(8977,	49)
	(8978,	50)
	(8979,	50)
	(8980,	52)
	(8981,	52)
	(8982,	53)
	(8983,	53)
	(8984,	54)
	(8985,	54)
	(8986,	55)
	(8987,	55)
	(8988,	56)
	(8989,	57)
	(8990,	58)
	(8991,	58)
	(8992,	58)
	(8993,	58)
	(8994,	58)
	(8995,	59)
	(8996,	59)
	(8997,	59)
	(8998,	59)
	(8999,	61)
	(9000,	62)
};
